GreenMO: Virtualized User-proportionate MIMO

With the turn of new decade, wireless communications face a major challenge on connecting many more new users and devices, at the same time being energy efficient and minimizing its carbon footprint. However, the current approaches to address the growing number of users and spectrum demands, like traditional fully digital architectures for Massive MIMO, demand exorbitant energy consumption. The reason is that traditionally MIMO requires a separate RF chain per antenna, so the power consumption scales with number of antennas, instead of number of users, hence becomes energy inefficient. Instead, GreenMO creates a new massive MIMO architecture which is able to use many more antennas while keeping power consumption to user-proportionate numbers. To achieve this GreenMO introduces for the first time, the concept of virtualization of the RF chain hardware. Instead of laying the RF chains physically to each antenna, GreenMO creates these RF chains virtually in digital domain. This also enables GreenMO to be the first flexible massive MIMO architecture. Since GreenMO's virtual RF chains are created on the fly digitally, it can tune the number of these virtual chains according to the user load, hence always flexibly consume user-proportionate power. Thus, GreenMO paves the way for green and flexible massive MIMO. We prototype GreenMO on a PCB with eight antennas and evaluate it with a WARPv3 SDR platform in an office environment. The results demonstrate that GreenMO is 3x more power-efficient than traditional Massive MIMO and 4x more spectrum-efficient than traditional OFDMA systems, while multiplexing 4 users, and can save upto 40% power in modern 5G NR base stations.

==> background/background.tex <==
% !TEX root = ../paper.tex
\section{Background and Motivation}\label{sec:background}

\begin{figure}[t]
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    \input{results/rfe_pow_spectrum}
    \label{fig:compute_pow_spectrum}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    \input{results/compute_pow_spectrum}
    \label{fig:rfe_pow_spectrum}
    \end{subfigure}
    \caption{How today's multi-user techniques stand}
\end{figure}

\begin{table}[t]
    \centering
\begin{tabular}[t]{|c|c|c|c|c|}
      \hline
      Features       & FDMA & DBF & HBF & \textbf{\name} \\ \hline
      Spectrum Req.  & \textcolor{red}{\textbf{Nx}} & 1x & 1x & \textbf{1x} \\ \hline
      RFE Pow.       & 1x & \textcolor{red}{\textbf{$N_{ant}$x}} & $\sim$\textcolor{red}{\textbf{$\sim N_{ant}$x}} & \textbf{1x} \\ \hline
      Compute Pow.   & Nx & \textcolor{red}{\textbf{$N_{ant}$x}} & Nx & \textbf{Nx}  \\ \hline
      Sampling Pow.  & Nx & \textcolor{red}{\textbf{$N_{ant}$x}} & Nx & \textbf{Nx}\\ \hline
      Flexibility    & Yes & Yes & \textcolor{red}{\textbf{No}} & \textbf{Yes}\\ \hline
\end{tabular}
    \caption{Comparison of \name with existing techniques}
    \label{tab:comparison}
\end{table}

Recall that our goal is to achieve next-generation green communications which are spectrum-efficient.
The current gold-standard for spectrum-efficiency communications is Massive MIMO, and therefore in this section, we would review the state-of-art massive MIMO architectures and put them in perspective with green communications. 
The key idea behind massive MIMO is to use massive number of antennas $N_{\text{ant}}$ as compared to the number of users $N$ so  to capture enough degrees of freedom required to create $N$ spatial streams.
% \todo{todo what?, to create non-interfering... }. 
In that context, there are two popular multi-antenna architectures, digital beamforming and hybrid beamforming. 
To understand how green these architectures are, we study these in two aspects of power consumption in wireless transceivers 1) radio front-ends and 2) the sampling and compute for decoding. 

\subsection{Energy Consumption for radio front-ends }

Most popular architecture in sub-6 GHz is digital beamforming architecture (DBF). 
DBF basically connects each of the $N_{\text{ant}}$ antennas to radio frontend processing chains (RF chains), which downconvert the signals received by the antennae and get it ready for digital baseband sampling. 
% Recall that the goal of massive MIMO architecture to achieve N non-interfering spatial stream one for each user. 
The goal of DBF here is to procure the antenna's degrees of freedom at the digital baseband level, where signal processing can then create $N$ non-interfering spatial streams, one for each user.

In that context, digital beamforming is extremely inefficient in its power consumption at the front-end. 
Among the various analog components in the RF chain, the dominant power consuming operation is the downconversion of each $N_{\text{ant}}$ signals. 
The downconversion for each antenna needs high quality LO signal distributed, which is extremely power hungry and challenging process. Primarily, the quality of LO degrades as you split the signal power of the LO, therefore, the architecture needs active low-noise amplification circuits and distribute the LO. 
Furthermore, the LO for Massive MIMO operations need to be phase synchronized, which makes it complex and further adds to the power consumption\todo{delete this sentence}. 
The end result is that LO distribution dominates the power consumption, make it power hungry architecture continuously burning watts of constant power for just being operational. 

On the otherhand, Hybrid beamforming approaches try to reduce this power consumption by using analog pre-processing networks which constructs only $N$ outputs one for each user instead of $N_{\text{ant}} >> N $ ~\cite{beamforming,works}, downconvert post creation of N outputs.  
The analog circuits are typically network of phase shifters, and the phases are set such that the $N_{\text{ant}}$ degrees of freedom available at the RF front end are mapped to a well conditioned $N$ degrees of freedom at digital baseband; such that digital processing can then establish $N$ spatial streams without requiring downconversion of additional $N_{\text{ant}}-N$ streams\todo{I don't follow this}.
However, firstly, these hybrid beamformers 
% optimize only for the compute power consumption by reducing the number of backhaul streams but do not optimize for the front end RF-chain power consumption as they would 
still require $N$ physical RF-chains, so the LO distribution is still there (albeit reduced by a factor of $N_{\text{ant}}/N$). 
% Secondly, these phase shifter networks have high insertion losses, which puts stress on the power amplifier requirements; 
% this ends up increasing the non-linearities from the amplifier, and requiring a higher ENOB from digital sampling \todo{stay away from high ENOB, you would higher right??}.
% Recent papers have even suggested that hybrid beamformers actually end up having RF front end power consumption almost similar to digital counterparts ~\cite{recent,works,provingthis}.

% Fundamentally, both the existing strategies end up wasting a lot of power just at the RF front-end chains, and this is 
The true requirements of a green communications architecture, however is to put forward a system which can cut this RF front end power consumption to lowest of limits, that is be a constant $O(1)$ and not be $O(N)$, where $N$ is the number of users.
The $O(1)$ power consumption at RF front end is extremely critical since this is a a fixed power consumption just to set up the hardware.  
Clearly, none of the current approaches are even close to solving this RF front end power optimization problem, since for DBF power is $O(N_{\text{Ant}})$ and for even the most ideal HBF it is $O(N)$.
% if we can limit to the $1\times$ RF chain. 

\subsection{Energy consumption for sampling and compute}

In addition to the RF front end power consumption of multi-antenna architectures, it is also important for green architectures to consider the power consumption for digital sampling, and the data backhauling+compute power thereoff.
However, unlike RF front end power, this is not a fixed power consumption cost due to hardware, and depends on the user load.
Thus, the challenge to optimize this power consumption is different than that of front end; Truly green architectures need to \emph{flexibly} adjust the the sampling and compute power consumption to always be commensurate with the number of users supported (i.e. has to be $N$x).

For digital beamforming massive MIMO, each of the $N_{\text{ant}}$ antenna streams needs to be backhauled and computed in the digital signal processor, in order to obtain the $N$ interference free per-user streams. Thus, this makes DBF further inefficient, it has to firstly, deal with compute+sampling of $N_{\text{ant}}$ streams in addition to exacerbated power requirements already. On the other hand, the hybrid architectures $N_{\textit{ant}}$ to $N$ RF-chains via analog circuits and feedback only $N$ streams to efficiently use sample and compute. 
However, HBF today is a fixed architecture which optimizes compute+sampling only for $N$ users.
Since ideally the compute power should scale with $N$, it can not be optimized for a fixed number of users.
That is, if the number of users increase/decrease, HBF can not arbitarily scale to higher/lower RF chains required since the architecture relies heavily on the fixed laid down phase shifter network.
% Thus, HBF is not a flexible architecture, and this is one major hindrance on why even after years of research on HBF there are very few practical deployments.

% Alongside cutting down on power requirements, another advantage of \name is the flexibility arising from virtualization of RF chains.
% Since the number of RF chains can be controlled via software by tweaking the sampling+switching frequency of \name architecture, it allows \name to adaptively tune number of RF chains in response to user load.
% In contrast, HBF today is a fixed architecture which optimizes compute+sampling only for $N$ users. 
% If the number of users increase/decrease, it can not arbitarily scale to higher/lower RF chains required since the architecture relies heavily on laid down phase shifter network.
% Thus, HBF is not a flexible architecture, and this is one major hindrance on why even after years of research on HBF there are very few practical deployments.

In summary, requirements from a truly green architecture is two-fold with respect to power consumption: (1) Have O(1) power consumption at the RF front ends to minimize the setup power costs and (2) Have O(N) power consumption for sampling+compute to minimize the running power costs, flexibly in response to the corresponding $N$ users' load. In addition, (1) and (2) need to be met with spectrum efficiency. All the $N$ users need to share the same spectrum resource.


% Multi-user communication systems today either do FDMA, by separating users in frequency domain, or utilize massive MIMO, which separates user in spatial domain.
% FDMA is energy efficient and flexible; requires only a single RF chain and the base station has to only sample the relevant parts of spectrum where user's are transmitting, and this sampling can be controlled directly via software.
% Massive MIMO, on the other hand, allows users to use same frequency bands, by using multiple antennas to separate users spatially. 
% However, this comes at a cost of laying of dedicated hardware per antenna to downsample and digitize, referred to as `RF chains', which end up burning a lot of power.
% This massive MIMO architecture of having $1$ RF chain per antenna is referred to as `Digital beamforming'.
% % 

% The bottlenecks with digital beamforming architectures have been thought to be the power implications of the ADCs required to digitize these samples, and the deployment of multiple RF chains which guzzle up a lot of power from the local oscillators supplying the downconversion clocks.
% Hence, under these power consumption assumptions, at the onset of 5G standards, it was not considered that the digital beamforming architectures could even be practical and there was a lot of push towards doing beamforming in the analog RF domain, in order to prevent digitization of signals from each antenna required to perform the baseband digital beamforming. 
% In this process, these analog beamforming approaches add circuit elements like phase shifters, which contribute to a lot of insertion losses requiring increased LNA power consumption.
% Further these phase shifters have limited precision, and they are not wideband, which limits the total beamforming gains.
% Also analog architectures by themselves do not offer spatial multiplexing possibilities, requiring sophisticated directional MAC algorithms.

% However, as the technology evolves, it has actually become evident that ADC/DAC power consumption is going to go lower and has dropped considerably in the past few years itself \cite{yan2019performance}.
% Also, ADC/DAC power consumption is flexible, it can be further reduced by reducing the number of quantization bits on demand.
% Further, looking at the tradeoffs introduced by the analog beamforming; heavy insertion losses+sophisticated MAC algorithms, digital beamforming architectures have started becoming more preferred again, with multiple previous work even reporting the competitiveness of today's digital beamformers over analog in terms of power consumption \cite{barati2020energy,yan2019performance,dutta2019case,abdelghany2018towards,DOOSTMOHAMMADY2021107870}; at the same time preserving the flexibilities and spatial multiplexing possibilities offered by the digital architectures. 

% \subsection{Current system drawbacks and how \name addresses these}
% However, the digital beamformers of today are still facing two problems, first, the power consumption and technical difficulties of laying a synchronized downconversion LO distribution, and second, design of a flexible hybrid architecture which optimizes the amount of data backhauled and required signal processing.
% \name gives a solution to both these problems, and paves the way ahead for a new class of beamforming approaches; delivering robust spatial multiplexing gains while being both, spectrum efficient and power efficient.

% For the first problem, \name uses just a single physical RF chain, thus circumventing the LO distribution issues.
% Infact, studies show that the total power consumption of a synchronized distributed LO network is higher than that of ADCs/DACs \cite{yan2019performance}.
% Worse, given that there is an increasing trend towards moving higher frequencies, mmWave and THz bands, and the LO distribution problem is only going to become more challenging as our hardware advances.
% Instead of distributing these high frequency LO clocks, the clocks given to the RF switches in \name design are of the order of the signal bandwidth, and not carrier frequencies. 
% Thus, \name architecture is well adapt to next generation communication technologies.

% Second, it has been well acknowledged that to serve $N$ users reliably, massive MIMO required $N_{\text{ant}}>N$ antennas, and thus the total ADC sampling is going to be larger than number of users, with traditional massive MIMO architectures.
% Ideally, we should be sampling only $N$ users streams, but here we end up sampling $N_{\text{ant}}$ streams, which leads to increased ADC power consumption and more importantly, the digital signal processing is now working on higher number of samples; requiring much higher data rates to handle the huge amount of data generated via massive MIMO just to serve $N$ users \cite{yan2019performance,ding2020agora}.

% Hybrid analog-digital architectures attempt to address this problem, by laying an network of phase shifters and combiners which connect a larger number of $N_{\text{ant}}$ antennas to $N$ RF chains, and use analog beamforming to combine the $N_{\text{ant}}$ streams into $N$ sampled streams. Essentially, they project the larger number of $N_{\text{ant}}$ dimensions to create effective $N$ dimensional channels such that the $N$ users can get decoded.
% However, these architectures still end up wasting a lot of power in dealing with insertion losses from phase shifters, working with phase shifter quantization issues amongst the others.
% Further, these architectures are inflexible; when number of users reduce they still end up burning power in the set up physical RF chains.
% In comparison, \name architecture hybridizes easily, since all antennas are by default connected to the virtual RF chains, making it easier to just keep on adding antennas without worrying about fixed analog circuitry.
% \name also is a flexible architecture, when number of users reduce, we just reduce number of virtual RF chains on the fly.
% As compared to phase shifters, which have insertion losses around 10 dB, switches have minimal insertion losses, about just 0.5-1 dB which is minimal and does not increase burden on the LNA's.








%People want flexible solutions; in gen comm
%MIMO going reverse way
%Trends of softwarization: 

==> background/background_v1.tex <==
% !TEX root = ../paper.tex
\section{Background and Motivation}\label{sec:background}

\begin{figure}[t]
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    \input{results/rfe_pow_spectrum}
    \caption{}
    \label{fig:compute_pow_spectrum}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    \input{results/compute_pow_spectrum}
    \caption{}
    \label{fig:rfe_pow_spectrum}
    \end{subfigure}
    \vspace{5pt}
    \caption{Power and Spectrum efficiency comparison: (a) RF front end power compared vs spectrum efficiency (b) Compute Power vs Spectrum Efficiency. Showing how \name is the most optimal.}
    % \vspace{-5pt}
\end{figure}



Recall that our goal is to achieve next-generation green communications which are spectrum-efficient.
The current gold-standard for spectrum-efficiency communications is Massive MIMO, and therefore in this section, we would review the state-of-art massive MIMO architectures and put them in perspective with green communications. 
The key idea behind massive MIMO is to use massive number of antennas $N_{\text{ant}}$ as compared to the number of users $N$ so  to capture enough degrees of freedom required to create $N$ spatial streams.
In that context, there are two popular multi-antenna architectures, digital beamforming and hybrid beamforming. 
To understand how green these architectures are, we study these in two aspects of power consumption in wireless transceivers while maintaining spectral efficiency: (1) radio front-ends and (2) the sampling and compute for decoding. 

\subsection{Energy Consumption for radio front-ends }
Most popular architecture in sub-6 GHz is digital beamforming architecture (DBF)~\cite{ding2020agora,yan2019performance,araujo2016massive, hoydis2013massive,liu2012downlink, castaneda2016overview}. 
DBF basically connects each of the $N_{\text{ant}}$ antennas to radio frontend processing chains (RF chains), which downconvert the signals received by the antennae and get it ready for digital baseband sampling. 
The goal of DBF here is to procure the antenna's degrees of freedom at the digital baseband level, where signal processing can then create $N$ non-interfering spatial streams, one for each user.

This specific design of RF front end design makes the digital beamforming inefficient in its power consumption at the front-end. 
The reason behind this power inefficiency is that amongst the various analog components in the RF chain, the dominant power consuming operation is the downconversion of each $N_{\text{ant}}$ signals. 
This downconversion for each antenna needs high quality LO signal distributed, which is extremely power hungry and a challenging process. 
Primary reason for this is that the quality of LO degrades as you split the signal power of the LO~\cite{yan2019performance,swindlehurst2014millimeter,chung2020millimeter}, and therefore the architecture needs active low-noise amplification circuits to distribute the LO. 
Furthermore, these split LO's for Massive MIMO operations need to be phase synchronized with very low phase noise, which makes the process more power hungry~\cite{yan2019performance,lacaille2019optimizing}.
The end result of this complex LO distribution to serve $N$ users is that it dominates the power consumption, making the DBF's front end design constantly drawing watts of power for its spectrally efficient operations.


% \begin{adjustbox}{max width=\textwidth}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}[t]{|c|c|c|c|c|}
      \hline
      \textbf{Features}       & \textbf{FDMA} & \textbf{DBF} & \textbf{HBF} & \textbf{\name} \\ \hline
      \textbf{Spectrum Req. } & \textcolor{red}{O(N)} & $O(1)$ & O(1) & \textbf{$O(1)$} \\ \hline
      \textbf{RFE Pow.}       & $O(1)$ & \textcolor{red}{\textbf{$O(N_{ant})$}} & \textcolor{red}{\textbf{$\sim O(N_{ant})$}} & $O(1)$ \\ \hline
      \textbf{Compute Pow.}   & $O(N)$ & \textcolor{red}{\textbf{$O(N_{ant})$}} & $O(N)$ & \textbf{$O(N)$}  \\ \hline
      \textbf{Sampling Pow.}  & $O(N)$ & \textcolor{red}{\textbf{$O(N_{ant})$}} & $O(N)$ & \textbf{$O(N)$}\\ \hline
      \textbf{Flexibility}    & Yes & Yes & \textcolor{red}{No} & Yes\\ \hline
\end{tabular}
}
\vspace{4pt}
\caption{Comparison of \name with existing techniques}
\label{tab:comparison}
\vspace{-10pt}
\end{table}
% \end{adjustbox}

On the otherhand, there are Hybrid beamforming (HBF) approaches that try to reduce the RF front end power consumption by using analog pre-processing networks which constructs only $N$ outputs one for each user instead of $N_{\text{ant}} > N $ ~\cite{kim201828,kuhne2020bringing,ghasempour2018multi,xie2015hekaton,chen2020turbo, zhang2017hybridly,yu2016alternating,mondal201921, mondal201825, mondal201725,obara2015indoor, chen2017bush}.
These $N$ outputs are then downconverted to decode the user data.
These analog pre-processing networks are typically a network of phase shifters.
These phase shifters are configured such that it projects the $N_{\text{ant}}$ degrees of freedom available at the RF front end to well conditioned $N$ degrees of freedom at digital baseband.
This analog phase configuration establishes $N$ spatial streams without requiring downconversion of additional $N_{\text{ant}}-N$ streams
% \todo{I don't follow this}.
However, these phase shifters still require $N$ physical RF-chains, so that the power hungry LO distribution is still existing (albeit reduced by a factor of $N_{\text{ant}}/N$).
An additional point to note is that this analog phase shifting network has very high insertion losses (about 10dB)~\cite{kuhne2020bringing,barati2020energy,yan2019performance}. These insertion losses need to be compensated for via increased power consumption from the power-amplifiers. Often this additional power requirement from the amplifiers offsets the power savings at the RF front end due to reduction of RF chains from $N_{ant}$ to $N$. Thus making the HBF RF front end almost as power hungry as DBF as shown in Fig.~\ref{fig:rfe_pow_spectrum}.

Thus, we can see that both DBF and HBF consume power on the order of the number of antennas ($O(N_{\text{Ant}})$). 
But we know that, RF front end power consumption is a constant power requirement just to set up the hardware, and it should not scale upward with the number of antennas required for massive MIMO.
Thus, true requirements of a green communications architecture, should be to cut this RF front end power consumption to the lowest of limits, by making it a constant ($O(1)$) instead.
% and not be $O(N)$, where $N$ is the number of users.
% Clearly, none of the current approaches are even close to solving this RF front end power optimization problem, since for DBF power is $O(N_{\text{Ant}})$ and for even for HBF it is $\sim O(N_{\text{Ant}})$.

\subsection{Energy consumption for sampling and compute}

In addition to the RF front end power consumption of multi-antenna architectures, it is also important for green architectures to consider the power consumption for digital sampling, and the data backhauling+compute power thereoff.
However, unlike RF front end power, this is not a fixed power consumption cost due to hardware, and depends on the user load.
Thus, the challenge to optimize this power consumption is different than that of front end. 
That is for a truly green architecture we need to \emph{flexibly} adjust the sampling and the compute power consumption to always be order of number of users, $O(N)$.
% commensurate with the number of users supported (i.e. has to be $N$x).

Unfortunately DBF needs to backhaul and compute $N_{\text{ant}}$ antenna streams at the digital signal processor to obtain the $N$ interference free per-user streams.
% For DBF, each of the $N_{\text{ant}}$ antenna streams needs to be backhauled and computed in the digital signal processor, in order to obtain the $N$ interference free per-user streams. 
Thus, this makes DBF further inefficient, as it deals with compute+sampling of $N_{\text{ant}}$ streams in addition to exacerbated power requirements already. 
On the other hand, the hybrid architectures reduce the RF-chains from$N_{\textit{ant}}$ to $N$ via analog circuits and feedback only $N$ streams to efficiently use sample and compute. 
However, HBF today is a fixed architecture which optimizes compute+sampling only for $N$ users.
Since ideally the compute power should scale with $N$, it can not be optimized for a fixed number of users.
That is, if the number of users increase/decrease, HBF can not arbitarily scale to higher/lower RF chains required since the architecture relies heavily on the fixed laid down phase shifter network.

In summary, requirements from a truly green architecture are two-fold with respect to power consumption: (1) Have O(1) power consumption at the RF front ends to minimize the setup power costs and (2) Have O(N) power consumption for sampling+compute to minimize the running power costs, flexibly in response to the corresponding $N$ users' load. In addition, the green architecture needs to meet (1) and (2) while maintaining the spectrum efficiency, i.e., all the $N$ users need to share the same existing spectrum resource.


==> background/background_v2.tex <==
\section{Background and Motivation}
As we connect more users to the wireless networks, the base station has to handle more data generated by the new users, and thus would require  to do so are further going to scale up and worsen.
Under the best theoretic scenario, the power consumption is going to scale linearly with number of users, since each user brings forth new data which needs to be digitized and communicated, requiring proportional increase in the communication resources and hence power.
However, in practical scenarios, technologies like massive MIMO end up requiring many more communication resources (antennas) than number of users, and thus end up being power inefficient.
On the other hand, using a different communication resource (spectrum) via OFDMA we can trace this linear increase however at cost of exacerbating spectrum requirements.
\name shows how the best of both world solution ends up tracing the linear curve similar to OFDMA while having same spectrum requirements like Massive MIMO.


\subsection{Info-theoretic limits to power consumption}

When we have $N$ users, transmitting signals with $B$ bandwidth each, info-theoretically there can be two equivalent approaches to accommodate these users.
Either we can have these $N$ users occupy different $B$ bandwidth chunks and then to obtain the data an ADC (Analog to Digital Converter) can sample the thus generated data in the $NB$ net spectrum.
Otherwise, the users can occupy the same $B$ bandwidth spectrum chunk, 
and now we connect $N$ antennas to $N$ different ADCs to create a MIMO approach, each of which sample the $B$ bandwidth received signals from their respective antenna.
These $N$ antennas receive signals from $N$ users via different channels, and akin to solving $N$ equations with $N$ variables, the data of each user can be decoded.


In summary, info-theoretically we require either $N$ different $B$ bandwidth ADCs, or a single $NB$ bandwidth ADC.
Theoretically, the power consumption of ADCs sampling at $F_s$, assuming that the transmitters use $q$ bits quantization is given by
$P_{ADC}=\text{FoM}\times F_s \times 2^q$
where where \text{FoM} is a constant referred to as figure of merit. With the first approach, $P_1 = \text{FoM}\times NB \times 2^q$, and with the second, $P_2 = N(\text{FoM}\times B \times 2^q)$, and clearly $P_1=P_2$, and both approaches are linear with number of users $N$.
This is basically the power consumed at the base-station which is receiving the $N$ users data.
In addition to this, to attain the target SNR to transmit at $q$ bits level, the $N$ users would transmit at a certain power $P_t$, which would require a power amplifier, having certain power consumption $P_{PA}$, as well as a DAC to generate the $B$ bandwidth transmit signals, requiring $P_{DAC}$.
The power consumed at users would hence be $N*(P_{PA}+P_{DAC})$, with total theoretical power consumption being $P_{th} = N*(P_{PA}+P_{DAC}+\text{FoM}B2^q)$, linear in $N$.
The transmit and receive roles of base-stations and user devices can be inverted to arrive at the roughly the same power calculations at an info-theoretic level.

\subsection{Power/Spectrum inefficiency of existing technologies}

When we transition to practical wireless communication circuits, we need to start adding concepts of center frequency, up/down conversion blocks, insertion losses of practical circuits etc. Hence in addition to the theoretical power requirements, there are some extra circuit power requirements $P_{total}=P_{th}+P_{hardware}$.
Thus, we can define efficiency via the following metric: $\frac{P_{th}}{P_{total}}*100$, since in order to get $P_{th}$ worth useful power to communicate $N$ users data at $B$ bandwidth each at a certain SNR, we are investing $P_{total}$ power.
For green communications architectures, it is essential to minimize the $P_{hardware}$.

In case of practical MIMO deployments, $P_{total}$ ends up being severely worse than $P_{th}$, as in realistic channel settings to serve $N$ users we need $M>>N$ antennas, also referred to as massive MIMO (mMIMO). Motivation behind mMIMO is that a $N\times N$ MIMO system may not have invertible channel matrices, or undergo severe noise boosting which would affect SNR.
Hence, $P_{mMIMO} \approx P_{th}+(M-N)*(P_{ADC})+M*P_{circuits}$, where $(M-N)*P_{ADC}$ are the extra power requirements from extra number of ADCs required, and $M*P_{circuits}$ is the total power required in LNA+downconversion chains of the $M$ antennas' signals.
Even though today massive MIMO is gold standard for its robustness in handling $N$ users, it is an extremely power-inefficient architecture for serving $N$ users.
If we consider the other approach of OFDMA, the extra hardware required there is just a single antenna, and hence for OFDMA
$P_{OFDMA} \approx P_{th}+P_{circuits}$, and often $P_{circuits}$ is miniscule compared to $P_{th}$ which increases linearly with $N$.
Some typical numbers for these metrics when $N$=4, would be $P_{circuits}= $, $P_{ADC}=$, and $P_{th}=$, \cite{} which gives $\eta_{mMIMO} = 30\%$, and $\eta_{OFDMA} = 95\%$.
However, OFDMA gets this power efficiency at cost of exacerbating spectrum requirements.

One potential method to bridge this tradeoff is to create hybrid beamformers, which map $M$ antennas to $N$ streams via an analog network, usually consisting of phase shifters.
Basically, these hybrid beamformers map the $M>>N$ antenna dimensions to a well conditioned $N$ streams dimension such that MIMO works equivalently with $N$ streams by itself. 
This approach has $P_{HBF} \approx P_{th}+M*P_{circuits_HB}$ this still requires the analog network which often has high insertion losses and requires higher circuit power than massive MIMO ($P_{circuits_{HB}}>P_{circuits_{mMIMO}}$.
Further, since the analog network is fixed $M:N$ network, hybrid beamformers loose their optimality when $N$ changes, hence are not flexible.
Typical efficiency metrics with a $16:4$ network when evaluated at $N=4$\cite{} would be $70\%$ (still not as high as OFDMA because of extra circuit power), which drops down to $40\%$ when $N=2$.

\name achieves the power efficiency of OFDMA, while being as spectrally efficient as massive MIMO, with a new architecture which basically virtualizes a single RF chain over multiple antennas and cut down on the the hardware power requirements, infact bringing it down to the OFDMA levels. The reason this works out is that \name creates virtual RF chains over the sampled bandwidth of a single ADC, and this enables \name to be flexible in addition as well. \name is truly the first architecture which bridges this severe tradeoff between power and spectrum efficiency.




% More importantly, under practical scenarios, the first approach of sampling $NB$ bandwidth for $N$ users also referred to as OFDMA, doesn't scale with number of users $N$ since the spectrum demands are exacerbating.
% Whereas the other approach of enabling MIMO using $N$ antennas to serve $N$ users, also referred to as mu-MIMO doesn't work in practise either since the required interference cancellation ends up requiring $M>>N$ number of antennas, also called as massive MIMO.
% Requiring many more antennas ends up requiring more ADCs in massive MIMO. In addition, each antenna requires it's own down/up conversion hardware and there is extra power required there as well.
% Hence we have $P_{massive MIMO} = N*(P_{PA}+P_{DAC}+P_{UP})+M*()$
% All these blocks are theoretically not required, but in practical deployments wireless communication needs to happen at certain frequency bands which requires the customized up/downconversion.
% However, as our IC technology gets better, these extra circuit blocks demand lesser power than the theoretical power requirements, for example an info-theoretic OFDMA system would require 


% Multi-antenna systems form an integral part of the next generation wireless communication networks. 

==> background/background_v3.tex <==
\section{Background and Motivation}

Increasing throughput is central to the growth of wireless networks, it allows newer applications demanding high data rates, and also allows networks to connect more users.
However, with the turn of new decade, an important consideration is that wireless networks become greener by being power efficient.
A metric of power efficiency here could be comparing the power consumed by different networks to attain similar throughput. 
If a particular network can support same throughput at a lower power bill, it is going to be greener, as well as cheaper, and the effects would distill down to end users having lower network bills.
Hence in this section, first we will show the throughput versus power metrics of the two popular wireless approaches of getting increased throughput, by either procuring more spectrum, or adding more antennas to get increased throughput.
Then we will briefly touch upon how a smarter fusion of these two approaches can push the efficiency metrics as close to ideal as possible, as well as enable scalable growth of wireless networks.

\subsection{Power efficiency of OFDMA, and today's MIMO (muMIMO \& mMIMO)}

In order to meet the increasing throughput demands, the two popular techniques have been either to add a large number of antennas and utilize the spatial dimension (mu-MIMO, mMIMO), or increase the sampled spectrum (OFDMA).
The latter approach almost always requires simpler hardware, a single antenna and downconversion chain and a ADC which supports the associated sampling requirements.
In order to scale to higher throughput, the hardware remains same, and just the sampling rate of ADC increases which leads to a linear increase in power \footnote{ADC power scales linearly with sampling frequency}.
Said differently, to get $N$ times throughput, the ADC starts sampling $N$ times spectrum.
However, this technique is not scalable in the sense that, operators need to buy more spectrum which goes through a complicated process through the FCC and is very expensive.
Further, as the user demand reduces, this increased spectrum purchased is not utilized fully leading to spectrally-inefficient deployments.

On the flipside, an other approach is to add more antennas to support increased throughput. Availability of more antennas can either enable beamforming towards a single user to get increased data rate, or allow the capability to handle multiple interfering users, improving the net throughput in the process, and this is intended goal of various MIMO approaches.
However, interfacing to multiple antennas requires more sophisticated hardware than OFDMA, since MIMO requires multiple synchronized downconversion chains and multiple ADCs to implement what is also referred to as digital beamforming. 
Hence, even the simplest MIMO deployment having $N$ antennas to get $N$ times throughput (mu-MIMO\cite{}) is not as power efficient as OFDMA.
Worse yet, in practical deployments, we often massive number of antennas, $M$ to get the required $N$ times throughput gain (massive MIMO, or mMIMO with $M>>N$), since mu-MIMO requires well conditioned environment which is more often not the case with realistic settings.
Requiring even more downconversion chains, and more ADCs, mMIMO ends up being even more power inefficient, since OFDMA, with requirement of higher spectrum requires simpler hardware and is power efficient.

Hence, we see a big spectrum grab today \cite{}, even though we have MIMO solutions to make wireless networks spectrally efficient. 
This is simply because the operators having more spectrum would end up having lower power bills, and simpler to manage network.

\subsection{Can MIMO get to the OFDMA levels of power efficiency?}

Hence the question really boils down to, if the spectrally efficient MIMO can ever hit the power efficiency of OFDMA \cite{}. There have been papers which have already concluded otherwise \cite{} and shown a tradeoff between power efficiency and spectrum efficiency of wireless deployments \cite{}. As a consequence, there are works which look at systems like NOMA \cite{}, 1 bit ADCs \cite{} which try to make MIMO power-efficient but are not universally deployable and work only in certain scenarios.

However, one hint towards solving this tradeoff is existence of hybrid beamformers (HBF). The idea is that thes $M>>N$ antennas are connected to $N$ downconversion chains via a compressive analog network which tries to capture the useful aspects of $M$ antennas into the sampled $N$ streams and reach the mMIMO performance. These hybrid beamformers theoretically reach power efficiency of mu-MIMO, however, in practical deployments the analog compressive network has higher losses which need to be compensated appropriately with amplifiers and hence starts becoming power inefficient. 
More importantly, HBF are fixed point deployment constructed to solve a particular $M:N (\text{fixed N})$ usecase, and even the theoretical optimality doesn't hold as the user load varies.

Hence, as a hypothesis, a HBF which has simple analog network with low losses, and is flexible in deployment where $M:N(\text{variable N})$ and not a fixed network, we can infact break the tradeoff.
In this paper, we basically show that this hypothesis is true and we can design such a special flexible HBF.
The design of such a flexible HBF marries the two fundamental approaches of higher sampled spectrum and many antennas in an interesting way.
Basically, we make the approach that we can connect all the $M$ antennas to a single configurable downconversion chain where the sampled IF spectrum can be varied akin to OFDMA to get the compressi


==> background/old_background.tex <==
% !TEX root = paper.tex
\section{Background and Motivation}\label{sec:background}

\begin{figure}[t]
    % \begin{adjustwidth}{-15pt}{} 
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/compute_pow_spectrum}
    % \caption{Power \& Spectrum Required}
    \label{fig:compute_pow_spectrum}
    \end{subfigure}
    % \end{adjustwidth}
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.8\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/rfe_pow_spectrum}
    % \caption{Power \& Spectrum Required}
    \label{fig:rfe_pow_spectrum}
    \end{subfigure}
        % \vspace{7pt}
    % \begin{subfigure}[b]{0.5\textwidth}
    
    % \end{subfigure}
    \caption{How today's multi-user techniques stand}
\end{figure}

\begin{table}[t]
    \centering
\begin{tabular}[t]{|c|c|c|c|c|}
      \hline
      Features       & FDMA & DBF & HBFF & \textbf{\name} \\ \hline
      Spectrum Req.  & \textcolor{red}{\textbf{Nx}} & 1x & 1x & \textbf{1x} \\ \hline
      RFE Pow.       & 1x & \textcolor{red}{\textbf{$N_{ant}$x}} & \textcolor{red}{\textbf{$\sim N_{ant}$x}} & \textbf{1x} \\ \hline
      Compute Pow.   & Nx & \textcolor{red}{\textbf{$N_{ant}$x}} & Nx & \textbf{Nx}  \\ \hline
      Sampling Pow.  & Nx & \textcolor{red}{\textbf{$N_{ant}$x}} & Nx & \textbf{Nx}\\ \hline
      Flexibility    & Yes & Yes & \textcolor{red}{\textbf{No}} & \textbf{Yes}\\ \hline
\end{tabular}
    \caption{Comparison of \name with existing techniques}
    \label{tab:comparison}
\end{table}

    

% table
% People want to reduce power; analog domain has insertion losses+imperfections+MAC requirements on top
% digital offers advantages
% reduce bits; loose capability to do higher constellations + imperfections; tradeoff
% We present a no-tradeoff approach to DBF

% judicious use of ADC: use only when required

% Massive MIMO has been touted as one of the most promising technologies which would enable spectral-efficient communications and finally address the spectrum crunch issue we face today.
% Today, massive MIMO faces an immense challenge to implement

% make it more structured

Currently, the gold-standard to enable spatial-efficient communications is massive MIMO, which has $N_{\text{ant}}$ antennas to serve $N$ interfering users, via the digital beamforming architecture (DBF).
DBF basically connects each of the $N_{\text{ant}}$ antennas to RF front end processing chains (RF chains), which downconvert and filter the signals received by the antennas and get it ready for digital sampling.
However, massive MIMO is highly power inefficient; to obtain $N$ user streams it has to firstly, deal with compute+sampling of $N_{\text{ant}}$ streams, as well as the RF front-end (RFE) power consumed by the laid out hardware for $N_{\text{ant}}$ RF chains.

Hybrid beamformers (HBF) attempt to address the sampling and compute power inefficiencies of DBF (Fig. \ref{fig:computpow_spectrum}), by using analog beamforming to project the $N_{\text{ant}}$ antenna signals to $N$ sampled streams via a network of analog phase shifters.
In an ideal scenario, HBF would end up reducing RF front end power consumption as well, since it would require only $N$ (instead of $N_{\text{ant}}$) RF chains. 
However due to the high insertion losses in the phase shifter networks, HBF ends up consuming considerable power resources to amplify the signal to compensate for these losses.
Hence, the recent works~\cite{recent,works,provingthis} have shown that the front end power consumption of a practical HBF is in fact of the same orders as that of DBF (Fig. \ref{fig:rfe_pow_spectrum}).

The most impactful contribution of \name's architecture is to cut down drastically on RFE power consumption; since \name architecture uses just a single RF chain.
Alongwith requirement of unique switching strategies in \name architecture, a key design choice we put forward is to use a ADC sampling at $NB$, where we have $N$ users occupying the same $B$ bandwidth spectrum.
\name proposes to create virtual RF chains in this $NB$ sampled spectrum from the single laid physical RF chain.
On the other hand, to serve $N$ users, the previous ideal approaches proposed to use $N$ different ADCs sampling $B$ bandwidth each.
The \textit{ADC power scales linearly with sampling frequency \cite{RFtextbooks, datasheets}}, with the power equation:
$$P{_{ADC}} =  \text{FoM}*2^q*F_s$$
where, FoM is the figure of merit, $q$ is the number of quantization bits and $F_s$ is the sampling frequency.
Thus, power of $N$ $B$ bandwidth ADCs would be same as a single $NB$ bandwidth ADC, and hence both these design choices are equivalent and consume $Nx$ total sampling power.
However, using just a single $NB$ ADC allows creation of virtual RF chains, and thus reduces the RFE power consumption considerably.

A common misconception with beamforming architectures today is to ignore the RFE power consumption and assume that the power requirements are bottlenecked via the ADC sampling.
However, it is in fact the opposite.
Today's multi-antenna architectures guzzle up a lot of power in order to synchronize and distribute the LO required for coherent MIMO downconversion.
Further, as the technology evovles, the sampling and compute will become more power efficient, but as the communication frequencies go higher, to mmWave and THz now, the RFE power consumption is going to become far more critical parameter to optimize and can no longer be neglected.

Alongside cutting down on power requirements, another advantage of \name is the flexibility arising from virtualization of RF chains.
Since the number of RF chains can be controlled via software by tweaking the sampling+switching frequency of \name architecture, it allows \name to adaptively tune number of RF chains in response to user load.
In contrast, HBF today is a fixed architecture which optimizes compute+sampling only for $N$ users. 
If the number of users increase/decrease, it can not arbitarily scale to higher/lower RF chains required since the architecture relies heavily on laid down phase shifter network.
% Thus, HBF is not a flexible architecture, and this is one major hindrance on why even after years of research on HBF there are very few practical deployments.

\name is the first work which optimizes the RFE power; at the same time there is no tradeoff and \name also optimizes the compute and sampling powers (Table \ref{tab:comparison}), all the while being flexible to react adaptively on the user load.
Thus, \name outperforms any of the present beamforming architectures, and paves the way ahead with the first architecture which can do power-efficient, spectrum-efficient green wireless communications.



% Multi-user communication systems today either do FDMA, by separating users in frequency domain, or utilize massive MIMO, which separates user in spatial domain.
% FDMA is energy efficient and flexible; requires only a single RF chain and the base station has to only sample the relevant parts of spectrum where user's are transmitting, and this sampling can be controlled directly via software.
% Massive MIMO, on the other hand, allows users to use same frequency bands, by using multiple antennas to separate users spatially. 
% However, this comes at a cost of laying of dedicated hardware per antenna to downsample and digitize, referred to as `RF chains', which end up burning a lot of power.
% This massive MIMO architecture of having $1$ RF chain per antenna is referred to as `Digital beamforming'.
% % 

% The bottlenecks with digital beamforming architectures have been thought to be the power implications of the ADCs required to digitize these samples, and the deployment of multiple RF chains which guzzle up a lot of power from the local oscillators supplying the downconversion clocks.
% Hence, under these power consumption assumptions, at the onset of 5G standards, it was not considered that the digital beamforming architectures could even be practical and there was a lot of push towards doing beamforming in the analog RF domain, in order to prevent digitization of signals from each antenna required to perform the baseband digital beamforming. 
% In this process, these analog beamforming approaches add circuit elements like phase shifters, which contribute to a lot of insertion losses requiring increased LNA power consumption.
% Further these phase shifters have limited precision, and they are not wideband, which limits the total beamforming gains.
% Also analog architectures by themselves do not offer spatial multiplexing possibilities, requiring sophisticated directional MAC algorithms.

% However, as the technology evolves, it has actually become evident that ADC/DAC power consumption is going to go lower and has dropped considerably in the past few years itself \cite{yan2019performance}.
% Also, ADC/DAC power consumption is flexible, it can be further reduced by reducing the number of quantization bits on demand.
% Further, looking at the tradeoffs introduced by the analog beamforming; heavy insertion losses+sophisticated MAC algorithms, digital beamforming architectures have started becoming more preferred again, with multiple previous work even reporting the competitiveness of today's digital beamformers over analog in terms of power consumption \cite{barati2020energy,yan2019performance,dutta2019case,abdelghany2018towards,DOOSTMOHAMMADY2021107870}; at the same time preserving the flexibilities and spatial multiplexing possibilities offered by the digital architectures. 

% \subsection{Current system drawbacks and how \name addresses these}
% However, the digital beamformers of today are still facing two problems, first, the power consumption and technical difficulties of laying a synchronized downconversion LO distribution, and second, design of a flexible hybrid architecture which optimizes the amount of data backhauled and required signal processing.
% \name gives a solution to both these problems, and paves the way ahead for a new class of beamforming approaches; delivering robust spatial multiplexing gains while being both, spectrum efficient and power efficient.

% For the first problem, \name uses just a single physical RF chain, thus circumventing the LO distribution issues.
% Infact, studies show that the total power consumption of a synchronized distributed LO network is higher than that of ADCs/DACs \cite{yan2019performance}.
% Worse, given that there is an increasing trend towards moving higher frequencies, mmWave and THz bands, and the LO distribution problem is only going to become more challenging as our hardware advances.
% Instead of distributing these high frequency LO clocks, the clocks given to the RF switches in \name design are of the order of the signal bandwidth, and not carrier frequencies. 
% Thus, \name architecture is well adapt to next generation communication technologies.

% Second, it has been well acknowledged that to serve $N$ users reliably, massive MIMO required $N_{\text{ant}}>N$ antennas, and thus the total ADC sampling is going to be larger than number of users, with traditional massive MIMO architectures.
% Ideally, we should be sampling only $N$ users streams, but here we end up sampling $N_{\text{ant}}$ streams, which leads to increased ADC power consumption and more importantly, the digital signal processing is now working on higher number of samples; requiring much higher data rates to handle the huge amount of data generated via massive MIMO just to serve $N$ users \cite{yan2019performance,ding2020agora}.

% Hybrid analog-digital architectures attempt to address this problem, by laying an network of phase shifters and combiners which connect a larger number of $N_{\text{ant}}$ antennas to $N$ RF chains, and use analog beamforming to combine the $N_{\text{ant}}$ streams into $N$ sampled streams. Essentially, they project the larger number of $N_{\text{ant}}$ dimensions to create effective $N$ dimensional channels such that the $N$ users can get decoded.
% However, these architectures still end up wasting a lot of power in dealing with insertion losses from phase shifters, working with phase shifter quantization issues amongst the others.
% Further, these architectures are inflexible; when number of users reduce they still end up burning power in the set up physical RF chains.
% In comparison, \name architecture hybridizes easily, since all antennas are by default connected to the virtual RF chains, making it easier to just keep on adding antennas without worrying about fixed analog circuitry.
% \name also is a flexible architecture, when number of users reduce, we just reduce number of virtual RF chains on the fly.
% As compared to phase shifters, which have insertion losses around 10 dB, switches have minimal insertion losses, about just 0.5-1 dB which is minimal and does not increase burden on the LNA's.








%People want flexible solutions; in gen comm
%MIMO going reverse way
%Trends of softwarization: 

==> conclusion/scal_bk.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={Number of Users},
ymin=0,
ymax=9000,
ylabel style={font=\color{white!15!black}},
ylabel={Power Requirement (mW)},
axis background/.style={fill=white},
legend style={at={(0.01,0.504)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize},
ylabel shift={-4pt}
]
\addplot [color=mycolor1, line width=4.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
4	349.876966085977\\
8	673.876966085977\\
12	997.876966085977\\
16	1321.87696608598\\
20	1645.87696608598\\
24	1969.87696608598\\
28	2293.87696608598\\
32	2617.87696608598\\
36	2941.87696608598\\
40	3265.87696608598\\
44	3589.87696608598\\
48	3913.87696608598\\
};
\addlegendentry{K antenna TIMO}

\addplot [color=mycolor2, line width=4.0pt, mark=asterisk, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
4	463.507864343909\\
8	927.015728687819\\
12	1390.52359303173\\
16	1854.03145737564\\
20	2317.53932171955\\
24	2781.04718606346\\
28	3244.55505040736\\
32	3708.06291475127\\
36	4171.57077909518\\
40	4635.07864343909\\
44	5098.586507783\\
48	5562.09437212691\\
};
\addlegendentry{K antenna digital}

\addplot [color=mycolor3, dotted, line width=4.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
4	723.507864343909\\
8	1447.01572868782\\
12	2170.52359303173\\
16	2894.03145737564\\
20	3617.53932171955\\
24	4341.04718606346\\
28	5064.55505040737\\
32	5788.06291475127\\
36	6511.57077909518\\
40	7235.07864343909\\
44	7958.586507783\\
48	8682.09437212691\\
};
\addlegendentry{2K antenna hybrid}

\addplot [color=mycolor4, dotted, line width=4.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
4	353.876966085977\\
8	681.876966085977\\
12	1009.87696608598\\
16	1337.87696608598\\
20	1665.87696608598\\
24	1993.87696608598\\
28	2321.87696608598\\
32	2649.87696608598\\
36	2977.87696608598\\
40	3305.87696608598\\
44	3633.87696608598\\
48	3961.87696608598\\
};
\addlegendentry{2K antenna TIMO}

\addplot [color=black, dashdotted, line width=4.0pt]
  table[row sep=crcr]{%
4	320\\
8	640\\
12	960\\
16	1280\\
20	1600\\
24	1920\\
28	2240\\
32	2560\\
36	2880\\
40	3200\\
44	3520\\
48	3840\\
};
\addlegendentry{K streams ADC power}

\end{axis}

\begin{axis}[%
width=1.227\figurewidth,
height=1.227\figureheight,
at={(-0.16\figurewidth,-0.135\figureheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize}
]
\end{axis}
\end{tikzpicture}%

==> conclusion/scal_discuss.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={Number of Users},
ymin=0,
ymax=10000,
ylabel style={font=\color{white!15!black}},
ylabel={Power Requirement (mW)},
axis background/.style={fill=white},
legend style={at={(0.02,0.484)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize},
ylabel shift={-4pt}
]

\addplot [color=mycolor3, dotted, line width=1.5pt, mark=diamond, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
4	784.04890956485\\
8	1568.0978191297\\
12	2352.14672869455\\
16	3136.1956382594\\
20	3920.24454782425\\
24	4704.2934573891\\
28	5488.34236695395\\
32	6272.3912765188\\
36	7056.44018608365\\
40	7840.4890956485\\
44	8624.53800521335\\
48	9408.5869147782\\
};
\addlegendentry{2K antenna hybrid}


\addplot [color=mycolor2, dotted, line width=1.5pt, mark=asterisk, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
4	524.04890956485\\
8	1048.0978191297\\
12	1572.14672869455\\
16	2096.1956382594\\
20	2620.24454782425\\
24	3144.2934573891\\
28	3668.34236695395\\
32	4192.3912765188\\
36	4716.44018608365\\
40	5240.4890956485\\
44	5764.53800521335\\
48	6288.5869147782\\
};
\addlegendentry{K antenna digital}


\addplot [color=mycolor4, dotted, line width=1.5pt, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
4	385.012227391213\\
8	729.012227391213\\
12	1073.01222739121\\
16	1417.01222739121\\
20	1761.01222739121\\
24	2105.01222739121\\
28	2449.01222739121\\
32	2793.01222739121\\
36	3137.01222739121\\
40	3481.01222739121\\
44	3825.01222739121\\
48	4169.01222739121\\
};
\addlegendentry{2K antenna TIMO}

\addplot [color=mycolor1, dotted, line width=1.5pt, mark=x, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
4	365.012227391213\\
8	689.012227391213\\
12	1013.01222739121\\
16	1337.01222739121\\
20	1661.01222739121\\
24	1985.01222739121\\
28	2309.01222739121\\
32	2633.01222739121\\
36	2957.01222739121\\
40	3281.01222739121\\
44	3605.01222739121\\
48	3929.01222739121\\
};
\addlegendentry{K antenna TIMO}

\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
4	300\\
8	620\\
12	940\\
16	1260\\
20	1580\\
24	1900\\
28	2220\\
32	2540\\
36	2860\\
40	3180\\
44	3500\\
48	3820\\
};
\addlegendentry{ADC with K streams}

\end{axis}

\begin{axis}[%
width=1.227\figurewidth,
height=1.227\figureheight,
at={(-0.16\figurewidth,-0.135\figureheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize}
]
\end{axis}
\end{tikzpicture}%

==> conclusion/scal_discuss_sajjad.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={\textbf{Number of Users (K)}},
ymin=0,
ymax=10000,
ylabel style={font=\color{white!15!black}},
ylabel={\textbf{Power Requirement (mW)}},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.01,0.54)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
nodes={scale=0.9, transform shape},
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize},
ylabel shift={-4pt},
xlabel shift={-4pt}
]

\addplot [color=mycolor3, dotted, line width=1.5pt, mark=diamond, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
4	784.04890956485\\
8	1568.0978191297\\
12	2352.14672869455\\
16	3136.1956382594\\
20	3920.24454782425\\
24	4704.2934573891\\
28	5488.34236695395\\
32	6272.3912765188\\
36	7056.44018608365\\
40	7840.4890956485\\
44	8624.53800521335\\
48	9408.5869147782\\
};
\addlegendentry{2K antenna hybrid}


\addplot [color=mycolor2, dotted, line width=1.5pt, mark=asterisk, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
4	524.04890956485\\
8	1048.0978191297\\
12	1572.14672869455\\
16	2096.1956382594\\
20	2620.24454782425\\
24	3144.2934573891\\
28	3668.34236695395\\
32	4192.3912765188\\
36	4716.44018608365\\
40	5240.4890956485\\
44	5764.53800521335\\
48	6288.5869147782\\
};
\addlegendentry{K antenna digital}


\addplot [color=mycolor4, dotted, line width=1.5pt, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
4	385.012227391213\\
8	729.012227391213\\
12	1073.01222739121\\
16	1417.01222739121\\
20	1761.01222739121\\
24	2105.01222739121\\
28	2449.01222739121\\
32	2793.01222739121\\
36	3137.01222739121\\
40	3481.01222739121\\
44	3825.01222739121\\
48	4169.01222739121\\
};
\addlegendentry{2K antenna TIMO}

\addplot [color=mycolor1, dotted, line width=1.5pt, mark=x, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
4	365.012227391213\\
8	689.012227391213\\
12	1013.01222739121\\
16	1337.01222739121\\
20	1661.01222739121\\
24	1985.01222739121\\
28	2309.01222739121\\
32	2633.01222739121\\
36	2957.01222739121\\
40	3281.01222739121\\
44	3605.01222739121\\
48	3929.01222739121\\
};
\addlegendentry{K antenna TIMO}

\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
4	300\\
8	620\\
12	940\\
16	1260\\
20	1580\\
24	1900\\
28	2220\\
32	2540\\
36	2860\\
40	3180\\
44	3500\\
48	3820\\
};

\addlegendentry{ADC with K streams}


%uncomment if require: \path (0,380); %set diagram left start at 0, and has height of 380

%Straight Lines [id:da056473852988744744] 

\addplot [color=red, line width=1.6pt]
  table[row sep=crcr]{%
40	5390\\
40	7590\\
};
\addplot [color=red,  line width=1.6pt]
  table[row sep=crcr]{%
39.2 7200\\
40	 7590\\
};

\addplot [color=red,  line width=1.6pt]
  table[row sep=crcr]{%
40.8 7200\\
40	 7590\\
};

\addplot [color=red,  line width=1.6pt]
  table[row sep=crcr]{%
40.8 5780\\
40	 5390\\
};

\addplot [color=red,  line width=1.6pt]
  table[row sep=crcr]{%
39.2 5780\\
40	 5390\\
};

\addplot [color=green, line width=1.5pt]
  table[row sep=crcr]{%
41.5	3200\\
41.5	3800\\
};

\addplot [color=green, line width=1.1pt]
  table[row sep=crcr]{%
41.5	3220\\
41	    3350\\
};

\addplot [color=green, line width=1.1pt]
  table[row sep=crcr]{%
41.5	3220\\
42	    3350\\
};

\addplot [color=green, line width=1.1pt]
  table[row sep=crcr]{%
41.5	3780\\
41	    3550\\
};

\addplot [color=green, line width=1.1pt]
  table[row sep=crcr]{%
41.5	3780\\
42	    3550\\
};

% \draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (40,5382) -- (40,7800) ;

% \draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1]    (39.5,7200) -- (40,7800) ;

% \draw [shift={(40,28.43)}, rotate = 270] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% \draw [shift={(40,20.43)}, rotate = 90] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


\end{axis}

\begin{axis}[%
width=1.227\figurewidth,
height=1.227\figureheight,
at={(-0.16\figurewidth,-0.135\figureheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
xlabel style={font=\footnotesize},ylabel style={font=\footnotesize},legend style={font=\scriptsize},ticklabel style={font=\scriptsize}
]
\end{axis}
\end{tikzpicture}%

==> design/design.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
% Assuming till here time diversity has been motivated
\subsection{Creating temporal variations at increased IF bandwidth}
\noindent In any wireless network, it is assumed that the base station has to sample at twice the aggregate bandwidth occupied by the users transmission. Thus, a natural solution to increase the capacity would be to increase this bandwidth by getting more spectrum. However, this requires change in standards, as well as tedious issues in procuring more spectrum from FCC.

In order to further increase the network capacity, \name makes a key observation. The problem at hand with current networks is not that each user wants more bandwidth, but that the net bandwidth which gets added up as the number of users increase exacerbates the requirements. Thus, in order to skirt around the issues of  procuring extra over the air bandwidth, we ask what if we can increase the IF bandwidth at the base station, and perform time multiplexing with the extra sub-sample time slots created in the process. This way, we utilize the full intended benefit of increased bandwidth, without actually increasing the RF bandwidth.

So, what are the key changes required to harness this higher IF bandwidth for multi-user settings? First and foremost, the ADCs need to sample faster, to support an increased IF bandwidth, and this is the easiest modification required, since anyways, these ADC's were overdesigned and already performing sampling at a higher rate, albeit to alleviate the discontinuities in OFDM packets by interpolating and oversampling. This leads to increased SNR and reduced non-idealities like PAPR among others. However, the key challenge here is how to actually use this increased sampling capability to fit in data of multiple users? That is, say if we increase the IF bandwidth $K$ times, and thus the ADC samples $K$times faster, can we fit in the $K$ users data streams in this increased capability?

\name's key insight here, to utilize these ADCs higher sampling rate for multi-user support is to create local IF changes in the wireless channel, which emulate the user transmissions themselves to be with increased bandwidth.
To create these changes, we need to introduce a circuit element which can introduce this dynamicness, as fast as the ADC can sample.
The fastest and the most intuitive way to do this would be to toggle the RF chain on and off at the sampling rate, using RF switches, effectively multiplying the received signal having reduced bandwidth B, with a 0-1 code of increased bandwidth $KB$, where $K$ is the factor by which the ADC oversamples.
As compared to $K$ users each having bandwidth $B$ occupying different parts of the whole $KB$ RF spectrum, when we increase only the IF bandwidth to $KB$, each users signal also gets multiplied by the same 0-1 $KB$ bandwidth code, and hence all the $K$ users interfere in the increased $KB$ bandwidth. So, how do we solve for this created interference, without actually increasing the RF bandwidth.

\subsection{Supplementing the increased bandwidth with a single wire antenna array}

A major challenge to utilizing the increased $KB$ IF bandwidth in order to read data from $K$ $B$ bandwidth users, is to handle the interference caused because all the $K$ users actually occupy the same $B$ bandwidth RF spectrum. To counter this interference, \name comes up with a unique solution, where we create a single wire antenna array, which allows us to use the increased dimensionality due to dealing with multiple antennas, in order to cancel out the interference. Traditional methods to do this involve digital beamforming, which need one RF chain for each antenna. In comparison, \name's antenna array just needs one RF chain, with the outputs of the antennas combined into a single RF chain.

That is, in order to handle the interference due to $K$ users transmitting simultaneously, \name's antenna array consists of $K$ antennas, all combined to a single RF chain with a wilkinson network.
But, in that case, if the antennas outputs are combined to one RF chain, how do we actually use the gains entitled by using multiple antennas? 
This is where our increased IF bandwidth comes to the rescue. 
We augment our antenna array design to combine across $K$ `switched-antennas' instead of just normal antennas.
By `switched-antenna', we mean that each antenna is connected to a RF switch which toggles this antenna on-off, with the switched output being the input to the combining network (Fig.), 
% and the $K$ antennas with $K$ RF switches are then combined to a single wire interface with a wilkinson network.
The intuiton we have here is that the $KB$ wideband code applied to the received $B$ bandwidth signals, allows us to isolate the signals from each of the $K$ switched-antennas.

To see how this switched-antenna RF chain behaves, we model the scenario mathematically, with the $K$ users transmitting signals $x_{1,2,\ldots K}(t)$, and the complex time-invariant channel seen by user $i$ to the $j$-th antenna represented as $h_{ij}$. We consider that the $j-th$ antenna toggles on-off with a bit sequence $b_j(t)$ via the RF switch, where $b_j(t) \in \{0,1\}$. The combined received signal $y(t)$ across the $K$ switched antennas with $K$ users interfering, can be represented as:

\begin{equation}
    y(t) = \sum_{i=1}^K \sum_{j=1}^K (h_{ij}*x_i(t))\cdot b_j(t)
\label{eqn:combined_codes}
\end{equation}

This combined signal $y(t)$ goes through downconversion, and then ADC sampling at $KB$ to get sampled baseband signal

\begin{equation}
    Y[n] \equiv y(nT_s) = \sum_{i=1}^K \sum_{j=1}^K (h_{ij}*X_i[n])\cdot B_j[n]
\label{eqn:combined_codes}
\end{equation}

Now, to isolate the signal from $j$-th antenna, we choose the codes $B_{1,2,\ldots K}[n]$ such that $B_{j_1}[n]\cdot B_{j_2}[n] = 0$ if $j_1 \neq j_2$. For example, these codes can be identity codes, say $K=4$, for which the IF bandwidth quadruples, and we choose $B_1[n] = [1,0,0,0]_n$, $B_2[n] = [0,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,0,1]_n$, where $[\cdot]_n$ shows that the code gets repeated, that is $B_1[n] = 1,0,0,0,1,0,0,0,\ldots$.
Such codes allow us to isolate the signals from the individual antennas, since multiplying $Y[n]$ with a self copy of the code, sets all other codes to 0, since,

\begin{equation}
\begin{split}
Y[n]\cdot B_j[n] &= \sum_{i=1}^K \sum_{j'=1}^K (h_{ij'}*X_i[n]))\cdot (B_{j'}[n]\cdot B_j[n])\\
                &= \sum_{i=1}^K (h_{ij}*X_i[n])B_{j}[n]
\end{split}
\label{eqn:isolated_codes}    
\end{equation}

Thus, $Y[n]\cdot B_j[n]$ does not have any contribution from any other antenna, apart from antenna $j$, which allows us to use the $K$ $h_{ij}$ channels from each $K$ users to the $j$-th antenna. Further, multiplying with $B_j[n]$ appropriately downsamples the $KB$ bandwidth $Y[n]$ to useful $B$ bandwidth $Y_j[n]$, where we get $Y_j[n]$ by removing the zeros from $Y[n]\cdot B_j[n]$. For example, when $K=4$ and identity codes as described before,
$Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$.

This allows us to obtain the $4$ channels $h_{i1}, h_{i2}, h_{i3}, h_{i4}$ for each of the $i$-th user, from $Y_1[n],Y_2[n],Y_3[n],Y_4[n]$ respectively, even if the outputs from the 4 switched antennas were combined into a single stream $Y[n]$.
% This gives another requirement for the increased IF bandwidth to serve multi-user scenarios, that is to disambiguate this interference, we need to have increased antennas, so that we can combine across the antenna streams and cancel out the interference from each other. 
% A challenge here is to do so without actually increasing the number of RF chains, since otherwise the solution will not be scalable and useful.
% Thus, \name comes up with a creative solution, where we combine signals from multiple antennas into one combined RF chain, effectively utilizing the increased antenna space dimensionality to cancel interference, and using just one RF chain in the process. 
% However, this is not enough, since 
% Normally, wireless channels remain relatively stable over time, 
% and some reasoning for this is that the clients by-at-average don't
% move fast, and the sampling rate for receivers is reasonably high, 
% which allows the receivers to sample at a faster rate, which further 
% gives the sense that channels don't change much over multiple samples.

% So, how do we create dynamicness in the channel, which allows opportunities 
% to tap in the time diversity. The key 
\subsection{Time combining to suppress interference}
Now that we have used the codes to isolate the signals from each antenna, we have shown how a single wire antenna array can be used with increased bandwidth IF codes without losing down on channels of each antenna. This draws a parallel to how in a normal digital beamforming system, we get channels per each RF chain from a single antenna. So the next natural question arises, if we can use these individual channels to do beamforming with this extra time varying diveristy introduced because of fast sampling and RF switch coding?

Recall that in a $K$-user, $K$-antenna setting, the sampled signal associated with antenna $j$ is denoted as, $Y_j[n] =  Y[Kn+1] = \sum_{i=1}^K h_{ij}*X_i[Kn+j-1]$. In order to sucessfully combine across $Y_{1,2\ldots K}[n]$, we need to co-phase them, that is, we need to delay the signals so that each stream has the same temporal signal $X_i[\cdot]$. That is, we delay 
\begin{equation}
Y^{\mathcal{D}}_{j}[n] = \mathcal{D}(Y_j[n], K-j) =  \sum_{i=1}^K h_{ij}*X_i[Kn+K-1]    
\end{equation}

The delay can be implemented using $\text{delayseq}(\cdot)$ function, which applies this fractional delay in the frequency domain. 
Because we oversample $K$ times anyways, this delay operation is exact as per the Shannon-Nyquist theorem, and we do not loose any information with $X_i[n]$ since we assume $X_i[n]$ is $B$ bandwidth.
Now, all $Y^{\mathcal{D}}_{1,2\ldots K}$ have the same input signal $X_i[Kn+K-1]$, which allows us to combine across these signals, similar to how we traditionally combine across signals from multiple RF chains. 
Further, we can re-write the comvolution as a multiplication by taking fourier transform of $Y^{\mathcal{D}}_{1,2\ldots K}$. This allows for a matrix representation,

\begin{equation}
\begin{bmatrix}
 Y_1^{\mathcal{D}}(f) \\
 Y_2^{\mathcal{D}}(f)\\
 \cdot \\
 \cdot \\
 Y_K^{\mathcal{D}}(f)\\
\end{bmatrix}
=
\begin{bmatrix}
 H_{11}(f) & H_{21}(f) & \cdot & \cdot & H_{K1}(f)\\
 H_{12}(f) & H_{22}(f) & \cdot & \cdot & H_{K2}(f)\\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 H_{1K}(f) & H_{2K}(f) & \cdot & \cdot & H_{KK}(f)\\
 \end{bmatrix}
 \begin{bmatrix}
 X_1(f) \\
 X_2(f)\\
 \cdot \\
 \cdot \\
 X_K(f)\\
\end{bmatrix}
\label{eqn:expanded_matrx}
\end{equation}

which we can write in shorthand as $\mathbf{Y}=\mathbf{H}\mathbf{X}$, where $\mathbf{Y}$ is the $K\times 1$ column obtained by stacking the $K$ different delayed streams, $\mathbf{H}$ is the $K\times K$ channel matrix, with $H_{ij}$ being channel from user $i$ to antenna $j$, and $\mathbf{X}$ being the column vector of the K users transmitted signal in frequency domain.

Now, to isolate signal of user $1$ from other users, we take the matrix $\mathbf{H}$ and remove the first column to get a $K-1 \times K$ matrix $\mathbf{H}_{1^{\_}}$, which because of reduced number of columns, will have a $K\times 1$ column-space null vector $\mathbf{N}_1$ belonging to the null space of the matrix $\mathbf{H}_{1^{\_}}$. When we take the inner product of the $K\times 1$ complex vectors, $\mathbf{N}_1$ with $\mathbf{Y}$, we see that

\begin{equation}
    \begin{split}
    R_1(f) &= \mathbf{N}_1\cdot \mathbf{Y} =\mathbf{N}_1 \cdot \begin{bmatrix} 
        \mathbf{H}_1\quad \mathbf{H}_{1^{\_}}
        \end{bmatrix}\\
        &=
        [\mathbf{N}_1\cdot\mathbf{H}_1\quad \mathbf{N}_1\cdot\mathbf{H}_{1^{\_}}]
        \mathbf{X}\\
        &= \begin{bmatrix} 
        \mathbf{N}_1 \cdot \mathbf{H}_1\quad \mathbf{0}_{K-1 \times K}
        \end{bmatrix}
        \mathbf{X}\\
        & = (\mathbf{N}_1\cdot \mathbf{H}_1)X_1(f)
    \end{split}    
\end{equation}

since $\mathbf{N}_1$ will null out the $\mathbf{H}_{1^{\_}}$ sub-matrix. Thus, using the vector $\mathbf{N}_1$ to combine across the $K$ delayed sample vector $\mathbf{Y}$ we can null out all other users apart from user 1, and hone onto the signal from user 1. Note that we can generate such nulling vectors for all the $K$ users, since there is nothing special about the user 1. Thus we can get $\mathbf{N}_{1,2,\ldots K}$ for all the $K$ users, from the null spaces of appropriate matrices $\mathbf{H}_{j^{\_}}$ by removing the $j$-th column associated to $j$-th user. Thus, we can get the vector $\mathbf{R}(f) = {\begin{bmatrix}
 R_1(f) 
 R_2(f)
 \cdot 
 \cdot 
 R_K(f)
\end{bmatrix}}^T$, such that

\begin{equation}
\begin{split}
\mathbf{R}(f) &= [\mathbf{N}_1 \mathbf{N}_2 \cdot \cdot \mathbf{N}_K ] \cdot Y  \\
& = \begin{bmatrix}
 \mathbf{N}_1\cdot \mathbf{H}_1 & 0 & \cdot & \cdot & 0\\
 0 & \mathbf{N}_2\cdot \mathbf{H}_2 & \cdot & \cdot & 0\\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 0 & 0 & \cdot & \cdot &  \mathbf{N}_K\cdot \mathbf{H}_K \\
 \end{bmatrix}
 \begin{bmatrix}
 X_1(f) \\
 X_2(f)\\
 \cdot \\
 \cdot \\
 X_K(f)\\
\end{bmatrix}
\end{split}
\end{equation}
% \begin{split}

Since here, the vector $\mathbf{R}$ is a product of diagonal matrix and the vector having signals of all the $K$-users, using just a single RF chain with $K$ switched antennas, and the ADC, RF switches toggling at $KB$ rate, we can get data of $K$ users each having over the air bandwidth of $B$.

\subsection{Spatio-temporal combining}

The above analysis to get $K$ users data from one RF chains can be further generalized when there are multiple $S$ different RF chains. Usually, when we have $S$ RF chains, it is assumed that the design can serve $S$ interfering users simultaneously. However, with the $K$ times increased local IF bandwidth, we can actually even increase the number of users to $S\times K$. 

Since now we need to serve $SK$ users, we would need to combine in $SK$ dimensions, and thus we have $SK$ number of switched antennas per RF chain (Fig.). In this scenario, from a single RF chain, we can only get $K\times 1$ vector $\mathbf{Y}^s$ from the $K$ number of orthogonal codes we can design when we increase the IF bandwidth $K$ times, however, we need to serve $SK$ users. The first key insight which we make here, is that now instead of using the identity codes, we will turn multiple antennas on simultaneously, and thus, the channels which we measure with the $K$

% To do so, we need to have $SK$ number of antennas, and in the multi RF chain setting, these $SK$ antennas are mapped to $S$ RF chains, instead of just $1$ RF chain. That is, there are $S$ different combiner networks, each combining $SK$ antennas with $SK$ RF switches to a single RF chain (Fig. ). Thus, in this scenario, we will have $S^2K$ number of RF switches, so that we can have $S$ different combiner networks for the $SK$ antennas.

% Considering that now we will get $K\times 1$ vector $\mathbf{Y}^{s}$ from the $s$-th RF chain, we can model it similar to the previous analysis and write it as $\mathbf{Y}^{s} = \mathbf{H}\mathbf{X}$, however, here $\mathbf{H}$ is $SK\times SK$, and $\mathbf{X}$ is $SK \times 1$. Thus, the null space vector here will be $SK\times 1$, and thus it is not enough to combine it with the $K\times 1$ vector $Y^s$

% \noindent Antenna Switching creates artificial time-faded channels -> \\
% Combined with oversampling creates virtual RF chains with separate channels across time->\\
% More antennas allows existance of null spaces ->\\
% Wideband null space combining cancels interference\\

% For example, when $K=4$ and identity codes as described before,
% $Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$. In general, if we do not have these identity codes, that is, say $B_1[n] = [1,0,0,1]_n$, $B_2[n] = [1,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,1,1]_n$, we will observe $h_{i1}+h_{i2}, h_{i2}, h_{i3}+h_{i4}, h_{i4}+h_{i1}$ on the 4 delayed streams. Thus, the measured channels are actually matrix multiplication of the $K\times K$ channel matrix , $\mathbf{H} = [h_1 h_2 h_3 h_4]$, with $K\times K$ code matrix 
% $\mathbf{B} = \begin{bmatrix} 
% B_1
% B_2
% B_3
% B_4
% \end{bmatrix}^T$ $\mathbf{H}\cdot \mathbf{B}$. If we choose codes such that $\mathbf{B}$ is invertible, we can estimate the $K$ antenna channels simultaneously 

==> design/design2.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
% Assuming till here time diversity has been motivated
\subsection{Creating temporal variations at increased IF bandwidth}
\noindent In any wireless network, it is assumed that the base station has to sample at twice the aggregate bandwidth occupied by the users transmission. Thus, a natural solution to increase the capacity would be to increase this bandwidth by getting more spectrum. However, this requires change in standards, as well as tedious issues in procuring more spectrum from FCC.

In order to further increase the network capacity, \name makes a key observation. The problem at hand with current networks is not that each user wants more bandwidth, but that the net bandwidth which gets added up as the number of users increase exacerbates the requirements. Thus, in order to skirt around the issues of  procuring extra over the air bandwidth, we ask what if we can increase the IF bandwidth at the base station, and perform time multiplexing with the extra sub-sample time slots created in the process. This way, we utilize the full intended benefit of increased bandwidth, without actually increasing the RF bandwidth.

So, what are the key changes required to harness this higher IF bandwidth for multi-user settings? First and foremost, the ADCs need to sample faster, to support an increased IF bandwidth, and this is the easiest modification required, since anyways, these ADC's were overdesigned and already performing sampling at a higher rate, albeit to alleviate the discontinuities in OFDM packets by interpolating and oversampling. This leads to increased SNR and reduced non-idealities like PAPR among others. However, the key challenge here is how to actually use this increased sampling capability to fit in data of multiple users? That is, say if we increase the IF bandwidth $K$ times, and thus the ADC samples $K$times faster, can we fit in the $K$ users data streams in this increased capability?

\name's key insight here, to utilize these ADCs higher sampling rate for multi-user support is to create local IF changes in the wireless channel, which emulate the user transmissions themselves to be with increased bandwidth.
To create these changes, we need to introduce a circuit element which can introduce this dynamicness, as fast as the ADC can sample.
The fastest and the most intuitive way to do this would be to toggle the RF chain on and off at the sampling rate, using RF switches, effectively multiplying the received signal having reduced bandwidth B, with a 0-1 code of increased bandwidth $KB$, where $K$ is the factor by which the ADC oversamples.
As compared to $K$ users each having bandwidth $B$ occupying different parts of the whole $KB$ RF spectrum, when we increase only the IF bandwidth to $KB$, each users signal also gets multiplied by the same 0-1 $KB$ bandwidth code, and hence all the $K$ users interfere in the increased $KB$ bandwidth. So, how do we solve for this created interference, without actually increasing the RF bandwidth.

\subsection{Supplementing the increased bandwidth with a single wire antenna array}

A major challenge to utilizing the increased $KB$ IF bandwidth in order to read data from $K$ interfering users having the same $B$ bandwidth. That is, we need to handle the interference caused because all the $K$ users actually occupy the same $B$ bandwidth RF spectrum. To counter this interference, \name comes up with a unique solution, where we create a single wire antenna array, which allows us to use the increased dimensionality due to dealing with multiple antennas, in order to cancel out the interference. Traditional methods to do this involve digital beamforming, which need one RF chain for each antenna. In comparison, \name's antenna array just needs one RF chain, with the outputs of the antennas combined into a single RF chain.

That is, in order to handle the interference due to $K$ users transmitting simultaneously, \name's antenna array consists of $K$ antennas, all combined to a single RF chain with a wilkinson network.
But, in that case, if the antennas outputs are combined to one RF chain, how do we actually use the gains entitled by using multiple antennas? 
This is where our increased IF bandwidth comes to the rescue. 
We augment our antenna array design to combine across $K$ `switched-antennas' instead of just normal antennas.
By `switched-antenna', we mean that each antenna is connected to a RF switch which toggles this antenna on-off, with the switched output being the input to the combining network (Fig. \ref{fig:digital_vs_name}), 
% and the $K$ antennas with $K$ RF switches are then combined to a single wire interface with a wilkinson network.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/arch1.pdf}
    \caption{\name vs traditional digital beamformers}
    \label{fig:digital_vs_name}
\end{figure}
The intuiton we have here is that the $KB$ wideband code applied to the received $B$ bandwidth signals, allows us to isolate the signals from each of the $K$ switched-antennas.

To see how this switched-antenna RF chain behaves, we model the scenario mathematically, with the $K$ users transmitting signals $x_{1,2,\ldots K}(t)$, and the complex time-invariant channel seen by user $i$ to the $j$-th antenna represented as $h_{ij}$. We consider that the $j-th$ antenna toggles on-off with a bit sequence $b_j(t)$ via the RF switch, where $b_j(t) \in \{0,1\}$. The combined received signal $y(t)$ across the $K$ switched antennas with $K$ users interfering, can be represented as:

\begin{equation}
    y(t) = \sum_{i=1}^K \sum_{j=1}^K (h_{ij}*x_i(t))\cdot b_j(t)
\label{eqn:combined_codes}
\end{equation}

This combined signal $y(t)$ goes through downconversion, and then ADC sampling at $KB$ to get sampled baseband signal

\begin{equation}
    Y[n] \equiv y(nT_s) = \sum_{i=1}^K \sum_{j=1}^K (h_{ij}*X_i[n])\cdot B_j[n]
\label{eqn:combined_codes}
\end{equation}

Now, since we oversample $K$ times, we have $K$ sub-sampled time slots in one data-slot of $X_i$. 
Thus, to isolate the $K$ antenna channels, we utilize these sub-sampled time slot and leverage smart design of $B_j[n]$.
For an example, consider $K=4$, and we design $B_1[n] = [1,0,0,0]_n$, where $_n$ indicates that the code gets repeated, that is $B_1[n]=1,0,0,0,1,0,0,0\ldots$. 
So with this code design, the first antenna is `on' for every `4n+1' samples.
Similarly, say $B_2[n] = [0,1,0,0]_n, B_3[n] = [0,0,1,0]_n, B_4[n] = [0,0,0,1]_n$, such that no other antenna is `on' for the $(4n+1)$-th samples.
Now, when we evaluate $Y[4n+1]$, we get

\begin{equation}
\begin{split}
    Y[4n+1] &= \sum_{i=1}^4 \sum_{j=1}^4 (h_{ij}*X_i[4n+1]))\cdot B_{j}[4n+1] \\
            &= \sum_{i=1}^4 (h_{i1}*X_i[4n+1]))\\
\end{split}
\label{eqn:identity}
\end{equation}

since $B_1[4n+1] = 1$, whereas $B_{2,3,4}[4n+1]=0$. 
Observe that, $Y[4n+1]$ does not have any contribution from any other antenna, apart from antenna $1$, which allows us to use the $K$ $h_{i1}$ channels from each $K$ users to the $1$-st antenna.
We can get channels to antennas $2,3,4$ in similar way by observing $Y[4n+2], Y[4n+3], Y[4n+4]$ respectively.

More generally, $Y_1[n] \equiv Y[4n+1]$, captures the antennas which were toggled `on' for the $4n+1$ samples, that is if $B_1[n] = [1,0,0,1]_n, B_2[n] = [1,1,0,0]_n, B_3[n] = [0,0,1,0]_n, B_4[n] = [0,1,1,1]_n$, $Y[4n+1]$ will observe $h_{i1}+h_{i2}$ since antennas 1,2 were `on' for 4n+1 samples, and $Y[4n+2], Y[4n+3], Y[4n+4]$ will observe $h_{i2}+h_{i4}, h_{i3}+h_{i4}, h_{i1}+h_{i4}$ respectively.  Hence, we can modify \eqref{eqn:identity} as
\begin{equation}
Y[4n+j] = \sum_{i=1}^4 (\sum_{k=1}^K (h_{ik}b_{kj}))*X_i[4n+j])\\
\label{eqn:identity}
\end{equation}
where $k$ sums over the $K$ antennas and their on-off states for $4n+j$ samples $b_{kj}$, and this is similar to dot product of two vectors $\mathbf{h}_k$ and $\mathbf{b}_k$. 
Thus, we can write the codes in a $4\times 4$ matrix $\mathbf{B} = [B_1 B_2 B_3 B_4]$, $i$-th column denotes the on-off code for antenna $i$, the $j$-th row represents which antenna was on for $Y[4n+j]$ sample, and similarly the channels as a $4\times 4$ matrix $\mathbf{H} = [\mathbf{h}_{1} \mathbf{h}_{2} \mathbf{h}_{3} \mathbf{h}_{4}]^T$, where each row $\mathbf{h}_{i}$ denotes the $4\times 1$ vector of all $4$ users channel with antenna $i$.

Thus, combinedly, 
$Y[4n+1], Y[4n+2], Y[4n+3], Y[4n+4]]$ are associated with channels $\mathbf{H}\cdot\mathbf{B}$, and if the matrix $\mathbf{B}$ is invertible, we can estimate the individual channels from the single wire oversampled $Y[n]$. More simply, $\mathbf{B}$ can be chosen as identity matrix, as in the simplest example described before, and the codes can be different later on to get constructive combining gains by adding up in-phase antennas. To generalize now to $K$ users, we represent $Y[Kn+j]$, as $Y_j[n] \equiv Y[Kn+j]$, which give channels $\mathbf{H}\cdot\mathbf{B}$.
This allows us to obtain the $K$ channels $h_{i1}, h_{i2}, \ldots, h_{iK}$ for each of the $i$-th user and all the $K$ antennas, from $Y_1[n],Y_2[n],\ldots,Y_K[n]$ respectively, even if the outputs from the $K$ switched antennas were combined into a single stream $Y[n]$.

% Now, to isolate the signal from $j$-th antenna, we choose the codes $B_{1,2,\ldots K}[n]$ such that $B_{j_1}[n]\cdot B_{j_2}[n] = 0$ if $j_1 \neq j_2$. For example, these codes can be identity codes, say $K=4$, for which the IF bandwidth quadruples, and we choose $B_1[n] = [1,0,0,0]_n$, $B_2[n] = [0,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,0,1]_n$, where $[\cdot]_n$ shows that the code gets repeated, that is $B_1[n] = 1,0,0,0,1,0,0,0,\ldots$.
% Such codes allow us to isolate the signals from the individual antennas, since multiplying $Y[n]$ with a self copy of the code, sets all other codes to 0, since,

% \begin{equation}
% \begin{split}
% Y[n]\cdot B_j[n] &= \sum_{i=1}^K \sum_{j'=1}^K (h_{ij'}*X_i[n]))\cdot (B_{j'}[n]\cdot B_j[n])\\
%                 &= \sum_{i=1}^K (h_{ij}*X_i[n])B_{j}[n]
% \end{split}
% \label{eqn:isolated_codes}    
% \end{equation}

% Thus, $Y[n]\cdot B_j[n]$ does not have any contribution from any other antenna, apart from antenna $j$, which allows us to use the $K$ $h_{ij}$ channels from each $K$ users to the $j$-th antenna. Further, multiplying with $B_j[n]$ appropriately downsamples the $KB$ bandwidth $Y[n]$ to useful $B$ bandwidth $Y_j[n]$, where we get $Y_j[n]$ by removing the zeros from $Y[n]\cdot B_j[n]$. For example, when $K=4$ and identity codes as described before,
% $Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$.

% This allows us to obtain the $4$ channels $h_{i1}, h_{i2}, h_{i3}, h_{i4}$ for each of the $i$-th user, from $Y_1[n],Y_2[n],Y_3[n],Y_4[n]$ respectively, even if the outputs from the 4 switched antennas were combined into a single stream $Y[n]$.
% This gives another requirement for the increased IF bandwidth to serve multi-user scenarios, that is to disambiguate this interference, we need to have increased antennas, so that we can combine across the antenna streams and cancel out the interference from each other. 
% A challenge here is to do so without actually increasing the number of RF chains, since otherwise the solution will not be scalable and useful.
% Thus, \name comes up with a creative solution, where we combine signals from multiple antennas into one combined RF chain, effectively utilizing the increased antenna space dimensionality to cancel interference, and using just one RF chain in the process. 
% However, this is not enough, since 
% Normally, wireless channels remain relatively stable over time, 
% and some reasoning for this is that the clients by-at-average don't
% move fast, and the sampling rate for receivers is reasonably high, 
% which allows the receivers to sample at a faster rate, which further 
% gives the sense that channels don't change much over multiple samples.

% So, how do we create dynamicness in the channel, which allows opportunities 
% to tap in the time diversity. The key 
\subsection{Time combining to suppress interference}
Now that we have used the codes to isolate the signals from each antenna, we have shown how a single wire antenna array can be used with increased bandwidth IF codes without losing down on channels of each antenna. This draws a parallel to how in a normal digital beamforming system, we get channels per each RF chain from a single antenna. So the next natural question arises, if we can use these individual channels to do beamforming with this extra time varying diveristy introduced because of fast sampling and RF switch coding?

Recall that in a $K$-user, $K$-antenna setting, the sampled signal associated with antenna $j$ is denoted as, $Y_j[n] =  Y[Kn+1] = \sum_{i=1}^K \sum_{k=1}^{K}(h_{ik}b_{kj})*X_i[Kn+j]$. In order to sucessfully combine across $Y_{1,2\ldots K}[n]$, we need to co-phase them, that is, we need to delay the signals so that each stream has the same temporal signal $X_i[\cdot]$. That is, we delay 
\begin{equation}
Y^{\mathcal{D}}_{j}[n] = \mathcal{D}(Y_j[n], K-j) =  \sum_{i=1}^K \sum_{k=1}^K(h_{ij}b_{kj})*X_i[Kn+K]    
\end{equation}

The delay can be implemented using $\text{delayseq}(\cdot)$ function, which applies this fractional delay in the frequency domain. 
Because we oversample $K$ times anyways, this delay operation is exact as per the Shannon-Nyquist theorem, and we do not loose any information with $X_i[n]$ since we assume $X_i[n]$ is $B$ bandwidth.
Now, all $Y^{\mathcal{D}}_{1,2\ldots K}$ have the same input signal $X_i[Kn+K]$, which allows us to combine across these signals, similar to how we traditionally combine across signals from multiple RF chains. 
Further, we can re-write the convolution as a multiplication by taking fourier transform of $Y^{\mathcal{D}}_{1,2\ldots K}$. This allows for a matrix representation,

\begin{equation}
\begin{bmatrix}
 Y_1^{\mathcal{D}}(f) \\
 Y_2^{\mathcal{D}}(f)\\
 \cdot \\
 \cdot \\
 Y_K^{\mathcal{D}}(f)\\
\end{bmatrix}
=
% \begin{bmatrix}
%  H_{11}(f) & H_{21}(f) & \cdot & \cdot & H_{K1}(f)\\
%  H_{12}(f) & H_{22}(f) & \cdot & \cdot & H_{K2}(f)\\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  H_{1K}(f) & H_{2K}(f) & \cdot & \cdot & H_{KK}(f)\\
%  \end{bmatrix}
\mathbf{H}
\cdot
\mathbf{B}
\cdot
 \begin{bmatrix}
 X_1(f) \\
 X_2(f)\\
 \cdot \\
 \cdot \\
 X_K(f)\\
\end{bmatrix}
\label{eqn:expanded_matrx}
\end{equation}

which we can write in shorthand as $\mathbf{Y}=\mathbf{H}\mathbf{B}\mathbf{X}$, where $\mathbf{Y}$ is the $K\times 1$ column obtained by stacking the $K$ different delayed streams, $\mathbf{H}, \mathbf{B}$ are the $K\times K$ channel, code matrix, and $\mathbf{X}$ being the column vector of the K users transmitted signal in frequency domain. For brevity, let $\tilde{\mathbf{H}}= \mathbf{H}\cdot \mathbf{B}$.

Now, to isolate signal of user $1$ from other users, we take the matrix $\tilde{\mathbf{H}}$ and remove the first column to get a $K-1 \times K$ matrix $\tilde{\mathbf{H}}_{1^{\_}}$, which because of reduced number of columns, will have a $K\times 1$ column-space null vector $\mathbf{N}_1$ belonging to the null space of the matrix $\tilde{\mathbf{H}}_{1^{\_}}$. When we take the inner product of the $K\times 1$ complex vectors, $\mathbf{N}_1$ with $\mathbf{Y}$, we see that

\begin{equation}
    \begin{split}
    R_1(f) &= \mathbf{N}_1\cdot \mathbf{Y} =\mathbf{N}_1 \cdot \begin{bmatrix} 
        \tilde{\mathbf{H}}_1\quad \tilde{\mathbf{H}}_{1^{\_}}
        \end{bmatrix}\\
        &=
        [\mathbf{N}_1\cdot\tilde{\mathbf{H}}_1\quad \mathbf{N}_1\cdot\tilde{\mathbf{H}}_{1^{\_}}]
        \mathbf{X}\\
        &= \begin{bmatrix} 
        \mathbf{N}_1 \cdot \tilde{\mathbf{H}}_1\quad \mathbf{0}_{K-1 \times K}
        \end{bmatrix}
        \mathbf{X}\\
        & = (\mathbf{N}_1\cdot \tilde{\mathbf{H}}_1)X_1(f)
    \end{split}    
\end{equation}

since $\mathbf{N}_1$ will null out the $\tilde{\mathbf{H}}_{1^{\_}}$ sub-matrix. Thus, using the vector $\mathbf{N}_1$ to combine across the $K$ delayed sample vector $\mathbf{Y}$ we can null out all other users apart from user 1, and hone onto the signal from user 1. Note that we can generate such nulling vectors for all the $K$ users, since there is nothing special about the user 1. Thus we can get $\mathbf{N}_{1,2,\ldots K}$ for all the $K$ users, from the null spaces of appropriate matrices $\tilde{\mathbf{H}}_{j^{\_}}$ by removing the $j$-th column associated to $j$-th user. Thus, we can get the vector $\mathbf{R}(f) = {\begin{bmatrix}
 R_1(f) 
 R_2(f)
 \cdot 
 \cdot 
 R_K(f)
\end{bmatrix}}^T$, such that

\begin{equation}
\begin{split}
\mathbf{R}(f) &= [\mathbf{N}_1 \mathbf{N}_2 \cdot \cdot \mathbf{N}_K ] \cdot Y  \\
& = \begin{bmatrix}
 \mathbf{N}_1\cdot \tilde{\mathbf{H}}_1 & 0 & \cdot & \cdot & 0\\
 0 & \mathbf{N}_2\cdot \tilde{\mathbf{H}}_2 & \cdot & \cdot & 0\\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 \cdot     & \cdot     & \cdot & \cdot & \cdot \\
 0 & 0 & \cdot & \cdot &  \mathbf{N}_K\cdot \tilde{\mathbf{H}}_K \\
 \end{bmatrix}
 \begin{bmatrix}
 X_1(f) \\
 X_2(f)\\
 \cdot \\
 \cdot \\
 X_K(f)\\
\end{bmatrix}
\end{split}
\end{equation}
% \begin{split}

\noindent Since here, the vector $\mathbf{R}$ is a product of diagonal matrix and the vector having signals of all the $K$-users, using just a single RF chain with $K$ switched antennas, and the ADC, RF switches toggling at $KB$ rate, we can get data of $K$ users each having over the air bandwidth $B$.

\subsection{Spatio-temporal combining}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/arch2.pdf}
    \caption{Different multi-RF chain implementations of \name's swtiched antenna array}
    \label{fig:multiname}
\end{figure}

The above analysis to get $K$ users data from one RF chains can be further generalized when there are multiple $S$ different RF chains. Usually, when we have $S$ RF chains, it is assumed that the design can serve $S$ interfering users simultaneously. However, with the $K$ times increased local IF bandwidth, we can actually even increase the number of users to $S\times K$. 

Since now we need to serve $SK$ users, we would need to combine in $SK$ dimensions, and thus we have $SK$ number of switched antennas per RF chain (Fig. \ref{fig:multiname}). In this scenario, from a single RF chain, we can only get $K\times 1$ vector $\mathbf{Y}^s$ from the $K$ number of orthogonal codes we can design when we increase the IF bandwidth $K$ times, however, we need to serve $SK$ users. 
Since now we have $S$ different RF chains, if we can combine across these $S$ spatial streams, as well as the individual $K$ streams per RF chains, we can indeed serve $SK$ users.

First, since we have more number of antennas ($SK$) than number of orthogonal codes due to oversampling ($K$), we need to generalize to not using identity codes and turning multiple antennas on simultaneously, to effectively utilize the 
$SK$ antennas.

% To do so, we need to have $SK$ number of antennas, and in the multi RF chain setting, these $SK$ antennas are mapped to $S$ RF chains, instead of just $1$ RF chain. That is, there are $S$ different combiner networks, each combining $SK$ antennas with $SK$ RF switches to a single RF chain (Fig. ). Thus, in this scenario, we will have $S^2K$ number of RF switches, so that we can have $S$ different combiner networks for the $SK$ antennas.

% Considering that now we will get $K\times 1$ vector $\mathbf{Y}^{s}$ from the $s$-th RF chain, we can model it similar to the previous analysis and write it as $\mathbf{Y}^{s} = \mathbf{H}\mathbf{X}$, however, here $\mathbf{H}$ is $SK\times SK$, and $\mathbf{X}$ is $SK \times 1$. Thus, the null space vector here will be $SK\times 1$, and thus it is not enough to combine it with the $K\times 1$ vector $Y^s$

% \noindent Antenna Switching creates artificial time-faded channels -> \\
% Combined with oversampling creates virtual RF chains with separate channels across time->\\
% More antennas allows existance of null spaces ->\\
% Wideband null space combining cancels interference\\

% For example, when $K=4$ and identity codes as described before,
% $Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$. In general, if we do not have these identity codes, that is, say $B_1[n] = [1,0,0,1]_n$, $B_2[n] = [1,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,1,1]_n$, we will observe $h_{i1}+h_{i2}, h_{i2}, h_{i3}+h_{i4}, h_{i4}+h_{i1}$ on the 4 delayed streams. Thus, the measured channels are actually matrix multiplication of the $K\times K$ channel matrix , $\mathbf{H} = [h_1 h_2 h_3 h_4]$, with $K\times K$ code matrix 
% $\mathbf{B} = \begin{bmatrix} 
% B_1
% B_2
% B_3
% B_4
% \end{bmatrix}^T$ $\mathbf{H}\cdot \mathbf{B}$. If we choose codes such that $\mathbf{B}$ is invertible, we can estimate the $K$ antenna channels simultaneously 

==> design/design4.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
In this section, we present the design of \name. First, we describe how \name can create numerous virtual RF chains with a single RF chain, saving down-conversion and LO (Local Oscillator) sharing complexity. Next, we discuss how \name can achieve flexibility, by showing the analysis that \name can behave like both, a true digital beamformer, as well as a hybrid beamformer. Finally, we will discuss an algorithm to make the multiplexing gains from \name architecture robust, and conclude by having an overview of our design before moving to the implementation and evaluation of \name.

\subsection{Creation of time interleaved RF chains with TIMO architecture}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{design/design_fig1.pdf}
    \caption{RF switches connect $i$-th antenna to every $4n+i$-th samples, creating time interleaved RF chains $y_i$ from a single sampled stream $y[n]$. Thus \name obtains multiplexing gains by leveraging the multiple antenna channels across the $4$ virtual RF chains.}
    \label{fig:design_subsec1}
    \vspace{5pt}
\end{figure*}

% The goal of \name architecture is to serve $K$ users transmitting concurrently and in the same frequency band. This leads to interference amongst all the users as their signals get summed over-the-air as they propagate towards the receiver. 
\name creates virtual RF chains to support multiple user. Let's assume, \name attempts to handle $K$-user by creating $K$ virtual RF chains interleaved across time samples of a single downconverted stream sampled by an ADC sampling $K$ times faster the bandwidth of the users, $B_t$. In this section, before we generalize to $M>K$ scenario, we would motivate \name's design for a simple $M=K$ setting. To further simplify the representations and for brevity we take an example case of $K=4$.

The intuition behind creation of these $K=4$ virtual RF chain is that sampling at $4B_t$ to decode $B_t$ bandwidth user, we get $4$ extra time slots at our disposal, and for these $4$ extra slots we can toggle different antennas on-off using RF switches to capture different antenna's signal in each of the $4$ slots. 
That is, say if we had a bandlimited signal $x[n]$, and we oversample it by $4$ times to obtain $y[n]$. To downsample $y[n]$ now, we have $4$ possible ways, we can do $y_0[n] = y[4n], y_1[n]=y[4n+1],y_2[n] = y[4n+2],y_3[n] = y[4n+3]$. Each of these $y_k$'s can be independently used to recover the original signal $x[n]$. 

This simple idea of $4$ independent ways to downsample $y[n]$ forms the intuitive prior behind \name's approach. That is, we can use switch different antennas on for these different sampling instants corresponding to each of the 4 $y_k$'s and use them as virtual RF chains interleaved over time. The concrete idea here is to keep the first switched antenna to be \emph{on} for $0,4,8,\ldots,4n$-th samples, the second switched antenna \emph{on} for $1,5,9,\ldots,4n+1$-th samples, and so on. This basically abstracts down to making each $y_k$ as a virtual RF chain for antenna $k$.  

To understand how this virtual RF chain actually captures the wireless channel at $k$-th antenna, let us model the scenario with $K=4$ users transmitting signals as $x_{i}(t), i\in\{1,2,3,4\}$, and the complex time-invariant channel seen by user $i$ to the $k$-th antenna represented as $h_{ik}$. 
We also know that at any time instant, $t$, each of the RF switch for the $k^{th}$ antenna is either \emph{on} or \emph{off}, which we can model as the switching signal $s_k(t) \in\{0,1\}$.
The combined interference signal $y(t)$ due to the $4$ users indexed via $i$, and $4$ switched antennas indexed via $k$, can be represented as:
\begin{equation}
    y(t) = \sum_{i=1}^4 \sum_{k=1}^4 (h_{ik}(t)*x_i(t))\cdot s_k(t).
\label{eqn:combined_codes}
\end{equation}
This combined signal $y(t)$ then goes through  one single downconversion, and a single ADC sampling at $4B_t$ to get one single combined digitized signal, $y[n]$ as follows:
\begin{equation}
    y[n] \equiv y(nT_s) = \sum_{i=1}^4 \sum_{k=1}^4 (h_{ik}[n]*x_i[n])\cdot s_k[n].
\label{eqn:combined_codes}
\end{equation}
Now, in order to untangle the individual virtual RF-chain signals $y_k[n], k\in\{1,2,3,4\}$ we need to ensure that only antenna $1$ is \emph{on} for every $4n$-th sample  corresponding to $y_0$ and \emph{off} for $4n+k, k\in\{1,2,3\}$-th samples and so on. We can enable this by choosing the switching vectors $s_k[n], k\in\{1,2,3,4\}$ as $s_1[n] = [1,0,0,0]_n$, $s_2[n] = [0,1,0,0]_n$, $s_3[n] = [0,0,1,0]_n$ and $s_4[n] = [0,0,0,1]_n$, where $[\cdot]_n$ shows that the sequence gets repeated, that is $s_1[n] = 1,0,0,0,1,0,0,0,\ldots$ as shown in Fig. \ref{fig:design_subsec1}.
% This choice of switching sequence essentially selects $y_k$-th virtual RF chain for antenna $k$.
% That is, antenna $1$ is \emph{on} for every $4n$-th samples corresponding to $y_0$ and \emph{off} for $y_1,y_2,y_3$, antenna $2$ is on only for every $4n+1$-th samples, corresponding to $y_1$ and so on (Fig. \ref{fig:design_subsec1}).
Thus, the oversampled signal $y[n]$ is interleaved with samples from each of the antennas.
This forms the core idea behind TIMO's approach of time interleaved RF chains.
We can now write these $K=4$ virtual RF chains, $y_1,y_2,y_3,y_4$ as
\begin{equation}
\begin{split}
y_k[n] &= \sum_{i=1}^4 (h_{ik}[4n+k]*x_k[4n+k])s_k[4n+k]\\
        &= \sum_{i=1}^4 (h_{ik}[4n+k]*x_k[4n+k]) \\
        &\approx \sum_{i=1}^4 (h_{ik}[4n]*x_k[4n+k]),
\label{eqn:equation_yj_id}    
\end{split}
\end{equation}

\noindent where the second step follows from $s_k[4n+k]$ being equal to 1 from definition, and the last step assumes that the wireless channels $h_{ik}[4n] \approx h_{ik}[4n+1] \approx h_{ik}[4n+2] \approx h_{ik}[4n+3]$, which is generally true as the coherence time for channels is usually much larger than duration of $4$ samples. Note that we are not assuming that the channel stays same across the entire packet length, but only local stationarity for a $4$ sample length.

\noindent Thus our $k$-th virtual RF chain $y_k$ effectively consists of convolution of all the $K$ users signals with channels between the users and the $k$-th antenna, as only $k$-th antenna is \emph{on} for the samples used to derive $y_k[n]$ from the single combined stream $y[n]$. 
This draws a parallel to how in a normal digital beamforming system, we get channels from a RF chain connected to a single antenna. 
Wherein, we can combine across $y_k$'s in order to cancel the interference, similar to how digital beamformer utilizes separate spatial RF chains for the same purpose.
While, we show only a case for $M=K=4$ for brevity, the above \name's design principles for obtaining virtual RF chains by utilizing switching sequences can be generalized to $M=K$.



\subsection{\name's equivalence to both digital and hybrid beamforming}

In the previous section, we have shown how we can obtain these virtual RF chains $y_k$ by utilizing the switching sequences $s_k$ and using RF switches to implement it with hardware. Before we understand how we perform combining in \name, let us generalize the setting to $K$ interfering users and $M>K$ number of antennas. 
This generalization will concretely reveal how \name's single-RF chain architecture can behave as both a digital beamformer, as well as a hybrid beamformer for the traditional multi-RF chain MIMO settings.


To understand how the single-RF chain based \name's architecture can perform the same as a physically laid multi-RF chain ideal digital or hybrid beamformer, let us first generalize \name's combining to $M>k$ setting and understand how \name can identify $y_k[n], k={1,2,\cdots,K}$. Firstly, let us stack up the switching sequences as rows of a combined $M \times K$ switching matrix $\mathbf{S}$. An element $s_{mk}\in\{0,1\}$ in the matrix $\mathbf{S}$ now
represents the on-off states for each of the $m=1,2,3,\ldots,M$ antennas for $k=1,2,3,\ldots,K$ virtual RF chains. 
In the example in previous section we had $\mathbf{S}$ as an identity matrix, as only one antenna was \emph{on} at a time. 
More generally, with $i$ indexing $i=1,2,\ldots K$ users, $m$ indexing $1,2,\ldots M$ antennas and $k$ indexing $1,2,\ldots K$ virtual RF chains, we can write Eqn \eqref{eqn:equation_yj_id} as
\begin{equation}
    y_k[n] = \sum_{i=1}^K \sum_{m=1}^{M} (h_{im}[Kn]*x_i[Kn+k])\cdot s_{mk},
\end{equation}
and since $s_{mk}$ can be either $0$ or $1$ for each antenna $m$ and is independent of the user's tranmission we can re-write the above equation as
\begin{equation}
y_k[n] = \sum_{i=1}^K \left(\left(\sum_{m=1}^{M} h_{im}[Kn]s_{mk}\right)*x_i[Kn+k]\right),
\label{eqn:equation_yj_gen}    
\end{equation}

Now to make the analysis simpler and to draw easier equivalences with the digital and hybrid beamforming, we can take the Fourier transform to go to the frequency domain as follows:
\begin{equation}
Y_k[f] = \sum_{i=1}^K \left(\left(\sum_{m=1}^{M} \tilde{H}_{im}[f]s_{mk}\right)\mathcal{F}(x_i[Kn+k])\right),\\
\end{equation}
\noindent where $\tilde{H}_{im}[f]$ represents the Fourier transform of channel  $\tilde{h}_{im}[n]\approx h_{im}[Kn] \approx h_{im}[Kn+1] \ldots \approx h_{im}[Kn+K-1]$, since the channel is assumed to be stationary for every $K$ samples. For brevity, we will drop tilde from the expression and write it simply as $H_{im}[f]$.  We can write $\mathcal{F}(x_i[Kn+k]) =  e^{j2\pi f k}\mathcal{F}(x_i[Kn]) = e^{j2\pi f k}X_i[f]$ by using Fourier identities for time delayed signals and using the fact that $x_i(t)$ has been oversampled by $K$ times. Thus we get the simplified equation,
\begin{equation}
Y_k[f] = \sum_{i=1}^K \left(\left(\sum_{m=1}^{M} H_{im}[f]s_{mk}\right)e^{j2\pi f k} X_i[f]\right).\\
\end{equation}
Now, note that $\sum_{m=1}^M H_{im}[f]s_{mk}$ is nothing but the $(i,k)$-th element in the matrix multiplication between $K\times{M}$ channel matrix $\mathbf{H}[f]$, and the ${M}\times K$ switching matrix $\mathbf{S}$. Note that for $Y_k$ we need to remove the phase due to group delay in the Fourier transform, which can be done by multiplying $Y_k$ by $e^{-j2\pi f k}$, and we can write the delay compensated vector $\mathbf{Y^\mathcal{D}}[f] = [Y_0[f]\; Y_1[f]e^{-j2\pi f}\;\ldots\; Y_{K-1}[f]e^{-j2\pi f (K-1)}]^{\top}$. 
This vector $\mathbf{Y^\mathcal{D}}[f]$ consists of phase delay compensated Fourier transforms of $y_k[n]$ which were obtained by collecting $Kn+k$ samples in the oversampled signal $y[n]$, and this step is similar to how the popular function $\text{delayseq}(.)$\cite{delayseq} removes fractional delays.
Denoting $\mathbf{X}[f]$ to be $[X_1[f] X_2[f]\ldots X_K[f]]^{\top}$, to get a much simpler equation in terms of matrix products, 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f].
\label{eq:timo_matrix}
\end{equation}

This equation is akin to what hybrid analog-digital beamformers use, since $\mathbf{S}$ here is implemented by the analog switching network, and we observe $\mathbf{HS}$ equivalent $K\times K$ channel with digital streams which can then be combined over digitally.

In digital beamforming systems with $M=K$, we obtain $y_r[n]$ for each of the $r$-th RF chains, $r=0,1,\ldots K-1$, we get the equation 
\begin{equation}
\mathbf{Y^\text{RF}}[f] = \mathbf{H}[f]\mathbf{X}[f].
\end{equation}
For $M=K$ case, we can set the switching matrix $\mathbf{S}$ to be identity, we get a clear equivalence between \name and traditional digital beamforming, even though \name implements $\mathbf{S}$ in analog domain using switches. However, having $M=K$ is not a very robust operating point to serve $K$ users, since the channel may not always be full rank. Hence, it is always preferred to have $M>K$ in order to serve $K$ users.

Connecting more number of antennas to lesser number of physical RF chains usually requires changing the normal structure of the beamformer and creating specialised analog network with phase shifters.
In \name's architecture, we have the humble RF switch, which implements this switching network, similar to how setting this network to identity matrix gave \name an equivalence to digital beamforming. 
The main benefit of having $M>K$ antennas for $K$ virtual RF chains is that this allows us to harden the multiplexing gains of $K$ for any user configuration, irrespective of the underlying channels for the $K$ users. 

\subsection{Harnessing power of multiple antennas for robust multiplexing gains}
In previous section, we saw how \name provides a much more natural solution to hybridize the digital architecture, by scaling up the number of switched-antennas \emph{without} requiring any additional sampling or downconversion chains cost, or any specialised hardware like phase shifters. 
In contrast, we have seen that \name can easily generalize to $M>K$ antenna scenario and harden the multiplexing gains by $K\times$ with a single RF-chain. 

We have seen from Eq~\ref{eq:timo_matrix} that when we have $K$ users and $M>K$ antennas the equivalent channel $\mathbf{H}[f]\mathbf{S}$ still remains $K\times K$, and the digital combining part operates on this $K\times K$ equivalent channel $\mathbf{H}[f]\mathbf{S}$. So the idea here is to choose the matrix $\mathbf{S}$ in a way such that the digital combining operates on a full rank uncorrelated $K\times K$ equivalent channel in order to increase the performance.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_fig2.pdf}
    % \vspace{2pt}
    \caption{By strategically choosing $\mathbf{S}$ to implement binarized analog beamforming per user, we ensure that the effective $K\times K$ channel is as uncorrelated as possible.}
    \vspace{4pt}
    \label{fig:smatrix__choice}
\end{figure}
In order to achievve this full-rank equivalent channel matrix $\mathbf{H}[f]\mathbf{S}$, we need to choose $\mathbf{S}$. TO choose $\mathbf{S}$, we have $2^{M\times K}$ possible choices, as each of the $M$ antenna can be turned on/off for each of the $K$ slots. Hence, a brute force optimization would not be scalable, considering $M=8$ and $K=4$, we have $2^{32}$ choices, and it will take a considerable amount of time to go over these possibilities, which would exceed the channel coherence time. Hence, instead of a brute force search for an optimal $\textbf{S}$ we need a smart and compute efficient way of estimating a relevant matrix $\mathbf{S}$. 

Here, we make a key observation. We have $K$ users, and the goal is to create equivalent channel $\mathbf{H}[f]\mathbf{S}$ which is as uncorrelated as possible. The way to do this would be to basically use each of the $K$ time slots to prioritize one user at a time, that is, to select column $i$ of $\mathbf{S}$ such that signal power of user $i$ is maximised in that slot.
This way the equivalent channel $\mathbf{H}[f]\mathbf{S}$ will have higher diagonal values than non-diagonal, which will decrease correlations, as one user is getting prioritized at a time.

To increase the signal power of user $i$, the theoretically exact way to do so would be to conjugate the user $i$'s channels for each antenna, thus implementing analog beamforming, which would co-phase the user's signals received at each antenna, to give constructive combining gains.
However, we do not have accurate phase shifters, and infact in our design we just have RF switches which can toggle on-off, thus providing only one-bit control over the phases. But, at the same time, we just need to increase the signal power for user $i$ and we actually do not need very accurate beamforming for this. This can also be achieved by turning \emph{on} the maximal set of antennas whose phases would add up constructively (Fig. \ref{fig:smatrix__choice}). We call this algorithm as binarized analog beamforming (BABF) algorithm, as it takes the analog beamforming solution and finds the closest representative of that in the binary RF switch implementable solution.

To achieve the best uncorrelated equivalent channel matrix $\mathbf{H}[f]\mathbf{S}$, in binarized analog beamforming algorithm, we go one antenna by one to calculate the number of other antennas whose phases lie within an acute angle ($\pi/3$ in our implementation) of each other.
We select the group of in-phase antennas having the highest cardinality, since that would entail higher constructive combining gain and thus higher power for user $i$.
Thus, this makes the algorithm to be $O(M)$, as we have to choose from $M$ number of groups.
We repeat this procedure for each $k$-th user for $k$-th time slot to create a matrix $\mathbf{S}$ that enables maximally uncorrelated equivalent channel matrix.
A further detailed implementation of the BABF algorithm is described in Algorithm \ref{Alg1} (in Appendix section). 

We note that the BABF method of choosing $\mathbf{B}$ to prioritize signal power instead of utilizing $\mathbf{B}$ to cancel interference is a common theme on how hybrid beamformers \cite{chen2020turbo,ghasempour2018multi} choose their analog weights. This is because increasing signal power is an easier operation, and allows for inaccuracies because whatever is in-phase will ultimately add up and serve the purpose of increased signal power. On the other hand choosing an analog network such that signals are cancelled requires more careful calibration, as well as an requirement to generalize to wideband. Hence, in line with previous approaches to utilize analog networks for creation of such rank achieving equivalent channels, we also propose an algorithm to increase the signal power, however using just RF switches instead of quantized phase shifters. 
The final task of combining across the signals with arbitrary accuracy and wideband generalization are better handled in the digital domain, and thus the digital combining with $(HB)^{-1}$ across the virtual RF chains will cancel out the interference and give $N$ user's interference-free data streams.

\subsection{Final digital combining step in \name}

The key insight which \name delivers is that to handle $K$ users transmitting $B_t$ bandwidth signals $\mathbf{X}$, we can sample a single signal $y$ at $KB_t$ bandwidth by utilizing a switched antenna array with number of antennas $M>K$ and switching sequences for each of the $M$ antennas and the extra $K$ slots created due to higher sampling rate denoted by $\mathbf{S}$ to get the equation 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f],
\end{equation}
where $\mathbf{Y^\mathcal{D}}$ are the delay compensated $K$ streams derived from $y$. We get an equivalent channel $\mathbf{H}[f]\mathbf{S}$ created due to the switching network, and we choose $\mathbf{S}$ such that the obtained $K\times K$ channel is as uncorrelated as possible, so that all the $K$ users can be served with sufficient SINR. 

Now, to recover individual data symbols for each user $\mathbf{X}[f]$ from the obtained interfered samples $\mathbf{Y}[f]$,  we can utilize a $K\times K$ beamforming matrix $\mathbf{V}[f] =[v_1 v_2 \ldots v_K]^{\top}$ which is a collection of $K\times 1$ beamforming vectors $v_i, i=0,1,\ldots K-1$.  When we take the inner product of $v_i$ with $\mathbf{Y}[f]$, the hope is that we recover $x_i[f]$. To cancel out interference, the best method is to use a ZF combiner \cite{rebato2019performance} .
In \name's case, the matrix $\mathbf{V}[f]$ selects pseudo inverse of $\mathbf{H}[f]\mathbf{S}$ as the digital combiner matrix $\mathbf{V}$. 
Thus after utilizing the digital combiner, we get
\begin{equation}
\mathbf{V}\mathbf{Y^\mathcal{D}}[f] = \text{pinv}(\mathbf{H}[f]\mathbf{S})(\mathbf{H}[f]\mathbf{S})\mathbf{X}[f] \approx \mathbf{X}[f], 
\end{equation}
which allows us to remove the interference and recover each of the $K$ symbols $\mathbf{X}=[X_1,X_2,\ldots X_K]^{\top}$. An important point to note is that since this combining happens in digital domain, we can do arbitrary combinations for each frequency bin $[f]$ which allows for resilient wideband operation, as well as accurate phase values so that the interference are cancelled perfectly.

\textbf{Extending \name to handle downlink multi-user transmissions}: So far we have presented analysis of \name's beamforming approach applied to an uplink channel with AP receiving multiple-user's interfering signals. In an equivalent downlink setting, almost the same generalization can apply naturally.  given the channel measurements at the clients are fed-back to \name. \name would then utilize the RF switch based architecture to create spatial transmissions which essentially null other users' signals while trying to communicate to an intended user, allowing for downlink multi-user transmissions. 



%\todo{Add reciprocity argument that TIMO can work as a transmitter as well.}

==> design/design_LO.tex <==
% architecture
% how this architecture can be green fixed hybrid
% how this architecture can flex through mu-MIMO and massive MIMO
% what is deployed: mu-MIMO, what is proposed massive MIMO
% LO
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{design/design_re_fig1.pdf}
    \caption{Toy example demonstrating \name's approach to create virtual RF chain from one physically laid chain \todo{Ish: Add caption to sub-figures} }
    % \vspace{5pt}
    \label{fig:virt_rfc}
\end{figure*}


\section{Design}

\name attempts to build a new multi-user communications architecture, which is as power-efficient+flexible as FDMA, and spectrum-efficient as massive MIMO. 
In this section, first we will describe how \name bridges the gap between massive MIMO and FDMA by using just a single physical RF chain like FDMA, and at the same time obtains signals from multiple antennas by `virtualizing' RF chains across the captured spectrum.
Then, we will provide a generalization to \name architecture, which allows \name architecture to scale with number of antennas easily without increasing RF chains, saving on the amount of data getting processed and leading to a green architecture.
% Further, this generalization helps adapt to averse channel conditions, if channel conditions are bad \name can tap into further diversity gains to help increase the 


% Multi-antenna MIMO architectures have played a critical role in helping wireless networks scale with number of users without adding new spectrum. 
% Each antenna brings about a new degree of freedom, and capturing these degrees of freedom is what allows MIMO systems to handle multiple users communicating together.
% Capturing these degrees of freedom today requires connecting dedicated circuitry, referred to as a RF chain, per antenna, which does not allow for seamless software control and goes against the recent trends of virtualization of communication networks.
% In this section, first we will explain how we can capture these degrees of freedom via a new architecture which can offer software-level control, by essentially virtualizing these RF chains.
% Then, we will show the two applications which are made possible by our new architecture, namely, green communication circuits made possible by digital processing and sampling commensurate with number of users, and a flexible mode of operation where the worse channel conditions can be countered by scaling the sampling rate of the architecture.


\subsection{Virtualizing RF chains}

% \todo{Ish: First line summarize the paragraph}

% Massive MIMO architectures today need multiple downconversion RF chains, which make it power hungry. 
% Downconversion requires distribution of the LO clock across all these RF chains.
% Due to high frequency of these LO clocks (in GHz), the distribution networks are lossy and further synchronization requirements increase the power consumption. 
% This problem is only going to intensify further as the communication frequencies increase from GHz to mmWave to THz.
% The RF chains in a typical receive MIMO architecture basically perform three tasks, they amplify the weak signal at the antenna, downconvert the signal to baseband and finally sample it via an ADC to get digital baseband samples from the antenna.
% All this requires dedicated hardware per antenna, and thus it is common knowledge to assume the requirement of physically laid RF chains to get these digitized baseband samples per antenna.
% One of the biggest challenges going ahead with power consumption in these RF chains is the total LO power draw, and required synchronization of the clocks across RF chains, required for massive MIMO, and this problem is only going to intensify further as the communication frequencies increase from GHz to mmWave to THz.

% \name circumvents these power consumption challenges posed by multiple physical RF chains, by designing a novel architecture which just uses a single physically laid RF chain connected to all the antennas, thus not requiring LO distribution and synchronisation.
% The core concept is that \name creates different virtual RF chains from the single physically laid chain.
% This enables hardware re-use of downconversion chains for all antennas which optimizes power consumption, and the virtualization leads to flexible number of RF chains as well, since the number of created RF chains can be controlled via software.
\name creates a flexible, power efficient multi-antenna architecture by creating multiple virtual RF chains from a singly laid physical RF chain.
This circumvents challenges in LO distribution across physically laid RF chains as all virtual RF chains share the same downconversion path. 
Since these virtual RF chains are created digitally, they can be abstracted in software, allowing \name architecture to be flexible, and increase/decrease the virtual RF chains based on channel conditions and the number of users.

\todo{write the next two paragraphs in a direct way, say how \name does it, then you can explain a bit why those parameters are used.}

In order to create virtual RF chains, \name tries to tweak the circuit parameters of the single laid RF chain.
But what are the parameters which any RF chain exposes to the controlling software? We have the gain settings for LNA, the mixer's center frequency and the ADC sampling frequency. Definitely tweaking the LNA gains or varying the downconverting frequency won't do us any good for virtualization. 
However, varying the ADC sampling frequency would imply sampling more bandwidth digitally, allowing for more digital control over the multi-antenna hardware.
% The idea is to somehow try and map signals from each antenna across the increased sampling frequency of the ADC; that way each RF chain appears across
This can possibly allow to fit each antenna's signals across the increased bandwidth; creating virtual RF chains across the sampled spectrum.
This is similar to how FDMA utilizes assymetricity in transmit bandwidth per user and the total sampled spectrum; \name asks the question that can this assymetricity be also used for creation of virtual RF chains across the sampled spectrum.
% However, when all the antennas share a common downconversion chain, their signals will get combined.
% Thus after downconversion, baseband sampling will get a summed signal across antennas, and not individual antenna signals required for MIMO processing.

\noindent\textbf{Toy example to show \name's working:}

\noindent However, merely increasing ADC rate does not by itself create these virtual RF chains. 
The succinct reason for that by itself, increasing the ADC sampling rate does not give any new diversity, since there are no signals in the new parts of spectrum ADC captures when it's sampling rate increases.
This is better explained via a toy example of a $2$ antenna array. 
As an abstraction, consider first antenna receives a rectangular pulsed signal and the second antenna receives a triangular signal.
Today's way of capturing the 2 degrees of freedom offered by the array is to have 2 physically laid RF chains, which downconvert and sample these rectangular and triangular signals directly  (Fig. \ref{fig:virt_rfc}(a)). 
% \todo{Ish: Go slow here, explain the (b) architecture that it uses a single RF chain for two antennas.}
% Now, a naive attempt at replacing multiple RF chains in (a) by virtualizing the chains over a single physically laid RF chain, by merely increasing the ADC rate (b)
Now, \ref{fig:virt_rfc}(b) shows a naive attempt at replacing multiple RF chains in (a) by virtualizing the chains over a single physically laid RF chain, however, by merely increasing the ADC rate.
This leads to combining of the signals from the antennas before getting downconverted by the RF chain, which gives a raised triangular signal in this scenario. 
Hence, there's no way of separating them now, and by doubling ADC sampling here would not capture any new diversity but only the noise in the neighbour band, and thus \ref{fig:virt_rfc}(b) fails to create these 2 virtual RF chains with the triangular and rectangular signals in them.

% How \name enables this creation of virtual RF chains by tweaking ADC's sampling rate is by introducing RF switches which toggle in synchronity with the ADC's sampling clock.
The key concept behind \name architecture is to create useful signal copies in the neighbour bands, instead of just noise; so that when ADC sampling rate increases it gets diversity gains due to sampling more bandwidth.
For this purpose, we need to create signal variations in the neighbour bands, before the signals get downconverted through the RF chain.
But how does \name enable this, that too in a low-power way to stay true to the requirements of a power-efficient architecture?
Our insight here is that we can augment the antenna array with RF switches (\ref{fig:virt_rfc}(c)) toggling with \emph{on-off} codes having time period, commensurate to signal bandwidth.
Similar toggling RF switches have also been used for backscatter communications \todo{Cite}, which also demand low-power operation; RF switches in backscatter applications create frequency shifts in reflected signal to avoid interference with line of sight signal.
Hence, \name basically uses RF switches for something similar, to create frequency shifts of the RF signals before they get downconverted, and now with frequency shifts the higher sampling rate ADC will be useful as it will capture diversity in signals instead of just noise. 

Thus, in order to create these virtual RF chains over a singly laid physical RF chain, \name uses strategic toggling of the RF switches, combined with ADCs increased sampling rate.
We first explain this strategic toggling using the same toy example of 2 virtual RF chains, and then extend it to creation of $N$ RF chains.
When \name wants to create 2 virtual RF chains, the ADCs would be sampling at $2B$, where $B$ is the signal bandwidth, to accommodate the $2$ signals from each RF chain.
Thus, a single ADC sample will occupy total time of $\frac{1}{2B}$, and in order to shift the signals by frequency $B$, the switching code has to repeat every $2$ ADC samples.
This presents us two possible codes $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$.
When we supply these codes to one of the 2 antennas, we have one antenna being toggled \emph{on} for odd samples, and the other antenna toggled \emph{on} for even samples.

This strategic toggling actually creates sum of the $2$ antenna signals in the first nyquist band ($(-B/2)<f<(B/2)$) and difference of the $2$ antenna signals in the second band ($(-B)<f<(-B/2)$ and $(B/2)<f<(B)$), as shown in \ref{fig:virt_rfc}(c).
The reason is that $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$ are basically $\pi$ shifted versions of the same frequency codes, and hence the frequency shifted copies they create will reflect this $\pi$ shift, leading to creation of subtracted signals in second band.
This basically then allows us to separate the per-antenna signals by simple signal processing, first add the signals extracted from each nyquist band and then take the difference.

In order to explain mathematically on why this effect happens, say the antenna signals were $s_1(t), s_2(t)$, these signals are $B$ bandwidth. 
The codes $c_1 = 0,1,0,1,\ldots$ $c_2 = 1,0,1,0,\ldots$ are basically 50\% duty cycled codes with frequency $B$, and RF switches implement these codes in RF domain before downconversion and ADC sampling.
Thus, the ADC finally samples the waveform $s_1(t)c_1(t)+s_2(t)c_2(t)$, at $2B$.
In addition to a constant DC component, these switches also produce harmonics at $\pm B$.
Since $c_2$ is \emph{on} for odd samples and $c_1$ is \emph{on} for even samples, $c_1$'s harmonic at $\pm B$ will basically be $\pm \pi$ of $c_2$. 
This is because the codes are having frequency $B$, thus time period $\frac{1}{B}$, and the associated time delay between $c_1,c_2$ is $0.5(\frac{1}{B})$, thus the phase associated with this time delay would be $(\frac{2\pi}{\frac{1}{B}})0.5(\frac{1}{B}) = \pi$.
The DC component of $c_1,c_2$ however would be the same, since the DC component depends on the average energy, which is a measure of how much time the codes had value $1$ which is same for both.

Thus, as shown in Fig. \ref{fig:virt_rfc}(c) the frequency domain view of the signal sampled by ADC, which was $s_1(t)c_1(t)+s_2(t)c_2(t)$, would have $0.5*(s_1(t)+s_2(t))$ in the first nyquist band, ($-\frac{B}{2}<f<\frac{B}{2}$) and $0.5*(s_1(t)-s_2(t))$ in the second nyquist band, ($(-B<f<-\frac{B}{2}) \cup (\frac{B}{2}<f<B)$). A simple digital processing step can now get us back $s_1, s_2$ by simply adding the subtracting these signals in the two nyquist bands.

Thus, \name utilizes RF switches with different phase codes, coupled with an oversampling ADC in order to virtualize the RF chains. This is also supported by recent trends of having faster ADCs, which offer other benefits as well, like simplified baseband filter design, reduced quantization noise amongst others.
With \name's architecture, virtualization of RF chain concept would be another advantage of faster ADC design.

\noindent\textbf{Generalization to $N$ antennas}
The method of obtaining these virtual RF chains from a single physically laid chain can be easily generalized when we have $N$ antennas with $N$ RF switches and an ADC which is doing $N*B$ times sampling where $B$ is the signal bandwidth.
In this generalized scenario, we will now have $N$ codes $c_1,c_2\ldots c_n$, which will be codes of length $N$ with  $c_1 = {1,0,0,\ldots,0,0}$, $c_2 = {0,1,0,\ldots,0,0}$, $\ldots$, $c_{n-1} = {0,0,0,\ldots,1,0}$ and $c_{n-1} = {0,0,0,\ldots,0,1}$.
Since these are $1/N$ duty cycled codes they will have frequency images at every integral multiple of $B$ and thus total $N$ images at frequencies $\text{fftshift}(0,B,2B,\ldots N)$.
In addition, code $c_i$ is delayed by $\frac{(i-1)}{NB}$, and thus the $j$-th harmonic of $c_i$ will have phases $\frac{(i-1)}{NB}*\frac{2\pi}{\frac{1}{jB}} = (i-1)*j*\frac{2\pi}{N}$.

The ADC is sampling at $NB$, and thus we will have $N$ $B$ bandwidth zones obtained from the ADC sampled stream $R$, denoted by $R^B_1, R^B_2, R^B_3\ldots R^B_N = \mathbf{R^B}$, with $\mathbf{R^B}$ being a $N\times N_s$ matrix which stores the $N_s$ samples correpsonding to each of the $N$-th $B$ bandwidth zone, and we can obtain our virtualized RF chains $S_1,S_2,\ldots S_N = \mathbf{S}$, $S$ being $N \times N_s$ as well, via phase inversion of the $N\times N$ phase matrix $\mathbf{P}$ corresponding to $j$-th harmonic phase of $c_i$:

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{design/design_re_fig2.pdf}
    % \vspace{3pt}
    \caption{How switching changes the signal spectrum: example where $N=4$, code $c_2$. Due to time delay of $1/(4*B)$, the phases at harmonics $B,2B,(3B=-B)$ are $1*(2\pi)/4 = 90^o$, $2*(2\pi)/4 = 180^o$ and $3*(2\pi)/4 = 270^o$}
    % \vspace{5pt}
    \label{fig:virt_rfc_gen}
\end{figure}

\begin{equation}
    \mathbf{S} = (\mathbf{e}^{(-\mathbf{P})})* \mathbf{R^B}
\end{equation}

where $\mathbf{e}^{(\cdot)}$ applies the exponential function to each element of the matrix. The matrix $\mathbf{P}$ in detail looks like this:

\begin{equation*}
  \mathbf{P}=
  \begin{blockarray}{*{5}{c} l}
    \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
      0 & B & 2B & $\ldots$ & (N-1)B & \\
    \end{block}
    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
      0 & 0 & 0 & $\ldots$ & 0 \bigstrut[t]& $c_1$ \\
      0 & \frac{2\pi}{N} & \frac{4\pi}{N} & $\ldots$ & \frac{2(N-1)\pi}{N} & $c_2$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(i-1)}{N} & \frac{4\pi(i-1)}{N} & $\ldots$ & \frac{2(N-1)(i-1)\pi}{N} & $c_i$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(N-1)}{N} & \frac{4\pi(N-1)}{N} & $\ldots$ & \frac{2(N-1)(N-1)\pi}{N} & $c_n$ \\
    \end{block}
  \end{blockarray}
\end{equation*}

The reason this generalization works out is because all these are different series of roots of unity, and by doing phase inversion one set of the roots become all co-phased and thus their virtual RF chain component adds up, and the other sets of roots still remain phase shifted versions of their previous versions and add up to 0, which allows \name to extract the RF chain per antenna from the increased sample rate ADC stream.

\noindent\textbf{Using virtual RF chains for spatial-multiplexing}

Once we are able to obtain the per-antenna waveforms $\mathbf{S}$, the process to obtain the spatially multiplexed output is straightforward and follows the same method as compared to usual way with physically laid RF chains.
In the scenario when we have $N$ antennas and $N$ RF chains, and say we have $N$ users, we can perform MIMO channel estimation with the $N$ virtual RF chains to get the $N\times N$ channel matrix for all $N$ users and $N$ antennas.
\todo{Tell linear non-linear similar to agora}
Now, we can choose any precoding strategy, like MMSE, BD or ZF to suppress the signals from other users to get individual streams for each of the $N$ users. For example if we use a simple ZF precoding would multiply the $N\times N$ matrix $\mathbf{H}^{-1}$ to the obtained virtual RF chain matrix $\mathbf{S}$ to get individual interference free $N_s$ samples of each $N$-th users data, stored in the $N\times N_s$ matrix $\mathbf{U}$. 

\begin{equation}
    \mathbf{U} = \mathbf{H}^{-1}\mathbf{S}
\end{equation}

Thus, by using just 1 physically laid RF chain, we can enable creation of $N$ virtual RF chains with $N$ antennas and $N$ RF switches which allows for a possible $N$ times spatial multiplexing gain, by allowing $N$ users to communicate simultaneously on the same spectrum.


\subsection{Enabling green communications with \name}
\todo{image to explain this subsection}

A traditional mu-MIMO system strives to serve $N$ users with $N$ antennas, and for this it lays down $N$ physical RF chains.
However, in practical scenarios, often we need many more number of antennas $N_{\text{ant}}>>N$ number of users in order to serve all the users with a good quality wireless link, and this system is referred to as Massive MIMO.
The reason is that we need more degrees of freedom than $N$ as the channels of the $N$ users to the base station are often correlated, especially when the users are located close to each other. 
Thus, having more antennas leads to more degrees of freedom which allows the base station to serve $N$ users effectively.
Although massive MIMO is info theoretically sound, it is challenging to deploy due to requirement of a massive number of RF chains as well.
Further, it is not a `green' architecture, since it needs to sample $N_\text{ant}$ data streams, much more than the required number of $N$ data streams to serve $N$ users.
Also, it is wasteful in terms of the digital processing done after sampling on $N_\text{ant}$ streams, as well as communication of $N_\text{ant}$ streams to the DSP where these algorithms are implemented.

Hence, it would be ideal to somehow have only $N$ data streams to serve $N$ users and at the same time use $N_{\text{ant}}$ antennas.
Here \name gives a perfect solution, where we can always reduce the number of virtual RF chains by reducing the ADC sampling rate, and still use $N_{\text{Ant}}$ antennas connected to one physical RF chain.
When we have $N_{\text{Ant}}$ antennas but only $N$ times oversampling ADC, we can not create $N_{\text{Ant}}$ separate virtual RF chains, but only $N$ virtual RF chains.
The key insight which allows \name to still effectively use $N_{\text{Ant}}$ antennas' degrees of freedom is that we try and increase the signal power for user $i$ in the $i$-th virtual RF chain, by supplying same code $c_i$ to antennas which are in-phase for user $i$ (that is, have the channel angles within $\pm \pi/2$).
We make an observation that $c_i = \{0,\ldots,1,\ldots,0\}$, which has a $1$ at the $i$-th position is orthogonal to any $c_j$, $j\neq i$.
Thus, we can add these codes when we want to have antennas to appear in more than one virtual RF chains.
Say for an example, we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
So, here, for antennas $\{1,6\}$, which is to be selected for both the users, we will give the code $c_1+c_2$. For antennas $\{3,5\}$, we will give the code $c_1$, and for $\{2,7,8\}$ we will give $c_2$.
This will ensure that for virtual RF chain $1$ corresponding to $c_1$, the signals from antennas $\{1,3,5,6\}$ would be combined and for virtual RF chain $2$, we will get combined signals from $\{1,2,6,7,8\}$.

Now, generalizing this idea, based on the $N_{\text{ant}}\times N$ channel $\mathbf{H}$, we would determine the maximal group of antennas in-phase for user $i$, corresponding to $c_i$ which generates the virtual RF chain $i$.
We name this algorithm to select the maximal in-phase antennas as $\text{BABF}(\cdot)$ (Algorithm \ref{Alg1}), where BABF stands for Binarized Analog Beamforming.
Essentially, for each virtual RF chain we try to beamform towards individual users using the $0-1$ bit control we have over the switched antenna array.

\begin{algorithm}
  \caption{BABF, Input: $\textbf{H},\phi$, Output: $\mathbf{B}$}
  \begin{algorithmic}[1]
  \label{algo:switch_selection}
  \STATE $\phi$=$\pi/3$;\
  \FOR{ $1 \le i \le K$}{
      \FOR{ $1 \le m \le M$}{
      \STATE $\Tilde{\textbf{b}}_{i,m}=[0, 0 , \ldots , 0]_{1\times M}$;\
      \STATE $\textbf{g}_{i,m}=\textbf{H}_{i}h^*_{i,m}$;\
      \STATE $\boldsymbol{\theta}_{i,m}$=$\angle{\textbf{g}_{i,m}}$;\
      \STATE $\Tilde{\textbf{b}}_{i,m}(m)$=$|\boldsymbol{\theta}_{i,m}|<\phi$;\
      \STATE $score_{i,m}=$ Number of elements equal to $1$ in $\Tilde{\textbf{b}}_{i,m}$;
      }
      \ENDFOR
  }
  \ENDFOR
  \STATE $\mathbb{B} :=$ Set of all possible permutations of $score_{i,m}, 1 \le i \le K, 1 \le m \le M$\;
  \STATE $l=1$;\
  \STATE Select $score^*\in \mathbb{B}$ that provides the $l^{\text{th}}$ highest score;\
  \STATE $\mathbf{B}=\mathbf{B}^*$ (corresponding to $score^*$);\
  \IF{$\mathbf{H}\mathbf{B}$ is full rank}
  \STATE $\mathbf{B}$ is the optimal switch configuration;\
  \ELSE
  \STATE $l=l+1$;\
  \STATE Go to line 13;\
  \ENDIF
\end{algorithmic}
\label{Alg1}
\end{algorithm}

That is, the BABF algorithm we get a switching matrix $\mathbf{B}$, where $\mathbf{B}$ is $N_{\text{Ant}}\times N$, which increases signal power of user $i$ in the $i$-th virtual RF chain, by turning $N_{\text{Ant}}$ antennas on-off.
Although each virtual RF chain prioritizes one user, there is significant interference terms still present in the virtual RF chains at this stage.
However, this can be handled easily by digital combining, that is the virtual RF chains are now capturing the $N \times N$ channel $HB$, which can be inverted via ZF approach, and that cancels out the interference terms.
Hence, using the BABF algorithm and the orthogonality of $c_i$ codes, we can project the $N_{\text{Ant}}\times N$ channel $\mathbf{H}$ onto an effective $N\times N$ channel $\mathbf{(HB)}$.

\begin{equation}
    \mathbf{U} = \mathbf{(HB)}^{-1}\mathbf{S}
\end{equation}

\ifflex

\subsection{Adapting to averse channel conditions with high sampling rate}
\todo{Draw a channel phase figure here}
In the last section we showed how \name's architecture can enable green communications by restricting only to $N$ times ADC sampling to serve $N$ users, at the same time using a $N_{\text{Ant}}>N$ antennas.
However, there might be scenarios where channel conditions are so bad that it is required to really bump up the sampling rate.
By increasing the sampling rate, we can get more control over the projected channel $\mathbf{HB}$.
However, we need to generalize our projection matrix generation when we bump up the sampling rate.

For an example, consider we have $8$ antennas, $2$ users and we oversample by a factor of $4$, which gives us $4$ virtual RF chains. In the previous section, we used $2$ times oversampling to handle 2 users, and used $2$ codes $c_0,c_1$ to implement the BABF matrix $\mathbf{B}$. The BABF algorithm basically selected antennas which are maximally \emph{in-phase}, i.e. their channel angles are within $-\pi/2,\pi/2$ of each other.
When we have $4$ chains at our disposal for $2$ users, we can then infact, select the antennas which were turned off before in the other $2$ spare codes, and do the phase aligning in digital domain to get more SNR gain for the user.
In a way, this is a way of refining the beamforming weights by implementing precise phase rotations across the digital samples, instead of simple $0/1$ as compared to previous section.

Put mathematically, we have $c_0$ implementing the maximal antenna set for user $1$, $c_1$ implementing the complimentary set for user $2$, and $c_2,c_3$ doing the same for user $2$.
Taking the same example as before, say we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
$c_0$ will turn on $\{1,3,5,6\}$, $c_1$ will turn on $\{2,4,7,8\}$, $c_2$ will do $\{1,2,6,7,8\}$ and finally $c_4$ will do $\{3,4,5\}$.
Then the virtual RF chain corresponding to $c_0$ will be added to $e^{j\pi}$ times that of $c_1$ to get everything phase aligned, and same with $c_1,c_2$.
Thus, we will get the following $\mathbf{B}$ matrix:


\begin{equation*}
  \begin{blockarray}{*{8}{c} l}
    % \begin{block}{*{8}{>{$\footnotesize}c<{$}} l}
    \begin{block}{*{8}{c}>{$\footnotesize}l<{$}}
     1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Ant. index\\
    \end{block}
    \begin{block}{[*{8}{c}]>{$\footnotesize}l<{$}}
      1 & e^{j\pi} & 1 & e^{j\pi} & 1 & 1 & e^{j\pi} & e^{j\pi}\bigstrut[t]& User 1 \\
      1 & 1 & e^{j\pi} & e^{j\pi} & e^{j\pi} & 1 & 1 & 1 & User 2 \\
    \end{block}
  \end{blockarray}
\end{equation*}


To generalize this, to say $N_O$ times oversampling with $N$ users, we would select the antennas whose phases are within $-\frac{\pi}{(N_O/N)},\frac{\pi}{(N_O/N)}$ using the $\phi$ parameter in the BABF code. Then we will perform the phase aligning across the virtual RF chains by multiplying each of the codes by the respective angles which will align them with the maximally selected set, and thus this will give more control over the generation of the projection matrix $\mathbf{B}$.
Since the phases to select in the groups tighten as $N_O$ increases, once the oversampling factor $N_O$ becomes equal to $N_{\text{Ant}}$, we can just do one antenna per virtual RF chain and handle all the processing in the digital domain. 
At this point \name basically becomes a full blown massive MIMO architecture.
Thus, \name shows a very flexible architecture: which can be tuned to behave like a green hybrid beamformer to a full massive MIMO architecture, all via software level control of the singly laid physical RF chain.

\fi 

% construct matrix

% This process of virtual RF chain creation is what makes \name's architecture flexible, as the number of these virtual RF chains can be easily controlled via software itself.
% To enable this process of virtual RF chain creation, \name's architecture uses RF switches connected to each antenna, as shown in Fig. 1. \todo{cite} have also used similar architectures with RF switches connected to antennas, but they were typically used in static scenarios to extend the array factor, in order to get selection combining gains or improved spatial localization accuracies. 
% However, the real power of these switched architectures is that these switches can really be toggled very fast, and this fast toggling is the essential essence which allows \name to use it for the creation of these virtual RF chains. To the best of our knowledge, \name is the first paper which makes the connection of fast switching with virtual RF chain creation.

% Thus, the natural question becomes, how exactly does \name use fast switching for RF chain virtualization? 
% Let's take a simple example first with $4$ antennas connected to a single RF chain with $4$ switches, similar to Fig. 1.
% Here, in the worst case, we would want $4$ RF chains to be created, one per antenna.
% A flexible architecture would be able to tune down the number of RF chains, i.e. have just 2 RF chains when conditions are good to save on power consumption.
% So the target here is to have a flexible way of generating either 2, or 4 RF chains. 



% Say we have a signal with certain bandwidth $BW$. 
% If we consider a switch with switching frequency $f_s$, that is it has a certain duty cycled 0,1 pattern which repeats after $T_s = 1/f_s$.
% Considering a simple 50\% duty cycled switching rate at $f_s$, we will have frequency components at $0, \pm f_s, \pm 3 f_s$ and so on.
% When the signal with $BW$ bandwidth goes through a $f_s$ rate switch, it basically gets frequency shifted and copies are created at these frequency components of the switch.
% If we want to prevent any interference due to these copies, we need to have sufficient gap between the two copies, that is, we need to have $f_s>BW$.


==> design/design_LO_2.tex <==
% architecture
% how this architecture can be green fixed hybrid
% how this architecture can flex through mu-MIMO and massive MIMO
% what is deployed: mu-MIMO, what is proposed massive MIMO
% LO
\section{Design}

To achieve the two-fold requirements for a green architecture set in ~\cref{sec:background}, \name aims to develop next generation Base Stations that optimize for both the setup power costs at the RF front-end and running power costs of sampling+compute.
In this section, we first dive into the idea of how \name's architecture drastically cuts down on the RF front end power costs in \cref{sec:design-virtual}. Then we show how \name optimizes the running costs by minimizing the sampled data, and data backhauling+compute thereof in \cref{sec:design-babf}.

\subsection{\name's solution to optimize RF front end power}\label{sec:design-virtual}

The first design challenge that \name attempts to solve is to be extremely power efficient at the RF front end.
The requirements are severe; somehow \name has to figure out a method to have constant power in the front-end irrespective of the number of users being served by the architectures.
The reason being that the front end power consumption is like fixed setup cost for the architecture.
This power will be consumed no matter how the user load varies, since it is associated with just the setting up of the physical hardware being used by the architecture.

The current spectrum efficient systems like Massive MIMO, are not power efficient as their power consumption is proportional to the number of RF-chains laid down, which at best is loosely proportional to the maximum number of users they intend to serve.
The fixed power these architectures consumed thus is $O(N)$.
As a consequence, these architectures are designed for maximum number if users $N_{max}$ and then irrespective of the user load the architecture experiences, the architectures will keep on guzzling $O(N_{max})$ power, thus not being green at all.
% As discussed in ~\cref{sec:background} while the existing massive MIMO algorithms try to achieve spectral efficiency by increasing the number of RF-chains to support the spatial diversity, which in turn increases the power consumption because of requirement to have multiple physical RF chains. 
Thus the key design principle which \name overcomes these shortcomings is by laying one single physical RF-chain connecting all the antennas, minimizing the power consumption to $O(1)$.

However, if \name uses multiple antennas connected to a single RF chain, how does \name get back the required degrees of freedom? In attempts to do so, \name borrows certain concepts from OFDMA. 
Recall that, in order to serve $N$ $B$ bandwidth users, OFDMA would widen the sampled bandwidth to $NB$ and have the $N$ users in $N$ different non-intefering frequency bands.
What if \name could do the same, but with antennas instead of users? That is, sample more bandwidth, and try to fit antennas signals into the sampled bandwidth.

At first glance, it may seem that we are trading off the front-end power consumption to the sampling power consumption, by using $NB$ bandwidth to get $N$ antenna signals.
However, this is not the case.
The reason is that ADC's power scales linearly with frequency\cite{yan2019performance,barati2020energy}, with the ADC power equation being
$$P_{ADC}=\text{FoM}\times F_s \times 2^q$$
where \text{FoM} is a constant referred to as figure of merit, $F_s$ is sampling frequency and $q$ is the quantization bits used in ADC.
What we are proposing here is to replace the traditionally used $N$ different ADCs sampling at $B$ each, with a single ADC sampling at $NB$.
Due to linearity of ADC power consumption with sampling frequency, power consumption of $NB$ ADC will be the same as $N$ different $B$ ADCs.
% \name creates a flexible, power efficient multi-antenna architecture by creating multiple virtual RF chains from a singly laid physical RF chain.
% This circumvents challenges in LO distribution across physically laid RF chains as all virtual RF chains share the same downconversion path. 
% Since these virtual RF chains are created digitally, they can be abstracted in software, allowing \name architecture to be flexible, and increase/decrease the virtual RF chains based on channel conditions and the number of users.

% \todo{write the next two paragraphs in a direct way, say how \name does it, then you can explain a bit why those parameters are used.}
Henceforth, \name's design principle is to have multiple antennas connected to a single ADC, which will be sampling at $N$x rate to capture $N$ RF chains abstracted over the sampled bandwidth.
We refer to this concept of creating RF chains over the ADC's digitized samples as `virtual RF chain' creation, since in a way, we virtualize the concept of many virtual RF chains created from a single high-speed physical RF chain.
What virtualization gives us is a design which works with just a single downconnversion chain, which meets the $O(1)$ power requirements.
In addition, we get flexibility on adaptively increasing/decreasing number of RF chains by just tweaking the ADC's sampling rate, leading to a flexible design.
A natural question at this point would be, how does \name actually enable this virtual RF chain creation?
That is, how does \name guarantee that antennas' signal can be accomodated across the $NB$ sampled ADC bandwidth, so that \name can create these virtual RF chains?
% In contrast, \name's design enables it to create multiple virtual RF chains that fit $N$ user signals of $B$ bandwidth each across a $NB$ sampled spectrum.
% To fit these $N$ user signals of $B$ bandwidth each across $NB$ sampled spectrum, \name's ADC needs to firstly sample $NB$ bandwidth digitally. 
% However, merely increasing ADC rate does not by itself create these virtual RF chains. The succinct reason for that by itself, increasing the ADC sampling rate does not give any new diversity, since there are no signals in the new parts of spectrum ADC captures when it's sampling rate increases. 
% So, just blindly increasing the ADC sampling rate to $NB$ would lead the ADC to sample just noise. 
% Instead in \name, we borrow ideas from the backscatter communication that enable them to be low-power, wherein we switch each individual
% \name tries to tweak the circuit parameters of the single laid RF chain.
% But what are the parameters which any RF chain exposes to the controlling software? We have the gain settings for LNA, the mixer's center frequency and the ADC sampling frequency. Definitely tweaking the LNA gains or varying the downconverting frequency won't do us any good for virtualization. 
% However, varying the ADC sampling frequency would imply sampling more bandwidth digitally, allowing for more digital control over the multi-antenna hardware.
% This can possibly allow to fit each antenna's signals across the increased bandwidth; creating virtual RF chains across the sampled spectrum.
% This is similar to how FDMA utilizes assymetricity in transmit bandwidth per user and the total sampled spectrum; \name asks the question that can this assymetricity be also used for creation of virtual RF chains across the sampled spectrum.

\noindent\textbf{Toy example to show virtual RF chain creation}
We attempt to first explain the concept of virtual RF chain creation with help of a simple toy example, where we have a $2$ antenna array. 
As an abstraction, consider first antenna receives a triangular signal and the second antenna receives a rectangular pulsed signal, both signals in frequency domain having bandwidth $B$.
Today's way of capturing the 2 degrees of freedom offered by the array is to have 2 physically laid RF chains, which downconvert and sample these rectangular and triangular signals directly  (Fig. \ref{fig:virt_rfc_naive}(a)). 

Now, \ref{fig:virt_rfc_naive}(b) shows a naive attempt at replacing multiple RF chains in (a) by virtualizing the chains over a single physically laid RF chain, however, by merely increasing the ADC rate.
This leads to combining of the signals from the antennas before getting downconverted by the RF chain, which gives a raised triangular signal in this scenario. 
Since the antenna signals have got combined, \ref{fig:virt_rfc}(b) fails to create these 2 virtual RF chains with isolated triangular and rectangular signals in them.
Thus, merely increasing ADC rate does not by itself create these virtual RF chains, as by increasing the ADC sampling rate we actually did not get any new information on how to untangle the combined antenna signals. 
This is because there is just noise and no antenna signals in the neighbour parts of spectrum captured by the ADC, when it's sampling rate is doubled in hopes of creating $2$ virtual RF chains.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_re_fig1a.pdf}
    \caption{Toy example demonstrating \name's approach to create virtual RF chain from one physically laid chain }
    % \vspace{5pt}
    \label{fig:virt_rfc_naive}
\end{figure}

The key concept behind \name architecture is to create useful signal copies in the neighbour bands, instead of just noise as compared to the naive example considered before; so that when ADC sampling rate increases to accomodate virtual RF chains, it gets the capability to untangle the combined antenna signals to successfully create the virtual RF chains.
To create these signal copies, we need to somehow shift the antenna signals to neighbour bands, before the signals get downconverted through the RF chain.
But how does \name enable this, that too in a low-power way to stay true to the requirements of a power-efficient architecture?

Our insight here is that we can augment the antenna array with RF switches (Fig. \ref{fig:virt_rfc_switch}) toggling with \emph{on-off} codes having time period, equal to signal bandwidth to perform this frequency shifting.
Similar toggling RF switches have also been used for backscatter communications \todo{Cite}, which also demand low-power operation; RF switches in backscatter applications create frequency shifts in reflected signal to avoid interference with line of sight signal.
Hence, \name basically uses RF switches for something similar, to create frequency shifts of the RF signals before they get downconverted, and now with frequency shifts of the antenna signals, the higher sampling rate ADC will be useful as it will capture different frequency shifted antenna signals instead of just neighbour band noise. 

Thus, in order to create these virtual RF chains over a singly laid physical RF chain, \name uses strategic toggling of the RF switches, combined with ADCs increased sampling rate.
We first explain this strategic toggling using the same toy example of 2 virtual RF chains, and later extend it to creation of $N$ RF chains.
When \name wants to create 2 virtual RF chains, the ADCs would be sampling at $2B$, where $B$ is the signal bandwidth, to accommodate the $2$ signals from each RF chain.
Thus, a single ADC sample will occupy total time of $\frac{1}{2B}$, and in order to shift the signals by frequency $B$, the switching code has to repeat every $2$ ADC samples.
This presents us two possible codes $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$.
When we supply these codes to one of the 2 antennas, we have one antenna being toggled \emph{on} for odd samples, and the other antenna toggled \emph{on} for even samples.

This strategic toggling actually creates sum of the $2$ antenna signals in the first nyquist band ($(-B/2)<f<(B/2)$) and difference of the $2$ antenna signals in the second band ($(-B)<f<(-B/2)$ and $(B/2)<f<(B)$), as shown in Fig. \ref{fig:virt_rfc_switch}.
The reason is that $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$ are basically $\pi$ shifted versions of the same frequency codes, and hence the frequency shifted copies they create will reflect this $\pi$ shift, leading to creation of subtracted signals in second band.
This basically then allows us to separate the per-antenna signals by simple signal processing, first add the signals extracted from each nyquist band and then take the difference.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_re_fig1b.pdf}
    \caption{Toy example demonstrating \name's approach to create virtual RF chain from one physically laid chain }
    % \vspace{5pt}
    \label{fig:virt_rfc_switch}
\end{figure}


In order to explain mathematically on why this effect happens, say the antenna signals were $s_1(t), s_2(t)$, these signals are $B$ bandwidth. 
The codes $c_1 = 0,1,0,1,\ldots$ $c_2 = 1,0,1,0,\ldots$ are basically 50\% duty cycled codes with frequency $B$, and RF switches implement these codes in RF domain before downconversion and ADC sampling.
Thus, the ADC finally samples the waveform $s_1(t)c_1(t)+s_2(t)c_2(t)$, at $2B$.
In addition to a constant DC component, these switches also produce harmonics at $\pm B$.
Since $c_2$ is \emph{on} for odd samples and $c_1$ is \emph{on} for even samples, $c_1$'s harmonic at $\pm B$ will basically be $\pm \pi$ of $c_2$. 
This is because the codes are having frequency $B$, thus time period $\frac{1}{B}$, and the associated time delay between $c_1,c_2$ is $0.5(\frac{1}{B})$, thus the phase associated with this time delay would be $(\frac{2\pi}{\frac{1}{B}})0.5(\frac{1}{B}) = \pi$.
The DC component of $c_1,c_2$ however would be the same, since the DC component depends on the average energy, which is a measure of how much time the codes had value $1$ which is same for both.

Thus, as shown in Fig. \ref{fig:virt_rfc_switch} the frequency domain view of the signal sampled by ADC, which was $s_1(t)c_1(t)+s_2(t)c_2(t)$, would have $0.5*(s_1(t)+s_2(t))$ in the first Nyquist band, ($-\frac{B}{2}<f<\frac{B}{2}$) and $0.5*(s_1(t)-s_2(t))$ in the second Nyquist band, ($(-B<f<-\frac{B}{2}) \cup (\frac{B}{2}<f<B)$). A simple digital processing step can now get us back $s_1, s_2$ by simply adding the subtracting these signals in the two Nyquist bands.

Hence, \name utilizes RF switches with different phase codes, coupled with an increased sampling rate ADC in order to virtualize the RF chains. 
This design effectively marries OFDMA to massive MIMO, we end up using more sampling bandwidth to create virtual RF chains over frequency, which allows \name to be as spectrum efficient as massive MIMO and as power efficient as OFDMA.
% This is also supported by recent trends of having faster ADCs, which offer other benefits as well, like simplified baseband filter design, reduced quantization noise amongst others.
% With \name's architecture, virtualization of RF chain concept would be another advantage of faster ADC design.

\noindent\textbf{Generalization to $N$ antennas}:\\
The method of obtaining these virtual RF chains from a single physically laid chain can be easily generalized when we have $N$ antennas with $N$ RF switches and an ADC which is doing $N*B$ times sampling where $B$ is the signal bandwidth.
In this generalized scenario, we will now have $N$ codes $c_1,c_2\ldots c_n$, which will be codes of length $N$ with  $c_1 = {1,0,0,\ldots,0,0}$, $c_2 = {0,1,0,\ldots,0,0}$, $\ldots$, $c_{n-1} = {0,0,0,\ldots,1,0}$ and $c_{n-1} = {0,0,0,\ldots,0,1}$.
Since these are $1/N$ duty cycled codes they will have frequency images at every integral multiple of $B$ and thus total $N$ images at frequencies $\text{fftshift}(0,B,2B,\ldots N)$.
In addition, code $c_i$ is delayed by $\frac{(i-1)}{NB}$, and thus the $j$-th harmonic of $c_i$ will have phases $\frac{(i-1)}{NB}*\frac{2\pi}{\frac{1}{jB}} = (i-1)*j*\frac{2\pi}{N}$.

The ADC is sampling at $NB$, and thus we will have $N$ $B$ bandwidth zones obtained from the ADC sampled stream $R$, denoted by $R^B_1, R^B_2, R^B_3\ldots R^B_N = \mathbf{R^B}$, with $\mathbf{R^B}$ being a $N\times N_s$ matrix which stores the $N_s$ samples correpsonding to each of the $N$-th $B$ bandwidth zone, and we can obtain our virtualized RF chains $S_1,S_2,\ldots S_N = \mathbf{S}$, $S$ being $N \times N_s$ as well, via phase inversion of the $N\times N$ phase matrix $\mathbf{P}$ corresponding to $j$-th harmonic phase of $c_i$:

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{design/design_re_fig2.pdf}
%     % \vspace{3pt}
%     \caption{How switching changes the signal spectrum: example where $N=4$, code $c_2$. Due to time delay of $1/(4*B)$, the phases at harmonics $B,2B,(3B=-B)$ are $1*(2\pi)/4 = 90^o$, $2*(2\pi)/4 = 180^o$ and $3*(2\pi)/4 = 270^o$}
%     % \vspace{5pt}
%     \label{fig:virt_rfc_gen}
% \end{figure}

\begin{equation}
    \mathbf{S} = (\mathbf{e}^{(-\mathbf{P})})* \mathbf{R^B}
\end{equation}

where $\mathbf{e}^{(\cdot)}$ applies the exponential function to each element of the matrix. The matrix $\mathbf{P}$ in detail looks like this:

\begin{equation*}
  \mathbf{P}=
  \begin{blockarray}{*{5}{c} l}
    \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
      0 & B & 2B & $\ldots$ & (N-1)B & \\
    \end{block}
    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
      0 & 0 & 0 & $\ldots$ & 0 \bigstrut[t]& $c_1$ \\
      0 & \frac{2\pi}{N} & \frac{4\pi}{N} & $\ldots$ & \frac{2(N-1)\pi}{N} & $c_2$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(i-1)}{N} & \frac{4\pi(i-1)}{N} & $\ldots$ & \frac{2(N-1)(i-1)\pi}{N} & $c_i$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(N-1)}{N} & \frac{4\pi(N-1)}{N} & $\ldots$ & \frac{2(N-1)(N-1)\pi}{N} & $c_n$ \\
    \end{block}
  \end{blockarray}
\end{equation*}

The reason this generalization works out is because all these are different series of roots of unity, and by doing phase inversion one set of the roots become all co-phased and thus their virtual RF chain component adds up, and the other sets of roots still remain phase shifted versions of their previous versions and add up to 0, which allows \name to extract the RF chain per antenna from the increased sample rate ADC stream.

\noindent\textbf{Using virtual RF chains for spatial-multiplexing}:
\noindent Once we are able to obtain the per-antenna waveforms $\mathbf{S}$, the process to obtain the spatially multiplexed output is straightforward and follows the same method as compared to usual way with physically laid RF chains.
In the scenario when we have $N$ antennas and $N$ RF chains, and say we have $N$ users, we can perform MIMO channel estimation with the $N$ virtual RF chains to get the $N\times N$ channel matrix for all $N$ users and $N$ antennas.

Now, we can choose any precoding strategy to suppress the signals from other users to get individual streams for each of the $N$ users.
For example if we use a simple ZF precoding would multiply the $N\times N$ matrix $\mathbf{H}^{-1}$ to the obtained virtual RF chain matrix $\mathbf{S}$ to get individual interference free $N_s$ samples of each $N$-th users data, stored in the $N\times N_s$ matrix $\mathbf{U}$. 

\begin{equation}
    \mathbf{U} = \mathbf{H}^{-1}\mathbf{S}
\end{equation}

We choose to implement only the linear precoding schemes, like MMSE, BD or ZF, since these schemes, in particular, ZF have been experimentally verified to meet the system capacities \cite{ding2020agora}, while the non-linear precoding methods like THP are still under theoretical research.

Thus, by using just 1 physically laid RF chain, we can enable creation of $N$ virtual RF chains with $N$ antennas and $N$ RF switches, while using just $O(1)$ power consumption at the front-end.


\subsection{\name's solution to optimize sampling+compute power}\label{sec:design-babf}

% A traditional mu-MIMO system strives to serve $N$ users with $N$ antennas, and for this it lays down $N$ physical RF chains.
% However, in practical scenarios, often we need many more number of antennas $N_{\text{ant}}>>N$ number of users in order to serve all the users with a good quality wireless link, and this system is referred to as Massive MIMO.
% The reason is that we need more degrees of freedom than $N$ as the channels of the $N$ users to the base station are often correlated, especially when the users are located close to each other. 
% Thus, having more antennas leads to more degrees of freedom which allows the base station to serve $N$ users effectively.
% Although massive MIMO is info theoretically sound, it is challenging to deploy due to requirement of a massive number of RF chains as well.
% Further, it is not a `green' architecture, since it needs to sample $N_\text{ant}$ data streams, much more than the required number of $N$ data streams to serve $N$ users.
% Also, it is wasteful in terms of the digital processing done after sampling on $N_\text{ant}$ streams, as well as communication of $N_\text{ant}$ streams to the DSP where these algorithms are implemented.

In practical scenarios, it is infeasible to serve $N$ users interfering with just $N$ antennas. 
The reason is that the channel matrix $\mathbf{H}$ often endsup being non-invertible and ill-conditioned to support $N$ spatial stream generation.
Today's massive MIMO architectures, both digital beamforming and hybrid beamforming, use $N_{\text{ant}}>N$ antennas in order to serve $N$ users in a robust manner. 
The reasoning behind the $N_{\text{ant}}>N$ antennas requirement is to capture more than enough degrees of freedom to allow creation of robust $N$ spatial streams, one for each user.

However, to optimize for sampling+compute power it would be ideal to somehow have only $N$ data streams to serve $N$ users and at the same time use $N_{\text{ant}}$ antennas.
Thus, in order to optimize for sampling power \name can  create $N$ virtual RF chains connected to $N_{\text{Ant}}$ antennas, by utilizing $N$ times oversampling ADC. 
However, using $N$ virtual RF chains for handling $N_{\text{Ant}}$ antennas does not allow for separate virtual RF chain per antenna as assumed in the previous sections.
So a natural question is, how does \name's techniques scale to larger number of antennas than number of virtual RF chains, and how does \name still tap into the $N_{ant}$ degrees of freedom with just $N$ virtual RF chains?

The key advantage of \name architecture which allows to effectively use $N_{\text{Ant}}$ antennas' degrees of freedom is that virtual RF chains do not split up antenna array amongst themselves.
Traditional beamformers which connect $N_{\text{Ant}}$ antennas with $N_{\text{Ant}}$ analog circuit elements, to $N$ physical RF chains, end up dividing the antenna array between the $N$ RF chains.
For example, say we have $8$ antennas and $4$ physical RF chains, we would get only $2$ antennas per physical RF chain.
However, virtual RF chains are an abstraction over the single physically laid RF chain, and since all the $8$ antennas here are connected to the single physical RF chain, the entire array is available to each of the virtual RF chain as well.

But how does \name use these degrees of freedom to optimize for sampling+compute power?
The insight here is to configure the antenna array differently for different virtual RF chain.
The idea is that we can dedicate one virtual RF chain to just try and maximise the signal power for one user, and not worry about the interference suppression in the process.
This is because the interference suppression can be taken care of via the digital precoding methods.


Put simply, we try and increase the signal power for user $i$ in the $i$-th virtual RF chain.
In order to do so, we would determine the maximal group of antennas in-phase for user $i$, and turn these antennas on for that virtual RF chain $i$.
We name this algorithm to select the maximal in-phase antennas as $\text{BABF}(\cdot)$ (Algorithm \ref{Alg1}), where BABF stands for Binarized Analog Beamforming.
Essentially, for each virtual RF chain we try to beamform towards individual users using the $0-1$ bit control we have over the switched antenna array.

\begin{algorithm}
  \caption{BABF, Input: $\textbf{H}$, Output: $\mathbf{B}$}
  \begin{algorithmic}[1]
  \label{algo:switch_selection}
  \STATE $\phi$=$\pi/3$;\
  \FOR{ $1 \le i \le K$}{
      \FOR{ $1 \le m \le M$}{
      \STATE $\Tilde{\textbf{b}}_{i,m}=[0, 0 , \ldots , 0]_{1\times M}$;\
      \STATE $\textbf{g}_{i,m}=\textbf{H}_{i}h^*_{i,m}$;\
      \STATE $\boldsymbol{\theta}_{i,m}$=$\angle{\textbf{g}_{i,m}}$;\
      \STATE $\Tilde{\textbf{b}}_{i,m}(m)$=$|\boldsymbol{\theta}_{i,m}|<\frac{\pi}{4}$;\
      \STATE $score_{i,m}=$ Number of elements equal to $1$ in $\Tilde{\textbf{b}}_{i,m}$;
      }
      \ENDFOR
  }
  \ENDFOR
  \STATE $\mathbb{B} :=$ Set of all possible permutations of $score_{i,m}, 1 \le i \le K, 1 \le m \le M$\;
  \STATE $l=1$;\
  \STATE Select $score^*\in \mathbb{B}$ that provides the $l^{\text{th}}$ highest score;\
  \STATE $\mathbf{B}=\mathbf{B}^*$ (corresponding to $score^*$);\
  \IF{$\mathbf{H}\mathbf{B}$ is full rank}
  \STATE $\mathbf{B}$ is the optimal switch configuration;\
  \ELSE
  \STATE $l=l+1$;\
  \STATE Go to line 13;\
  \ENDIF
\end{algorithmic}
\label{Alg1}
\end{algorithm}

That is, with the BABF algorithm we get a switching matrix $\mathbf{B}$, where $\mathbf{B}$ is $N_{\text{Ant}}\times N$, which increases signal power of user $i$ in the $i$-th virtual RF chain, by turning $N_{\text{Ant}}$ antennas on-off strategically.
In summary, BABF algorithm to prioritize 1 user per virtual RF chain ends up projecting the $N\times N_{\text{Ant}}$ channel matrix $\mathbf{H}$, to an equivalent $N\times N$ channel matrix $\mathbf{HB}$.
By prioritizing signal power for one user per virtual RF chain, we make 
$\mathbf{HB}$ as close to identity matrix as possible, by increasing the diagonal entries power (diagonal entries correspond to channel powers for user $i$ for $i$-th virtual RF chain)

Hence, the BABF algorithm chosen $\mathbf{B}$ creates a projected channel $\mathbf{HB}$ such that the remaining interference terms in $\mathbf{HB}$ can be handled easily by digital combining by be inverting this effective channel matrix via ZF approach.

\begin{equation}
    \mathbf{U} = \mathbf{(HB)}^{-1}\mathbf{S}
\end{equation}

The overall approach behind BABF is very similar to how hybrid beamformers optimize the analog part to maximize for signal power and digital part to minimize the interference terms.
Hence, similar to physical hybrid counterparts using analog circuits to connect more antennas to less number of physical RF chains, \name's virtual architecture can also hybridize to support more number of antennas than virtual RF chains. This allows \name to effectively project the $N_{ant}$ degrees of freedom to $N$ streams, which optimizes for sampling+compute power.


%  by supplying same code $c_i$ corresponding to the $i$-th RF chain, to antennas which are in-phase for user $i$ (that is, have the channel angles within $\pm \pi/4$).
% We make an observation that $c_i = \{0,\ldots,1,\ldots,0\}$, which has a $1$ at the $i$-th position is orthogonal to any $c_j$, $j\neq i$.
% Thus, we can add these codes when we want to have antennas to appear in more than one virtual RF chains.
% Say for an example, we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
% So, here, for antennas $\{1,6\}$, which is to be selected for both the users, we will give the code $c_1+c_2$. For antennas $\{3,5\}$, we will give the code $c_1$, and for $\{2,7,8\}$ we will give $c_2$.
% This will ensure that for virtual RF chain $1$ corresponding to $c_1$, the signals from antennas $\{1,3,5,6\}$ would be combined and for virtual RF chain $2$, we will get combined signals from $\{1,2,6,7,8\}$.

% \ifflex

% \subsection{Adapting to averse channel conditions with high sampling rate}
% \todo{Draw a channel phase figure here}
% In the last section we showed how \name's architecture can enable green communications by restricting only to $N$ times ADC sampling to serve $N$ users, at the same time using a $N_{\text{Ant}}>N$ antennas.
% However, there might be scenarios where channel conditions are so bad that it is required to really bump up the sampling rate.
% By increasing the sampling rate, we can get more control over the projected channel $\mathbf{HB}$.
% However, we need to generalize our projection matrix generation when we bump up the sampling rate.

% For an example, consider we have $8$ antennas, $2$ users and we oversample by a factor of $4$, which gives us $4$ virtual RF chains. In the previous section, we used $2$ times oversampling to handle 2 users, and used $2$ codes $c_0,c_1$ to implement the BABF matrix $\mathbf{B}$. The BABF algorithm basically selected antennas which are maximally \emph{in-phase}, i.e. their channel angles are within $-\pi/2,\pi/2$ of each other.
% When we have $4$ chains at our disposal for $2$ users, we can then infact, select the antennas which were turned off before in the other $2$ spare codes, and do the phase aligning in digital domain to get more SNR gain for the user.
% In a way, this is a way of refining the beamforming weights by implementing precise phase rotations across the digital samples, instead of simple $0/1$ as compared to previous section.

% Put mathematically, we have $c_0$ implementing the maximal antenna set for user $1$, $c_1$ implementing the complimentary set for user $2$, and $c_2,c_3$ doing the same for user $2$.
% Taking the same example as before, say we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
% $c_0$ will turn on $\{1,3,5,6\}$, $c_1$ will turn on $\{2,4,7,8\}$, $c_2$ will do $\{1,2,6,7,8\}$ and finally $c_4$ will do $\{3,4,5\}$.
% Then the virtual RF chain corresponding to $c_0$ will be added to $e^{j\pi}$ times that of $c_1$ to get everything phase aligned, and same with $c_1,c_2$.
% Thus, we will get the following $\mathbf{B}$ matrix:


% \begin{equation*}
%   \begin{blockarray}{*{8}{c} l}
%     % \begin{block}{*{8}{>{$\footnotesize}c<{$}} l}
%     \begin{block}{*{8}{c}>{$\footnotesize}l<{$}}
%      1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Ant. index\\
%     \end{block}
%     \begin{block}{[*{8}{c}]>{$\footnotesize}l<{$}}
%       1 & e^{j\pi} & 1 & e^{j\pi} & 1 & 1 & e^{j\pi} & e^{j\pi}\bigstrut[t]& User 1 \\
%       1 & 1 & e^{j\pi} & e^{j\pi} & e^{j\pi} & 1 & 1 & 1 & User 2 \\
%     \end{block}
%   \end{blockarray}
% \end{equation*}


% To generalize this, to say $N_O$ times oversampling with $N$ users, we would select the antennas whose phases are within $-\frac{\pi}{(N_O/N)},\frac{\pi}{(N_O/N)}$ using the $\phi$ parameter in the BABF code. Then we will perform the phase aligning across the virtual RF chains by multiplying each of the codes by the respective angles which will align them with the maximally selected set, and thus this will give more control over the generation of the projection matrix $\mathbf{B}$.
% Since the phases to select in the groups tighten as $N_O$ increases, once the oversampling factor $N_O$ becomes equal to $N_{\text{Ant}}$, we can just do one antenna per virtual RF chain and handle all the processing in the digital domain. 
% At this point \name basically becomes a full blown massive MIMO architecture.
% Thus, \name shows a very flexible architecture: which can be tuned to behave like a green hybrid beamformer to a full massive MIMO architecture, all via software level control of the singly laid physical RF chain.

% \fi 

% construct matrix

% This process of virtual RF chain creation is what makes \name's architecture flexible, as the number of these virtual RF chains can be easily controlled via software itself.
% To enable this process of virtual RF chain creation, \name's architecture uses RF switches connected to each antenna, as shown in Fig. 1. \todo{cite} have also used similar architectures with RF switches connected to antennas, but they were typically used in static scenarios to extend the array factor, in order to get selection combining gains or improved spatial localization accuracies. 
% However, the real power of these switched architectures is that these switches can really be toggled very fast, and this fast toggling is the essential essence which allows \name to use it for the creation of these virtual RF chains. To the best of our knowledge, \name is the first paper which makes the connection of fast switching with virtual RF chain creation.

% Thus, the natural question becomes, how exactly does \name use fast switching for RF chain virtualization? 
% Let's take a simple example first with $4$ antennas connected to a single RF chain with $4$ switches, similar to Fig. 1.
% Here, in the worst case, we would want $4$ RF chains to be created, one per antenna.
% A flexible architecture would be able to tune down the number of RF chains, i.e. have just 2 RF chains when conditions are good to save on power consumption.
% So the target here is to have a flexible way of generating either 2, or 4 RF chains. 



% Say we have a signal with certain bandwidth $BW$. 
% If we consider a switch with switching frequency $f_s$, that is it has a certain duty cycled 0,1 pattern which repeats after $T_s = 1/f_s$.
% Considering a simple 50\% duty cycled switching rate at $f_s$, we will have frequency components at $0, \pm f_s, \pm 3 f_s$ and so on.
% When the signal with $BW$ bandwidth goes through a $f_s$ rate switch, it basically gets frequency shifted and copies are created at these frequency components of the switch.
% If we want to prevent any interference due to these copies, we need to have sufficient gap between the two copies, that is, we need to have $f_s>BW$.


==> design/design_SAM_BABF.tex <==
% !TEX root = ../paper.tex
\section{Design}~\label{sec:design}

% Contribution 1: create virtual RF chains on the go, idea: single physical chain with multuple virtual chains carved from the samples spectrum

% Contribution 2: Virtualization entails that all antennas are connected to all virtual chains: how do you de-multiplex and the key ideas behind antenna switching

% Contribution 3: Antenna switching algorithm to put it all together.


\name designs a new multi-user communication architecture which is able to serve multiple users with a single physically laid RF chain connected to multiple antennas via a network of RF switches.
In this section, first we will describe \name Switched Antenna Multiplexing (SAM), which multiplexes the received interfered signals of $N$ users and $B$ bandwidth at each antenna into multiple frequency shifted copies, by switching at $NB$ rate on-off codes.
Second, we describe \name's Binarized Analog Beamforming (BABF) which carves out $N$ separate $B$ bandwidth virtual RF chains, with each RF chain separately maximizing one user's signal power.
Then, to put it all together and get interference-free per-user signals, we describe how \name combines across the created virtual RF chains with digital-wideband precision in order to cancel any residual interference left in the virtual RF chains.

% handle ADC in B&M

%Onion layers:
% 1. Tease multiplexing, why it is required and the name of technique
% 2. SAM does bandwidth widening: no need to tell RF switches etc
% 3. Naive solution: Cant just widen bandwidth at receive
\subsection{\name SAM: Switched Antenna Multiplexing }\label{sec:design-virtual}

% Introduce antenna multiplexing first time
\name creates a new multi-user communication architecture  which is green, flexible and spectrum efficient, as a consequence of using a single physical RF chain connected to multiple antennas.
Since all the antennas share the same RF chain, a central requirement is to somehow multiplex the antennas' signals.
Multiplexing the antennas' outputs would prevent loss of degrees of freedom captured by the single physically laid RF chain, and allow carving of virtual RF chains flexibly in response to user load.
\name achieves this via the Switched Antenna Multiplexing (SAM) technique. 

% SAM overview
The key idea behind SAM is to take the $B$ bandwidth received signal at an antenna and spread it into a wider $MB$ intermediate bandwidth. 
Each of the $M$ antennas do this in a distinct manner with a different spreading strategy.
Hence, the $MB$ signals from each antenna gets combined across these $M$ antennas to create a single $MB$ bandwidth signal which is downconverted and sampled by the single physical RF chain.
Since each antenna spreads $B$ bandwidth onto $MB$ in a distinct manner, it is possible to isolate the original $B$ bandwidth signals received at $M$ antennas from the single $MB$ sampled signal.
Hence, in a way, SAM enables antennas to get mapped to the net sampled bandwidth of the single RF chain.
The sampled bandwidth in \name architecture can be increased/reduced in response to user load, and then SAM can adaptively be used to control the degrees of freedom, which leads to a flexible architecture.
Further, virtualization of downconversion hardware leads to both silicon, as well as power savings, further bolstering \name as a green communication architecture.

% naive solution
However, SAM can not be enabled by merely playing around with sampled bandwidth of the RF chain.
\noindent To explain this, we consider a simple toy example, where we have a $M=2$ antenna array.
As an abstraction, consider first antenna receives a triangular signal and the second antenna receives a rectangular pulsed signal, both signals in frequency domain having bandwidth $B$  (Fig. \ref{fig:virt_rfc_naive}(a)).
Fig.~\ref{fig:virt_rfc_naive}(b) shows the naive attempt at antenna multiplexing by merely increasing the ADC rate to $2B$ in hopes of capturing the signals from the two antennas.
Since the antenna signals have got combined into a raised triangular signal before downconversion and sampling, \ref{fig:virt_rfc_naive}(b) fails to isolate the triangular and rectangular signals.
Thus, merely increasing ADC rate does not by itself does not allow for multiplexing, as by increasing the ADC sampling rate we actually did not get any new information on how to untangle the combined antenna signals. 
This is because there is just noise and no antenna signals in the additional spectrum $2$ times sampled bandwidth of ADC to get antenna multiplexing.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_re_fig1a.pdf}
    \caption{Toy example showing (a) $2$ physical RF chains and (b) a naive approach towards virtualization by increasing merely the ADC sampling rate}
    % \vspace{5pt}
    \label{fig:virt_rfc_naive}
\end{figure}

% Now start telling SAM. Piece of info: RF switch and hamronics (Fig. 2a)
So, to actually enable antenna multiplexing, it is required to create useful signal copies in the neighbour bands, instead of just noise as compared to the naive example considered before.
To create signal copies in the additionally sampled bands, we need to somehow shift the antenna signals to neighbour bands.
\name's insight here is to augment the antenna array with RF switches toggling with \emph{on-off} codes which create frequency shifted harmonics and thus help create these frequency shifted signal copies, hence creating SAM.
Similar toggling RF switches have also been used for backscatter communications \cite{zhang2017freerider,zhang2016hitchhike,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, at minimal power operation to even enable low-power batteryless operation of such frequency shift methods. 
\name uses these low-power RF switches to create frequency shifts of the RF signals and enable the required antenna multiplexing via a singly laid RF chain, and hence we refer it as SAM (Switched Antenna Multiplexing). SAM also enables the higher sampling rate ADC to be useful as it will capture different frequency shifted antenna signals instead of just neighbour band noise. 
% The idea behind \name SAM is to use $N$ distinct $B$ bandwidth toggling codes to create $N$ times multiplexing across antennas with $NB$ bandwidth sampling ADC.

% SAM discussion: 1/N duty cycled codes (Fig 2b)
SAM essentially uses $1/M$ duty cycled on-off $B$ frequency codes (shown in Fig. \ref{fig:duty_fig} (a)), and sample these with $MB$ bandwidth, we get $M$ copies of frequency shifted signals at frequencies $0,B,2B\ldots (M-1)B$.
% To understand how SAM works, we denote the received $B$ bandwidth signal at an antenna as $s(t)$, which goes through a RF switch toggling with $c(t)$ on-off code. 
% Due to switching, the received signal basically gets multiplied by the code in the time domain to give $s(t)c(t)$, corresponding to  
% convolution in frequency domain $S(f)*C(f)$.
% SAM designs the code $c(t)$ such that the corresponding frequency transform $C(f)$ has $M$ different harmonics $B$ bandwidth apart to fill the $MB$ sampled spectrum and create useful frequency shifted signal copies.
% Show how 1/N gives N distinct spikes equal level 
Without loss of generality let us see how SAM works for $M=4$.
When we have $M$ = 4, we have codes repeating after $T=1/B$ period and getting sampled at $T_s = 1/4B$.
With this, we can have $4$ distinct codes: 
$c_0[n]= c_0(nT_s) = \{1,0,0,0,1,0,0,0\ldots\}$,
$c_1[n]=\{0,1,0,0,0,1,0,0\ldots\}$,
$c_2[n]=\{0,0,1,0,0,0,1,0\ldots\}$,
and $c_3[n]=\{0,0,0,1,0,0,0,1\ldots\}$ (Fig. Fig. \ref{fig:duty_fig} (c)).
Since the sampling period $T_s = 1/4B$ and as these codes repeat after $4$ samples, the time period of codes is $1/B$.
% Each of these codes essentially have the same frequency components as these are the same codes just separated out in phase as denoted by the location of $``1"$ in these codes.

% Hence, when a signal $s[n]$ is switched with one of these codes, say $c_0[n]$, we get $s[n]c_0[n]$ since the signal in a way gets multiplied by ``1"s and ``0"s.
% Equivalently, in the frequency domain, the $B$ bandwidth signals $s[n]$ get convolved with the codes it creates the signal copies centered at each of these center frequencies where the codes have delta functions, hence populating the entire $4B$ sampled spectrum with these $4$ signal copies.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/des_fig2.pdf}
    \caption{\name SAM codes: continuous and discrete time}
    \label{fig:duty_fig}
\end{figure}

The fourier transform of these codes gives $4$ delta functions centered at these $4$ frequencies, $0,B,2B,3B$.
Intuitively, what is happening is that although the continuous time fft of the $1/4$ duty cycle $B$ frequency code gives harmonics spread according to a sinc sequence, when this code is sampled with $4B$ bandwidth, the copies alias around to give $4$ distinct peaks at $0,B,2B,3B$ (Fig. \ref{fig:duty_fig}(b,d)), with different $c_i$ giving different phases at each of these peaks.
To see how the $4$ codes give equal magnitude delta functions at the 4 frequencies, and see in detail how different codes give different phases across the copies, we mathematically analyze the fourier transform for these codes.
For the code $c_i[n]$, we get $C_i[f]$ which gives the delta functions and the phases,
\begin{equation}
c_i[n] = \begin{cases}
1,\text{if }n=4k+i\\
0,\text{otherwise}
\end{cases}
\end{equation}
\begin{equation}
C_i[f] = \sum_{n=0}^{N} c[n]e^{-j2\pi f nT_s} = \sum_{n=4k+i,k=0}^{k<[\frac{N}{4}]}e^{-j2\pi f \frac{(4k+i)}{4B}}
\end{equation}
\begin{equation}
    \therefore C_i[f] = e^{\frac{(-j2\pi f i)}{4B}}\sum_{k=0}^{k<[\frac{N}{4}]}e^{\frac{(-j2\pi f k)}{B}} = \begin{cases}
    e^{\frac{(-j2\pi f i)}{4B}}(N/4)\\\text{ if } f=0,B,2B,3B\\
    0, \text{ otherwise}
    \end{cases}
\end{equation}

Hence, depending on choice of $i$, the $4$ $N/4$ peaks at $f=0,B,2B,3B$ have the different phases $e^{\frac{(-j2\pi fi)}{4B}}$ (In case of $M=4$, these phases are multiples of $90^{o}$, as shown in Fig. \ref{fig:duty_fig}(b)). Intuitively, what happens is that when you sample the $1/4$ duty cycled codes of frequency $B$ with $4B$ sampling frequency, the harmonics alias and give equal peaks at the 4 frequencies within the sampling frequency (Fig.). 
Note that here, we consider frequencies $f=0,B,2B,3B$ which can be equivalently written as $f=0,B,-2B,-B$ after taking a fftshift. 
Since the peaks are $B$ bandwidth separated out, when the $B$ bandwidth signals are passed via the RF switches, they undergo frequency domain convolution and these delta functions create $4$ signal copies around these $4$ center frequencies.
Since we have different phases across the $4$ codes, we can use these codes to capture $4$ degrees of freedom since this multiplexing allows to pack $4$ antennas $B$ bandwidth signal across the $4B$ sampled bandwidth of the single RF chain.

\subsection{Creating Virtual RF chains from SAM}

Now we have shown how SAM enables creation of $N$ degrees of freedom from a single downconversion chain sampling at $N$ times.
However, SAM by itself does not provide isolated degrees of freedom since we have $N$ different phase copies getting added over the $NB$ bandwidth sampled bandwidth.
The key insight which allows \name to isolate the degrees of freedom generated by the distinct codes is that we can separate out the $N$ different $B$ bandwidth regions of the $NB$ sampled bandwidth to generate $N$ different linear equations.
These $N$ equations are generated by different ways of combining the $N$ different degrees of freedom (unknown) from the antennas from the $N$ different (known) codes, and hence can be solved for the unknowns to isolate the $N$ degrees of freedom.

As a toy example, consider $N=2$.
When \name wants to create 2 virtual RF chains, SAM would require the ADCs to sample at $2B$, to accommodate the $2$ signals from each antenna, and switch the antennas via the two codes $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$.
Hence, for the first sequence $i=0$, we have $0$ phase signal copies in both the $0-B$ and $B-2B$ band.
For the second sequence with $i=1$, we have $0$ phase in the $0-B$ band and $e^{-j2\pi B/(2B)} = e^{-j\pi}$ in the $B-2B$ band.
Hence SAM creates sum of the $2$ antenna signals in the first Nyquist band and difference of the $2$ antenna signals in the second band, as shown in Fig. \ref{fig:virt_rfc_switch}.
This then allows us to separate the per-antenna signals by simple signal processing, first add the signals extracted from each Nyquist band and then take the difference as illustrated in Fig. \ref{fig:virt_rfc_switch}. Thus \name creates these virtual RF chains with a single physically laid RF chain and isolate the per antenna signals.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_re_fig1b.pdf}
    \caption{Toy example demonstrating \name's approach to create virtual RF chain from $N=2$ SAM }
    % \vspace{5pt}
    \label{fig:virt_rfc_switch}
\end{figure}

% connection to 2 antennas
\noindent\textbf{Generalization to $M$ antennas}:\\
The method of obtaining these virtual RF chains from a single physically laid chain can be easily generalized from $2$ to a general $M$ antennas with $M$ RF switches and an ADC which is doing $MB$ times sampling.
In this generalized scenario, we will now have $M$ codes $c_0,c_1\ldots c_{M-1}$, which are $1/M$ duty cycled codes having delta functions at every integral multiple of $B$ and thus total $N$ images at frequencies $\text{fftshift}(0,B,2B,\ldots N)$.
In addition, code $c_i$ is delayed by $\frac{(i-1)}{MB}$, and thus the $j$-th harmonic of $c_i$ will have phases $\frac{(i-1)}{MB}*\frac{2\pi}{\frac{1}{jB}} = (i-1)j\frac{2\pi}{M}$.

The ADC is sampling at $MB$, and thus we will have $M$ $B$ bandwidth zones obtained from the ADC sampled stream $R$, denoted by $R^B_1, R^B_2, R^B_3\ldots R^B_N = \mathbf{R^B}$, with $\mathbf{R^B}$ being a $M\times N_s$ matrix which stores the $N_s$ samples correpsonding to each of the $M$-th $B$ bandwidth zone, and we can obtain our virtual RF chains $S_1,S_2,\ldots S_M = \mathbf{S}$, $S$ being $N \times N_s$ as well, via phase inversion of the $N\times N$ phase matrix $\mathbf{P}$ corresponding to $j$-th harmonic phase of $c_i$:

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{design/design_re_fig2.pdf}
%     % \vspace{3pt}
%     \caption{How switching changes the signal spectrum: example where $N=4$, code $c_2$. Due to time delay of $1/(4*B)$, the phases at harmonics $B,2B,(3B=-B)$ are $1*(2\pi)/4 = 90^o$, $2*(2\pi)/4 = 180^o$ and $3*(2\pi)/4 = 270^o$}
%     % \vspace{5pt}
%     \label{fig:virt_rfc_gen}
% \end{figure}

\begin{equation}
    \mathbf{S} = (\mathbf{e}^{(-\mathbf{P})})* \mathbf{R^B}
\end{equation}

where $\mathbf{e}^{(\cdot)}$ applies the exponential function to each element of the matrix. The matrix $\mathbf{P}$ in detail looks like this:

\begin{equation*}
  \mathbf{P}=
  \begin{blockarray}{*{5}{c} l}
    \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
      0 & B & 2B & $\ldots$ & (N-1)B & \\
    \end{block}
    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
      0 & 0 & 0 & $\ldots$ & 0 \bigstrut[t]& $c_1$ \\
      0 & \frac{2\pi}{N} & \frac{4\pi}{N} & $\ldots$ & \frac{2(N-1)\pi}{N} & $c_2$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(i-1)}{N} & \frac{4\pi(i-1)}{N} & $\ldots$ & \frac{2(N-1)(i-1)\pi}{N} & $c_i$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(N-1)}{N} & \frac{4\pi(N-1)}{N} & $\ldots$ & \frac{2(N-1)(N-1)\pi}{N} & $c_n$ \\
    \end{block}
  \end{blockarray}
\end{equation*}

The reason this generalization works out is because all these are different series of roots of unity, and by doing phase inversion one set of the roots become all co-phased and thus their virtual RF chain component adds up, and the other sets of roots still remain phase shifted versions of their previous versions and add up to 0, which allows \name to extract the RF chain per antenna from the increased sample rate ADC stream.

Hence, this simple signal processing step allows \name to isolate the $M$ degrees of freedom generated via the $M$ different $1/M$ duty cycle codes via SAM, thus creating the $M$ virtual RF chains.

% \noindent\textbf{Using virtual RF chains for spatial-multiplexing}:
% \noindent Once we are able to obtain the per-antenna waveforms $\mathbf{S}$, the process to obtain the spatially multiplexed output is straightforward and follows the same method as compared to usual way with physically laid RF chains.
% In the scenario when we have $N$ antennas and $N$ RF chains, and say we have $N$ users, we can perform MIMO channel estimation with the $N$ virtual RF chains to get the $N\times N$ channel matrix $H$ for all $N$ users and $N$ antennas.

% Now, we can choose any precoding strategy to suppress the signals from other users to get individual streams for each of the $N$ users.
% For example if we use a simple ZF precoding would multiply the $N\times N$ matrix $\mathbf{H}^{-1}$ to the obtained virtual RF chain matrix $\mathbf{S}$ to get individual interference free $N_s$ samples of each $N$-th users data, stored in the $N\times N_s$ matrix $\mathbf{U}$. 

% \begin{equation}
%     \mathbf{U} = \mathbf{H}^{-1}\mathbf{S}
% \end{equation}

% We choose to implement only the linear precoding schemes, like MMSE, BD or ZF, since these schemes, in particular, ZF have been experimentally verified to meet the system capacities \cite{ding2020agora}, while the non-linear precoding methods like THP are still under theoretical research.

% Thus, by using just 1 physically laid RF chain and SAM implemented via RF switches, we can enable creation of $M$ virtual RF chains with $M$ antennas and $M$ RF switches

\subsection{Having N$>>$M antennas with $MB$ bandwidth RF chain}

Till now we have shown how SAM creates $M$ degrees of freedom in the $MB$ sampled bandwidth, and how these degrees of freedom become the $M$ virtual RF chains via a simple signal processing step.
These virtual RF chains contain the $B$ bandwidth signal received at each of the $M$ antennas (denoted by $\mathbf{S}$), which can then be further used to serve $M$ intefering users, by further solving for $M$ users channels across the $M$ antennas, denoted by $M\times M$ matrix $\mathbf{H}$ (can be obtained by $\text{channel\_estimation}(\mathbf{S})$) and then inverting the channels to get interference free streams $\mathbf{U} = H^{-1}S$.

However, often, with real world channels, this inversion of $M\times M$ matrix doesn't give good SINR performance, and there are mainly two reasons for this.
First, if the users are located close to each other this matrix might not be invertible since the channels are very similar to each other and the matrix doesn't really have a full rank.
Secondly, such channel inversion can cause noise boosting when users' signal powers are comparable across the RF chains.
As an example, consider a simple toy case with $2$ users where the channel matrix is $H=\begin{bmatrix} 1 & -1 \\
                1 & 1
\end{bmatrix}$.
Here to obtain the interference free streams $U$, we need to add and subtract the two $1\times N_s$ vectors $S_1$, $S_2$, that is 
$U = \begin{bmatrix} S_1+S_2 \\
                S_1-S_2
\end{bmatrix}$.
On hardware, we won't have the true $S_1, S_2$, we would have $\hat{S}_1,\hat{S_2} = S_1+n_1, S_2+n_2$ respectively, where $n_1,n_2$ can be assumed iid $\mathcal{N}(0,N_0)$.
Hence, the obtained $U = \begin{bmatrix} S_1+S_2+n_1+n_2 \\
                S_1-S_2+n_1-n_2
\end{bmatrix}$.
Since $n_1,n_2$ are iid, both $n_1+n_2, n_1-n_2$ would be $\mathcal{N}(0,2N_0)$, since noise powers always add up.
Hence, even though the channel inversion step handles interference, it boosts the noise power to double it's value and worsens the final obtained SINR.

In comparison, say the toy channel was  $H=\begin{bmatrix} 2 & -1 \\
                1 & 2
\end{bmatrix}$.
Now, $U = \begin{bmatrix} S_1+\frac{S_2}{2}+n_1+\frac{n_2}{2} \\
                -\frac{S_1}{2}+S_2+\frac{n_1}{2}-n_2
\end{bmatrix}$.
Here, $n_1+\frac{n_2}{2}, -\frac{n_1}{2}+n_2$ would be $\mathcal{N}(0,1.25N_0)$, and thus the noise would not be boosted as much.
Thus, the general idea is that the channel matrix $\mathbf{H}$, in addition to being well conditioned such that inverse exists, needs to have higher diagonal terms as possible to avoid noise boosting.

In order to achieve this behaviour, and enable interference suppression without noise boosting, a common approach is to increase number of antennas to $N>>M$ where $M$ is number of users, as is the case with massive MIMO and traditional hybrid beamforming.
In \name we utilize $N>>M$ antennas to create artificial $M\times M$ channels, which has higher on-diagonal entries in the channel matrix.
In other words, the $N$ antennas are toggled such that the created $M$ virtual RF chains from the $M$ DoF SAM have higher signal power for one user than the others, such that the channel matrix is structured in the desired diagonal heavy manner.
To achieve this, \name idea is to introduce BABF, short for Binarized Analog BeamForming.

BABF basically selects the maximal group of antennas which are in-phase to a particular user $i$, and turns them on for the corresponding $i$-th virtual chain by supplying $c_i$ code to all the antennas in the maximal group.
In this manner, all the antennas' signal combine in the thus created $i$-th virtual chain, and since these are in-phase for the particular user, the user's power increases because of constructive combining, whereas the same doesn't happen for the other users. 
This basically creates the desired diagonal heavy channel structure and helps digital interference suppression without noise boosting.
But, in realistic scenario, the maximal group of antennas for one user could have common antennas with other user's group as well.
Hence, this would require these common antennas to be "on" for both the user's virtual chains.
This is easily made possible since the codes $c_i, c_j$ are orthogonal, and when we need to turn an antenna "on" for virtual chain $i,j$ corresponding to user $i,j$ we can do that by supplying $c_i+c_j$ to that antenna.

Hence, the SAM and virtual RF chain creation mechanism allows controlling which antennas turn on for any virtual chain, and multiple antennas can be one for the same chain, as well as one antenna can be on for a particular virtual chain.
Thus, mathematically, SAM+virtual chain creation allows us to project the $M\times N$ channel $\mathbf{H}$ into an equivalent $M\times M$ channel $\tilde{\mathbf{H}} = \mathbf{H}\mathbf{B}$ via a binary $N \times M$ matrix $\mathbf{B}$ which tells if antenna $n$ was ``on" or ``off" for virtual chain $m$.

The matrix $\mathbf{B}$ is chosen via the BABF approach to create diagonal heavy $\tilde{\mathbf{H}}$. 
The process of virtual RF chain creation then gives the $M\times N_s$ streams $\mathbf{S}$ formed due to the combination of the $N$ antennas turned "on" for each of the $M$ virtual chains in $\mathbf{S}$.
A simple channel inversion step allows us to compute the interference free streams from $\mathbf{S}$ via $\mathbf{U} = \tilde{\mathbf{H}}^{-1}S$.
Since $\tilde{\mathbf{H}}=\mathbf{H}\mathbf{B}$ is designed to be diagonal heavy, this inversion process suppresses interference without boosting noise by a lot and thus allowing $M$ interfering to be served via just $M$ DoFs captured via the SAM technique using $MB$ bandwidth chain and $1/M$ duty cycled codes.



% The frequency domain of each of these codes represent delta functions at frequencies $0,B,2B,3B$ and hence when a $B$ bandwidth signal is convolved with these codes it creates signal copies centered around these $4$ delta functions.

% We denote the $4$ codes as $c_i[n]$ where $i={0,1,2,3}$ appropriately, and $c_i[n]$ has $1$ at positions $4k+i$ where $k$ is an integer.






% let us revisit the aforementioned toy example of 2 virtual RF chains and it can easily be extended to creation of $N$ RF chains that is discussed later.
% So, for the 2 antenna toy example, when \name wants to create 2 virtual RF chains, the ADCs would be sampling at $2B$, where $B$ is the signal bandwidth, to accommodate the $2$ signals from each RF chain.
% Thus, a single ADC sample will occupy total time of $\frac{1}{2B}$, and in order to shift the signals by frequency $B$, the switching code has to repeat every $2$ ADC samples.
% This presents us two possible codes $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$.
% When we supply these codes to one of the 2 antennas, we have one antenna being toggled \emph{on} for odd samples, and the other antenna toggled \emph{on} for even samples.

% This strategic toggling actually creates sum of the $2$ antenna signals in the first Nyquist band ($(-B/2)<f<(B/2)$) and difference of the $2$ antenna signals in the second band ($(-B)<f<(-B/2)$ and $(B/2)<f<(B)$), as shown in Fig. \ref{fig:virt_rfc_switch}.
% The reason is that $0,1,0,1,0,1,\ldots$ and $1,0,1,0,1,0,\ldots$ are basically $\pi$ shifted versions of the same frequency codes, and hence the frequency shifted copies they create will reflect this $\pi$ shift, leading to creation of subtracted signals in second band.
% Fundamentally, this then allows us to separate the per-antenna signals by simple signal processing, first add the signals extracted from each Nyquist band and then take the difference as illustrated in Fig. \ref{fig:virt_rfc_switch}. Thus \name creates these virtual RF chains with a single physically laid RF chain and strategically toggles the multiple switches connected to the multiple antennas to serve multiple users in a low-power and spectrum efficient fashion.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{design/design_re_fig1b.pdf}
%     \caption{Toy example demonstrating \name's approach to create virtual RF chain from one physically laid chain }
%     % \vspace{5pt}
%     \label{fig:virt_rfc_switch}
% \end{figure}


% To further provide some mathematical intuition on why this effect happens, say the antenna signals were $s_1(t), s_2(t)$, these signals are $B$ bandwidth. 
% The codes $c_1 = 0,1,0,1,\ldots$ $c_2 = 1,0,1,0,\ldots$ are basically 50\% duty cycled codes with frequency $B$, and RF switches implement these codes in RF domain before downconversion and ADC sampling.
% Thus, the ADC finally samples the waveform $s_1(t)c_1(t)+s_2(t)c_2(t)$, at $2B$.
% In addition to a constant DC component, these switches also produce harmonics at $\pm B$.
% Since the codes have a frequency $B$, thus time period $\frac{1}{B}$, and the associated time delay between $c_1,c_2$ is $0.5(\frac{1}{B})$, thus the phase associated with this time delay would be $(\frac{2\pi}{\frac{1}{B}})0.5(\frac{1}{B}) = \pi$.

% Thus, as shown in Fig. \ref{fig:virt_rfc_switch} the frequency domain view of the signal sampled by ADC, would have a summed up signal ($0.5*(s_1(t)+s_2(t))$) in the first Nyquist band, ($-\frac{B}{2}<f<\frac{B}{2}$) and a differential signal ($0.5*(s_1(t)-s_2(t))$) in the second Nyquist band, ($(-B<f<-\frac{B}{2}) \cup (\frac{B}{2}<f<B)$). A simple digital processing step can now get us back $s_1, s_2$ by simply adding the subtracting these signals in the two Nyquist bands.

% Hence, \name utilizes RF switches with different phase codes, coupled with an increased sampling rate ADC in order to virtualize the RF chains. 
% This design effectively marries OFDMA to massive MIMO, we end up using more sampling bandwidth to create virtual RF chains over frequency, which allows \name to be as spectrum efficient as massive MIMO and as power efficient as OFDMA.

==> design/design_flex.tex <==
% architecture
% how this architecture can be green fixed hybrid
% how this architecture can flex through mu-MIMO and massive MIMO
% what is deployed: mu-MIMO, what is proposed massive MIMO
\section{Design}
Multi-antenna MIMO architectures have played a critical role in helping wireless networks scale with number of users without adding new spectrum. 
Each antenna brings about a new degree of freedom, and capturing these degrees of freedom is what allows MIMO systems to handle multiple users communicating together.
Capturing these degrees of freedom today requires connecting dedicated circuitry, referred to as a RF chain, per antenna, which does not allow for seamless software control and goes against the recent trends of virtualization of communication networks.
In this section, first we will explain how we can capture these degrees of freedom via a new architecture which can offer software-level control, by essentially virtualizing these RF chains.
Then, we will show the two applications which are made possible by our new architecture, namely, green communication circuits made possible by digital processing and sampling commensurate with number of users, and a flexible mode of operation where the worse channel conditions can be countered by scaling the sampling rate of the architecture.

\subsection{Virtualizing RF chains}

\subsubsection{Toy example to show \name's working}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{design/design_re_fig1.pdf}
    \caption{Toy example demonstrating \name's approach to create virtual RF chain from one physically laid chain}
    % \vspace{5pt}
    \label{fig:virt_rfc}
\end{figure*}

The RF chains in a typical receive MIMO architecture basically perform three tasks, they amplify the weak signal at the antenna, downconvert the signal to baseband and finally sample it via an ADC to get digital baseband samples from the antenna.
All this requires dedicated hardware per antenna, and thus it is common knowledge to assume the requirement of physically laid RF chains to get these digitized baseband samples per antenna.
\name presents a novel architecture which just uses a single physically laid RF chain, connected to all the antennas, which allows hardware re-use and optimizes power-consumption.
The core concept is that \name creates different virtual RF chains from the single physically laid chain.

The idea is that, in order to virtualize the RF chain, \name will tweak the parameters from a software level, of a single laid RF chain. But what are the parameters which any RF chain exposes to the controlling software? We have the gain settings for LNA, the mixer's center frequency and the ADC sampling frequency. Definitely tweaking the LNA gains or varying the downconverting frequency won't do us any good for virtualization. 
However, varying the ADC sampling frequency could possibly allow us to sample more bandwidth, and we can then fit the virtual RF chains over this increased bandwidth to allow for the RF chain virtualization.

However, just increasing ADC rate does not give virtual RF chains. To understand the intuition behind how \name enables creation of these virtual RF chains, we take a toy example of a $2$ antenna array. As an abstraction, consider first antenna receives a rectangular pulsed signal and the second antenna receives a triangular signal.
Today's way of capturing the 2 degrees of freedom offered by the array is to have 2 physically laid RF chains, which downconvert and sample these signals directly  (Fig. \ref{fig:virt_rfc}(a)).
Now, a naive attempt at virtualization with a single oversampled RF chain would try to increase the ADC sampling rate in hopes of attaining the $2$ degrees of freedom  (Fig. \ref{fig:virt_rfc}(b)). 
However, this wont work because the signals from the antennas would have added and there's no way of separating them now, and sampling at 2x rate will not help.

How \name enables this creation of virtual RF chains by tweaking ADC's sampling rate is by introducing RF switches which toggle in synchronity with the ADC's sampling clock.
Basically, we augment the antenna array design with RF switches to create a switched antenna array.
These RF switches are then toggled \emph{on-off} in a strategic manner, with one antenna being toggled \emph{on} for odd samples, and the other antenna toggled \emph{on} for even samples.
Say the antenna signals were $s_1(t), s_2(t)$ and the \emph{on-off} codes implemented via the RF switch are $c_1(t),c_2(t)$.
The ADC finally samples the waveform $s_1(t)c_1(t)+s_2(t)c_2(t)$, at 2 times the nyquist sampling rate corresponding to $s_1,s_2$.
The codes $c_1, c_2$ are basically 50\% duty cycled codes with frequency corresponding to the bandwidth $B$ of signals $s_1,s_2$.
Thus in addition to a constant DC component, these switches also produce harmonics at $\pm B$.
Since $c_2$ is \emph{on} for odd samples and $c_1$ is \emph{on} for even samples, $c_1$'s harmonic at $\pm B$ will basically be $\pm \pi$ of $c_2$. 
This is because the codes are having frequency $B$, thus time period $\frac{1}{B}$, and the associated time delay between $c_1,c_2$ is $0.5(\frac{1}{B})$, thus the phase associated with this time delay would be $(\frac{2\pi}{\frac{1}{B}})0.5(\frac{1}{B}) = \pi$.
The DC component of $c_1,c_2$ however would be the same, since the DC component depends on the average energy, which is a measure of how much time the codes had value $1$ which is same for both.

Thus, as shown in Fig. \ref{fig:virt_rfc}(c) the frequency domain view of the signal sampled by ADC, which was $s_1(t)c_1(t)+s_2(t)c_2(t)$, would have $0.5*(s_1(t)+s_2(t))$ in the first nyquist band, ($-\frac{B}{2}<f<\frac{B}{2}$) and $0.5*(s_1(t)-s_2(t))$ in the second nyquist band, ($(-B<f<-\frac{B}{2}) \cup (\frac{B}{2}<f<B)$). A simple digital processing step can now get us back $s_1, s_2$ by simply adding the subtracting these signals in the two nyquist bands.

Thus, \name utilizes RF switches with different phase codes, coupled with an oversampling ADC in order to virtualize the RF chains. This is also supported by recent trends of having faster ADCs, which offer other benefits as well, like simplified baseband filter design, reduced quantization noise amongst others.
With \name's architecture, virtualization of RF chain concept would be another advantage of faster ADC design.

\subsubsection{Generalization to $N$ antennas}
The method of obtaining these virtual RF chains from a single physically laid chain can be generalized easily when we have $N$ antennas with $N$ RF switches and an ADC which is doing $N*B$ times sampling where $B$ is the signal bandwidth.
So here, we will have codes $c_1,c_2\ldots c_n$ which will be codes of length $N$ with  $c_1 = {1,0,0,\ldots,0,0}$, $c_2 = {0,1,0,\ldots,0,0}$, $\ldots$, $c_{n-1} = {0,0,0,\ldots,1,0}$ and $c_{n-1} = {0,0,0,\ldots,0,1}$.
Since these are $1/N$ duty cycled codes they will have frequency images at every integral multiple of $B$ and thus total $N$ images at frequencies $\text{fftshift}(0,B,2B,\ldots N)$.
In addition, code $c_i$ is delayed by $\frac{(i-1)}{NB}$, and thus the $j$-th harmonic of $c_i$ will have phases $\frac{(i-1)}{NB}*\frac{2\pi}{\frac{1}{jB}} = (i-1)*j*\frac{2\pi}{N}$.
We will have $N$ $B$ bandwidth zones obtained from the ADC sampled stream $R$, denoted by $R^B_1, R^B_2, R^B_3\ldots R^B_N = \mathbf{R^B}$, with $\mathbf{R^B}$ being a $N\times N_s$ matrix which stores the $N_s$ samples correpsonding to each of the $N$-th $B$ bandwidth zone, and we can obtain our virtualized RF chains $S_1,S_2,\ldots S_N = \mathbf{S}$, $S$ being $N \times N_s$ as well, via phase inversion of the $N\times N$ phase matrix $\mathbf{P}$ corresponding to $j$-th harmonic phase of $c_i$:

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{design/design_re_fig2.pdf}
    % \vspace{3pt}
    \caption{How switching changes the signal spectrum: example where $N=4$, code $c_2$. Due to time delay of $1/(4*B)$, the phases at harmonics $B,2B,(3B=-B)$ are $1*(2\pi)/4 = 90^o$, $2*(2\pi)/4 = 180^o$ and $3*(2\pi)/4 = 270^o$}
    % \vspace{5pt}
    \label{fig:virt_rfc_gen}
\end{figure}

\begin{equation}
    \mathbf{S} = (\mathbf{e}^{(-\mathbf{P})})* \mathbf{R^B}
\end{equation}

where $\mathbf{e}^{(\cdot)}$ applies the exponential function to each element of the matrix. The matrix $\mathbf{P}$ in detail looks like this:

\begin{equation*}
  \mathbf{P}=
  \begin{blockarray}{*{5}{c} l}
    \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
      0 & B & 2B & $\ldots$ & (N-1)B & \\
    \end{block}
    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
      0 & 0 & 0 & $\ldots$ & 0 \bigstrut[t]& $c_1$ \\
      0 & \frac{2\pi}{N} & \frac{4\pi}{N} & $\ldots$ & \frac{2(N-1)\pi}{N} & $c_2$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(i-1)}{N} & \frac{4\pi(i-1)}{N} & $\ldots$ & \frac{2(N-1)(i-1)\pi}{N} & $c_i$ \\
      $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\
      0 & \frac{2\pi(N-1)}{N} & \frac{4\pi(N-1)}{N} & $\ldots$ & \frac{2(N-1)(N-1)\pi}{N} & $c_n$ \\
    \end{block}
  \end{blockarray}
\end{equation*}

The reason this generalization works out is because all these are different series of roots of unity, and by doing phase inversion one set of the roots become all co-phased and thus their virtual RF chain component adds up, and the other sets of roots still remain phase shifted versions of their previous versions and add up to 0, which allows \name to extract the RF chain per antenna from the oversampled ADC stream.

\subsubsection{Using virtual RF chains for spatial-multiplexing}

Once we are able to obtain the per-antenna waveform $\mathbf{S}$, the process to obtain the spatially multiplexed output is straightforward and follows the same method as compared to usual way with physically laid RF chains.
In the scenario when we have $N$ antennas and $N$ RF chains, and say we have $N$ users, we can perform MIMO channel estimation with the $N$ virtual RF chains to get the $N\times N$ channel matrix for all $N$ users and $N$ antennas.
Now, we can choose any precoding strategy, like MMSE, BD or ZF to suppress the signals from other users to get individual streams for each of the $N$ users. For example if we use a simple ZF precoding would multiply the $N\times N$ matrix $\mathbf{H}^{-1}$ to the obtained virtual RF chain matrix $\mathbf{S}$ to get individual interference free $N_s$ samples of each $N$-th users data, stored in the $N\times N_s$ matrix $\mathbf{U}$. 

\begin{equation}
    \mathbf{U} = \mathbf{H}^{-1}\mathbf{S}
\end{equation}

Thus, by using just 1 physically laid RF chain, we can enable creation of $N$ virtual RF chains with $N$ antennas and $N$ RF switches which allows for a possible $N$ times spatial multiplexing gain, by allowing $N$ users to communicate simultaneously on the same spectrum.

\subsection{Enabling green communications with \name}
A traditional mu-MIMO system strives to serve $N$ users with $N$ antennas, and for this it lays down $N$ physical RF chains.
However, in practical scenarios, often we need many more number of antennas $N_{\text{ant}}>>N$ number of users in order to serve all the users with a good quality wireless link, and this system is referred to as Massive MIMO.
The reason is that we need more degrees of freedom than $N$ as the channels of the $N$ users to the base station are often correlated, especially when the users are located close to each other. 
Thus, having more antennas leads to more degrees of freedom which allows the base station to serve $N$ users effectively.
Although massive MIMO is info theoretically sound, it is challenging to deploy due to requirement of a massive number of RF chains as well.
Further, it is not a `green' architecture, since it needs to sample $N_\text{ant}$ data streams, much more than the required number of $N$ data streams to serve $N$ users.
Also, it is wasteful in terms of the digital processing done after sampling on $N_\text{ant}$ streams, as well as communication of $N_\text{ant}$ streams to the DSP where these algorithms are implemented.

Hence, it would be ideal to somehow have only $N$ data streams to serve $N$ users and at the same time use $N_{\text{ant}}$ antennas.
Here \name gives a perfect solution, where we can always reduce the number of virtual RF chains by reducing the ADC sampling rate, and still use $N_{\text{Ant}}$ antennas connected to one physical RF chain.
When we have $N_{\text{Ant}}$ antennas but only $N$ times oversampling ADC, we can not create $N_{\text{Ant}}$ separate virtual RF chains, but only $N$ virtual RF chains.
The key insight which allows \name to still effectively use $N_{\text{Ant}}$ antennas' degrees of freedom is that we try and increase the signal power for user $i$ in the $i$-th virtual RF chain, by supplying same code $c_i$ to antennas which are in-phase for user $i$ (that is, have the channel angles within $\pm \pi/2$).
We make an observation that $c_i = \{0,\ldots,1,\ldots,0\}$, which has a $1$ at the $i$-th position is orthogonal to any $c_j$, $j\neq i$.
Thus, we can add these codes when we want to have antennas to appear in more than one virtual RF chains.
Say for an example, we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
So, here, for antennas $\{1,6\}$, which is to be selected for both the users, we will give the code $c_1+c_2$. For antennas $\{3,5\}$, we will give the code $c_1$, and for $\{2,7,8\}$ we will give $c_2$.
This will ensure that for virtual RF chain $1$ corresponding to $c_1$, the signals from antennas $\{1,3,5,6\}$ would be combined and for virtual RF chain $2$, we will get combined signals from $\{1,2,6,7,8\}$.

Now, generalizing this idea, based on the $N_{\text{ant}}\times N$ channel $\mathbf{H}$, we would determine the maximal group of antennas in-phase for user $i$, corresponding to $c_i$ which generates the virtual RF chain $i$.
We name this algorithm to select the maximal in-phase antennas as $\text{BABF}(\cdot)$ (Algorithm \ref{Alg1}), where BABF stands for Binarized Analog Beamforming.
Essentially, for each virtual RF chain we try to beamform towards individual users using the $0-1$ bit control we have over the switched antenna array.

\begin{algorithm}
  \caption{BABF, Input: $\textbf{H}$, Output: $\mathbf{B},\phi$}
  \begin{algorithmic}[1]
  \label{algo:switch_selection}
  \STATE $\phi$=$\pi/3$;\
  \FOR{ $1 \le i \le K$}{
      \FOR{ $1 \le m \le M$}{
      \STATE $\Tilde{\textbf{b}}_{i,m}=[0, 0 , \ldots , 0]_{1\times M}$;\
      \STATE $\textbf{g}_{i,m}=\textbf{H}_{i}h^*_{i,m}$;\
      \STATE $\boldsymbol{\theta}_{i,m}$=$\angle{\textbf{g}_{i,m}}$;\
      \STATE $\Tilde{\textbf{b}}_{i,m}(m)$=$|\boldsymbol{\theta}_{i,m}|<\phi$;\
      \STATE $score_{i,m}=$ Number of elements equal to $1$ in $\Tilde{\textbf{b}}_{i,m}$;
      }
      \ENDFOR
  }
  \ENDFOR
  \STATE $\mathbb{B} :=$ Set of all possible permutations of $score_{i,m}, 1 \le i \le K, 1 \le m \le M$\;
  \STATE $l=1$;\
  \STATE Select $score^*\in \mathbb{B}$ that provides the $l^{\text{th}}$ highest score;\
  \STATE $\mathbf{B}=\mathbf{B}^*$ (corresponding to $score^*$);\
  \IF{$\mathbf{H}\mathbf{B}$ is full rank}
  \STATE $\mathbf{B}$ is the optimal switch configuration;\
  \ELSE
  \STATE $l=l+1$;\
  \STATE Go to line 13;\
  \ENDIF
\end{algorithmic}
\label{Alg1}
\end{algorithm}

That is, the BABF algorithm we get a switching matrix $\mathbf{B}$, where $\mathbf{B}$ is $N_{\text{Ant}}\times N$, which increases signal power of user $i$ in the $i$-th virtual RF chain, by turning $N_{\text{Ant}}$ antennas on-off.
Although each virtual RF chain prioritizes one user, there is significant interference terms still present in the virtual RF chains at this stage.
However, this can be handled easily by digital combining, that is the virtual RF chains are now capturing the $N \times N$ channel $HB$, which can be inverted via ZF approach, and that cancels out the interference terms.
Hence, using the BABF algorithm and the orthogonality of $c_i$ codes, we can project the $N_{\text{Ant}}\times N$ channel $\mathbf{H}$ onto an effective $N\times N$ channel $\mathbf{(HB)}$.

\begin{equation}
    \mathbf{U} = \mathbf{(HB)}^{-1}\mathbf{S}
\end{equation}

\subsection{Adapting to averse channel conditions with high sampling rate}
\todo{Draw a channel phase figure here}
In the last section we showed how \name's architecture can enable green communications by restricting only to $N$ times ADC sampling to serve $N$ users, at the same time using a $N_{\text{Ant}}>N$ antennas.
However, there might be scenarios where channel conditions are so bad that it is required to really bump up the sampling rate.
By increasing the sampling rate, we can get more control over the projected channel $\mathbf{HB}$.
However, we need to generalize our projection matrix generation when we bump up the sampling rate.

For an example, consider we have $8$ antennas, $2$ users and we oversample by a factor of $4$, which gives us $4$ virtual RF chains. In the previous section, we used $2$ times oversampling to handle 2 users, and used $2$ codes $c_0,c_1$ to implement the BABF matrix $\mathbf{B}$. The BABF algorithm basically selected antennas which are maximally \emph{in-phase}, i.e. their channel angles are within $-\pi/2,\pi/2$ of each other.
When we have $4$ chains at our disposal for $2$ users, we can then infact, select the antennas which were turned off before in the other $2$ spare codes, and do the phase aligning in digital domain to get more SNR gain for the user.
In a way, this is a way of refining the beamforming weights by implementing precise phase rotations across the digital samples, instead of simple $0/1$ as compared to previous section.

Put mathematically, we have $c_0$ implementing the maximal antenna set for user $1$, $c_1$ implementing the complimentary set for user $2$, and $c_2,c_3$ doing the same for user $2$.
Taking the same example as before, say we have $2$ users and $8$ antennas, and for user $1$ the antennas $\{1,3,5,6\}$ are in-phase and for user $2$ the antennas $\{1,2,6,7,8\}$ are in phase.
$c_0$ will turn on $\{1,3,5,6\}$, $c_1$ will turn on $\{2,4,7,8\}$, $c_2$ will do $\{1,2,6,7,8\}$ and finally $c_4$ will do $\{3,4,5\}$.
Then the virtual RF chain corresponding to $c_0$ will be added to $e^{j\pi}$ times that of $c_1$ to get everything phase aligned, and same with $c_1,c_2$.
Thus, we will get the following $\mathbf{B}$ matrix:


\begin{equation*}
  \begin{blockarray}{*{8}{c} l}
    % \begin{block}{*{8}{>{$\footnotesize}c<{$}} l}
    \begin{block}{*{8}{c}>{$\footnotesize}l<{$}}
     1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Ant. index\\
    \end{block}
    \begin{block}{[*{8}{c}]>{$\footnotesize}l<{$}}
      1 & e^{j\pi} & 1 & e^{j\pi} & 1 & 1 & e^{j\pi} & e^{j\pi}\bigstrut[t]& User 1 \\
      1 & 1 & e^{j\pi} & e^{j\pi} & e^{j\pi} & 1 & 1 & 1 & User 2 \\
    \end{block}
  \end{blockarray}
\end{equation*}


To generalize this, to say $N_O$ times oversampling with $N$ users, we would select the antennas whose phases are within $-\frac{\pi}{(N_O/N)},\frac{\pi}{(N_O/N)}$ using the $\phi$ parameter in the BABF code. Then we will perform the phase aligning across the virtual RF chains by multiplying each of the codes by the respective angles which will align them with the maximally selected set, and thus this will give more control over the generation of the projection matrix $\mathbf{B}$.
Since the phases to select in the groups tighten as $N_O$ increases, once the oversampling factor $N_O$ becomes equal to $N_{\text{Ant}}$, we can just do one antenna per virtual RF chain and handle all the processing in the digital domain. 
At this point \name basically becomes a full blown massive MIMO architecture.
Thus, \name shows a very flexible architecture: which can be tuned to behave like a green hybrid beamformer to a full massive MIMO architecture, all via software level control of the singly laid physical RF chain.

% construct matrix

% This process of virtual RF chain creation is what makes \name's architecture flexible, as the number of these virtual RF chains can be easily controlled via software itself.
% To enable this process of virtual RF chain creation, \name's architecture uses RF switches connected to each antenna, as shown in Fig. 1. \todo{cite} have also used similar architectures with RF switches connected to antennas, but they were typically used in static scenarios to extend the array factor, in order to get selection combining gains or improved spatial localization accuracies. 
% However, the real power of these switched architectures is that these switches can really be toggled very fast, and this fast toggling is the essential essence which allows \name to use it for the creation of these virtual RF chains. To the best of our knowledge, \name is the first paper which makes the connection of fast switching with virtual RF chain creation.

% Thus, the natural question becomes, how exactly does \name use fast switching for RF chain virtualization? 
% Let's take a simple example first with $4$ antennas connected to a single RF chain with $4$ switches, similar to Fig. 1.
% Here, in the worst case, we would want $4$ RF chains to be created, one per antenna.
% A flexible architecture would be able to tune down the number of RF chains, i.e. have just 2 RF chains when conditions are good to save on power consumption.
% So the target here is to have a flexible way of generating either 2, or 4 RF chains. 



% Say we have a signal with certain bandwidth $BW$. 
% If we consider a switch with switching frequency $f_s$, that is it has a certain duty cycled 0,1 pattern which repeats after $T_s = 1/f_s$.
% Considering a simple 50\% duty cycled switching rate at $f_s$, we will have frequency components at $0, \pm f_s, \pm 3 f_s$ and so on.
% When the signal with $BW$ bandwidth goes through a $f_s$ rate switch, it basically gets frequency shifted and copies are created at these frequency components of the switch.
% If we want to prevent any interference due to these copies, we need to have sufficient gap between the two copies, that is, we need to have $f_s>BW$.


==> design/design_new.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
% Assuming till here time diversity has been motivated
\subsection{Increasing sampling bandwidth without adding new spectrum}

% What is the problem at hand, how to utilize extra bandwidth
\noindent Typically in a wireless network, we have a single AP connected to multiple clients. 
The clients are typically consumer devices like smartphones or tablets which employ generic chipsets to transmit/receive, whereas the AP can have more dedicated and sophisticated hardware capabilities to maintain the network of clients it is connected to.
Thus, in most networks today, the AP has far more capable hardware than the clients, which usually translates to a higher sampling rate, more antennas and powerful processors to employ specialized communication algorithms as well.

To leverage this assymetricity in the capability of communications hardware between the AP and the clients, modern WiFi protocols have been utilizing protocols like OFDMA. In OFDMA systems, the AP utilizes a wider sampling bandwidth than the clients, and fits multiple clients in different frequency bands so that they don't interfere (Fig. ). More concretely, say there are $K$ users utilizing a transmit bandwidth of $B_t$, and the receiver utilizes a bandwidth of $B_r=kB_t$. 
The receiver is tuned to a center frequency $f_c$, and thus it samples the spectrum from $f_c\pm \frac{B_r}{2}$.
To serve all the $K$ users simultaneously, the OFDMA protocol would require the transmitters to occupy $K$ different contiguous $B_t$ frequency bands in the frequency range from $[f_c- \frac{KB_t}{2},f_c+ \frac{KB_t}{2}]$, such that user $1$ occupies $[f_c- \frac{KB_t}{2},f_c- \frac{(K-1)B_t}{2}]$, user $2$ occupies $[f_c- \frac{(K-1)B_t}{2},f_c- \frac{(K-2)B_t}{2}]$, and so on till user $K$ who occupies $[f_c+ \frac{(K-1)B_t}{2},f_c+ \frac{(K)B_t}{2}]$.

Thus, the aggregate over-the air bandwidth ($K$ different $B_t$ frequency bands) occupied by the clients is the same as the sampling bandwidth, $B_r=KB_t$ of the AP. As our technologies mature, and we get capability to develop ADCs which can sample at GHz frequencies, that would necessitate a large requirement on the over the air bandwidth, which may not always be possible. Infact, this is the major reason to push for mmWave bands as they are capable of furnishing 1 GHz over the air bandwidths.

However, the majority of the devices today operate in sub-6 band, so to design \name, we concretely ask this question, how can we utilize the $K$ times higher sampling bandwidth available without asking the clients to be spaced apart in different frequency bands (Fig. ). In this scenario, although the AP is utilizing a wider bandwidth to sample, all the clients are within the smaller over the air bandwidth. So, unlike OFDMA, here all the users utilize the same over-the-air bandwidth to $B_t$, i.e. all the users transmit at the same center frequency $f_c$, and occupy the same spectrum from $f_c\pm \frac{B_t}{2}$. The receiver is tuned to the same frequency, however samples at a higher bandwidth $f_c\pm \frac{KB_t}{2}$. 

Even though the receiver is able to sample at $K$ times the bandwidth, this will not help much here by itself as there are $K$ users interfering in the $[-\frac{B_t}{2},\frac{B_t}{2}]$ band and nothing elsewhere, unlike in OFDMA where each of the $K$ users were occupying the different $K$ $B_t$ bands.
Thus the challenge here to use higher sampling bandwidth without actually increasing the spectrum is to somehow handle the $K$ user interference in the transmitted bandwidth.




% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
 
% \end{tabular}
% \end{center}

% \begin{table}
% \fontsize{10}{10}
% % \newcolumntype{b}{>{\hsize=0.9\hsize}X}
% \newcolumntype{s}{>{\hsize=0.2\hsize}X}   
%     \begin{tabularx}{\columnwidth}{|s|s|s|s|}
%         \hline
%          Technology & Digital Beamf. (mu-MIMO) & OFDMA & \name \\ \hline
%          TX Bandwidth & BW & BW & BW \\  \hline
%          Multiplexing Gain & m & m & m \\ \hline 
%          RF Bandwidth & BW & m*BW & BW \\ \hline 
%          Sampling Bandwidth & BW & m*BW & m*BW \\ \hline
%          Number of Antennas & m & 1 & m \\ \hline 
%          Number of RF Chains & m & 1 & 1 \\ \hline 
%     \end{tabularx}
%     \caption{Comparison of \name with other multiplexing techniques today}
%     \label{table: design_comparison}
% \end{table}

\subsection{Switched antenna array with a higher sampling bandwidth}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{design/design_fig1.pdf}
    \caption{Separating per-antenna channel estimates from a single wire switched-antenna stream containing time interleaved samples from each antenna}
    \label{fig:design_subsec1}
\end{figure*}


Now one method to deal with $K$ users interfering in the $[-\frac{B_t}{2},\frac{B_t}{2}]$ bandwidth is to utilize digital beamforming, which would do this by having $K$ antennas connected to $K$ downconversion chain with $K$ ADCs. By utilizing channel estimates for each of the $K$ users across $K$ antennas, we have a system with $K$ equations and $K$ variables, to isolate each of the $K$ users signals. There have been various techniques to do this, with the most popular ones being ZF, MMSE and Null Beamforming \todo{Cite}. 

Interestingly, digital beamforming utilizes $K$ ADCs which need to at least sample $B_t$ bandwidth to handle $K$ users having bandwidth $B_t$. The fundamental question we ask is, if we can utilize a single ADC which can sample $K$ times faster to sample the bandwidth $B_r=KB_t$ without requiring $K$ slower ADCs in parallel. If so, we would utilize the faster sampling rate ADCs by itself in order to serve multiple users, and this design would also cut down on number of downconversion chains, as a single downconversion chain with a $K$ times faster ADC can achieve the same effect as $K$ separate downconversion chains each connected to a slower ADC.

To this end, \name comes up with a unique solution, where we create a single wire antenna array along with a faster sampling ADC, which utilizes faster sampling and increased dimensionality due to having multiple antennas to serve multiple clients. That is, in order to handle the interference due to $K$ users transmitting simultaneously, \name's antenna array consists of $K$ antennas, whose outputs are combined via a series of combiners in order to form a single wire interface for the antenna array.
But, in that case, if the antennas outputs are combined to one RF chain, the antenna array will act as a single big antenna, and thus it won't be possible to utilize the increased dimensionality from having multiple antennas.
This is where our increased sampling bandwidth comes to the rescue.
We augment our antenna array design to combine across $K$ `switched-antennas' instead of just normal antennas.
By `switched-antenna', we mean that each antenna is connected to a RF switch which toggles this antenna on-off, with the switched output being the input to the combining network (Fig.), 
% and the $K$ antennas with $K$ RF switches are then combined to a single wire interface with a wilkinson network.

The intuition in using a switched antenna array is that because we are sampling $K$ times faster than the required sampling rate to decode $B_t$ bandwidth user, we have $K$ extra time slots at our disposal. 
That is, say if we had a bandlimited signal $x[n]$, and we oversample it by $K$ times to obtain $y[n]$. To downsample $y[n]$ now, we have $K$ possible ways, we can do $y_0[n] = y[Kn], y_1[n]=y[Kn+1],\ldots,y_i[n] = y[Kn+i], \ldots y_{K-1}[n]=y[Kn+K-1]$. From nyquist theorem, apart from varying group delays depending on the value of $i$ to choose one of $y_i$'s, all these can be independently used to recover the original signal $x[n]$. Now, think of $x[n]$ as the transmitted $B_t$ limited signal and $y[n]$ as the oversampled signal at the receiver. We have $K$ different ways to downsample $y[n]$, depending on which of the $i$-th delayed $y_i$ to choose from. The concrete idea here is to keep the first switched antenna to be \emph{on} for samples $0,K,2K\ldots nK$, the second switched antenna \emph{on} from $1,K+1,2K+1\ldots nK+1$ and so on. What this will enable is that instead of all the $y_i$'s being redundant in terms of the information they carry, now each $y_i$ would essentially be utilizing the channel at antenna $i$ (Fig. \ref{fig:design_subsec1}).  

To see how this switched-antenna RF chain behaves, we model the scenario mathematically, with the $K$ users transmitting signals $x_{1,2,\ldots,k, \ldots K}(t)$, and the complex time-invariant channel seen by user $k$ to the $i$-th antenna represented as $h_{ki}$. We consider that the $i$-th antenna toggles on-off with a bit sequence $s_i(t)$ via the RF switch, where $s_i(t) \in \{0,1\}$. The combined received signal $y(t)$ across the $K$ users indexed via $k$, and $K$ switched antennas indexed via $i$, can be represented as:

\begin{equation}
    y(t) = \sum_{k=1}^K \sum_{i=1}^K (h_{ki}(t)*x_k(t))\cdot s_i(t)
\label{eqn:combined_codes}
\end{equation}

This combined signal $y(t)$ goes through downconversion, and then ADC sampling at $KB_t$ to get sampled baseband signal

\begin{equation}
    y[n] \equiv y(nT_s) = \sum_{k=1}^K \sum_{i=1}^K (h_{ki}[n]*x_k[n])\cdot s_i[n]
\label{eqn:combined_codes}
\end{equation}

For sake of brevity, assume $K=4$. Now, to isolate the signal from each of the antennas, we choose $s_1[n] = [1,0,0,0]_n$, $s_2[n] = [0,1,0,0]_n$, $s_3[n] = [0,0,1,0]_n$ and $s_4[n] = [0,0,0,1]_n$, where $[\cdot]_n$ shows that the sequence gets repeated, that is $s_1[n] = 1,0,0,0,1,0,0,0,\ldots$.
Hence, antenna $1$ is \emph{on} for every $4n$-th samples and \emph{off} for others, antenna $2$ is on only for every $4n+1$-th samples, antenna $3$ is on only for every $4n+2$-th samples and antenna $4$ is on only for every $4n+3$-th samples.
Thus, the oversampled signal $y[n]$ is interspersed with samples from each of the antennas.
Now, when we write the $K=4$ $y_1,y_2,y_3,y_4$ different ways of downconverting $y[n]$, given by $y_i[n] =y[4n+i]$, we get
\begin{equation}
\begin{split}
y_i[n] &= \sum_{k=1}^K (h_{ki}[4n+i]*x_k[4n+i])s_i[4n+i]\\
        &= \sum_{k=1}^K (h_{ki}[4n+i]*x_k[4n+i]) \\
        &\approx \sum_{k=1}^K (h_{ki}[4n]*x_k[4n+i])
\label{eqn:equation_yj_id}    
\end{split}
\end{equation}



\noindent where the second step follows from $s_i[4n+i]$ being = 1 from definition, and the last step assumes that the wireless channels $h_{ki}[4n] \approx h_{ki}[4n+1] \approx h_{ki}[4n+2] \approx h_{ki}[4n+3]$, which is generally true as the coherence time for channels is usually much larger than duration of $4$ samples. 

Note that we are not assuming that the channel stays same across the entire packet length, but only local stationarity for every $4$ samples. Hence, \noindent $y_i$ effectively consists of convolution of all the $K$ users signals with channels between the users and the $i$-th antenna, as only $i$-th antenna is on for the samples used to derive $y_i$ from $y$. 
Thus, setting $s_1[n] = [1,0,0,0]_n$, $s_2[n] = [0,1,0,0]_n$, $s_3[n] = [0,0,1,0]_n$ and $s_4[n] = [0,0,0,1]_n$ allows us to obtain the $4$ antenna channels $h_{k1}, h_{k2}, h_{k3}, h_{k4}$ for each of the $k$-th user, from $y_1[n],y_2[n],y_3[n],y_4[n]$ respectively, even if the outputs from the 4 switched antennas were combined into a single stream $y[n]$. 
This draws a parallel to how in a normal digital beamforming system, we get channels per each RF chain from a single antenna. 
Hence, we can then combine across $y_i$'s in order to cancel the interference, similar to how digital beamformer utilizes separate spatial RF chains for the same purpose.
% This gives another requirement for the increased IF bandwidth to serve multi-user scenarios, that is to disambiguate this interference, we need to have increased antennas, so that we can combine across the antenna streams and cancel out the interference from each other. 
% A challenge here is to do so without actually increasing the number of RF chains, since otherwise the solution will not be scalable and useful.
% Thus, \name comes up with a creative solution, where we combine signals from multiple antennas into one combined RF chain, effectively utilizing the increased antenna space dimensionality to cancel interference, and using just one RF chain in the process. 
% However, this is not enough, since 
% Normally, wireless channels remain relatively stable over time, 
% and some reasoning for this is that the clients by-at-average don't
% move fast, and the sampling rate for receivers is reasonably high, 
% which allows the receivers to sample at a faster rate, which further 
% gives the sense that channels don't change much over multiple samples.

% So, how do we create dynamicness in the channel, which allows opportunities 
% to tap in the time diversity. The key 
\subsection{Time combining and its equivalence to digital beamforming}
We have now shown how we can recover per-antenna channel streams by utilizing the switching sequences $s_i$ and using RF switches to implement in  
This is because we have $i$-th antenna turning \emph{on} for every $4n+i$-th samples in the oversampled $y[n]$. 

Before we move ahead in explaining how the combining is finally performed, we will generalize the setting to utilize arbitrary switching sequences. We can represent all the switching sequences as rows of a combined switching matrix $S$. In the example discussed before to use per antenna channel estimates, we had $S$ as an identity matrix, as only one antenna was \emph{on} at a time. For a element $s_{ij}$ in the matrix $S$, row $i$ represent the on-off states for antenna $i$, and column $j$ represents which of the $K$ antennas were on at time slots $Kn+j$ samples. Thus, more generally, we can write Eqn \eqref{eqn:equation_yj_id}as,
\begin{equation}
\begin{split}
y_j[n] &= \sum_{k=1}^K \sum_{i=1}^K (h_{ki}[Kn]*x_k[Kn+j])\cdot s_{i}[Kn+j]\\
       &= \sum_{k=1}^K \sum_{i: s_{ij}=1} (h_{ki}[Kn]*x_k[Kn+j])\\
       &= \sum_{k=1}^K \left(\left(\sum_{i: s_{ij}=1} h_{ki}[Kn]\right)*x_k[Kn+j]\right)\\
       &= \sum_{k=1}^K \left(\left(\sum_{i}^K h_{ki}[Kn]s_{ij}\right)*x_k[Kn+j]\right)\\
\end{split}
\label{eqn:equation_yj_gen}    
\end{equation}

\noindent the third step follows from superposition principles of LTI analysis, and the last two steps are equivalent as $s_{ij}\in{0,1}$. To get a more concise expression and convert convolutions to multiplications, we can take the fourier transform to go to the frequency domain,
\begin{equation}
Y_j[f] = \sum_{k=1}^K \left(\left(\sum_{i}^K \tilde{H}_{ki}[f]s_{ij}\right)\mathcal{F}(x_k[Kn+j])\right)\\
\end{equation}
\noindent $\tilde{H}_{ki}[f]$ represents the fourier transform of channel  $\tilde{h}_{ki}[n]\approx h_{ki}[Kn] \approx h_{ki}[Kn+1] \ldots \approx h_{ki}[Kn+K-1]$, since the channel is assumed to be stationary for every $K$ samples. For brevity, we will drop tilde from the expression and write it simply as $H_{ki}[f]$.  We can write $\mathcal{F}(x_k[Kn+j]) =  e^{j2\pi f j}\mathcal{F}(x_k[Kn]) = e^{j2\pi f j}X_k[f]$ by using fourier identities for time delayed signals and using the fact that $x_k(t)$ has been oversampled by $K$ times. Thus we get the simplified equation,
\begin{equation}
Y_j[f] = \sum_{k=1}^K \left(\left(\sum_{i}^K H_{ki}[f]s_{ij}\right)e^{j2\pi f j} X_k[f]\right)\\
\end{equation}
Now, note that $\sum_{i}^K H_{ki}[f]s_{ij}$ is nothing but the $k,j$-th element in the matrix multiplication between $K*K$ channel matrix $\mathbf{H}[f]$ and the $K*K$ switching matrix $\mathbf{S}$. Note that for $Y_j$ we need to remove the phase due to group delay in the fourier transform, which can be done by multiplying $Y_j$ by $e^{-j2\pi f j}$, and we can write the delay compensated vector $\mathbf{Y^\mathcal{D}}[f] = [Y_0[f] e^{-j2\pi f}Y_1[f]\ldots e^{-j2\pi f (K-1)}Y_K-1[f]]^T$, and denote $\mathbf{X}[f]$ to be $[X_1[f] X_2[f]\ldots X_k[f]]^T$, to get a much simpler equation in terms of matrix products, 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f]
\end{equation}
Note that the vector $\mathbf{Y^\mathcal{D}}[f]$ consists of phase delay compensated fourier transforms of $y_i[n]$ which were obtained by collecting $Kn+i$ samples in the oversampled signal $y[n]$. In traditional beamforming systems, where we obtain $y_r[n]$ for each of the $r$-th RF chains, $r=0,1,\ldots K-1$, we get the equation 
\begin{equation}
\mathbf{Y^\text{RF}}[f] = \mathbf{H}[f]\mathbf{X}[f]
\end{equation}
Thus, by setting the switching matrix $\mathbf{S}$ to be identity, we get an equivalence between the two methods. 

To recover individual data symbols for each user $\mathbf{X}[f]$ from the obtained interfered samples $\mathbf{Y}[f]$, and assuming knowledge of channel matrix $\mathbf{H}[f]$, we can utilize a $K\times K$ beamforming matrix $\mathbf{V}[f] =[v_1 v_2 \ldots v_K]^T$ which is a collection of $K\times 1$ beamforming vectors $v_i$.  When we take the inner product of $v_i$ with $\mathbf{Y}[f]$, the hope is that we recover $x_i[f]$. 
Basically, when evaluating the inner product, we have the expression $P_i=v_i^TH[f]$, and $P_i$ is another $K\times 1$ vector and the SIR obtained by the combining operation would then be $\frac{|P_{ii}|^2}{\sum_{j\neq i}|P_{ij}|^2} $, where $P_{ij}$ denotes $j$-th element of $P_i$. To obtain these beamforming vectors, we can use multiple methods, ranging from ZF, which basically multiplies $\mathbf{Y}$ by $\mathbf{H}^{-1}$, or using a MMSE, or null space beamforming. All these combining methods would work similarly for both \name's $\mathbf{Y^\mathcal{D}}$ as well as digital beamforming's $\mathbf{Y^\text{RF}}$. An important point to note is that since this combining happens in digital domain, we can do arbitrary combinations for each frequency bin $[f]$ which allows for resilient wideband operation, as well as accurate phase values for both methods, as compared to analog beamforming approaches which utilize phase combining at center frequency and runs into issues of beam squinting and phase quantization noise.

% The more recent papers \todo{CITE TurboHB} advocate the usage of null space beamformers which weed out the interference terms most effectively. 
% Here, $v_i$ is computed from null space of matrix $\mathbf{H}_{i^{\_}}$, which is obtained after removing $i$-th column from the chanel matrix $\mathbf{H}[f]$. $\mathbf{H}_{i^{\_}}$ has reduced number of columns (K-1) than rows (K), we will have a $K\times 1$ column-space null vector belonging to the null space of the matrix $\mathbf{H}_{i^{\_}}$.

\subsection{Harnessing power of multiple antennas for robust multiplexing gains}

In the previous section, we proved how \name performs equivalent to digital beamforming approaches, at the same time utilizing just one RF chain and a higher sampling rate bandwidth.
Usually digital beamforming solutions are designed to equate number of users to number of antennas, in order to utilize a $K\times K$ channel between each of the $K$ users and $K$ antennas. 
This is done to use the $K$ RF chains for maximal multiplexing gains, since we are putting in $K$ ADCs we should have the operating point as $K$ spatial streams from $K$ users.
However, in reality, this is not a robust operating point, since the ability to serve $K$ users depends on having a full rank channel, as well as highly uncorrelated channel between the users to get a higher SINR performance.
If this pre-condition is not met, the SINR degrades drastically, and the only way of resolving this is utilizing smart user-selection to choose only those users where spatial multiplexing gain is possible to achieve \todo{CITE LATTE}.

However, \name provides a much more natural solution to this problem, by scaling up the number of switched-antennas \emph{without} requiring any additional sampling or downconversion chain costs. Say we utilize $K_{\text{ant}}$ number of switched-antennas, with $K_{\text{ant}}>K$. Our analysis in the previous section generalizes very naturally to this usecase, where we still have the equation 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f]
\end{equation}

Here $\mathbf{H}[f]$ is $K\times K_{\text{ant}}$, and $\mathbf{S}$ is $K_{\text{ant}}\times K$ instead of both matrices being $K\times K$. This is because we still have $K$ extra slots because of $KB_t$ sampling bandwidth, but we have $K_{\text{ant}}$ antennas to toggle on-off in these $K$ extra slots. The equivalent channel $\mathbf{H}[f]\mathbf{S}$ still remains $K\times K$, and the digital combining part operates on this $K\times K$ equivalent channel. So the idea here is to choose the matrix $\mathbf{S}$ in a way such that the digital combining operates on a full rank uncorrelated $K\times K$ equivalent channel in order to increase the performance. The intuition to use multiple antennas and less number of effective RF chains is on the lines of Hybrid beamforming architectures in mmWave literature, where there is an analog combining network across multiple antennas supported by a reduced number of RF chains.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_fig2.pdf}
    \caption{Utilizing more antennas than number of RF chains}
    \label{fig:my_label}
\end{figure}
Now, to choose $S$ we have $2^{K_{\text{ant}}*K}$ possible choices, as each of the $K_{\text{ant}}$ antenna can be turned on/off for each of the $K$ slots. Hence, a brute force optimization would not be scalable, considering even smallest of the cases with $K_{\text{ant}}=8$ and $K=4$, we have $2^{32}$ choices, and it will take a considerable amount of time to go over these possibilities, which would exceed the channel coherence time. Hence, instead of a brute force search for an optimal $\textbf{S}$ we need a smart and compute efficient way of estimating a relevant matrix $\mathbf{S}$. 

So, in order to do so we make a key observation. We need to find on-off states for $K_{\text{ant}}$ antennas for each of the $K$ extra time slots for the $K_{\text{ant}}\times K$ matrix $\mathbf{S}$. At the same time we have $K$ users, and the goal is to create equivalent channel $\mathbf{H}[f]\mathbf{S}$ which is as uncorrelated as possible. The way to do this would be to basically use each of the $K$ time slots to prioritize 1 user at a time, that is, to select column $i$ of $\mathbf{S}$ such that signal power of user $i$ is maximised in that slot.
This way the equivalent channel $\mathbf{H}[f]\mathbf{S}$ will have higher diagonal values than non-diagonal, which will decrease correlations, as one user is getting prioritized at a time.

Now, the ideal way to do this would be to co-phase the signals from user $i$ by implementing conjugate channel $\mathbf{H}_i^*$ phases using a network of phase shifters connected to each antenna. However, we do not have accurate phase shifters, and infact in our design we just have RF switches which can toggle on-off, thus providing only one-bit control over the phases. But, at the same time, we just need to increase the signal power for user $i$ and we actually do not need very accurate beamforming for this. This can also be achieved by turning \emph{on} the maximal set of antennas whose phases would add up constructively (Fig. ). 

The algorithm is simple, we go one antenna by one, and calculate the number of other antennas whose phases lie within an acute angle of each other.
We select the group having the highest number of antennas.
Thus, this makes the algorithm to be $O(K_{\text{ant}})$, as we have to choose from $K_{\text{ant}}$ number of groups.
We repeat this procedure for each $k$-th user for $k$-th time slot to create a matrix $\mathbf{S}$.
One another important thing is that we need to choose a full rank matrix $\mathbf{S}$, in order for $\mathbf{H}[f]\mathbf{S}$ to serve all the $K$ users.
Thus, in some cases if the matrix $\mathbf{S}$ turns out to be not full rank, mostly because the antenna configuration selected was same for 2 users, in that case the algorithm tries to create another matrix by selecting the second highest number of antennas group for $\mathbf{S}$. The detailed algorithm is described in Algorithm 1. 

\subsection{Putting it all together: The end-to-end algorithm}

The key insight which \name delivers is that to handle $K$ users transmitting $B_t$ bandwidth signals $\mathbf{X}$, we can sample a single signal $y$ at $KB_t$ bandwidth by utilizing a switched antenna array with number of antennas $K_{\text{ant}}>K$ and switching sequences for each of the $K_{\text{ant}}$ antennas and the extra $K$ slots created due to higher sampling rate denoted by $\mathbf{S}$ to get the equation 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f]
\end{equation}
where $\mathbf{Y^\mathcal{D}}$ are the delay compensated $K$ streams derived from $y$. We get an equivalent channel $\mathbf{H}[f]\mathbf{S}$ created due to the switching network, and we choose $\mathbf{S}$ such that the obtained $K\times K$ channel is as uncorrelated as possible, so that all the $K$ users can be served with sufficient SINR. 
Finally, we will go over the method we use to digitally combine across $\mathbf{Y^\mathcal{D}}$ in order to recover $X[f]$. Denote by $\tilde{\mathbf{H}}[f] = \mathbf{H}[f]\mathbf{S}$, the digital combining matrix $\mathbf{V}$ has to be estimated such that 
To recover $\mathbf{X}[f]$, we would then use a digital combiner matrix $\mathbf{V}$ such that $\mathbf{V}$. To cancel out interference, the best method is to use a ZF combiner, which selects pseudo inverse of $\mathbf{H}[f]\mathbf{S}$ as the digital combiner matrix $\mathbf{V}$. Thus after utilizing the digital combiner, we get
\begin{equation}
\mathbf{V}\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})^{-1}(\mathbf{H}[f]\mathbf{S})\mathbf{X}[f] \approx \mathbf{X}[f] 
\end{equation}
which allows us to remove the interference and recover each of the $K$ symbols $\mathbf{X}=[X_1,X_2,\ldots X_K]^T$
% Hence, to choose the column $S^i$ such that user $i$'s signal power is increased, we first determine the best beamforming vector for user $i$, given by conjugate of the channel for user $i$ given by the $i$-th row of channel matrix, giving the $K_{\text{ant}}\times 1$ vector $v_i = \mathbf{H}_i^*$. Now, we select antenna $j$, and multiply the conjugate phase of the beamforming vector associated with antenna j, given by $v^*_{ij}$, to get $v^j_i = v_iv^*_{ij}$. We then compute the angles of the of $\angle v^j_i$

% Going ahead, for brevity we drop the $[f]$ however we make the point that because we are implementing this combining across the digitized samples $y[n]$ we can perform arbitrary combinations across frequencies and utilize wideband beamforming. To recover $\mathbf{X}$ we can use multiple methods, ranging from ZF, which basically multiplies $\mathbf{Y}$ by $\mathbf{H}^{-1}$, or using a MMSE solution, as well as null space beamforming advocated by more recent paperrs for the same. Essentially, the aim is to design a combining matrix $\mathbf{V}$ such that $VY\approx $ 

% The more recent papers \todo{CITE TurboHB} advocate the usage of null space beamformers which weed out the interference terms most effectively. to compute the null space beamforming weights, consider an example of isolating signal of user $1$ from other users, we take the matrix $\mathbf{H}$ and remove the first column to get a $K-1 \times K$ matrix $\mathbf{H}_{1^{\_}}$, which because of reduced number of columns, will have a $K\times 1$ column-space null vector $\mathbf{N}_1$ belonging to the null space of the matrix $\mathbf{H}_{1^{\_}}$. When we take the inner product of the $K\times 1$ complex vectors, $\mathbf{N}_1$ with $\mathbf{Y}$, we see that

% \begin{equation}
%     \begin{split}
%     R_1 &= \mathbf{N}_1\cdot \mathbf{Y} =\mathbf{N}_1 \cdot \begin{bmatrix} 
%         \mathbf{H}_1\quad \mathbf{H}_{1^{\_}}\mathbf{X}
%         \end{bmatrix}\\
%         &=
%         [\mathbf{N}_1\cdot\mathbf{H}_1\quad \mathbf{N}_1\cdot\mathbf{H}_{1^{\_}}]
%         \mathbf{X}\\
%         &= \begin{bmatrix} 
%         \mathbf{N}_1 \cdot \mathbf{H}_1\quad \mathbf{0}_{K-1 \times K}
%         \end{bmatrix}
%         \mathbf{X}\\
%         & = (\mathbf{N}_1\cdot \mathbf{H}_1)X_1(f)
%     \end{split}    
% \end{equation}

% since $\mathbf{N}_1$ will null out the $\mathbf{H}_{1^{\_}}$ sub-matrix. Thus, using the vector $\mathbf{N}_1$ to combine across the $K$ delayed sample vector $\mathbf{Y}$ we can null out all other users apart from user 1, and hone onto the signal from user 1. Note that we can generate such nulling vectors for all the $K$ users, since there is nothing special about the user 1. Thus we can get $\mathbf{N}_{1,2,\ldots K}$ for all the $K$ users, from the null spaces of appropriate matrices $\mathbf{H}_{j^{\_}}$ by removing the $j$-th column associated to $j$-th user. Thus, we can get the vector $\mathbf{R}(f) = {\begin{bmatrix}
%  R_1(f) 
%  R_2(f)
%  \cdot 
%  \cdot 
%  R_K(f)
% \end{bmatrix}}^T$, such that

% \begin{equation}
% \begin{split}
% \mathbf{R}(f) &= [\mathbf{N}_1 \mathbf{N}_2 \cdot \cdot \mathbf{N}_K ] \cdot Y  \\
% & = \begin{bmatrix}
%  \mathbf{N}_1\cdot \mathbf{H}_1 & 0 & \cdot & \cdot & 0\\
%  0 & \mathbf{N}_2\cdot \mathbf{H}_2 & \cdot & \cdot & 0\\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  0 & 0 & \cdot & \cdot &  \mathbf{N}_K\cdot \mathbf{H}_K \\
%  \end{bmatrix}
%  \begin{bmatrix}
%  X_1(f) \\
%  X_2(f)\\
%  \cdot \\
%  \cdot \\
%  X_K(f)\\
% \end{bmatrix}
% \end{split}
% \end{equation}
% % \begin{split}

% Since here, the vector $\mathbf{R}$ is a product of diagonal matrix and the vector having signals of all the $K$-users, using just a single RF chain with $K$ switched antennas, and the ADC, RF switches toggling at $KB$ rate, we can get data of $K$ users each having over the air bandwidth of $B$.

% \subsection{Spatio-temporal combining}

% The above analysis to get $K$ users data from one RF chains can be further generalized when there are multiple $S$ different RF chains. Usually, when we have $S$ RF chains, it is assumed that the design can serve $S$ interfering users simultaneously. However, with the $K$ times increased local IF bandwidth, we can actually even increase the number of users to $S\times K$. 

% Since now we need to serve $SK$ users, we would need to combine in $SK$ dimensions, and thus we have $SK$ number of switched antennas per RF chain (Fig.). In this scenario, from a single RF chain, we can only get $K\times 1$ vector $\mathbf{Y}^s$ from the $K$ number of orthogonal codes we can design when we increase the IF bandwidth $K$ times, however, we need to serve $SK$ users. The first key insight which we make here, is that now instead of using the identity codes, we will turn multiple antennas on simultaneously, and thus, the channels which we measure with the $K$

% To do so, we need to have $SK$ number of antennas, and in the multi RF chain setting, these $SK$ antennas are mapped to $S$ RF chains, instead of just $1$ RF chain. That is, there are $S$ different combiner networks, each combining $SK$ antennas with $SK$ RF switches to a single RF chain (Fig. ). Thus, in this scenario, we will have $S^2K$ number of RF switches, so that we can have $S$ different combiner networks for the $SK$ antennas.

% Considering that now we will get $K\times 1$ vector $\mathbf{Y}^{s}$ from the $s$-th RF chain, we can model it similar to the previous analysis and write it as $\mathbf{Y}^{s} = \mathbf{H}\mathbf{X}$, however, here $\mathbf{H}$ is $SK\times SK$, and $\mathbf{X}$ is $SK \times 1$. Thus, the null space vector here will be $SK\times 1$, and thus it is not enough to combine it with the $K\times 1$ vector $Y^s$

% \noindent Antenna Switching creates artificial time-faded channels -> \\
% Combined with oversampling creates virtual RF chains with separate channels across time->\\
% More antennas allows existance of null spaces ->\\
% Wideband null space combining cancels interference\\

% For example, when $K=4$ and identity codes as described before,
% $Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$. In general, if we do not have these identity codes, that is, say $B_1[n] = [1,0,0,1]_n$, $B_2[n] = [1,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,1,1]_n$, we will observe $h_{i1}+h_{i2}, h_{i2}, h_{i3}+h_{i4}, h_{i4}+h_{i1}$ on the 4 delayed streams. Thus, the measured channels are actually matrix multiplication of the $K\times K$ channel matrix , $\mathbf{H} = [h_1 h_2 h_3 h_4]$, with $K\times K$ code matrix 
% $\mathbf{B} = \begin{bmatrix} 
% B_1
% B_2
% B_3
% B_4
% \end{bmatrix}^T$ $\mathbf{H}\cdot \mathbf{B}$. If we choose codes such that $\mathbf{B}$ is invertible, we can estimate the $K$ antenna channels simultaneously 

==> design/design_no31.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
In this section, we present the design of \name. First, we describe how \name can create numerous virtual RF chains with a single RF chain, saving down-conversion and LO (Local Oscillator) sharing complexity. Next, we discuss how \name can achieve flexibility, by showing the analysis that \name can behave like both, a true digital beamformer, as well as a hybrid beamformer. Finally, we will discuss an algorithm to make the multiplexing gains from \name architecture robust, and conclude by having an overview of our design before moving to the implementation and evaluation of \name.

%First, we describe intuitively how \name is able to create these time interleaved virtual RF chains by building up on the toy example discussed in Section \ref{sec:intro}.

% \todo{this is good...proceed... features first then techniques...  :) }
\subsection{Creation of time interleaved RF chains with TIMO architecture}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{design/design_fig1.pdf}
    \caption{RF switches connect $i$-th antenna to every $4n+i$-th samples, creating time interleaved RF chains $y_i$ from a single sampled stream $y[n]$. Thus \name obtains multiplexing gains by leveraging the multiple antenna channels across the $4$ virtual RF chains.}
    \label{fig:design_subsec1}
    \vspace{5pt}
\end{figure*}

The goal of \name architecture is to serve $K$ users transmitting concurrently and in the same frequency band. 
This leads to interference amongst all the users as their signals get summed over-the-air as they propagate towards the receiver.
\name attempts to handle this $K$-user interference by creating $K$ virtual RF chains interleaved across time samples of a single downconverted stream sampled by an ADC sampling $K$ times faster the bandwidth of the users, $B_t$. In this section, before we generalize to $M>K$ scenario, we would motivate \name's design for a simple $M=K=4$ setting.
% Traditional approaches like digital beamforming create $K$ physical RF chain by having $K$ ADCs, and all these $K$ ADCs also need to sample $B_t$ bandwidth individually. 
% Thus, in terms of overall ADC sampling of $KB_t$ total samples, both these approaches are equivalent.
% However, the traditional approaches requires $K$ downconversion chains, whereas \name's architecture can create $K$ virtual RF chains by having just one downconverting mixer.

% To create these $K$ virtual RF chains with just a single downconversion chain, we utilize an antenna array with RF switches, and  
The intuition behind creation of these $K=4$ virtual RF chain is that sampling at $4B_t$ to decode $B_t$ bandwidth user, we get $4$ extra time slots at our disposal, and for these $4$ extra slots we can toggle different antennas on-off using RF switches to capture different antenna's signal in each of the $4$ slots. 
That is, say if we had a bandlimited signal $x[n]$, and we oversample it by $4$ times to obtain $y[n]$. To downsample $y[n]$ now, we have $4$ possible ways, we can do $y_0[n] = y[4n], y_1[n]=y[4n+1],y_2[n] = y[4n+2],y_3[n] = y[4n+3]$. Each of these $y_k$'s can be independently used to recover the original signal $x[n]$. 

This simple idea of $4$ independent ways to downsample $y[n]$ forms the intuitive prior behind \name's approach. That is, we can use switch different antennas on for these different sampling instants corresponding to each of the 4 $y_k$'s and use them as virtual RF chains interleaved over time. The concrete idea here is to keep the first switched antenna to be \emph{on} for $0,4,8,\ldots,4n$-th samples, the second switched antenna \emph{on} for $1,5,9,\ldots,4n+1$-th samples, and so on. This basically abstracts down to making each $y_k$ as a virtual RF chain for antenna $k$.  

To see how this virtual RF chain actually captures the wireless channel at $k$-th antenna, we model the scenario mathematically, with the $4$ users transmitting signals as $x_{1,2,3,4}(t)$, and the complex time-invariant channel seen by user $i$ to the $k$-th antenna represented as $h_{ik}$. We model the effect of RF switches tunring on-off for different sampling instants as a bit sequence $s_k[n]$, where $s_k[n] \in \{0,1\}$ and decides if switch $k$ corresponding to antenna $k$ is on or off for sample $n$. The combined interference signal $y(t)$ due to the $4$ users indexed via $i$, and $4$ switched antennas indexed via $k$, can be represented as:
\begin{equation}
    y(t) = \sum_{i=1}^4 \sum_{k=1}^4 (h_{ik}(t)*x_i(t))\cdot s_k(t).
\label{eqn:combined_codes}
\end{equation}
This combined signal $y(t)$ goes through downconversion, and ADC sampling at $4B_t$ to get digitzed signal
\begin{equation}
    y[n] \equiv y(nT_s) = \sum_{i=1}^4 \sum_{k=1}^4 (h_{ik}[n]*x_i[n])\cdot s_k[n].
\label{eqn:combined_codes}
\end{equation}
Now, we set $s_1[n] = [1,0,0,0]_n$, $s_2[n] = [0,1,0,0]_n$, $s_3[n] = [0,0,1,0]_n$ and $s_4[n] = [0,0,0,1]_n$, where $[\cdot]_n$ shows that the sequence gets repeated, that is $s_1[n] = 1,0,0,0,1,0,0,0,\ldots$.
This choice of switching sequence essentially selects $y_k$-th virtual RF chain for antenna $k$.
That is, antenna $1$ is \emph{on} for every $4n$-th samples correspnding to $y_0$ and \emph{off} for $y_1,y_2,y_3$, antenna $2$ is on only for every $4n+1$-th samples, correspnding to $y_1$ and so on (Fig. \ref{fig:design_subsec1}).
Thus, the oversampled signal $y[n]$ is interleaved with samples from each of the antennas.
This forms the core idea behing TIMO's approach of time interleaved RF chains.
We can now write these $K=4$ virtual RF chains, $y_1,y_2,y_3,y_4$ as
\begin{equation}
\begin{split}
y_k[n] &= \sum_{i=1}^4 (h_{ik}[4n+k]*x_k[4n+k])s_i[4n+k]\\
        &= \sum_{i=1}^4 (h_{ik}[4n+k]*x_k[4n+k]) \\
        &\approx \sum_{i=1}^4 (h_{ik}[4n]*x_k[4n+k]),
\label{eqn:equation_yj_id}    
\end{split}
\end{equation}

\noindent where the second step follows from $s_k[4n+k]$ being = 1 from definition, and the last step assumes that the wireless channels $h_{ik}[4n] \approx h_{ik}[4n+1] \approx h_{ik}[4n+2] \approx h_{ik}[4n+3]$, which is generally true as the coherence time for channels is usually much larger than duration of $4$ samples. Note that we are not assuming that the channel stays same across the entire packet length, but only local stationarity for every $4$ samples.

\noindent Hence, our $k$-th virtual RF chain $y_k$ effectively consists of convolution of all the $K$ users signals with channels between the users and the $k$-th antenna, as only $k$-th antenna is on for the samples used to derive $y_k[n]$ from the single combined stream $y[n]$. 
% Thus, setting $s_1[n] = [1,0,0,0]_n$, $s_2[n] = [0,1,0,0]_n$, $s_3[n] = [0,0,1,0]_n$ and $s_4[n] = [0,0,0,1]_n$ allows us to obtain the $4$ antenna channels $h_{i1}, h_{i2}, h_{i3}, h_{i4}$ for each of the $i$-th user, from $y_1[n],y_2[n],y_3[n],y_4[n]$ respectively, even if the outputs from the 4 switched antennas were combined into a single stream $y[n]$. 
This draws a parallel to how in a normal digital beamforming system, we get channels per RF chain from a single antenna. 
Hence, we can then combine across $y_k$'s in order to cancel the interference, similar to how digital beamformer utilizes separate spatial RF chains for the same purpose.
% This gives another requirement for the increased IF bandwidth to serve multi-user scenarios, that is to disambiguate this interference, we need to have increased antennas, so that we can combine across the antenna streams and cancel out the interference from each other. 
% A challenge here is to do so without actually increasing the number of RF chains, since otherwise the solution will not be scalable and useful.
% Thus, \name comes up with a creative solution, where we combine signals from multiple antennas into one combined RF chain, effectively utilizing the increased antenna space dimensionality to cancel interference, and using just one RF chain in the process. 
% However, this is not enough, since 
% Normally, wireless channels remain relatively stable over time, 
% and some reasoning for this is that the clients by-at-average don't
% move fast, and the sampling rate for receivers is reasonably high, 
% which allows the receivers to sample at a faster rate, which further 
% gives the sense that channels don't change much over multiple samples.

% So, how do we create dynamicness in the channel, which allows opportunities 
% to tap in the time diversity. The key 
\subsection{\name's equivalence to both digital and hybrid beamforming}
In the previous section, we have shown how we can obtain these virtual RF chains $y_k$ by utilizing the switching sequences $s_k$ and using RF switches to implement it with hardware. Before we move ahead in explaining how the combining is finally performed, we will generalize the setting to $K$ interfering users and number of antennas $M>K$. 
This generalization will concretely reveal how \name architecture can behave as both a digital beamformer, as well as a hybrid beamformer.

We start by formalizing the representation of the switching sequences as rows of a combined $M \times K$ switching matrix $\mathbf{S}$. An element $s_{mk}\in\{0,1\}$ in the matrix $\mathbf{S}$, 
represents the on-off states for each of the $m=1,2,3,\ldots,M$ antennas for $k=1,2,3,\ldots,K$ virtual RF chains. 
In the example in previous section we had $\mathbf{S}$ as an identity matrix, as only one antenna was \emph{on} at a time. 
More generally, with $i$ indexing $i=1,2,\ldots K$ users, $m$ indexing $1,2,\ldots M$ antennas and $k$ indexing $1,2,\ldots K$ virtual RF chains, we can write Eqn \eqref{eqn:equation_yj_id} as
\begin{equation}
    y_k[n] = \sum_{i=1}^K \sum_{m=1}^{M} (h_{im}[Kn]*x_i[Kn+k])\cdot s_{mk},
\end{equation}
and since $s_{mk}$ can be either $0$ or $1$, we can also write it as all antennas $m$ such that $s_{mk}=1$,
\begin{equation}
\begin{split}
y_k[n] &= \sum_{i=1}^K \sum_{m: s_{mk}=1} (h_{im}[Kn]*x_i[Kn+k])\\
       &= \sum_{i=1}^K \left(\left(\sum_{m: s_{mk}=1} h_{im}[Kn]\right)*x_i[Kn+k]\right)\\
       &= \sum_{i=1}^K \left(\left(\sum_{m}^{M} h_{im}[Kn]s_{mk}\right)*x_i[Kn+k]\right),\\
\end{split}
\label{eqn:equation_yj_gen}    
\end{equation}

\noindent where the second step follows from superposition principles of LTI analysis, and the last two steps are equivalent as $s_{mk}\in\{0,1\}$. To get a more concise expression and convert convolutions to multiplications, we can take the Fourier transform to go to the frequency domain,
\begin{equation}
Y_k[f] = \sum_{i=1}^K \left(\left(\sum_{m}^{M} \tilde{H}_{im}[f]s_{mk}\right)\mathcal{F}(x_i[Kn+k])\right),\\
\end{equation}
\noindent where $\tilde{H}_{im}[f]$ represents the Fourier transform of channel  $\tilde{h}_{im}[n]\approx h_{im}[Kn] \approx h_{im}[Kn+1] \ldots \approx h_{im}[Kn+K-1]$, since the channel is assumed to be stationary for every $K$ samples. For brevity, we will drop tilde from the expression and write it simply as $H_{im}[f]$.  We can write $\mathcal{F}(x_i[Kn+k]) =  e^{j2\pi f k}\mathcal{F}(x_i[Kn]) = e^{j2\pi f k}X_i[f]$ by using Fourier identities for time delayed signals and using the fact that $x_i(t)$ has been oversampled by $K$ times. Thus we get the simplified equation,
\begin{equation}
Y_k[f] = \sum_{i=1}^K \left(\left(\sum_{m}^{M} H_{im}[f]s_{mk}\right)e^{j2\pi f k} X_i[f]\right).\\
\end{equation}
Now, note that $\sum_{m}^M H_{im}[f]s_{mk}$ is nothing but the $(i,k)$-th element in the matrix multiplication between $K\times{M}$ channel matrix $\mathbf{H}[f]$, and the ${M}\times K$ switching matrix $\mathbf{S}$. Note that for $Y_k$ we need to remove the phase due to group delay in the Fourier transform, which can be done by multiplying $Y_k$ by $e^{-j2\pi f k}$, and we can write the delay compensated vector $\mathbf{Y^\mathcal{D}}[f] = [Y_0[f]\; Y_1[f]e^{-j2\pi f}\;\ldots\; Y_{K-1}[f]e^{-j2\pi f (K-1)}]^{\top}$. 
This vector $\mathbf{Y^\mathcal{D}}[f]$ consists of phase delay compensated Fourier transforms of $y_k[n]$ which were obtained by collecting $Kn+k$ samples in the oversampled signal $y[n]$, and this step is similar to how the popular function $\text{delayseq}(.)$\cite{delayseq} removes fractional delays.
Denoting $\mathbf{X}[f]$ to be $[X_1[f] X_2[f]\ldots X_K[f]]^{\top}$, to get a much simpler equation in terms of matrix products, 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f].
\end{equation}

This equation is akin to what hybrid analog-digital beamformers use, since $\mathbf{S}$ here is implemented by the analog switching network, and we observe $\mathbf{HS}$ equivalent $K\times K$ channel with digital streams which can then be combined over digitally.

In digital beamforming systems with $M=K$, we obtain $y_r[n]$ for each of the $r$-th RF chains, $r=0,1,\ldots K-1$, we get the equation 
\begin{equation}
\mathbf{Y^\text{RF}}[f] = \mathbf{H}[f]\mathbf{X}[f].
\end{equation}
For $M=K$ case, we can set the switching matrix $\mathbf{S}$ to be identity, we get a clear equivalence between \name and traditional digital beamforming, even though \name implements $\mathbf{S}$ in analog domain using switches. However, having $M=K$ is not a very robust operating point to serve $K$ users, since the channel may not always be full rank. Hence, it is always preferred to have $M>K$ in order to serve $K$ users.

Connecting more number of antennas to lesser number of physical RF chains usually requires changing the normal structure of the beamformer and creating specialised analog network with phase shifters.
In \name's architecture, we have the humble RF switch, which implements this switching network, similar to how setting this network to identity matrix gave \name an equivalence to digital beamforming. 
The main benefit of having $M>K$ antennas than $K$ virtual RF chains is that this allows us to harden the multiplexing gains of $K$ for any user configuration, irrespective of the underlying channels for the $K$ users. 

% To recover individual data symbols for each user $\mathbf{X}[f]$ from the obtained interfered samples $\mathbf{Y}[f]$, and assuming knowledge of channel matrix $\mathbf{H}[f]$, we can utilize a $K\times K$ beamforming matrix $\mathbf{V}[f] =[v_1 v_2 \ldots v_K]^T$ which is a collection of $K\times 1$ beamforming vectors $v_i$.  When we take the inner product of $v_i$ with $\mathbf{Y}[f]$, the hope is that we recover $x_i[f]$. 
% Basically, when evaluating the inner product, we have the expression $P_i=v_i^TH[f]$, and $P_i$ is another $K\times 1$ vector and the SIR obtained by the combining operation would then be $\frac{|P_{ii}|^2}{\sum_{j\neq i}|P_{ij}|^2} $, where $P_{ij}$ denotes $j$-th element of $P_i$. To obtain these beamforming vectors, we can use multiple methods, ranging from ZF, which basically multiplies $\mathbf{Y}$ by $\mathbf{H}^{-1}$, or using a MMSE, or null space beamforming. All these combining methods would work similarly for both \name's $\mathbf{Y^\mathcal{D}}$ as well as digital beamforming's $\mathbf{Y^\text{RF}}$. An important point to note is that since this combining happens in digital domain, we can do arbitrary combinations for each frequency bin $[f]$ which allows for resilient wideband operation, as well as accurate phase values for both methods, as compared to analog beamforming approaches which utilize phase combining at center frequency and runs into issues of beam squinting and phase quantization noise.

% The more recent papers \todo{CITE TurboHB} advocate the usage of null space beamformers which weed out the interference terms most effectively. 
% Here, $v_i$ is computed from null space of matrix $\mathbf{H}_{i^{\_}}$, which is obtained after removing $i$-th column from the chanel matrix $\mathbf{H}[f]$. $\mathbf{H}_{i^{\_}}$ has reduced number of columns (K-1) than rows (K), we will have a $K\times 1$ column-space null vector belonging to the null space of the matrix $\mathbf{H}_{i^{\_}}$.

\subsection{Harnessing power of multiple antennas for robust multiplexing gains}
In previous section, we saw how \name provides a much more natural solution to hybridize the digital architecture, by scaling up the number of switched-antennas \emph{without} requiring any additional sampling or downconversion chain costs, or any specialised hardware like phase shifters. In this subsection, we will present a simple but powerful method to strategically chooe the switching matrix $\mathbf{S}$ in order to harden the multiplexing gains. After generalizing the switching sequences to $M$ antennas, we got the following relation,
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f].
\end{equation}

The equivalent channel $\mathbf{H}[f]\mathbf{S}$ still remains $K\times K$, and the digital combining part operates on this $K\times K$ equivalent channel $\mathbf{H}[f]\mathbf{S}$. So the idea here is to choose the matrix $\mathbf{S}$ in a way such that the digital combining operates on a full rank uncorrelated $K\times K$ equivalent channel in order to increase the performance. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/design_fig2.pdf}
    % \vspace{2pt}
    \caption{By strategically choosing $\mathbf{S}$ to implement binarized analog beamforming per user, we ensure that the effective $K\times K$ channel is as uncorrelated as possible.}
    \vspace{4pt}
    \label{fig:smatrix__choice}
\end{figure}
Now, to choose $\mathbf{S}$, we have $2^{M\times K}$ possible choices, as each of the $M$ antenna can be turned on/off for each of the $K$ slots. Hence, a brute force optimization would not be scalable, considering $M=8$ and $K=4$, we have $2^{32}$ choices, and it will take a considerable amount of time to go over these possibilities, which would exceed the channel coherence time. Hence, instead of a brute force search for an optimal $\textbf{S}$ we need a smart and compute efficient way of estimating a relevant matrix $\mathbf{S}$. 

Here, we make a key observation. We have $K$ users, and the goal is to create equivalent channel $\mathbf{H}[f]\mathbf{S}$ which is as uncorrelated as possible. The way to do this would be to basically use each of the $K$ time slots to prioritize one user at a time, that is, to select column $i$ of $\mathbf{S}$ such that signal power of user $i$ is maximised in that slot.
This way the equivalent channel $\mathbf{H}[f]\mathbf{S}$ will have higher diagonal values than non-diagonal, which will decrease correlations, as one user is getting prioritized at a time.

To increase the signal power of user $i$, the theoretically exact way to do so would be to conjugate the user $i$'s channels for each antenna, thus implementing analog beamforming, which would co-phase the user's signals received at each antenna, to give constructive combining gains.
However, we do not have accurate phase shifters, and infact in our design we just have RF switches which can toggle on-off, thus providing only one-bit control over the phases. But, at the same time, we just need to increase the signal power for user $i$ and we actually do not need very accurate beamforming for this. This can also be achieved by turning \emph{on} the maximal set of antennas whose phases would add up constructively (Fig. \ref{fig:smatrix__choice}). We call this algorithm as binarized analog beamforming (BABF) algorithm, as it takes the analog beamforming solution and finds the closest representative of that in the binary RF switch implementable solution.

This binarized analog beamforming algorithm is simple, we go one antenna by one, and calculate the number of other antennas whose phases lie within an acute angle ($\pi/3$ in our implementation) of each other.
We select the group of in-phase antennas having the highest cardinality, since that would entail higher constructive combining gain and thus higher power for user $i$.
Thus, this makes the algorithm to be $O(M)$, as we have to choose from $M$ number of groups.
We repeat this procedure for each $k$-th user for $k$-th time slot to create a matrix $\mathbf{S}$.
Our detialed implementation of BABF algorithm is described in Algorithm \ref{Alg1} (in Appendix section). 

The BABF method of choosing $\mathbf{S}$ to prioritize signal power instead of utilizing $\mathbf{S}$ to cancel interference is a common theme on how hybrid beamformers \cite{chen2020turbo,ghasempour2018multi} choose their analog weights. This is because increasing signal power is an easier operation, and allows for inaccuracies because whatever is in-phase will ultimately add up and serve the purpose of increased signal power. On the other hand choosing an analog network such that signals are cancelled requires more careful calibration, as well as an requirement to generalize to wideband. Hence, in line with previous approaches to utilize analog networks for creation of such rank achieveing equivalent channels, we also propose an algorithm to increase the signal power, however using just RF switches instead of quantized phase shifters. 
The final task of combining across the signals with arbitrary accuracy and wideband generalization are the tasks of the digital combining part of \name which will be described in the next section.

\subsection{Final digital combining step in \name}

The key insight which \name delivers is that to handle $K$ users transmitting $B_t$ bandwidth signals $\mathbf{X}$, we can sample a single signal $y$ at $KB_t$ bandwidth by utilizing a switched antenna array with number of antennas $M>K$ and switching sequences for each of the $M$ antennas and the extra $K$ slots created due to higher sampling rate denoted by $\mathbf{S}$ to get the equation 
\begin{equation}
\mathbf{Y^\mathcal{D}}[f] = (\mathbf{H}[f]\mathbf{S})\mathbf{X}[f],
\end{equation}
where $\mathbf{Y^\mathcal{D}}$ are the delay compensated $K$ streams derived from $y$. We get an equivalent channel $\mathbf{H}[f]\mathbf{S}$ created due to the switching network, and we choose $\mathbf{S}$ such that the obtained $K\times K$ channel is as uncorrelated as possible, so that all the $K$ users can be served with sufficient SINR. 

Now, to recover individual data symbols for each user $\mathbf{X}[f]$ from the obtained interfered samples $\mathbf{Y}[f]$,  we can utilize a $K\times K$ beamforming matrix $\mathbf{V}[f] =[v_1 v_2 \ldots v_K]^{\top}$ which is a collection of $K\times 1$ beamforming vectors $v_i, i=0,1,\ldots K-1$.  When we take the inner product of $v_i$ with $\mathbf{Y}[f]$, the hope is that we recover $x_i[f]$. To cancel out interference, the best method is to use a ZF combiner \cite{rebato2019performance} .
In \name's case, the matrix $\mathbf{V}[f]$ selects pseudo inverse of $\mathbf{H}[f]\mathbf{S}$ as the digital combiner matrix $\mathbf{V}$. 
Thus after utilizing the digital combiner, we get
\begin{equation}
\mathbf{V}\mathbf{Y^\mathcal{D}}[f] = \text{pinv}(\mathbf{H}[f]\mathbf{S})(\mathbf{H}[f]\mathbf{S})\mathbf{X}[f] \approx \mathbf{X}[f], 
\end{equation}
which allows us to remove the interference and recover each of the $K$ symbols $\mathbf{X}=[X_1,X_2,\ldots X_K]^{\top}$. An important point to note is that since this combining happens in digital domain, we can do arbitrary combinations for each frequency bin $[f]$ which allows for resilient wideband operation, as well as accurate phase values so that the interference are cancelled perfectly. \todo{Add reciprocity argument that TIMO can work as a transmitter as well.}
% Hence, to choose the column $S^i$ such that user $i$'s signal power is increased, we first determine the best beamforming vector for user $i$, given by conjugate of the channel for user $i$ given by the $i$-th row of channel matrix, giving the $M\times 1$ vector $v_i = \mathbf{H}_i^*$. Now, we select antenna $j$, and multiply the conjugate phase of the beamforming vector associated with antenna j, given by $v^*_{ij}$, to get $v^j_i = v_iv^*_{ij}$. We then compute the angles of the of $\angle v^j_i$


% To recover individual data symbols for each user $\mathbf{X}[f]$ from the obtained interfered samples $\mathbf{Y}[f]$, and assuming knowledge of channel matrix $\mathbf{H}[f]$, we can utilize a $K\times K$ beamforming matrix $\mathbf{V}[f] =[v_1 v_2 \ldots v_K]^T$ which is a collection of $K\times 1$ beamforming vectors $v_i$.  When we take the inner product of $v_i$ with $\mathbf{Y}[f]$, the hope is that we recover $x_i[f]$. 
% Basically, when evaluating the inner product, we have the expression $P_i=v_i^TH[f]$, and $P_i$ is another $K\times 1$ vector and the SIR obtained by the combining operation would then be $\frac{|P_{ii}|^2}{\sum_{j\neq i}|P_{ij}|^2} $, where $P_{ij}$ denotes $j$-th element of $P_i$. To obtain these beamforming vectors, we can use multiple methods, ranging from ZF, which basically multiplies $\mathbf{Y}$ by $\mathbf{H}^{-1}$, or using a MMSE, or null space beamforming. All these combining methods would work similarly for both \name's $\mathbf{Y^\mathcal{D}}$ as well as digital beamforming's $\mathbf{Y^\text{RF}}$. An important point to note is that since this combining happens in digital domain, we can do arbitrary combinations for each frequency bin $[f]$ which allows for resilient wideband operation, as well as accurate phase values for both methods, as compared to analog beamforming approaches which utilize phase combining at center frequency and runs into issues of beam squinting and phase quantization noise.
% Going ahead, for brevity we drop the $[f]$ however we make the point that because we are implementing this combining across the digitized samples $y[n]$ we can perform arbitrary combinations across frequencies and utilize wideband beamforming. To recover $\mathbf{X}$ we can use multiple methods, ranging from ZF, which basically multiplies $\mathbf{Y}$ by $\mathbf{H}^{-1}$, or using a MMSE solution, as well as null space beamforming advocated by more recent paperrs for the same. Essentially, the aim is to design a combining matrix $\mathbf{V}$ such that $VY\approx $ 

% The more recent papers \todo{CITE TurboHB} advocate the usage of null space beamformers which weed out the interference terms most effectively. to compute the null space beamforming weights, consider an example of isolating signal of user $1$ from other users, we take the matrix $\mathbf{H}$ and remove the first column to get a $K-1 \times K$ matrix $\mathbf{H}_{1^{\_}}$, which because of reduced number of columns, will have a $K\times 1$ column-space null vector $\mathbf{N}_1$ belonging to the null space of the matrix $\mathbf{H}_{1^{\_}}$. When we take the inner product of the $K\times 1$ complex vectors, $\mathbf{N}_1$ with $\mathbf{Y}$, we see that

% \begin{equation}
%     \begin{split}
%     R_1 &= \mathbf{N}_1\cdot \mathbf{Y} =\mathbf{N}_1 \cdot \begin{bmatrix} 
%         \mathbf{H}_1\quad \mathbf{H}_{1^{\_}}\mathbf{X}
%         \end{bmatrix}\\
%         &=
%         [\mathbf{N}_1\cdot\mathbf{H}_1\quad \mathbf{N}_1\cdot\mathbf{H}_{1^{\_}}]
%         \mathbf{X}\\
%         &= \begin{bmatrix} 
%         \mathbf{N}_1 \cdot \mathbf{H}_1\quad \mathbf{0}_{K-1 \times K}
%         \end{bmatrix}
%         \mathbf{X}\\
%         & = (\mathbf{N}_1\cdot \mathbf{H}_1)X_1(f)
%     \end{split}    
% \end{equation}

% since $\mathbf{N}_1$ will null out the $\mathbf{H}_{1^{\_}}$ sub-matrix. Thus, using the vector $\mathbf{N}_1$ to combine across the $K$ delayed sample vector $\mathbf{Y}$ we can null out all other users apart from user 1, and hone onto the signal from user 1. Note that we can generate such nulling vectors for all the $K$ users, since there is nothing special about the user 1. Thus we can get $\mathbf{N}_{1,2,\ldots K}$ for all the $K$ users, from the null spaces of appropriate matrices $\mathbf{H}_{j^{\_}}$ by removing the $j$-th column associated to $j$-th user. Thus, we can get the vector $\mathbf{R}(f) = {\begin{bmatrix}
%  R_1(f) 
%  R_2(f)
%  \cdot 
%  \cdot 
%  R_K(f)
% \end{bmatrix}}^T$, such that

% \begin{equation}
% \begin{split}
% \mathbf{R}(f) &= [\mathbf{N}_1 \mathbf{N}_2 \cdot \cdot \mathbf{N}_K ] \cdot Y  \\
% & = \begin{bmatrix}
%  \mathbf{N}_1\cdot \mathbf{H}_1 & 0 & \cdot & \cdot & 0\\
%  0 & \mathbf{N}_2\cdot \mathbf{H}_2 & \cdot & \cdot & 0\\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  \cdot     & \cdot     & \cdot & \cdot & \cdot \\
%  0 & 0 & \cdot & \cdot &  \mathbf{N}_K\cdot \mathbf{H}_K \\
%  \end{bmatrix}
%  \begin{bmatrix}
%  X_1(f) \\
%  X_2(f)\\
%  \cdot \\
%  \cdot \\
%  X_K(f)\\
% \end{bmatrix}
% \end{split}
% \end{equation}
% % \begin{split}

% Since here, the vector $\mathbf{R}$ is a product of diagonal matrix and the vector having signals of all the $K$-users, using just a single RF chain with $K$ switched antennas, and the ADC, RF switches toggling at $KB$ rate, we can get data of $K$ users each having over the air bandwidth of $B$.

% \subsection{Spatio-temporal combining}

% The above analysis to get $K$ users data from one RF chains can be further generalized when there are multiple $S$ different RF chains. Usually, when we have $S$ RF chains, it is assumed that the design can serve $S$ interfering users simultaneously. However, with the $K$ times increased local IF bandwidth, we can actually even increase the number of users to $S\times K$. 

% Since now we need to serve $SK$ users, we would need to combine in $SK$ dimensions, and thus we have $SK$ number of switched antennas per RF chain (Fig.). In this scenario, from a single RF chain, we can only get $K\times 1$ vector $\mathbf{Y}^s$ from the $K$ number of orthogonal codes we can design when we increase the IF bandwidth $K$ times, however, we need to serve $SK$ users. The first key insight which we make here, is that now instead of using the identity codes, we will turn multiple antennas on simultaneously, and thus, the channels which we measure with the $K$

% To do so, we need to have $SK$ number of antennas, and in the multi RF chain setting, these $SK$ antennas are mapped to $S$ RF chains, instead of just $1$ RF chain. That is, there are $S$ different combiner networks, each combining $SK$ antennas with $SK$ RF switches to a single RF chain (Fig. ). Thus, in this scenario, we will have $S^2K$ number of RF switches, so that we can have $S$ different combiner networks for the $SK$ antennas.

% Considering that now we will get $K\times 1$ vector $\mathbf{Y}^{s}$ from the $s$-th RF chain, we can model it similar to the previous analysis and write it as $\mathbf{Y}^{s} = \mathbf{H}\mathbf{X}$, however, here $\mathbf{H}$ is $SK\times SK$, and $\mathbf{X}$ is $SK \times 1$. Thus, the null space vector here will be $SK\times 1$, and thus it is not enough to combine it with the $K\times 1$ vector $Y^s$

% \noindent Antenna Switching creates artificial time-faded channels -> \\
% Combined with oversampling creates virtual RF chains with separate channels across time->\\
% More antennas allows existance of null spaces ->\\
% Wideband null space combining cancels interference\\

% For example, when $K=4$ and identity codes as described before,
% $Y_1[n] = Y[4n] = Y[4n]\cdot B_1[4n] = \sum_{i=1}^K h_{i1}*X_i[4n]$, since every $4$-th sample in $B_1[n]$ is $1$, all others are zero. Similarly, $Y_2[n] = Y[4n+1],Y_3[n] = Y[4n+2], Y_4[n] = Y[4n+3]$. In general, if we do not have these identity codes, that is, say $B_1[n] = [1,0,0,1]_n$, $B_2[n] = [1,1,0,0]_n$, $B_3[n] = [0,0,1,0]_n$ and $B_4[n] = [0,0,1,1]_n$, we will observe $h_{i1}+h_{i2}, h_{i2}, h_{i3}+h_{i4}, h_{i4}+h_{i1}$ on the 4 delayed streams. Thus, the measured channels are actually matrix multiplication of the $K\times K$ channel matrix , $\mathbf{H} = [h_1 h_2 h_3 h_4]$, with $K\times K$ code matrix 
% $\mathbf{B} = \begin{bmatrix} 
% B_1
% B_2
% B_3
% B_4
% \end{bmatrix}^T$ $\mathbf{H}\cdot \mathbf{B}$. If we choose codes such that $\mathbf{B}$ is invertible, we can estimate the $K$ antenna channels simultaneously 

==> design/design_quals.tex <==
\section{Design}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{new_figs/des_figa.png}
    \caption{How MIMO can be enabled via a single RF chain}
    \label{fig:des_fig_a}
\end{figure}

\name designs a new multi-user MIMO antenna array architecture which maximises both energy and spectrum efficiency (EE \& SE) by adapting to varying user loads and carving out user-proportionate number of virtual RF chains as demand-fit from a single physically laid RF chain.
The key design elements which enable \name are the analog spreading, digital de-spreading blocks which allow creation of these virtual RF chains, and BABF approach to beamform towards one user-per virtual chain via many more antennas than number of users
% and generalization of this concept towards more antennas than number of users to create narrower interference free beams.
In this section, we will first describe how \name realizes the analog spreading via RF switches, how it is de-spreaded in digital domain, then describe the BABF approach. 
Finally, we end with how all these design elements work together to handle the multi-user interference and enable spatial multiplexing
% In this section, first we will ease into how such an architecture is possible by hypothesising existence of certain circuit element which can spread the received signals $B$ bandwidth signals across a wider $NB$ bandwidth to accommodate $N$ spatial streams to serve $N$ users.
% We will then show that this hypothetical circuit element can be realized in form of simple RF switches toggling with strategically chosen, orthogonal on-off codes having certain duty-cycle, initial phase and time period.
% Finally, we would generalize this proposed architecture to $M>N$ antennas in order to tap-into gains from more antennas to attain SE while keeping to user-proportionate power to maintain EE.

\subsection{How to enable MIMO with OFDMA's single adaptable-bandwidth RF chain}
% end with challenges in designing such a 

In this section, we will motivate how with a hypothetical circuit element, we can enable MIMO to work with a single, adaptively sampling user-proportionate RF chain akin to single antenna frequency divisioning schemes. This new architecture would enable MIMO gains to be adaptable with users as we need not have multiple physically laid RF chains as is the case with traditional MIMO. 

We show how this hypothetical architecture is actually nothing but marrying the two different concepts of spatial multiplexing (MIMO) and frequency multiplexing (OFDMA) into a best of both worlds concept, as shown in Fig. \ref{fig:des_fig_a}. 
The idea is to adopt the multiple antennas aspect of MIMO, and the adaptable bandwidth aspect of OFDMA, shown via green shaded boxes in Fig. \ref{fig:des_fig_a}.
To serve $N$ users having $B$ bandwidth each, MIMO architectures would have a minimum of $N$ antennas served by $N$ different RF chains such that the interfered mix of signals is downconverted and sampled across all $N$ antennas, which can be then fed to a digital beamforming (DBF) block that inverts the channel and isolated the per-user signals (Fig. \ref{fig:des_fig_a}, yellow box).
In contrast, to serve $N$ users, OFDMA would simply ask all users to be in different $B$ bandwidth zones in a net $NB$ bandwidth spectrum, which is downconverted and digitized via a $NB$ bandwidth ADC, and the per-user signals can be then isolated by simply carving out these $N$ different $B$ bandwidth zones (Fig. \ref{fig:des_fig_a}, blue box).

The goal of the new proposed architecture armed with $N$ antennas and a single $NB$ bandwidth RF chain is to basically take the per-antenna interfered signals mix having $B$ bandwidth each and spread it across the $NB$ sampled digitzed bandwidth of the ADC. 
Then, post-digitization, the per-antenna signals can be isolated in digital domain by carving out the different $B$ bandwidth zones. 
This is similar to how OFDMA isolated the $N$ different per-user signals, but now it will isolate the $N$ per-antenna signals, spread across the $NB$ bandwidth via the special circuit element.
Once separated, these per-antenna signals can then be fed to a digital beamforming block exactly similar to how these $N$ signals were fed in a traditional MIMO architecture.
Hence, the new proposed architecture would in theory, work exactly similar to the traditional MIMO architecture from the perspective of digital beamforming block, by simply spreading the antenna signals across the $NB$ bandwidth and the isolating them across the $N$ different $B$ bandwidth zones.

Hence, the key essence in enabling single RF chain MIMO would be how can we design this circuit element which would create the desired signal spreading effect.
Also, an important aspect would be the power consumption of this circuit element, say denoted by $P_c$, as the power consumption of the new architecture would clearly be $NP_c+P_{OFDMA}$, where $P_{OFDMA}$ is the power consumption of the single $NB$ bandwidth RF chain in OFDMA architecture. 
This is because the new proposed architecture largely has these 3 parts, $N$ antennas, which by themselves are passive entities, $N$ special circuit components one per antenna, and a single OFDMA like RF chain.
Hence, to truly show power efficiencies akin to single antenna OFDMA systems, this $NP_c$ term has to be negligible as compared to OFDMA power so that $P_{new}=NP_c+P_{OFDMA} \sim P_{OFDMA}$ for reasonable values of $N$ like popular configurations having $64/128$ antennas. Thus this circuit component has to be designed keeping under these requirements of negligible power consumption.

However, one point in favor of this new architecture is that these requirements are not as harsh.
% Considering the fact that we need to perform frequency shifts of the order of bandwidth, which is akin to shifting the signals to adjacent channels in case of Wi-Fi.
We have infact backscatter architectures, which do something similar and give frequency shifts to the signals to adjacent channels, that too at $10\mu$W level which can even be made batteryless.
Hence, the question boils down to if we can adopt something similar in context of single chain MIMO, where similar RF circuit component can perform these frequency shifts at a minimal power overhead, allowing to build MIMO systems with power levels meeting that of single antenna systems.



\subsection{GreenMO's realization of single RF chain MIMO using RF switches}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{new_figs/des_figb.pdf}
    \caption{How RF switches create the required signal spreading effect}
    \label{fig:des_figb}
\end{figure}

To practically realize the desired single chain MIMO architecture, this special circuit would need to overcome two challenges in order to create the desired frequency spreading effect.
First challenge, here is that the signal spreading effect has to be created right next to antenna in the RF domain, where the signals have not been downconverted yet. 
Hence, it rules out any simple baseband freq. shift circuits which implement frequency shifting.
Second challenge is that this circuit element should be low-powered enough so that the extra cost of adding these $N$ different circuit blocks is minimal and the overall power requirements remain similar to OFDMA level.

\textcolor{red}{Make this para crisp, need to compare with mixers o/w defensive writing}
A naive approach here would be to use mixers to create the desired frequency spreading effect. 
The mixers can have the LO clock sources of the order of signal bandwidth, instead of center frequency, to shift the signals across the $NB$ spectrum.
Hence, as compared to mixers typically used for downconversion operation, these $NB$ mixers would be shifting frequencies in order of bandwidth instead of center frequency will have orders of magnitude lower active power draw, which is proportional to frequency of operation. This would be because the bandwidth is just a small fraction of center frequency, for eg, in Wi-Fi the center frequency would be 2.4/5 GHz whereas bandwidth is just 20 MHz.
Although mixers by themselves can be passive circuits, they typically have considerable insertion losses.
Because of these insertion losses, mixer architecture would require per-antenna amplifiers (PA/LNA) to offset the losses. 
Hence, even though mixers can work right at the RF level, it does not fit the second challenge well due to the insertion losses.
An added third challenge however, with LNA/PA+mixer system would be how to handle the undesired non-linearities they introduce because of mixing+amplifying, which can lead to performance tradeoffs.

Instead, we realize that both the challenges can be met by taking a leaf out of backscatter systems, which face similar constraints on RF ciircuits which spread frequencies.
These backscatter systems also need near zero power power operation to justify batteryless operation, and also can not tolerate insertion losses which would lead to reduced reflected signal power.
As a consequence, backscatter systems use simple RF switches, instead of mixers to meet these requirements.
Clearly, RF switches work directly at the RF frequencies as they have the capability to toggle the impinging RF signals on and off.
Further, this on-off toggling if done periodically with a on-off square wave of certain frequency create harmonics and spreads the signals.
Also, RF switches have minimal insertion losses, <1 dB, and hence do not require amplifiers and as a proof have been used successfully in backscatter systems without needing LNAs/PAs.

So basically, if we connect an antenna, receiving a signal $s(t)$ to a RF switch which toggles with a periodic on-off wave given by $c(t)$, we get multiplication in time domain $s(t)c(t)$, corresponding to convolution in frequency domain $S(f)*C(f)$.
If we take a $1/B$ time period on off sequence $c(t)$ it will fundamental frequency as $B$. 
Thus, the active power draw proportional to $B$ instead of $f_c$, working at orders of magnitude lower power than downconverters which requiring LO clocks with time period $1/f_c$.
Although the RF switches are able to work at RF level and with minimal power requirements, the $B$ frequency on-off codes will have harmonics at integral multiples of $B$ which would spread the signal much beyond the nyquist period $[-NB/2,NB/2)$.
This is visually illustrated in Fig. \ref{fig:des_figb} for $N=4$.

So a natural question is how do we obtain the required spreading effect only between $[-NB/2,NB/2)$ and remove the non-linearities?
A simple solution of to basically do a low pass filter before sampling so that would eliminate these copies altogether and we would sample only the band of interest.
However, this would end up wasting the signal power which has landed beyond the band, as these wold just get filtered out.
Instead, we realize that the non-linearities created by switching can infact be harnessed in a powerful way by simple sampling process.
We make the observation that by sampling at $NB$ rate, a $1/N$ duty cycled code of $B$ frequency basically gives equal harmonics at integral frequencies in the required nyquist range.
This is because the other harmonic components simply alias on top of the required peaks in the $[-NB/2,NB/2)$, as shown in Fig. \ref{fig:des_figb} for $N=4$.
Hence, instead of filtering these non-linearities, by sampling them via $NB$ ADC these harmonics fold on top of each other and thus make the system efficient by not wasting any received signal power in filtering.

Hence, while serving $N$ users, using RF swithes, we can make use of the required $NB$ bandwidth to handle these $N$ users by spreading each antenna signals into this wide bandwidth via RF switches, at minimal power overhead and efficiently without losing any signal power.
% However, a natural question is that RF switches, like mixers also would produce these harmonics at other frequencies and hence create non-linearities. 
% In this section, we would show how these non-linearities can be harnessed in order to create the signal replicas without any losses and create performance comparable to traditional MIMO systems.
% Hence, RF switches become a perfect fit to the requirements of the special circuit element for the single RF chain MIMO architecture.

\subsection{How \name carves out $N$ virtual RF chains from $NB$ sampled bandwidth}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{design/des_fig2.pdf}
    \caption{\name on-off codes: continuous and discrete time}
    \label{fig:duty_fig}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{new_figs/des_figc.pdf}
    \caption{Separating per antenna signals}
    \label{fig:des_figc}
\end{figure}

So far, we have seen how the RF switches can be used to spread the recieved $B$ bandwidth interfered signals into a $NB$ bandwidth sampled spectrum, for one antenna.
Now, we will show how we can isolate the $N$ individual per-antenna signals from this net sampled bandwidth, which in abstract notion can be thought of as creating $N$ virtual RF chains towards each antenna.
Even though there does not exist a physical RF chain to each antenna, the isolation of per-antenna signals in digital domain from the net $NB$ sampled bandwidth would lead to creation of virtual chains interfacing each antenna to the ADC, without any actual physical laid hardware.
In this subsection we will simplify the setting to one antenna per virtual chain, and the next subsection generalizes to multiple antennas per virtual chain.

The basic idea behind creation of multiple virtual RF chains from this spreaded bandwidth is that we can actually have $N$ orthogonal codes each with $1/N$ duty cycle but different starting phases, as shown in Fig. \ref{fig:duty_fig}. 
So, when these codes are sampled with $NB$ bandwidth, these codes basically represent different sample indexes in time domain, since time sample occupies $1/NB$ time and because of $1/N$ duty cycling they have different on-off samples.
Essentially, $c_0$ is on for every $Ni$ samples, $c_1$ is on for $Ni+1$ samples and generalizing $c_j$ is on for $Ni+j$ samples.
When the fourier transform of these discrete sequences are taken, all the codes show $N$ delta functions at every integral multiple of $B$ between $[-NB/2,NB/2)$.
Further, each $c_i$ shows a different phase at these delta functions, with each $c_i$'s phase following a routes of unity sequence, like $c_i$ has phases $\frac{\pi}{N}*i*j$ for different $j$ denoting the $N$ delta functions $-NB/2,-(N-1)B/2,\ldots (N-1)B/2$.
Detailed proof of fourier transform of these discrete sequences is in appendix section \textcolor{red}{ToDo}.
The codes and their frequency components are shown visually in Fig. \ref{fig:duty_fig}.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{new_figs/des_figd.pdf}
    \caption{Generalizing \name to multi-antenna architecture}
    \label{fig:des_figd}
\end{figure}


The same virtual RF chain isolation can be done in time domain as well, where these codes get isolated much more easily, since they occupy non-overlapping samples.
Essentially $c_j$ ensures that antenna $j$ which is getting toggles with $c_j$ is on for $Nk+j$ samples, $k=1,2,3,\ldots$ denoting the sample index.
Hence, as illustrated in Fig. \ref{fig:des_figc}, even after the signals from multiple antenna get combined and pass through a single downconversion chain, by just isolating every $Nk+j$ samples, we can get the samples corresponding to $j$-th antenna. 
Thus, in a way this switching+sampling operation enables separate signal path for each antenna, in a way the downconversion chain is virtualized over all the antennas.
This makes \name architecture with virtual RF chains a flexible architecture, as \name can adjust the number of virtual RF chains on the fly. 
If the number of users change from $N \to N'$, the architecture can respond by simply changing the sampling rate from $NB$ to $N'B$, which can then be used to carve out the needed $N'$ virtual RF chains.
In comparison, a traditional MIMO architecture can not increase/decrease number of RF chain in response to user demand as these RF chains have been laid physically, and can not be changed on the fly.
Hence, \name architecture can flexibly meet the user-proportionate power consumption demands.
However, till now we have assumed $N$ antennas for $N$ users, and to justify the required flexibility, we will generalize the architecture for $N$ users with $M>N$ antennas in the next subsection, so that the sampled bandwidth remains $NB$ while icnreasing antennas to $M$. 


\subsection{How \name flexibly generalizes to $M$ antennas for $N$ users}

Finally, we will show in this section how \name generalizes to $N$ users and $M>N$ antennas.
With $M$ antennas, we can serve at most $M$ users simultaneously from info-theoretic bounds \cite{}.
Hence, in order to be flexible to user demand and power-efficient, \name needs to adapt to the scenario when number of users $N$ are lesser than number of antennas $M$ ($M<N$).
By that we mean \name should consume power proportional to $N$ instead of number of antennas $M$ when user load decreases, in order to justify the user-proportionate power claim.

The key insight to this generalization is the fact that unlike a physical RF chain, which is connected to one antenna typically, the virtual RF chains are by default connected to all the RF chains simultaneously.
In other words, we can turn `on' multiple antennas per virtual RF chain instead of a single antenna, and also, an antenna can simultanoeusly be `on' for multiple virtual RF chains.
This multiple antenna to multiple virtual RF chain mapping is enabled by the orthogonality of the toggling sequences $c_j$.
That is, if we want to turn on antennas $i_1,i_2,i_3$ for the virtual RF chain created by $c_j$, we can supply the $c_j$ clock to each of these antennas indexed via $i_1,i_2,i_3$.
And if a particular $i$-th antenna has to be turned on for $j_1,j_2,j_3$ virtual RF chains, we can supply clocks $c_{j_1}+c_{j_2}+c_{j_3}$.
Since $c_{j_1}$, $c_{j_2}$ and $c_{j_3}$ don't overlap in time, adding these codes together would create a new toggling sequence which would be `on' for $Nk+j_1,Nk+j_2,Nk+j_3$ samples and hence turn on this antenna for all these $3$ virtual RF chains.
This is illustrated visually via inset in Fig. \ref{fig:des_figd}.


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/setup.pdf}
    \vspace{1pt}
    \caption{Hardware implementation of \name}
    \label{fig:pcb_pic}
\end{figure}

Putting this in a matrix form, because of this many to many mapping, where multiple antennas can be turned `on', `off' for multiple virtual RF chains, the switching network allows us to implement a binary matrix $\mathbf{S} \in \{0,1\}^{M*N}$ in analog domain, where $M$ is number of antennas and $N$ is number of users, as well as number of virtual RF chains to justify the user-proportionate computing claim.
Basically, this matrix projects the higher dimensional channel $\mathbf{H}$ which is complex valued $\mathbf{C}^{N*M}$ which represents the amplitude and phase of each $n$
-th user at $m$-th antenna, into an equivalent $\mathbf{C}^{N*N}$ chnanel $\tilde{\mathbf{H}}=\mathbf{HS}$ by toggling antennas on-off strategically.

Hence, to create user-proportionate $N$ virtual RF chains, \name architecture can project the $N*M$ antennas channel into $N*N$ equivalent channel via $\mathbf{S}$ matrix implemented in analog domain by RF switches and the supplied clocks.
The choice of this matrix when $M=N$ is obvious, we can just set it to identity matrix and continue, as was also motivated in the prior sections.
When $M>N$, we need to select the matrix $\mathbf{S}$ strategically such that we tap into the higher degrees of freedom offered by more antennas and project the higher dimensional matrix $\mathbf{H}$ into a well-formed $N*N$ equivalent $\tilde{\mathbf{H}}$.
To do so, our insight is that since we have $N$ virtual RF chains for $N$ users, we can user the high number of antennas to perform approximate on-off beamforming towards one user per virtual RF chain.
That is, for virtual RF chain $j$, we basically turn `on' the maximal set of antennas in-phase for user $j$, so that the signal power for user $j$ is boosted for $j$-th virtual chain.
This is visually illustrated in Fig. \ref{fig:des_figd}, with each virtual RF chain prioritising one particular user.

The matrix $\mathbf{S}$ which implements this is determined via BABF algorithm (Binarized analog beamforming) which takes the analog beamforming weights and basically quantizes it to binary $0-1$ level.
The exact algorithm is included in appendix and the idea is illustrated visually in Fig. \ref{fig:des_figd} for a particular `blue' user.
After the virtual RF chains are created, they are fed to the digital beamforming blocks which invert this equivalent matrix $\tilde{\mathbf{H}}^{-1}$.
The choice of switching matrix $\mathbf{S}$ ensures ivertability of $\tilde{\mathbf{H}}$, since by prioritizing one user per virtual RF chain, it basically makes the equivalent channel, $\tilde{\mathbf{H}}$ an approximate identity matrix, and hence enables the $N*N$ digital beamforming block to suppress interference with ease.


\textbf{Putting it all together}: So, to conclude the design section, we will briefly summarize and put the various design elements in context.
We started by hypothesing how we can marry the MIMO spatial multiplexing architectures with OFDMA frequency multiplexing architecture by means of a frequency spreading RF circuit element.
Then, we showed how to realize this hypothesis in form of strategically toggling RF switches, which enable the creation of separate virtual RF chains per user.
Via BABF algorithm to select switching matrix $\mathbf{S}$, we can beamform towards one user per virtual chain.
Finally, this equivalent $N*N$ channel $\tilde{\mathbf{H}}=\mathbf{H}\mathbf{S}$ can be fed to digital beamformer block which would invert this $\tilde{\mathbf{H}}^{-1}$to finally get the per-user signals.


\begin{figure*}[t]
    % \begin{subfigure}[t]{0.6\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{results/microbenchmarks/combiner_lowres.pdf}
    % \input{results/microbenchmarks/combiner} 
    \caption{(a) Shows the raw received signal from the single RF chain. The created virtual RF chains are shown in (b), after BABF which increases user $i$'s power in $i$-th virtual chain. Finally (c) shows the interference free per-user streams obtained after digital combining of the virtual chains. (d) and (e) show the raw constellations before and after interference cancellation.}
    \label{fig:ex_trace}
\end{figure*}
% However, in a practical setting, usually we require more antennas than number of users $N>M$ so that 


==> intros/intro_dig_hyb.tex <==
% !TEX root = paper.tex

\section{Introduction}

% Spectrum is scarce, TDMA is slow
The amount of devices connected to wireless networks has been blowing up as the networks become more accessible and robust. 
Today on an average, a single person carries multiple devices connected to the same network, like a phone, tablet and smart watches.
Thus, any wireless Access Point (AP) will almost always be connected to multiple devices.
The easiest way for the AP to handle multiple connections is to put the multiple devices in different time slots or non-overlapping frequency bands.
The first approach reduces throughput, whereas the second approach demands more spectrum.
However, spectrum is a scarce resource, and thus to scale to the number of devices without trading off throughput, we need concurrent user transmissions without adding new spectrum.

% MIMO has tried to solve this exact issue, fails
Enabling spectrum efficient multi user communications has been the core push behind mu-MIMO technologies, by utilizing digital beamforming. 
Digital beamforming techniques exploit the increased dimensionality from multiple antennas, in order to attempt create orthogonal spatial streams to multiple concurrently transmitting users sharing the same frequency band. 
In theory, digital beamforming can utilize $K$ antennas to create $K$ spatial streams to serve $K$ users simultaneously.
However, in practise this 1:1 mapping between number of antennas and number of users doesn't work, since often the channels between the users are highly correlated, and thus the spatial streams created by digital beamforming are not orthogonal and suffer from significant performance degradation. 
Resolving this issue with mu-MIMO has been the push behind massive MIMO, wherein the idea is to exploit a large number of antennas to leverage digital beamforming in a $K_{\text{ant}}=K_{\text{dim}}>K$ dimensional subspace where it is robustly possible to create these $K$ orthogonal spatial streams.

Thus, it is of utmost importance to extend the digital beamforming ideas to utilize higher number of antennas than before. 
A naive way to go by this is to keep on adding a separate RF chain for each antenna, consisting of a downconversion mixer and a sampling ADC alongwith other electronics.
However, this approach saturates the power and hardware requirements very quickly, alongwith the effort which goes into design of supporting interfaces like synchronised LO distribution across multiple RF chains.

Thus the adoption of digital beamforming architectures pose a big system level challenge to manage and operate. This had lead to limited adoption of the technology, and notable wireless networks like Wi-Fi moving ahead with OFDMA (tight scheduling of users in time/freq slots)  in WiFi-6, and 5G standards focussing on analog beamforming which typically use phased arrays with single RF chain. But none of these technologies actually enable spatial multiplexing, leaving the scalable multi-user wireless communications still an open problem. Hence, in this paper, \name asks if it is possible to achieve digital beamforming with multiple antennas, in a more scalable manner, with just a single RF chain. 
If we can achieve this elusive goal of multi-user reception with a single RF chain, this method of generating spatial multiplexing would be a new alternative to the usual method of laying multiple RF chains to get the same multiplexing gains. 


% Core concept of time combining
This leads to the first design principle of \name's solution for multi user networks, which is to leverage time as an alternate axis to space in order to generate these new spatial multiplexed streams.
The inspiration for this idea is simple, imagine if we have an antenna array wherein all the antennas' outputs are combined into a single wire interface, which then goes through a single downconversion chain and digital sampling. If we keep one antenna \emph{on}, and other antennas \emph{off} for certain time samples, during those time samples we can discern the channel observed at that particular antenna.
At some other time samples, we can turn a second antenna \emph{on}, and observe the channel at the second antenna, and so on.
Thus, by turning individual antennas on-off in an antenna array, we can use a single wire interface to isolate the channels observed across multiple antennas (Fig. \ref{fig:intro_time_interleaved_rfcs}).
This draws a parallel to how digital beamforming observes individual antenna channels. 
What digital beamforming achieves by utilizing samples across the ADCs sampling the antenna space directly, \name achieves though digital samples interleaved across time by toggling antennas \emph{on} and \emph{off}.

% practical implementations now
To practically implement digital beamforming, we require a separate downconversion chain and an individual ADC to sample the baseband signal after downconversion.
In stark contrast, we can implement \name by just using a RF switch per antenna, a simple wired combiner network across the antennas followed by a single downconversion chain and an ADC to digitize the samples. 
Essentially, the usage of RF switches help us create virtual RF chains over time, with the digital samples where one antenna is \emph{on} forming the virtual RF chain associated with that antenna, and similarly for the other antennas, we can collect the \emph{on} samples for that antenna and assign those to be a virtual RF chain for the other antenna.
Hence, for practical implementation of \name, we need an ADC which can sample at a higher rate to accommodate creation of these virtual RF chains per antenna.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virt.pdf}
    \caption{Time interleaved virtual RF chains: An antenna array with RF switches, which turn each antenna on turn by turn and thus the single ADC samples the combined stream having antenna signals interleaved with each other}
    \label{fig:intro_time_interleaved_rfcs}
\end{figure}

This leads us to the second design principle of \name, which is to utilize higher sampling bandwidth than what aggregate bandwidth transmitted by the users. 
In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. Thus, \name would utilize a $K$ times sampling bandwidth for the single ADC in its design, as compared to $K$ different ADCs sampling at lower rate as compared to digital beamforming. \name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.

% Note that \name utilizes just a higher sampling bandwidth and does not necessitate the total over-the-air bandwidth to be $K$ times higher (Fig. \ref{fig:introfig1}). The total over-the-air bandwidth still remains lower, thus \name's approach is spectrum efficient. This assymetricity in the sampling bandwidth and the total utilized spectrum can be regularly seen in everyday wireless networks, for example, in Wifi-6, modems are always capable of performing 160 MHz sampling, still there are modes in which they just sample aggregate bandwidth of $20/40/80$ MHz in crowded situations like Airport/Malls, where there are neighbourhood modems operating in the other occupied frequency bands in the exposed 160 MHz spectrum. \name provides a method to increasing the network capacity by enabling multiplexing gains due to creation of virtual RF chains using the higher sampling rate capability.

% The final design principle of \name is to utilize more number of antennas than number of virtual RF chains, creating a hybrid \name beamformer in order to harden the spatial multiplexing gains. 

Going one step further, we notice that a generalization of \name's switching based approach to more number of antennas than number of virtual RF chains is very natural. This leads to the final design principle of \name wherein we creating a hybrid \name beamformer in order to harden the spatial multiplexing gains from the created virtual RF chains. Basically, we can switch multiple antennas on for each of the virtual RF chain in order to utilize constructive combining gains from these antennas to our advantage. This draws a parallel to hybrid beamformers, which have more antennas than number of physical RF chains.

Interestingly, \name's hybrid virtual beamforming automatically creates a fully connected hybrid beamformer, the gold standard amongst the currently existing hybrid beamformers. This is because all antennas are connected to the created virtual RF chains by default. In comparison, fully connected hybrid beamformers for physical RF chains require the hardware cost of  having an extensive circuit network required to connect each antenna to each RF chain. In case of \name's hybrid generalization, since the RF chains are a virtual abstract of the single wire sampled signal, all the antennas are connected automatically to each virtual RF chains without requiring more amount of switches to the effect.

Utilizing more number of antennas than number of virtual RF chains allows \name to harden the multiplexing gains entailed by the number of virtual RF chains available. This is a very concrete problem with mu-MIMO approaches of today, that we can not actually have $K$ users reliably multiplexed with $K$ antenna digital beamformer \cite{}. Due to this, there has been research on creating mu-MIMO schedulers \cite{}, which would select the group of users which can be multiplexed successfully, in order to fully utilize the available RF chains. Unlike these approaches, \name solves the problem head-on, by utilizing more number of antennas and strategic switching sequences to create an uncorrelated equivalent channel, which always allows for robust multiplexing gains across any spatial user configuration. This is also backed by our evaluation, where we see a drastic improvement with hybrid architecture when number of users are same as number of virtual RF chains.

Thus, to summarize, \name designs a novel antenna array which utilizes a single wire interface at a higher sample rate to replicate what traditional digital beamformers typically do with multiple wire slower interfaces, at the same time avoiding requirement of multiple downconversion chains. Further, \name shows that such architectures are naturally generalizable to a fully connected hybrid architecture with more number of antennas than number of RF chains, which allows us to harden the multiplexing gains and allow for robust mu-MIMO operation. We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users by utilizing a hybrid architecture.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/intro_fig_1.pdf}
%     \caption{Comparison of \name with current wireless networks. Due to creation of new fractional time-slots by fast switching, \name can serve multiple users operating over the same time slot and frequency band}
%     \label{fig:introfig1}
% \end{figure}

% The benefits of this are two-fold, first, 
% gains, and second, if any system has more RF chains available, \name can work in tandem with digital beamforming to tap into even more multiplicative gain possible. Said simply, if \name with 1 RF chain can serve 4 users, \name with 2 RF chains can serve 8 users in accordance with the 2x multiplexing offered by an additional RF chain.






% and then be interpolated across to get the entire received signal at the antenna without requiring each antenna to be on for a long period of time. 


% that unlike transmitters which are external to the receiver and time divisioning has to respect the hardware constraints at the transmitter, this antenna switching is a local property of the receiver. 




% This forms the basis behind digital beamforming, which utilizes these digital samples across multiple antennas in order to utilize the high dimensional channels across the antennas to allow for multi-user transmissions. 
% However, digital beamformers 

% This is a required step since if we want to exploit the increased dimensionality, we need 
% Thus, in the WiFi 802.11ac protocol released back in 2016, mu-MIMO was introduced to commodity devices and was pitched to be a defining change for the future network design. 
% However, mu-MIMO failed to deliver on the promise of scaling well to multi-user transmissions, and infact there are reports that enabling mu-MIMO option in 802.11ac routers even leads to reduced performance metrics, as compared to scheduling users in different time slots.

% One of the main issues with mu-MIMO was that the assumption that we can always create independent spatial streams was not true for practical channels. 
% Creation of independent spatial streams is a very channel dependent property, and works well only if the channels for one user is uncorrelated with the other.
% One way to ensure creation of independent spatial streams is to increase the dimensionality by utilizing multiple antennas, which forms the goal behind massive MIMO\cite{}.
% Massive MIMO proposes to use a very large number of antennas in order to tap in the large dimensionality to create independent spatial streams.
% However, this requires connecting each antenna to a separate downconversion chain and sample the received signals, which requires an extensive network of RF chains requiring multiple ADCs and synchronised LO distribution networks for the downconvertors.
% All these make massive MIMO 

% Time is an untapped dimension
% doing it faster, opens up opportunities at sub 6
% our solution

==> intros/intro_dimension.tex <==
% !TEX root = paper.tex

\section{Introduction}

% Spectrum is scarce, TDMA is slow
The amount of devices connected to wireless networks has been blowing up as the networks become more accessible and robust. 
Today on an average, a single person carries multiple devices connected to the same network, like a phone, tablet and smart watches.
Hence, in today's digital environment, wireless networks need to be designed to prioritize handling multi-user connectivity.
The easiest method to handle multiple devices connected to a network is to have the devices talk to the network access point (AP) in different time slots. 
This however requires tight scheduling, or a distributed scheduling based MAC protocol, and in general reduce the throughput as number of devices scale up in the network.
To avoid this, a possibility is to have the devices transmit in different frequency bands, which allows for concurrent transmissions across multiple users, at the expense of higher spectrum requirement.
However, spectrum is a scarce resource, and thus to scale to the number of devices without trading off throughput, we need concurrent user transmissions without adding new spectrum to the mix.

% MIMO has tried to solve this exact issue, fails
Enabling spectrum efficient multi user communications has been the core push behind mu-MIMO technologies, by utilizing the high dimensionality offered by multiple antennas. 
This increased dimensionality allows enable creation of orthogonal spatial streams towards each device in the antenna space, allowing devices to be using same frequency band while transmitting concurrently.
However, the capability to create such orthogonal spatial streams is highly channel dependent, and in real-life channels with users carrying multiple devices with themselves, the channels to each device is extremely correlated, which creates cross-talk between these spatial streams and doesn't allow for orthogonal transmissions \cite{}.
This has been one of the core deterrents to achieve the promised multiplexing gains from mu-MIMO systems, and has plagues the mu-MIMO implementations after it got introduced into Wi-Fi 802.11ac \cite{},
Infact, there have even been reports that enabling mu-MIMO option in 802.11ac routers even leads to reduced performance metrics, as compared to scheduling users in different time slots.

%need for higher dimensionalities
The solution of this problem is to utilize much more antennas than number of spatial streams, at which point the terminology of mu-MIMO changes to massive MIMO \cite{}.
There have been theoretic papers which show that as number of antennas become infinitely large the multiplexing gains harden and become robust for any user configuration \cite{}.
However, to tap into these increased dimensionalities, we need to obtain the received digital samples from each antenna.
The way to do this digital sampling today is to connect each antenna to a downconversion chain followed by an ADC to sample these baseband signals.
These architectures are referred to as digital beamforming, and the challenges digital beamformers face today are issues with requirement of multiple ADCs, requiring an extensive synchronized LO network alongwith active circuit elements like mixers, all of which lead to exacerbating hardware requirement requiring a ton of powers.

% Some other way of getting this
Hence, the question \name attempts to answer is can this increased dimensionality be supported by some other means than requiring multiple downconversion chains and ADCs. 
The main element responsible for these increased dimensionalities are the multiple antennas, each capturing a different channel and opening up a new dimension.
So, can we just connect multiple antennas to a single downconversion chain, and still attempt to get the said dimensionalities?

% 
When we combine multiple antenna streams into one, the channels across each of the combined antennas get added into the one stream coming out, leading to superposition of channels. 
Thus instead of behaving like different antennas, we just observe the summed single channel of the combined array, and thus the array behaves like a single large antenna instead of different smaller antennas and does not offer the required dimensionalities. 
Here, \name comes up with a creative solution, which is to augment the antenna array with RF switches, and create artificial time diversity by switching the antennas on-off.
The core idea is simple, say at time instant one we switch off all the antennas apart from one, we start observing digital samples from that one antenna from the entire combined array.
Similarly, at second time instant, we can turn on a second antenna and turn off the others, which now starts giving channels of the second antenna. 
Thus, by toggling antennas on-off we can create temporal changes which allow \name to discern channels of each of the antennas in the combined array without requiring a different downconversion chain for each antenna.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/design_dim.pdf}
    \caption{Time interleaving RF chains: Shown in the figure is an antenna array with RF switches which turns each antenna on turn by turn and thus the ADC will sample the combined stream having antenna signals interleaved with each other.}
    \label{fig:time_interleaved_rfcs}
\end{figure}

However, a natural question here is, wouldn't this time divisioning of antennas entail reduced throughput, since to get multiple antenna channels we need multiple time slots to turn each of them on-off.
Here, \name makes a key connection, that these antenna samples can be time interleaved across the entire received samples (Fig. \ref{fig:time_interleaved_rfcs}), 
instead of one antenna being on for a long amount of time, then the second antenna and so on.
This will create time interleaved RF chains over a single sampled stream and thus would enable tapping into increased dimensionality offered by the antennas by using just a single RF chain.

% and then be interpolated across to get the entire received signal at the antenna without requiring each antenna to be on for a long period of time. 


% that unlike transmitters which are external to the receiver and time divisioning has to respect the hardware constraints at the transmitter, this antenna switching is a local property of the receiver. 




% This forms the basis behind digital beamforming, which utilizes these digital samples across multiple antennas in order to utilize the high dimensional channels across the antennas to allow for multi-user transmissions. 
% However, digital beamformers 

% This is a required step since if we want to exploit the increased dimensionality, we need 
% Thus, in the WiFi 802.11ac protocol released back in 2016, mu-MIMO was introduced to commodity devices and was pitched to be a defining change for the future network design. 
% However, mu-MIMO failed to deliver on the promise of scaling well to multi-user transmissions, and infact there are reports that enabling mu-MIMO option in 802.11ac routers even leads to reduced performance metrics, as compared to scheduling users in different time slots.

% One of the main issues with mu-MIMO was that the assumption that we can always create independent spatial streams was not true for practical channels. 
% Creation of independent spatial streams is a very channel dependent property, and works well only if the channels for one user is uncorrelated with the other.
% One way to ensure creation of independent spatial streams is to increase the dimensionality by utilizing multiple antennas, which forms the goal behind massive MIMO\cite{}.
% Massive MIMO proposes to use a very large number of antennas in order to tap in the large dimensionality to create independent spatial streams.
% However, this requires connecting each antenna to a separate downconversion chain and sample the received signals, which requires an extensive network of RF chains requiring multiple ADCs and synchronised LO distribution networks for the downconvertors.
% All these make massive MIMO 

% Time is an untapped dimension
% doing it faster, opens up opportunities at sub 6
% our solution

==> intros/intro_flex.tex <==
% !TEX root = paper.tex

% Flexible beamforming approach
% massive MIMO: softwarized etc
% HB: green, not SWrized

\section{Introduction}\label{sec:intro}

% Multiple-Input Multiple-Output (MIMO) communications enable multiple users to use the same spectrum simultaneously, thus helping the communication systems to scale up to number of users without need of buying/managing new spectrum \todo{cite}.
% This is made possible by using multiple antennas for communications, with each antenna bringing a new \textit{spatial} degree of freedom \todo{cite} allowing possibility of handling a new user.

% The wireless channel conditions and number of users in the network highly dictate on what can be achieved via these spatial dgerees of freedom. 
% That is, to serve $K$ users, we need minimum of $K$ degrees of freedom, which requires at least $K$ antennas.
% If the wireless channel between the base station and these $K$ users is favorable, we would require to exploit exactly $K$ antennas to serve each user successfully, whereas in some scenarios where the wireless channel is such that each new degree of freedom is not independent to other, and has some correlations, this number could be as high as $2*K$ or even higher. 
% Thus, it is highly favorable if we can capture these degrees of freedom in a flexible way, depending on channel conditions and how many interfering users exist, in order for an optimized multi-user system.

% However, none of the existing multi-antenna architectures can achieve this required flexibility. The mantra today is to design systems capable of `massive MIMO', referred to MIMO deployments having many more number of antennas than the number of users, to capture a lot of degrees of freedom and guaranteeing performance for a certain number of users. Massive MIMO implementation requires laying of a physical Radio frequency (RF) chain for each antenna to capture these degrees of freedom. 
% The RF chain essentially captures and amplifies the signal from an antenna, downconverts and finally digitizes the samples for MIMO processing, consuming certain amount of power in the process.
% % The RF chain essentially 
% Thus, when the wireless channel is favorable, or number of users are lesser, massive MIMO systems would end up burning a lot of power in the physically laid out RF chains. 

% % 
% A naive method of adding flexibility in traditional massive MIMO systems is to turn off some RF chains if conditions are favorable; however this comes at a price of reduced number of degrees of freedom, as turning off an RF chain amounts to dropping samples from the antenna it was connected to.

% A naive solution to this is to strategically turn off some RF chains depending on channel conditions, however this would mean inefficient utilization of the multiple antennas laid out, and wouldtradeoff the available degrees

% In order to utilize these degrees of freedom it is required to obtain the baseband samples of each antenna \todo{cite}.
% This is usually achieved by connecting each antenna to a separate Radio-Frequency (RF) chain, with a technique referred to as `Digital beamforming'.
% The RF chain has physically laid out 


% The RF chain essentially has circuit components like a power amplifier to boost the weak signals captured by the antenna, and a mixer to downconvert antenna's signal to baseband frequencies, in addition to requirement of a ADC to finally get the digital samples for MIMO processing from the downconverted-boosted signal input.

Multiple Input Multiple Output (MIMO) communications enable scaling of wireless networks to multiple users without adding new spectrum. 
The research and deployment trends over the past decade has evolved from muMIMO (multi-user MIMO) with number of antennas equalling number of users to massive MIMO, which uses many more antennas than number of users. 
The reasoning behind this shift has been simple, each antenna brings about a new degree of freedom and with lots of degrees of freedom massive MIMO can give performance gains which muMIMO had failed to deliver. 
However, in order to capture these lots of degrees of freedom, massive MIMO faces challenges in coming up with a green system architecture, which optimizes the power consumption.

%Virtualization gives hardware re-use, saves energy
The core reason behind this is the inflexibility of today's massive MIMO architectures. 
With current architectures, we need to have a physical RF chain laid out to each antenna for capturing the required degrees of freedom.
The RF chain essentially contains the hardware which downconverts and digitizes the signal from antennas for MIMO processing.
Since massive MIMO aims to capture higher number of degrees of freedom arising from having many antennas, it also needs to lay out these hardware chains to each of the antenna.
This is where the current solutions become over-engineered and inflexible; If the wireless channel conditions are favorable, or number of users to support decreases, it will not be required to have this many number of physically laid out RF chains.

% Virtualization gives software control, allows multiplexing

% A possible solution to make these networks flexible is to take a leaf out from an increasing trend of network virtualization. 
% That is, if these RF chains are not physically laid out, but captured in a way such that it is virtually abstracted out over reconfigurable hardware, we can then increase/decrease the number of these virtual RF chains at will, depending on channel conditions and user load.
% The core of this paper targets such an architecture which can virtualize these RF chains over a common laid out hardware.
% It is indeed possible, with slight changes to traditional antenna array architectures, to virtualize the concept of a RF chain.
% This virtualization leads to previously unforeseeable 



% Wherever possible, if we can replace traditional hardware 

% One naive solution to this is to possibly just turn off certain RF chains depending on the channel and number of users. 
% However, this also reduces the degrees of freedom captured as turning off an RF chain would mean dropping samples from the antenna it is connected to.
% Essentially, turning off the RF chains brings us back to the tried and failed mu-MIMO scenario which also captured limited degrees of freedom.
% Thus, a flexible way of tapping into the antenna's degrees of freedom without necessitating these multiple physically laid out RF chains is the need of the hour.

==> intros/intro_mcom_v0.tex <==
\section{Introduction}

Over the past decade, wireless networks have matured to provide reliable, ubiquitous and robust connectivity, and enabled numerous `killer' applications like video streaming/calling, instant messaging\cite{}.
However, this has come at a cost of humongous carbon footprint from the telecommunications sector, with the net carbon emissions rivalling that of aviation sector\cite{}.
At the same time, the predicted demand of wireless networks is expected to exponentiate even upwards over the next decade \cite{}.
This could be disastrous to the environment and worsen the already bad carbon footprint. 
Hence various case studies have shown that it is of utmost importance that wireless networks need to `\textbf{grow sustainably}' over the next decade\cite{}. Further, consumer sentiment also highlight this, with more than 70\% consumers willing to switch to a greener alternative\cite{}, as well as governments around the world pushing for greener industries \cite{}. 
Hence one `killer' selling point for next generation mobile networks could be how `green' they can grow while connecting more users, to cater towards both consumer, as well as sustainable incentive pushes. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{new_figs/intro_fig.pdf}
    \caption{\textcolor{red}{Better figure needed but this is general idea}\name maximises both SE and EE}
    \label{fig:intro_fig_new}
\end{figure}

Thus, it is imperative that we no longer just consider increasing net throughput as users increase as a golden metric for wireless network design, but need to consider the efficiency in generating the said throughput. 
That is, to grow sustainably, we need to advocate judicious use of the two key resources available in a wireless network, free spectrum and power at disposal.
Packing more bits per unit spectrum would support these more users by not exacerbating spectrum demands, whereas communicating more bits per joule energy spent would make the said communications greener.
Hence, the mobile network which would jointly optimize for both spectrum efficiency (SE) as well as energy efficiency (EE), while adding new users, will truly achieve the killer `green' mobile network selling point.

However, existing solutions for adding more users to mobile networks largely address these efficiencies in isolation. 
The most naive approach to add more users is to add more spectrum bands such that the users communicate at different frequencies in an interference-free manner.
This is also referred to as frequency multiplexing, implemented in today's networks via OFDMA.
% In comparison, OFDMA implements frequency multiplexing, which puts users in different spectrum bands. 
% Since the users have different frequency, there is no need to create a spatial beam and OFDMA can use a single antenna and hence a single RF chain. 
OFDMA requires sampling the aggregate spectrum, and hence the power consumption is proportional to the net sampling bandwidth, which in turn is user-proportionate.
Say if number of users are $N$ each having bandwidth $B$, OFDMA transmits/receives the aggregate RF bandwidth $NB$ to communicate the data to/from $N$ users. 
via an antenna
That is, 
In OFDMA, the single RF chain samples the aggregate bandwidth occupied by the number of users, and hence the single RF chain's power is user-proportionate.


but sacrifices SE by putting multiple users in different frequency band\cite{}, so the base station does not need to handle the interference.
As a consequence, OFDMA just needs a single antenna, hence a single RF chain, which needs to sample the net spectrum occupied by all the users.
For this, OFDMA would have sampling bandwidth proportionate to number of users, thus the power consumption is user-proportionate, making it achieve EE.
Multiple existing works have pointed to this SE-EE tradeoff\cite{}, and current research consensus is that the tradeoff can not be broken but needs to be addressed by careful design of networks that they operate on a compromised `green' point of operation.


MIMO approaches use multiple antennas to address SE by performing spatial multiplexing. 
Spatial multiplexing allows users to share the spectrum resources, since they are being served by distinct beams created via the multi-antenna array.
However, this requires specialized circuits , referred to as RF chains, to transmit/receive signals per-antenna.
Thus, the power consumption grows proportional to number of RF chains, and hence number of antennas, since each antenna needs its own RF chain. 
In practical implementations, like Massive MIMO, we require more antennas than number of users to create the required distinct beams\cite{}.
Hence, the power consumption is not user-proportionate, and massive MIMO sacrifices EE by setting up many more RF chains to serve a smaller number of users.

% This allows users to share the same spectrum, as they are separated in the spatial domain by the means of beamforming.
% This is achieved by creation of spatial beams towards each user by a concept also referred to as digital beamforming (DBF).
% However, this requires each antenna to have separate RF interfacing hardware\cite{} which interfaces the antenna with the baseband signal processing unit, also referred to as a `RF chain'. 
% which connect the baseband digital processor to the antenna and consists of various circuits like ADC/DAC, down/up conversion mixers, filters, LNA/PA.



Taking a step towards breaking this SE-EE tradeoff, in this paper we present \name, which for the first time, shows an architecture which can maximize both SE and EE. 
% The key insight here is to add low-power analog circuitry to each antenna such that 
The key insight which enables \name to do so, is that MIMO and OFDMA systems of today can be married together, by using configurable, low-power RF circuits per antenna, to get best of both worlds.
The idea is to have the multiple MIMO `configurable' antennas combinedly share the single user-proportionate sampling bandwidth RF chain of OFDMA. 
Each antenna in \name can be set to separate configurations to give unique identity to the antennas signal before they combine together and go through the RF chain.
By isolating the signals based on the unique identity, \name can isolate the per-antenna signals in the digital domain.
Hence, this approach basically creates a virtual signal path towards each separate antenna configuration in digital domain, and we dub this process as creation of `Virtual RF chains (VRF)'.
These VRFs also allow for grouping of multiple antennas by setting them to same configurations, so $N$ virtual RF chains can effectively share $M>N$ antennas among themselves.
This enables practical MIMO operation for $N$ interfering users, while harnessing advantages offered by $M>N$ antennas, and keeping power consumption to user-proportionate sampling level of single RF chain.
% Hence, the concrete approach behind \name is that, to serve $N$ users in a user-proportionate power manner via $M>N$ antennas, \name creates $N$ `virtual RF chains' from a single physical RF chain sampled at $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power efficiency of OFDMA.

% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.

% The basic idea is that we can use the increased sampling bandwidth of a single RF chain to carve out virtual signal paths to each antenna in the digital domain, in a process dubbed as creation of `virtual RF chains'.
% This way \name is able to harness MIMO operation by laying a single physical RF chain, and abstracting out multiple virtual RF chains as demand-fit.
% Further, this process is done in an optimal user-proportionate manner where \name can club together multiple antennas in a single virtual RF chain to harness the gains of many more antennas than number of users and show practical MIMO operation in realistic environments.
% This basically allows the single RF chain to get `virtualized' over the many antennas, in the sense that all antennas share the same RF chain but have a separate virtual digital path created , which allows for creation of virtual RF chains in the digital domain.
% Further, by 
% This is made possible by a combined analog-digital antenna combining approach which ensures that the required benefits of many more antennas than number of users get 
% Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

The first design consideration for \name is how to even realize this concept of a VRF? 
To motivate this, we first show how that the desired behaviour from the configurable RF circuit is to create a `frequency spreading' effect, so that the $B$ bandwidth user signals get spread into $NB$ total bandwidth.
However, a challenge here is that this spreading operation needs to be done with minimal power consumption, otherwise the net power requirements would end up being antenna proportionate as we need this circuit for each antenna.
Hence, \name inspires from backscatter communication's RF-switches that create frequency shifts with minimal <100uW power requirements \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, when toggled with certain frequency on-off clock.

% This rules out naive solutions like RF mixers which can create the intended frequency spreading effect, but at expense of insertion losses and non-negligible power consumption.
% Instead, \name uses RF switches, which also are capable of creating these frequency shifts when toggled with a certain frequency on-off clock.
% Further, this operation has minimal power requirements, and similar RF switches have been used for channel shifting purposes in backscatter systems with <10uW power requirements that can also be made batteryless \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}.
% The concrete idea here is that, to serve $N$ users in a user-proportionate power manner,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power efficiency of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
% It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
% We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

% Next, we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ different antenna groups so as to enable the creation of $N$ virtual RF chains. 
Thus, we can use RF switches to configure antennas on-off strategically to create VRFs. However, how exactly should we configure these switches such that we can create $N$ VRFs for $N$ different antenna groups?
For this, we show how \name can create $N$ orthogonal on-off clocks having $B$ frequency, corresponding to user bandwidth and $1/N$ duty cycle each, but different initial phases.
The idea is that a particular group of antennas antennas can be configured with one of these $N$ orthogonal on-off clocks, and signals of these antennas would get combined in the analog domain and get downconverted+digitized. 
Then in digital domain the summed signals from these different antennas can be isolated from since these summed combined signals would have the unique clock marking them different from the other groups using the rest $N-1$ clocks.
The key insight which allows separating these $N$ clocks from each other is that when
these $N$ different $B$ frequency codes are sampled at $NB$ they show up at different sample indexes in time, and this allows \name to separate the VRFs set up by each of the $N$ unique on-off clocks.

Finally, the last piece in the puzzle is how to select these $N$ different antenna groupings from the available $M$ antennas. One key feature of \name's VRFs is that it allows a many to many connection with antennas. That is, it not only allows us to turn on multiple antennas per VRF, we can also have one antenna showing up in multiple VRFs. This is because the clocks are orthogonal in time, and to have one antenna show up in two virtual chains, we can simply add two orthogonal clocks corresponding to the two VRFs. This allows \name to implement a switching matrix $\mathbf{S}$ in analog domain, which maps the user channels across $M$ antennas into $N$ user-proportionate VRFs. We also show a heuristic method, labelled as BABF, which beamforms towards one-user per VRF in order to enable practical user-proportionate MIMO.


% Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
% Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
% That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

% So far we have discussed how \name gets one antenna stream per virtual RF chain.
% But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
% A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
% Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
% Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


% To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
% The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
% In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
% Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
% \name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{new_figs/BM_fig.pdf}
    \caption{How power consumption varies with number of users for freq. \& spatial multiplexing, with typical values of power consumption tabulated}
    \label{fig:bm_fig_new}
\end{figure*}

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be green and drastically cut down both on RF front end power as well as sampling+compute power.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $3\times$ less power requirements, achieving the same network capacity as compared to FDMA with $4\times$ lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.


% Hence, massive MIMO ends up being  by having antenna proportionate power, as OFDMA can achieve the same goal by being user-proportionate.
% But, this comes at a cost of multiplicative increase in spectrum with OFDMA, which makes OFDMA power-inefficient.



% 


% Mainly these efficiency metrics can be either the traditionally considered spectral efficiency (bps per hertz) to advocate judicious use of spectrum, or energy efficiency
% both energy efficiency (bps per watt) and spectrum efficiency (bps per hertz). That is, in the coming decade, it is imperative to maximize both, how many bits can you communicate per watt usage, and number of bits packed in unit spectrum (Fig.). 



==> intros/intro_mcom_v1.tex <==
\section{Introduction}

Over the past decade, wireless networks have matured to provide reliable, ubiquitous and robust connectivity, and enabled numerous `killer' applications like video streaming/calling, instant messaging\cite{}.
However, this has come at a cost of humongous carbon footprint from the telecommunications sector, with the net carbon emissions rivalling that of aviation sector\cite{}.
At the same time, the predicted demand of wireless networks is expected to exponentiate even upwards over the next decade \cite{}.
This could be disastrous to the environment and worsen the already bad carbon footprint. 
Hence various case studies have shown that it is of utmost importance that wireless networks need to `\textbf{grow sustainably}' over the next decade\cite{}. Further, consumer sentiment also highlight this, with more than 70\% consumers willing to switch to a greener alternative\cite{}, as well as governments around the world pushing for greener industries \cite{}. 
Hence one `killer' selling point for next generation mobile networks could be how `green' they can grow while connecting more users\todo{or more throughput}, to cater towards both consumer, as well as sustainable incentive pushes. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{new_figs/intro_fig_simple.pdf}
    \caption{\todo{Better OFDMA figure}\name maximises both SE and EE}
    \label{fig:intro_fig_new}
\end{figure}

% \begin{figure}[t]
%     % \begin{adjustwidth}{-15pt}{} 
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \setlength{\figureheight}{0.6\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     % \input{results/8ant_multipos}    
%     \input{results/compute_pow_spectrum}
%     % \caption{Power \& Spectrum Required}
%     \label{fig:intro_fig_new}
%     \end{subfigure}
%     % \end{adjustwidth}
%     \caption{How today's multi-user techniques stand}
% \end{figure}


Thus, it is imperative that we no longer just consider increasing net throughput as users increase as a golden metric for wireless network design, but need to consider the efficiency in generating the said throughput. 
That is, to grow sustainably, we need to advocate judicious use of the two key resources available in a wireless network, spectrum and power at disposal.
Packing more bits per unit spectrum would support these more users by not exacerbating spectrum demands, whereas communicating more bits per joule energy spent would make the said communications greener.
Hence, the wireless network that would jointly optimize for both spectrum efficiency (SE) as well as energy efficiency (EE), while adding new users or more throughput, will truly achieve the killer `green' mobile network selling point. Furthermore, if such networks are energy-proportional and flexible, by energy-proportional they can scale up the throughput with linear increase in energy consumption and by flexible they can scale up and down as load varies.

Existing solutions for adding more users or more throughput to mobile networks largely address these efficiencies in isolation. 
A straightforward approach to add more users or more throughput is to add more spectrum bands such that the users communicate at different frequencies in an interference-free manner.
This is also referred to as frequency multiplexing\todo{do you want to call it OFDMA, keep it simple -- furthermore it could be channel bonding}, i.e., each user is provided $B$ bandwidth, but they are each assigned separate non-overlapping spectrum, consuming a total of $NB$ spectrum. In this case it achieves energy efficiency; as scaling to $N$ users with $B$ bandwidth goes towards receiving/transmitting $NB$ bandwidth, via a single RX/TX chain connected to an antenna, achieve a sub-linear scaling as such. Said differently, to support $NB$, the energy is consumed by single RX/TX chain is fixed, and the base-band power consumption scales linearly by $N$ to support $NB$ bandwidth, thus since we invest $N\times$ joules to sample $NB$, we are energy-proportionate as extra energy spent gives us the data bits proportionally. 
However, such an approach requires extra-ordinary spectrum to scale up, as shown in Fig. \ref{fig:intro_fig_new}. 


Another popular approach to add more users or throughput is to use MIMO or even massive MIMO spatial multiplexing using multiple antennas.
Spatial multiplexing works by creating narrow independent beams towards each user, this way even if the users communicate in same frequency bands they do not interfere as they are served via distinct beams.
Hence, spatial multiplexing can serve $N$ users having bandwidth $B$ with the fixed spectrum-cost of bandwidth $B$, i.e., packing in $N$ times more bits in the same $B$ spectrum improving the spectral efficiency by $N\times$ compared to frequency multiplexing.
% Thus even though OFDMA achieves EE, it is far less SE compared to MIMO.
However, these spectral-efficiency improvements come at cost of reduced energy-efficiency in MIMO. 
In practical MIMO implementations, like Massive MIMO, we require many more antennas, $M$ than number of users, $N$ ($M>>N$) to create the required distinct beams\cite{}.
Each antenna has its own RF-chains and base-band which receives/transmits the $B$ bandwidth signals to achieve MIMO operation, and hence the power consumption to serve $N$ users grows proportional to $M$.
Thus, we spent $M\times$ joules just to get $NB$ data bits across. Therefore, the energy consumption is antenna-proportionate instead of user-proportionate, MIMO sacrifices energy-efficiency to pack more bits in the same spectrum band. 
% It is 
% It is because as number of users increase, the sampling bandwidth increases proportionately, and all this sampled bandwidth contains proportionately many bits. 
% So the EE stays optimal as users increase.

% % In comparison, OFDMA implements frequency multiplexing, which puts users in different spectrum bands. 
% % Since the users have different frequency, there is no need to create a spatial beam and OFDMA can use a single antenna and hence a single RF chain. 
% % OFDMA requires sampling the aggregate spectrum, and hence the power consumption is proportional to the net sampling bandwidth, which in turn is user-proportionate.
% Say if number of users are $N$ each having bandwidth $B$, OFDMA transmits/receives the aggregate RF bandwidth $NB$ to communicate the data to/from $N$ users. 
% The hardware implementation of OFDMA is hence straightforward, consists of basically a single TX/RX chain which connects the digital processor to the antenna and communicates the $NB$ signals.
% The power consumption is user proportionate, as users in network increase/decrease OFDMA can increase/decrease the bandwidth and hence not waste power.
% via an antenna
% That is, 
% In OFDMA, the single RF chain samples the aggregate bandwidth occupied by the number of users, and hence the single RF chain's power is user-proportionate.


% but sacrifices SE by putting multiple users in different frequency band\cite{}, so the base station does not need to handle the interference.
% As a consequence, OFDMA just needs a single antenna, hence a single RF chain, which needs to sample the net spectrum occupied by all the users.
% For this, OFDMA would have sampling bandwidth proportionate to number of users, thus the power consumption is user-proportionate, making it achieve EE.
% Multiple existing works have pointed to this SE-EE tradeoff\cite{}, and current research consensus is that the tradeoff can not be broken but needs to be addressed by careful design of networks that they operate on a compromised `green' point of operation.


% As a consequence of MIMO not being EE, it limits usecase 
% MIMO approaches use multiple antennas to address SE by performing spatial multiplexing. 
% Spatial multiplexing allows users to share the spectrum resources, since they are being served by distinct beams created via the multi-antenna array.
% However, this requires specialized circuits , referred to as RF chains, to transmit/receive signals per-antenna.
% Thus, the power consumption grows proportional to number of RF chains, and hence number of antennas, since each antenna needs its own RF chain. 

% Hence, the power consumption is not user-proportionate, and massive MIMO sacrifices EE by setting up many more RF chains to serve a smaller number of users.

% This allows users to share the same spectrum, as they are separated in the spatial domain by the means of beamforming.
% This is achieved by creation of spatial beams towards each user by a concept also referred to as digital beamforming (DBF).
% However, this requires each antenna to have separate RF interfacing hardware\cite{} which interfaces the antenna with the baseband signal processing unit, also referred to as a `RF chain'. 
% which connect the baseband digital processor to the antenna and consists of various circuits like ADC/DAC, down/up conversion mixers, filters, LNA/PA.


\textbf{Hence, in this paper we show how to achieve MIMO multiplexing differently from traditional approach, and make it achieve both energy-efficiency and spectral-efficiency.}
In order to do so, we design a new MIMO architecture, dubbed as \name, which keeps energy consumption to user-proportionate ($N\times$) levels, while interfacing the required $M>>N$ antennas for MIMO operation.
\name achieves this by connecting all the $M$ MIMO antennas to OFDMA hardware, consisting of just a single $NB$ sampling RX/TX chain of OFDMA.
This way, power consumption remains to OFDMA levels, while we can use the $M$ antennas to create the required narrow beams for spatial multiplexing.

Clearly, the first challenge here is that how \name obtain the digitized per-antenna signals needed for MIMO processing from the single RX/TX chain? 
Since all the antennas share the same RX/TX chain, the signals would get combined into a single added signal, losing the per-antenna signature.
The first key insight of \name here is that since we have $NB$ bandwidth at disposal, and the user signals are $B$ bandwidth, we have extra $N$ degrees of freedom.
However, we
% So, in order to isolate the per-antenna signals, we can use these $N$ degrees of freedom to treat $N$ antennas as $N$ users and 
To utilize this higher bandwidth and the degree of freedom, we can spread the antenna signals via a distinct analog spreading code for each antenna, so that before getting combined each antenna gets a $NB$ bandwidth signature, as shown by different color boxes in Fig. \ref{fig:intro_spread}.
% This analog spreading effect basically preserves the antenna's signature before they get combined into a single RF chain, get downconverted and digitized.
After obtaining the $NB$ digitizes samples, we can de-spread the codes to isolate the per-antenna signature, and hence isolate the $B$ bandwidth original signal of that antenna.
Since we have $N$ degrees of freedom, we can generate $N$ such distinct orthogonal codes to isolate $N$ antennas signals even when they share the same RF chain.
In a way, this analog spreading + digital de-spreading creates `$N$ virtual RF chains' across the $NB$ bandwidth of the physically laid RF chain.
Even though there did not exist a physical path to $N$ antennas, it gets created virtually post-digitization.
% This is visually illustrated in Fig. \ref{fig:intro_spread}.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{new_figs/intro_spread_despread.pdf}
    \caption{Working principle behind \name}
    \label{fig:intro_spread}
\end{figure*}
% The second challenge here is how can we take this $N$ virtual RF chain concept and apply to $M>N$ antennas, to truly enable spatial multiplexing?

However, we started with $M>N$ antennas, but we have only $N$ virtual RF chains instead of $M$ with user-proportionate spreading-de-spreading.
Hence, a second challenge here is how do we use this concept of $N$ virtual RF chains with $M>N$ antennas?
The key insight here is that since virtual RF chains are created by analog spreading-digital despreading, we can have antennas co-phased for one user to spread with the same code, so that they constructively add up in the virtual RF chain generated by that code.
This way, we can have one virtual RF chain using a group of antenna beamforming towards it.
Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
A natural question here would be if $M$ antennas are split up amongst $N$ RF chains?
We show that infact $2$ virtual RF chains can share the same antenna since the spreading codes are orthogonal, so we can add the spreading codes of the $2$ virtual RF chains for one antenna to make it appear in both the RF chains.
Hence, this allows a many-to-many connection between the $M$ antennas and $N$ virtual RF chains, and effectively allows all the $N$ virtual chains to use the full array for beamforming.
This captures the required goal of narrow beams by using $M>N$ antennas, while using $N$ virtual RF chains.
% can we share the $N$ virtual RF chains effectively across higher number of antennas to create the required narrow beams?

% The key insight here is that unlike a physical RF chain, which is created by laying the physical hardware to each antenna, virtual RF chains are an abstraction created by the spreading-despreading effect.
% So, in \name we can group many antennas by spreading them in a similar way, so the de-spreading operation gives a combined signal across all these antennas.
% Further, we show that since the spreading codes are orthogonal, a single antenna can be spread across two virtual RF chains as well.
% So, \name allows a many to many connection between $M$ antennas and $N$ virtual RF chains.
% This allows \name to group antennas strategically such that they perform approximate analog beamforming towards one user per virtual RF chain.
% The residual interference left is then cancelled digitally by inverting the channels and doing zero-forcing post-coding  (shown after de-spreading block, Fig. \ref{fig:intro_spread}).


By addressing the two challenges listed above, \name truly enables `user-proportionate' spatial multiplexing with $M$ antennas connected via the `analog-spreading unit' to OFDMA hardware of a single RF chain.
Hence, the net power consumption of \name would be that of OFDMA + total power across the required analog spreading.
So, the last challenge in designing \name is how can the analog spreading be done at such minimal power requirements such that the power consumption dominated by OFDMA RF chain's power consumption.
To achieve this, we show that the required analog spreading operation can be achieved via simple RF switches toggling at strategically chosen $N$ distinct on-off codes, which give the required unique spreading for $N$ virtual RF chains.
RF switches enable this at $<1$mW power draw, which is minimal compared to $100$'s of mW power of OFDMA's RF chain.
This is not surprising, since in the field of backscatter communications, the same RF switches perform the frequency shifting operations at $\mu$W levels.


Thus, to summarize, \name designs a new MIMO architecture which connects $M$ antennas to single RF chain of OFDMA via $M$ RF switches. \name basically creates $N$ virtual RF chain via analog spreading effect of RF switches, and de-spread digitally in the $NB$ bandwidth OFDMA RF chain. 
\name also is a `flexible' architecture, it can create $N$ virtual RF chains on demand, so if there are lesser/more users it can adaptively reduce/increase the number of virtual chains.
At the same time, if there is a single MIMO capable user, \name can be used to serve multiple streams to one user instead of resticting to multi-user only scenarios.
By being almost same power level as OFDMA, as well as using multiple antennas to create mMIMO like narrow beams, \name achieves both EE and SE. 
We implement \name prototype with $M=8$ antennas to flexibly serve $2,3,4$ users. We test \name over multiple user positions in a conference room setting, as well as traditional MIMO and OFDMA baselines. Our key results include similar performance metrics with MIMO with $3\times$ less power requirements, achieving the same network capacity as compared to OFDMA with $4\times$ lesser spectrum requirements, which experimentally confirm the SE and EE claims.
We also show capability to handle multiple streams to increase throughput of single user by $3$ times.
Finally, we end with a case study on how \name can make various classes of base stations more energy efficient and cut down on power bills.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{new_figs/BM_fig.pdf}
%     \caption{How power consumption varies with number of users for freq. \& spatial multiplexing, with typical values of power consumption tabulated}
%     \label{fig:bm_fig_new}
% \end{figure*}

% and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.



% The main reason for MIMO not achieving EE is the requirement of separate RF chains for each antenna, and this issue 
% Taking a step towards breaking this SE-EE tradeoff, in this paper we present \name, which for the first time, shows an architecture which can maximize both SE and EE. 
% The key insight here is to add low-power analog circuitry to each antenna such that 
% The key insight which enables \name to do so, is that MIMO and OFDMA systems of today can be married together, by using configurable, low-power RF circuits per antenna, to get best of both worlds.
% The idea is to have the multiple MIMO `configurable' antennas combinedly share the single user-proportionate sampling bandwidth RF chain of OFDMA. 
% Each antenna in \name can be set to separate configurations to give unique identity to the antennas signal before they combine together and go through the RF chain.
% By isolating the signals based on the unique identity, \name can isolate the per-antenna signals in the digital domain.
% Hence, this approach basically creates a virtual signal path towards each separate antenna configuration in digital domain, and we dub this process as creation of `Virtual RF chains (VRF)'.
% These VRFs also allow for grouping of multiple antennas by setting them to same configurations, so $N$ virtual RF chains can effectively share $M>N$ antennas among themselves.
% This enables practical MIMO operation for $N$ interfering users, while harnessing advantages offered by $M>N$ antennas, and keeping power consumption to user-proportionate sampling level of single RF chain.
% % Hence, the concrete approach behind \name is that, to serve $N$ users in a user-proportionate power manner via $M>N$ antennas, \name creates $N$ `virtual RF chains' from a single physical RF chain sampled at $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power efficiency of OFDMA.

% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.

% The basic idea is that we can use the increased sampling bandwidth of a single RF chain to carve out virtual signal paths to each antenna in the digital domain, in a process dubbed as creation of `virtual RF chains'.
% This way \name is able to harness MIMO operation by laying a single physical RF chain, and abstracting out multiple virtual RF chains as demand-fit.
% Further, this process is done in an optimal user-proportionate manner where \name can club together multiple antennas in a single virtual RF chain to harness the gains of many more antennas than number of users and show practical MIMO operation in realistic environments.
% This basically allows the single RF chain to get `virtualized' over the many antennas, in the sense that all antennas share the same RF chain but have a separate virtual digital path created , which allows for creation of virtual RF chains in the digital domain.
% Further, by 
% This is made possible by a combined analog-digital antenna combining approach which ensures that the required benefits of many more antennas than number of users get 
% Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

% The first design consideration for \name is how to even realize this concept of a VRF? 
% To motivate this, we first show how that the desired behaviour from the configurable RF circuit is to create a `frequency spreading' effect, so that the $B$ bandwidth user signals get spread into $NB$ total bandwidth.
% However, a challenge here is that this spreading operation needs to be done with minimal power consumption, otherwise the net power requirements would end up being antenna proportionate as we need this circuit for each antenna.
% Hence, \name inspirchallengees from backscatter communication's RF-switches that create frequency shifts with minimal <100uW power requirements \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, when toggled with certain frequency on-off clock.

% This rules out naive solutions like RF mixers which can create the intended frequency spreading effect, but at expense of insertion losses and non-negligible power consumption.
% Instead, \name uses RF switches, which also are capable of creating these frequency shifts when toggled with a certain frequency on-off clock.
% Further, this operation has minimal power requirements, and similar RF switches have been used for channel shifting purposes in backscatter systems with <10uW power requirements that can also be made batteryless \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}.
% The concrete idea here is that, to serve $N$ users in a user-proportionate power manner,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power efficiency of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
% It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
% We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

% Next, we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ different antenna groups so as to enable the creation of $N$ virtual RF chains. 
% Thus, we can use RF switches to configure antennas on-off strategically to create VRFs. However, how exactly should we configure these switches such that we can create $N$ VRFs for $N$ different antenna groups?
% For this, we show how \name can create $N$ orthogonal on-off clocks having $B$ frequency, corresponding to user bandwidth and $1/N$ duty cycle each, but different initial phases.
% The idea is that a particular group of antennas antennas can be configured with one of these $N$ orthogonal on-off clocks, and signals of these antennas would get combined in the analog domain and get downconverted+digitized. 
% Then in digital domain the summed signals from these different antennas can be isolated from since these summed combined signals would have the unique clock marking them different from the other groups using the rest $N-1$ clocks.
% The key insight which allows separating these $N$ clocks from each other is that when
% these $N$ different $B$ frequency codes are sampled at $NB$ they show up at different sample indexes in time, and this allows \name to separate the VRFs set up by each of the $N$ unique on-off clocks.

% Finally, the last piece in the puzzle is how to select these $N$ different antenna groupings from the available $M$ antennas. One key feature of \name's VRFs is that it allows a many to many connection with antennas. That is, it not only allows us to turn on multiple antennas per VRF, we can also have one antenna showing up in multiple VRFs. This is because the clocks are orthogonal in time, and to have one antenna show up in two virtual chains, we can simply add two orthogonal clocks corresponding to the two VRFs. This allows \name to implement a switching matrix $\mathbf{S}$ in analog domain, which maps the user channels across $M$ antennas into $N$ user-proportionate VRFs. We also show a heuristic method, labelled as BABF, which beamforms towards one-user per VRF in order to enable practical user-proportionate MIMO.


% Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
% Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
% That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

% So far we have discussed how \name gets one antenna stream per virtual RF chain.
% But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
% A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
% Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
% Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


% To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
% The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
% In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
% Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
% \name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.




% Hence, massive MIMO ends up being  by having antenna proportionate power, as OFDMA can achieve the same goal by being user-proportionate.
% But, this comes at a cost of multiplicative increase in spectrum with OFDMA, which makes OFDMA power-inefficient.



% 


% Mainly these efficiency metrics can be either the traditionally considered spectral efficiency (bps per hertz) to advocate judicious use of spectrum, or energy efficiency
% both energy efficiency (bps per watt) and spectrum efficiency (bps per hertz). That is, in the coming decade, it is imperative to maximize both, how many bits can you communicate per watt usage, and number of bits packed in unit spectrum (Fig.). 



==> intros/intro_mcom_v2.tex <==
\section{Introduction}

Over the past decade, wireless networks have matured to provide reliable, ubiquitous and robust connectivity, and enabled numerous applications like video streaming/calling, instant messaging\cite{}.
However, this has come at a cost of humongous carbon footprint from the telecommunications sector, with the net carbon emissions rivalling that of aviation sector\cite{}.
At the same time, the predicted demand of wireless networks is expected to exponentiate even upwards over the next decade \cite{}.
Hence various case studies have highlighted the need for wireless networks to `\textbf{grow sustainably}' over the next decade\cite{}. Further, consumer sentiment also highlight this, with more than 70\% consumers willing to switch to a greener alternative\cite{}, as well as governments around the world pushing for greener industries \cite{}. Therefore one key selling point for next generation mobile networks would be how `green' they can grow while connecting more users and/or support higher throughput, 
to cater towards both consumer, as well as sustainable incentive pushes. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{new_figs/intro_arch.pdf}
    \caption{\name solves for energy efficiency by creating a new massive MIMO architecture with flexible user-proportionate power consumption}
    \label{fig:intro_fig_new}
\end{figure}

% \begin{figure}[t]
%     % \begin{adjustwidth}{-15pt}{} 
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \setlength{\figureheight}{0.6\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     % \input{results/8ant_multipos}    
%     \input{results/compute_pow_spectrum}
%     % \caption{Power \& Spectrum Required}
%     \label{fig:intro_fig_new}
%     \end{subfigure}
%     % \end{adjustwidth}
%     \caption{How today's multi-user techniques stand}
% \end{figure}

Thus, it is imperative that we no longer just consider increasing net throughput as users increase as a golden metric for wireless networks, but also the efficiency in generating this said throughput. 
That is, to grow sustainably, we need to advocate judicious use of the two key resources available in a wireless network, licensed spectrum and power at disposal.
Packing more bits per unit spectrum would support the growing data-rate by not exacerbating spectrum demand, thereby making systems spectrally efficient (SE).
However, in packing these more number of bits, energy has to be consumed in a proportionate manner, for making the networks energy efficient (EE).
In other words to achieve EE, it is imperative that energy consumption scales $N\times$ in a user proportionate manner to communicate $N$ streams of data towards $N$ users, whereas all $N$ users share spectrum judiciously to advocate for SE.
Further this EE and SE optimization should be flexible, as $N$ varies the energy proportionality should scale accordingly and spectrum usage should remain optimal.
% whereas communicating number of bits in a proportionate energy manner
% % should linear or sub-linearly increase the 
% per joule energy spent would make the networks greener. 
% Therefore, the expectation for future networks is to be
%the next generation wireless network that would jointly optimize for both spectrum efficiency (SE) as well as energy efficiency (EE), while adding new users or more throughput, will truly achieve the killer `green' mobile network selling point. 
%Furthermore, if such networks are 
% energy-proportional and flexible, by energy-proportional they can scale up the throughput with linear or sub-linear increase in energy consumption and by flexible they can scale up and down the energy consumption as load varies, besides optimizing for both spectrum efficiency (SE) as well as energy efficiency (EE).

Existing solutions for adding more users or more throughput to mobile networks largely address spectrum and energy efficiencies in isolation, and a rigid unflexible manner for fixed user numbers $N$. 
A energy-proportionate approach to add more users or more throughput is to add more spectrum bands such that the users communicate at different frequencies in an interference-free manner.
This is also referred to as frequency multiplexing, i.e., each user is provided $B$ bandwidth, and as a net $N$ users
% but they are each assigned separate non-overlapping spectrum, 
consume a total of $NB$ spectrum. 
% In this case it achieves throughput scaling which is energy proportional, 
% % as scaling to $N$ users with $B$ bandwidth 
% as the energy spent goes towards receiving/transmitting this $NB$ bandwidth
% , generally achieves linear scaling to first order. 
To support this $NB$ spectrum, the
% the energy consumed by front-end RX/TX chain is fixed at base-station and user, and the base-band 
power consumption scales linearly by $N$, and hence achieve EE.
This is because $N\times$ joules are used to receive/transmit the $NB$ signals, and this proportionate extra energy spent gives increased data bits proportionally\footnote{Contrary to traditional belief the ADC/DAC power consumption scale up linearly to a threshold point, beyond that they scale exponentially\todo{agrim: fix}}. 
However, such an approach 
% requires extra-ordinary spectrum to scale up, 
requires new spectrum band for each new user, which is an expensive and cumbersome process, 
but it achieves user/throughput proportionate energy scaling.
It also achieves flexibility since if number of user drops to $N' < N$, the transceiver could just sample $N'B$ bandwidth and therefore, would scale down the energy consumption as well. 
Hence the net sampling bandwidth of frequency multiplexing offers a simple design knob which can be adjusted in accordance to user load.

% Thus this sampling bandwidth can be abstracted to software layers and frequency multiplexing can be `vi

% In recent times, 
% another popular approach to add more users or throughput
An alternate to frequency multiplexing is massive MIMO (mMIMO), which creates spatial multiplexing.
% by many multiple antennas and used by both WiFi and 5G.
mMIMO creates $N$ distinct spatial beams via the massive number of antennas, to serve $N$ users sharing the same spectrum but different beams.
Thus, mMIMO has a spectrum-cost of fixed $B$ bandwidth, i.e., packing in $N$ times more bits via $N$ distinct spatial beams in the same $B$ band, improving SE by $N\times$ compared to frequency multiplexing.
This is achieved by digitally interfacing the $M>>N$ number of antennas, which creates the $N$ spatial beams in digital domain (mMIMO processing). 
This per-antenna digital interfacing requires each antenna to have its own RF interfacing hardware (for up/downcomversion, amplification) referred to as a RF chain, followed by the base-band processing chain which receives/transmits the $B$ bandwidth signals for all $M$ antennas, and performs the said mMIMO processing. 
Hence the energy consumption to serve $N$ users grows proportional to $M$.
% For mMIMO processing, the $M$ antenna signals are combined appropriately to isolate the $N$ user signals from the interfered signals mix at each antenna.
Thus, we spent $M\times$ joules just to get $NB$ data bits across. 
Therefore, the energy consumption is antenna-proportionate instead of user-proportionate, thus mMIMO sacrifices EE to pack more bits in the same spectrum band and achieve SE. 
Further, mMIMO architectures can not turn off energy proportionately if the number of users drop. 
% It is because the $M$ antennas and their RF chains have been laid physically and typical mMIMO implementations only backhaul the $N$ per-user streams with mMIMO processing implemented on the RF chips\cite{}.
At best mMIMO can turn off certain number of RF chains and hence drop some antennas, which would lead to performance degradation and thus this antenna selection process is not trivial \cite{}.
Thus, mMIMO does not posses a trivial design knob which can be changed to make it adapt to differing user-loads without dropping performance, hence lacks flexibility.
% , unlike the simple sampling bandwidth knob in frequency multiplexing.
% This is because the architecture mMIMO can not be virtualized, because of the complexity. 


% This is because it is not trivial to turn since the mMIMO backhauls only the per-user $N$ streams.
% the signals (massive-MIMO processing) from these many antennas  
% appropriately to 
% , this way all the users communicate in same frequency bands but the massive-MIMO processing creates interference-free signals per user. 

% Thus even though OFDMA achieves EE, it is far less SE compared to MIMO.
% However, these spectral-efficiency improvements come at cost of exponential energy-usage in massive-MIMO. 
% In massive-MIMO implementations, we require many more antennas, $M$ than number of users, $N$ ($M>>N$) to enable interference free signals per user\cite{}. 



% It is 
% It is because as number of users increase, the sampling bandwidth increases proportionately, and all this sampled bandwidth contains proportionately many bits. 
% So the EE stays optimal as users increase.

% % In comparison, OFDMA implements frequency multiplexing, which puts users in different spectrum bands. 
% % Since the users have different frequency, there is no need to create a spatial beam and OFDMA can use a single antenna and hence a single RF chain. 
% % OFDMA requires sampling the aggregate spectrum, and hence the power consumption is proportional to the net sampling bandwidth, which in turn is user-proportionate.
% Say if number of users are $N$ each having bandwidth $B$, OFDMA transmits/receives the aggregate RF bandwidth $NB$ to communicate the data to/from $N$ users. 
% The hardware implementation of OFDMA is hence straightforward, consists of basically a single TX/RX chain which connects the digital processor to the antenna and communicates the $NB$ signals.
% The power consumption is user proportionate, as users in network increase/decrease OFDMA can increase/decrease the bandwidth and hence not waste power.
% via an antenna
% That is, 
% In OFDMA, the single RF chain samples the aggregate bandwidth occupied by the number of users, and hence the single RF chain's power is user-proportionate.


% but sacrifices SE by putting multiple users in different frequency band\cite{}, so the base station does not need to handle the interference.
% As a consequence, OFDMA just needs a single antenna, hence a single RF chain, which needs to sample the net spectrum occupied by all the users.
% For this, OFDMA would have sampling bandwidth proportionate to number of users, thus the power consumption is user-proportionate, making it achieve EE.
% Multiple existing works have pointed to this SE-EE tradeoff\cite{}, and current research consensus is that the tradeoff can not be broken but needs to be addressed by careful design of networks that they operate on a compromised `green' point of operation.


% As a consequence of MIMO not being EE, it limits usecase 
% MIMO approaches use multiple antennas to address SE by performing spatial multiplexing. 
% Spatial multiplexing allows users to share the spectrum resources, since they are being served by distinct beams created via the multi-antenna array.
% However, this requires specialized circuits , referred to as RF chains, to transmit/receive signals per-antenna.
% Thus, the power consumption grows proportional to number of RF chains, and hence number of antennas, since each antenna needs its own RF chain. 

% Hence, the power consumption is not user-proportionate, and massive MIMO sacrifices EE by setting up many more RF chains to serve a smaller number of users.

% This allows users to share the same spectrum, as they are separated in the spatial domain by the means of beamforming.
% This is achieved by creation of spatial beams towards each user by a concept also referred to as digital beamforming (DBF).
% However, this requires each antenna to have separate RF interfacing hardware\cite{} which interfaces the antenna with the baseband signal processing unit, also referred to as a `RF chain'. 
% which connect the baseband digital processor to the antenna and consists of various circuits like ADC/DAC, down/up conversion mixers, filters, LNA/PA.


\textbf{Hence, in this paper we break the antenna-proportionate energy consumption required to achieve mMIMO multiplexing to user-proportionate energy consumption, while continuing to use all antennas for massive-MIMO operation, and achieving flexibility (dropping energy consumption as users drop) and spectral efficiency (using only bandwidth B).}
To this end, we present the design and implementation of a new massive-MIMO architecture, dubbed as \name.
% which keeps energy consumption to user-proportionate ($N\times$) levels, while interfacing the required $M>>N$ antennas for mMIMO operation.
\name connects each of the $M$ massive-MIMO antennas to an ultra-low power per-antenna configurable analog-network. 
Then \name combines signals from all the antennas configured uniquely, ensuring that the entire antenna array gain is available while only consuming a small amount of energy. 
The combined signal is passed through a single down-conversion chain and user-proportionate sampling rate , $NB$ digitization.
% thus consuming energy proportionate to the number of users supported. 
This digitized signal is passed through a digital computation network which isolates the per-antenna configurations to allow for massive-MIMO processing. 
The reverse operation can be conducted for transmission as well, to achieve user-proportionate energy consumption. 
Furthermore, \name energy consumption can be scaled flexibly via sampling bandwidth design knob, akin to frequency multiplexing.
That is, if the number of users drop to $N'$ users, the combined signal across the $M$ antennas is digitized at the $N'B$ sampling rate. 
% Thus \name offers the simple sampling bandwidth design knob for flexibility, akin to frequency multiplexing solution.

To achieve \name architecture, the first challenge is that how can \name create this ultra-low powered analog network, which allows \name to add more antennas easily without requiring complicated interfacing blocks.
\name's analog network simply combines output of all the $M$ antennas to a single downconversion chain via $M$ RF switches (shown in Fig. \ref{fig:intro_simple}).
This approach does not need per-antenna amplifiers, since RF switches have minimal ($<1$ dB) insertion losses, hence are energy efficient.
Further, they can be used to give `on-off' configurability to each antenna, hence providing it a distinct `on-off' signature.
This signature can then be used to isolate the per-antenna signal after the switched-signals across all the antennas get combined, downconverted and digitized by the single RF chain shared by all the antennas. 
% We build this analog network via RF switches connected to each antenna, which are energy efficient as they have extremely low insertion losses ($<1$ dB) an

% how do we design analog-pre-processing network such that each antenna signal identity is managed? 
Hence, the second challenge in \name architecture is how to strategically turn antennas `on-off' such that it enables isolation of per-antenna signals for mMIMO processing?
The first key insight of \name here is that since we have $NB$ bandwidth at disposal, and the user signals are $B$ bandwidth, we can use the wider bandwidth to fit $N$ antenna signals.
To use this $N\times$ higher bandwidth, we can spread the antenna signals via distinct $B$ frequency `on-off' codes which create signal harmonics and spread the $B$ bandwidth signal across $NB$ bandwidth.
We show how $N$ orthogonal $B$ frequency codes can be designed which spread the signals in an efficient manner across the $NB$ bandwidth and prevents signal leakage and distortions.
% However, we
% So, in order to isolate the per-antenna signals, we can use these $N$ degrees of freedom to treat $N$ antennas as $N$ users and 
% Since all the antennas share the same RX/TX chain, the signals would get combined into a single added signal, losing the per-antenna signature.
% analog spreading `on-off' codes for each antenna, so that before getting combined each antenna gets a unique $NB$ bandwidth signature.
% , as shown by different color boxes in Fig. \ref{fig:intro_spread}.

% By giving each antenna a $NB$ bandwidth signature, we preserve the per-antenna signatures even when they share a single downconversion chain.
% It is because we have $N$ different orthogonal methods to spread $B$ bandwidth signals into $NB$ bandwidth, and these orthogonal spreading methods can be then inverted to get back the per-antenna signals.

% allows for isolation of $N$
% This analog spreading effect basically preserves the antenna's signature before they get combined into a single RF chain, get downconverted and digitized.
% After obtaining the $NB$ digitizes samples, we can de-spread the codes to isolate the per-antenna signature, and hence isolate the $B$ bandwidth original signal of that antenna.
% Since we have $N$ degrees of freedom, we can generate $N$ such distinct orthogonal codes to isolate $N$ antennas signals even when they share the same RF chain.
Te third challenge is how \name then inverts this analog spreading effect of $N$ orthogonal codes to get back per antenna $B$ bandwidth-signals signals?
We show that these efficient $N$ spreading `on-off' codes are in-fact orthogonal in time, and can be inverted by isolating the different time samples occupied by each code.
This is done in the digital domain by simply splicing the digitized samples to ensure the de-spreading of codes.
In a way, this analog spreading + digital de-spreading via configurable RF switches creates `$N$ virtual RF chains' across the $NB$ bandwidth of the physically laid RF chain.
That is, even though there did not exist a physical path to $N$ antennas, it gets created virtually post-digitization.
Note that, similar to freq. multiplexing, we can use design knob of variable sampling bandwidth to vary the number of virtual chains as number of users $N$ varies.
% This is visually illustrated in Fig. \ref{fig:intro_spread}.

% The second challenge here is how can we take this $N$ virtual RF chain concept and apply to $M>N$ antennas, to truly enable spatial multiplexing?

However, we started with $M>N$ antennas, but we have only $N$ virtual RF chains from the spreading-de-spreading in $NB$ bandwidth.
Hence, the final challenge is how can \name use the entire array of $M$ antennas over these $N$ created virtual RF chains?
The two key insights here are that virtual RF chains allow for both, multiple antennas to be connected to a single virtual RF chain, as well as a single antenna connected to multiple RF chain.
This is made possible by the orthogonality of the codes, in the way that we can add to codes together for an antenna so that it shows up in both the spliced samples of virtual RF chain created by both these codes.
Further, giving same spreading code to multiple antennas allows them to be connected together in the same virtual chain.
% The basic principle why this works is that RF chains are created by the analog spreading + digital de-spreading effect which can be abstracted and applied across multiple antennas to enable a many to many connection between antennas and virtual RF chains, making the entire $M$ antenna array available to the $N$ virtual RF chains.
This way, we can have one virtual RF chain using a group of antennas which are co-phased for a user, and grouping them would in a way perform beamforming towards a particular user.
This allows \name to create narrower beams by using more number of $M$ antennas, than $N$ virtual chains, with the many-to-many connection allowing all antennas to be shared across all virtual chains.
Hence, \name achieves mMIMO like performance at user-proportionate power for $N$ virtual RF chains without being antenna-proportionate as mMIMO.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% This is because virtual RF chains are created by analog spreading via $N$ time-orthogonal codes, so to make two antennas appear in same virtual chain we can add the spreading codes for the particular antenna. 
% Hence, it would shows up in time-spliced samples post-digitization across both the virtual chains.
% Having multiple antennas for one virtual RF chain is straightforward, and can be done by supplying the particular spreading code to each antenna
% The key insight here is that since virtual RF chains are created by analog spreading-digital despreading, we can have antennas co-phased for one user to spread with the same code, so that they constructively add up in the virtual RF chain generated by that code.
% This way, we can have one virtual RF chain using a group of antenna beamforming towards it.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% A natural question here would be if $M$ antennas are split up amongst $N$ RF chains?
% We show that infact $2$ virtual RF chains can share the same antenna since the spreading codes are orthogonal, so we can add the spreading codes of the $2$ virtual RF chains for one antenna to make it appear in both the RF chains.
% Hence, this allows a many-to-many connection between the $M$ antennas and $N$ virtual RF chains, and effectively allows all the $N$ virtual chains to use the full array for beamforming.
% This captures the required goal of narrow beams by using $M>N$ antennas, while using $N$ virtual RF chains.
% can we share the $N$ virtual RF chains effectively across higher number of antennas to create the required narrow beams?

% The key insight here is that unlike a physical RF chain, which is created by laying the physical hardware to each antenna, virtual RF chains are an abstraction created by the spreading-despreading effect.
% So, in \name we can group many antennas by spreading them in a similar way, so the de-spreading operation gives a combined signal across all these antennas.
% Further, we show that since the spreading codes are orthogonal, a single antenna can be spread across two virtual RF chains as well.
% So, \name allows a many to many connection between $M$ antennas and $N$ virtual RF chains.
% This allows \name to group antennas strategically such that they perform approximate analog beamforming towards one user per virtual RF chain.
% The residual interference left is then cancelled digitally by inverting the channels and doing zero-forcing post-coding  (shown after de-spreading block, Fig. \ref{fig:intro_spread}).

% By addressing the challenges listed above, \name truly enables `user-proportionate' spatial multiplexing with $M$ antennas connected via the analog spreading network and a single $NB$ bandwidth RF chain.
% % Hence, the net power consumption of \name would be that of OFDMA + total power across the required analog spreading.
% % So, the last challenge in designing \name is how can the
% To design the analog network with ultra-low power consumption,we show that the required analog spreading operation can be achieved via simple RF switches toggling at strategically chosen $N$ distinct on-off codes, which give the required unique spreading for $N$ virtual RF chains.
% RF switches enable this at $<1$mW power draw, which is minimal compared to $100$'s of mW power draw of RF chains.
% This is not surprising, since in the field of backscatter communications, the same RF switches perform the frequency shifting operations at $\mu$W levels.


% Thus, to summarize, \name designs a new MIMO architecture which connects $M$ antennas to single RF chain of OFDMA via $M$ RF switches. \name basically creates $N$ virtual RF chain via analog spreading effect of RF switches, and de-spread digitally in the $NB$ bandwidth OFDMA RF chain. 
% \name also is a `flexible' architecture, it can create $N$ virtual RF chains on demand, so if there are lesser/more users it can adaptively reduce/increase the number of virtual chains.
% By being almost same power level as OFDMA, as well as using multiple antennas to create mMIMO like narrow beams, \name achieves both EE and SE. 
\todo{Improve last para}
We implement \name prototype with $M=8$ antennas to flexibly serve $2,3,4$ users. We test \name over multiple user positions in a conference room setting, as well as traditional MIMO and OFDMA baselines. Our key results include similar performance metrics with MIMO with $3\times$ less power requirements, achieving the same network capacity as compared to OFDMA with $4\times$ lesser spectrum requirements, which experimentally confirm the SE and EE claims.
At the same time, if there is a single MIMO capable user, \name can be used to serve multiple streams, and we show this by increasing throughput of single user by $3$ times.
Finally, we end with a case study on how \name can make various classes of base stations more energy efficient and cut down on power bills.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{new_figs/BM_fig.pdf}
%     \caption{How power consumption varies with number of users for freq. \& spatial multiplexing, with typical values of power consumption tabulated}
%     \label{fig:bm_fig_new}
% \end{figure*}

% and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.



% The main reason for MIMO not achieving EE is the requirement of separate RF chains for each antenna, and this issue 
% Taking a step towards breaking this SE-EE tradeoff, in this paper we present \name, which for the first time, shows an architecture which can maximize both SE and EE. 
% The key insight here is to add low-power analog circuitry to each antenna such that 
% The key insight which enables \name to do so, is that MIMO and OFDMA systems of today can be married together, by using configurable, low-power RF circuits per antenna, to get best of both worlds.
% The idea is to have the multiple MIMO `configurable' antennas combinedly share the single user-proportionate sampling bandwidth RF chain of OFDMA. 
% Each antenna in \name can be set to separate configurations to give unique identity to the antennas signal before they combine together and go through the RF chain.
% By isolating the signals based on the unique identity, \name can isolate the per-antenna signals in the digital domain.
% Hence, this approach basically creates a virtual signal path towards each separate antenna configuration in digital domain, and we dub this process as creation of `Virtual RF chains (VRF)'.
% These VRFs also allow for grouping of multiple antennas by setting them to same configurations, so $N$ virtual RF chains can effectively share $M>N$ antennas among themselves.
% This enables practical MIMO operation for $N$ interfering users, while harnessing advantages offered by $M>N$ antennas, and keeping power consumption to user-proportionate sampling level of single RF chain.
% % Hence, the concrete approach behind \name is that, to serve $N$ users in a user-proportionate power manner via $M>N$ antennas, \name creates $N$ `virtual RF chains' from a single physical RF chain sampled at $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power efficiency of OFDMA.

% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.

% The basic idea is that we can use the increased sampling bandwidth of a single RF chain to carve out virtual signal paths to each antenna in the digital domain, in a process dubbed as creation of `virtual RF chains'.
% This way \name is able to harness MIMO operation by laying a single physical RF chain, and abstracting out multiple virtual RF chains as demand-fit.
% Further, this process is done in an optimal user-proportionate manner where \name can club together multiple antennas in a single virtual RF chain to harness the gains of many more antennas than number of users and show practical MIMO operation in realistic environments.
% This basically allows the single RF chain to get `virtualized' over the many antennas, in the sense that all antennas share the same RF chain but have a separate virtual digital path created , which allows for creation of virtual RF chains in the digital domain.
% Further, by 
% This is made possible by a combined analog-digital antenna combining approach which ensures that the required benefits of many more antennas than number of users get 
% Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

% The first design consideration for \name is how to even realize this concept of a VRF? 
% To motivate this, we first show how that the desired behaviour from the configurable RF circuit is to create a `frequency spreading' effect, so that the $B$ bandwidth user signals get spread into $NB$ total bandwidth.
% However, a challenge here is that this spreading operation needs to be done with minimal power consumption, otherwise the net power requirements would end up being antenna proportionate as we need this circuit for each antenna.
% Hence, \name inspirchallengees from backscatter communication's RF-switches that create frequency shifts with minimal <100uW power requirements \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, when toggled with certain frequency on-off clock.

% This rules out naive solutions like RF mixers which can create the intended frequency spreading effect, but at expense of insertion losses and non-negligible power consumption.
% Instead, \name uses RF switches, which also are capable of creating these frequency shifts when toggled with a certain frequency on-off clock.
% Further, this operation has minimal power requirements, and similar RF switches have been used for channel shifting purposes in backscatter systems with <10uW power requirements that can also be made batteryless \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}.
% The concrete idea here is that, to serve $N$ users in a user-proportionate power manner,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power efficiency of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
% It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
% We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

% Next, we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ different antenna groups so as to enable the creation of $N$ virtual RF chains. 
% Thus, we can use RF switches to configure antennas on-off strategically to create VRFs. However, how exactly should we configure these switches such that we can create $N$ VRFs for $N$ different antenna groups?
% For this, we show how \name can create $N$ orthogonal on-off clocks having $B$ frequency, corresponding to user bandwidth and $1/N$ duty cycle each, but different initial phases.
% The idea is that a particular group of antennas antennas can be configured with one of these $N$ orthogonal on-off clocks, and signals of these antennas would get combined in the analog domain and get downconverted+digitized. 
% Then in digital domain the summed signals from these different antennas can be isolated from since these summed combined signals would have the unique clock marking them different from the other groups using the rest $N-1$ clocks.
% The key insight which allows separating these $N$ clocks from each other is that when
% these $N$ different $B$ frequency codes are sampled at $NB$ they show up at different sample indexes in time, and this allows \name to separate the VRFs set up by each of the $N$ unique on-off clocks.

% Finally, the last piece in the puzzle is how to select these $N$ different antenna groupings from the available $M$ antennas. One key feature of \name's VRFs is that it allows a many to many connection with antennas. That is, it not only allows us to turn on multiple antennas per VRF, we can also have one antenna showing up in multiple VRFs. This is because the clocks are orthogonal in time, and to have one antenna show up in two virtual chains, we can simply add two orthogonal clocks corresponding to the two VRFs. This allows \name to implement a switching matrix $\mathbf{S}$ in analog domain, which maps the user channels across $M$ antennas into $N$ user-proportionate VRFs. We also show a heuristic method, labelled as BABF, which beamforms towards one-user per VRF in order to enable practical user-proportionate MIMO.


% Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
% Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
% That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

% So far we have discussed how \name gets one antenna stream per virtual RF chain.
% But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
% A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
% Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
% Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


% To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
% The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
% In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
% Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
% \name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.




% Hence, massive MIMO ends up being  by having antenna proportionate power, as OFDMA can achieve the same goal by being user-proportionate.
% But, this comes at a cost of multiplicative increase in spectrum with OFDMA, which makes OFDMA power-inefficient.



% 


% Mainly these efficiency metrics can be either the traditionally considered spectral efficiency (bps per hertz) to advocate judicious use of spectrum, or energy efficiency
% both energy efficiency (bps per watt) and spectrum efficiency (bps per hertz). That is, in the coming decade, it is imperative to maximize both, how many bits can you communicate per watt usage, and number of bits packed in unit spectrum (Fig.). 



==> intros/intro_mcom_v3.tex <==
\section{Introduction}

Over the past decade, wireless networks have grown exponentially, and thereof have accrued humongous carbon footprint, with the net carbon emissions rivalling that of aviation sector\cite{footprint1,footprint2}.
% At the same time, the predicted demand of wireless networks is expected to exponentiate even upwards over the next decade .
Extensive case studies have highlighted the need for wireless networks to `\textbf{grow sustainably}' over the next decade\cite{}, and even consumer sentiment also highlight this, with more than 70\% consumers willing to switch to a greener alternative\cite{}. For wireless networks, the above translates to achieving efficient use of licensed spectrum and energy consumed.
Packing more bits per unit spectrum would support the growing data-rate by achieving spectrally efficient systems.
However, in communicating these more number of bits, the energy consumed should grow in a sub-linear manner, for making the wireless networks energy efficient. 
Ideally, wireless networks should achieve both spectral and energy efficiency (EE) and should be flexible, as number of users ($N$) decrease the energy used should proportional scale down.
% whereas communicating number of bits in a proportionate energy manner
% % should linear or sub-linearly increase the 
% per joule energy spent would make the networks greener. 
% Therefore, the expectation for future networks is to be
%the next generation wireless network that would jointly optimize for both spectrum efficiency (SE) as well as energy efficiency (EE), while adding new users or more throughput, will truly achieve the killer `green' mobile network selling point. 
%Furthermore, if such networks are 
% energy-proportional and flexible, by energy-proportional they can scale up the throughput with linear or sub-linear increase in energy consumption and by flexible they can scale up and down the energy consumption as load varies, besides optimizing for both spectrum efficiency (SE) as well as energy efficiency (EE).

%Therefore one key selling point for next generation mobile networks would be how `green' they can grow while connecting more users and/or support higher throughput, to cater towards both consumer, as well as sustainable incentive pushes. 
% Thus, it is imperative for wireless networks to not just keep increasing net throughput and/or users, but also maintaining or improving the energy efficiency.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{new_figs/intro_arch.pdf}
    \caption{\name solves for energy efficiency by creating a new massive MIMO architecture with flexible user-proportionate power consumption}
    \label{fig:intro_arch}
\end{figure}

% \begin{figure}[t]
%     % \begin{adjustwidth}{-15pt}{} 
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \setlength{\figureheight}{0.6\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     % \input{results/8ant_multipos}    
%     \input{results/compute_pow_spectrum}
%     % \caption{Power \& Spectrum Required}
%     \label{fig:intro_fig_new}
%     \end{subfigure}
%     % \end{adjustwidth}
%     \caption{How today's multi-user techniques stand}
% \end{figure}



Existing solutions for scaling wireless networks largely address spectrum and energy efficiencies in isolation, and are rigid. 
A energy-proportionate approach to scale wireless networks is to add more spectrum bands such that the users communicate at different frequencies in an interference-free manner (referred to as frequency multiplexing). Let's say each user is provided $B$ bandwidth, and therefore $N$ users consume a total of $NB$ spectrum. 
To support this $NB$ spectrum, the energy consumption scales by $N\times$ compared to supporting $B$ bandwidth. The extra energy is spent to support receiving/transmitting the $NB$ bandwidth signal\footnote{The ADC/DAC energy consumption scale up linearly to a threshold point, beyond that they scale exponentially\todo{agrim: may be talk about RF energy as well and citation?}}, resulting in linear scaling of energy proportionate to data bits ($N$).
% requires extra-ordinary spectrum to scale up, 
However, frequency multiplexing requires new spectrum band for each new user, which is an expensive and cumbersome process, 
but it achieves user/throughput proportionate energy scaling.
It also achieves flexibility since if the number of user drops to $K < N$, the transceiver could just sample $KB$ bandwidth and therefore, would scale down the energy consumption as well. 
Hence the net sampling bandwidth of frequency multiplexing offers a simple design knob which can be adjusted in accordance to user load.

% Thus this sampling bandwidth can be abstracted to software layers and frequency multiplexing can be `vi

% In recent times, 
% another popular approach to add more users or throughput
An alternate to frequency multiplexing is massive MIMO (mMIMO), which creates spatial multiplexing.
% by many multiple antennas and used by both WiFi and 5G.
mMIMO creates $N$ distinct spatial streams one for each user by performing linear combination of the massive number of antennas signals $M$, to serve $N$ users over the same spectrum. 
Thus, mMIMO has a spectrum-cost of fixed $B$ bandwidth, but packs in $N$ times more bits, improving spectral efficiency by $N\times$ compared to frequency multiplexing.
As shown in Fig. \ref{fig:intro_arch} (a), this is achieved by digitally interfacing the $M>>N$ number of antennas, which creates the $N$ spatial streams in digital domain (with mMIMO processing). Each antenna has its own RF interfacing hardware (for up/downcomversion, amplification) referred to as a RF chain, followed by the base-band unit which receives/transmits the $B$ bandwidth signals for each of the $M$ antennas, and performs digital computations O($MB$) to achieve mMIMO processing and generate $N$ user streams. 
Hence, mMIMO energy consumption is antenna proportional ($M\times$) to just get user-proportional ($N\times$) data bits across, thus super-linear energy consumption! 
% Thus, traditional mMIMO architecture sacrifices energy efficiency to pack more bits to achieve spectral efficiency. 
% For mMIMO processing, the $M$ antenna signals are combined appropriately to isolate the $N$ user signals from the interfered signals mix at each antenna.
% Therefore, the energy consumption is antenna-proportionate instead of user-proportionate, thus mMIMO sacrifices EE to pack more bits in the same spectrum band and achieve SE. 
Furthermore, mMIMO architectures are not flexible, that is they can not turn down energy consumption proportionately if the number of users drop. 
% It is because the $M$ antennas and their RF chains have been laid physically and typical mMIMO implementations only backhaul the $N$ per-user streams with mMIMO processing implemented on the RF chips\cite{}.
This is because if mMIMO turns off a certain number of RF chains, it has to drop some antennas, which would come at a performance degradation due to dropping to antennas as mMIMO would loose the degree-of-freedom~\cite{}.
Thus, traditional mMIMO architecture does not posses a trivial design knob which can be changed to make it adapt to differing user-loads without dropping performance, hence lacks flexibility.
% , unlike the simple sampling bandwidth knob in frequency multiplexing.
% This is because the architecture mMIMO can not be virtualized, because of the complexity. 


% This is because it is not trivial to turn since the mMIMO backhauls only the per-user $N$ streams.
% the signals (massive-MIMO processing) from these many antennas  
% appropriately to 
% , this way all the users communicate in same frequency bands but the massive-MIMO processing creates interference-free signals per user. 

% Thus even though OFDMA achieves EE, it is far less SE compared to MIMO.
% However, these spectral-efficiency improvements come at cost of exponential energy-usage in massive-MIMO. 
% In massive-MIMO implementations, we require many more antennas, $M$ than number of users, $N$ ($M>>N$) to enable interference free signals per user\cite{}. 



% It is 
% It is because as number of users increase, the sampling bandwidth increases proportionately, and all this sampled bandwidth contains proportionately many bits. 
% So the EE stays optimal as users increase.

% % In comparison, OFDMA implements frequency multiplexing, which puts users in different spectrum bands. 
% % Since the users have different frequency, there is no need to create a spatial beam and OFDMA can use a single antenna and hence a single RF chain. 
% % OFDMA requires sampling the aggregate spectrum, and hence the power consumption is proportional to the net sampling bandwidth, which in turn is user-proportionate.
% Say if number of users are $N$ each having bandwidth $B$, OFDMA transmits/receives the aggregate RF bandwidth $NB$ to communicate the data to/from $N$ users. 
% The hardware implementation of OFDMA is hence straightforward, consists of basically a single TX/RX chain which connects the digital processor to the antenna and communicates the $NB$ signals.
% The power consumption is user proportionate, as users in network increase/decrease OFDMA can increase/decrease the bandwidth and hence not waste power.
% via an antenna
% That is, 
% In OFDMA, the single RF chain samples the aggregate bandwidth occupied by the number of users, and hence the single RF chain's power is user-proportionate.


% but sacrifices SE by putting multiple users in different frequency band\cite{}, so the base station does not need to handle the interference.
% As a consequence, OFDMA just needs a single antenna, hence a single RF chain, which needs to sample the net spectrum occupied by all the users.
% For this, OFDMA would have sampling bandwidth proportionate to number of users, thus the power consumption is user-proportionate, making it achieve EE.
% Multiple existing works have pointed to this SE-EE tradeoff\cite{}, and current research consensus is that the tradeoff can not be broken but needs to be addressed by careful design of networks that they operate on a compromised `green' point of operation.


% As a consequence of MIMO not being EE, it limits usecase 
% MIMO approaches use multiple antennas to address SE by performing spatial multiplexing. 
% Spatial multiplexing allows users to share the spectrum resources, since they are being served by distinct beams created via the multi-antenna array.
% However, this requires specialized circuits , referred to as RF chains, to transmit/receive signals per-antenna.
% Thus, the power consumption grows proportional to number of RF chains, and hence number of antennas, since each antenna needs its own RF chain. 

% Hence, the power consumption is not user-proportionate, and massive MIMO sacrifices EE by setting up many more RF chains to serve a smaller number of users.

% This allows users to share the same spectrum, as they are separated in the spatial domain by the means of beamforming.
% This is achieved by creation of spatial beams towards each user by a concept also referred to as digital beamforming (DBF).
% However, this requires each antenna to have separate RF interfacing hardware\cite{} which interfaces the antenna with the baseband signal processing unit, also referred to as a `RF chain'. 
% which connect the baseband digital processor to the antenna and consists of various circuits like ADC/DAC, down/up conversion mixers, filters, LNA/PA.


In this paper we break the antenna-proportionate energy consumption required to achieve mMIMO multiplexing to user-proportionate energy consumption, while continuing to use all antennas for mMIMO operation, and achieving flexibility (dropping energy consumption as users drop) and spectral efficiency (using only bandwidth B).
To this end, we present the design and implementation of a new massive-MIMO architecture, dubbed as \name.
% which keeps energy consumption to user-proportionate ($N\times$) levels, while interfacing the required $M>>N$ antennas for mMIMO operation.
\name connects each of the $M$ massive-MIMO antennas to an ultra-low power per-antenna configurable analog-spreading-network, as shown in Fig \ref{fig:intro_arch} (b). This analog network can intuitively create a distinct signature for each antenna, by spreading it's signals in a distinct manner across a wider bandwidth with very minimal power. This spreaded+signatured output from each antennae is combined and passed through a single down-conversion chain, such an approach allows \name to add any number of antenna while only consuming minimal extra energy. The combined signal is then sampled at user-proportionate sampling rate ($NB$), to allows for de-spreading while keeping the digital computations at user-proportionate rate O($NB$). 

% thus consuming energy proportionate to the number of users supported. 
Hence, using the $NB$ sampled bandwidth, the digitized signal is passed through a digital de-spreading block which isolates the signature given to a particular antenna (to a limit of N antenna). 
% This analog spreading + digital de-spreading creates $N$ virtual RF chains, which are fed to MIMO processing to retrieve per-user streams. 
To ensure that the $M$ antennas diversity gains are captured correctly via the analog-spreading network, \name develops a algorithm to choose proper codes for analog-spreading, such that multiple antennas are grouped accordingly to create $N$ virtual RF chains.
That is, \name superimposes codes of multiple antennas strategically such that they beamform via the analog network towards one user per virtual RF chain, such that when, combined with the mMIMO processing it creates interference-free user streams.  
The digital de-spreading and analog-spreading operation can be conducted for transmission as well, to achieve user-proportionate energy consumption for both receive and transmit. 
Furthermore, \name energy consumption can be scaled flexibly via sampling bandwidth design knob, akin to frequency multiplexing.
That is, if the number of users drop to $K$ users, the combined signal across the $M$ antennas is digitized at the $KB$ sampling rate. 
% Thus \name offers the simple sampling bandwidth design knob for flexibility, akin to frequency multiplexing solution.

To achieve \name architecture, the first challenge is to how to create these spreaded bandwidth signatures in analog-network which allows creation of the virtual RF chains. 
Furthermore, we need to achieve this spreading operation in an ultra-low power fashion, which would allow \name to add more antennas easily without requiring exorbitant energy consumption. 
\name's solution to the two problems is to create a simple $M\to 1$ analog network of $M$ antennas each connected to faster-than-bandwidth RF switches with minimal loss ($<1$ dB) insertion losses, with active power draw of about 1mW.  
These switches are modulated with sub-sample level time-period on-off codes, which create the desired analog spreading signature.
This signature can then be used to control how different antenna groups can get combined in the analog network, before these go through the shared downconversion and digitization interface by the single RF chain. 

% Furthermore, the switches are modulated with code which uses `on-off' configurability at each antenna to provide a distinct `on-off' signature (code). 
% We build this analog network via RF switches connected to each antenna, which are energy efficient as they have extremely low insertion losses ($<1$ dB) an
% Recall that the digital sampling is conducted at 
% how do we design analog-pre-processing network such that each antenna signal identity is managed? 
Hence, the second challenge in \name architecture is how to isolate the $N$ 
The first key insight of \name here is that since we have $NB$ bandwidth at disposal, and the user signals are $B$ bandwidth, we can isolate $N$ antenna groups at a time.
To use this $N\times$ higher bandwidth, we can spread the antenna signals via distinct $B$ frequency `on-off' codes which create signal harmonics and spread the $B$ bandwidth signal across $NB$ bandwidth.
We show how $N$ orthogonal $B$ frequency codes can be designed which spread the signals in an efficient manner across the $NB$ bandwidth and prevents signal leakage and distortions.

% However, we
% So, in order to isolate the per-antenna signals, we can use these $N$ degrees of freedom to treat $N$ antennas as $N$ users and 
% Since all the antennas share the same RX/TX chain, the signals would get combined into a single added signal, losing the per-antenna signature.
% analog spreading `on-off' codes for each antenna, so that before getting combined each antenna gets a unique $NB$ bandwidth signature.
% , as shown by different color boxes in Fig. \ref{fig:intro_spread}.

% By giving each antenna a $NB$ bandwidth signature, we preserve the per-antenna signatures even when they share a single downconversion chain.
% It is because we have $N$ different orthogonal methods to spread $B$ bandwidth signals into $NB$ bandwidth, and these orthogonal spreading methods can be then inverted to get back the per-antenna signals.

% allows for isolation of $N$
% This analog spreading effect basically preserves the antenna's signature before they get combined into a single RF chain, get downconverted and digitized.
% After obtaining the $NB$ digitizes samples, we can de-spread the codes to isolate the per-antenna signature, and hence isolate the $B$ bandwidth original signal of that antenna.
% Since we have $N$ degrees of freedom, we can generate $N$ such distinct orthogonal codes to isolate $N$ antennas signals even when they share the same RF chain.
Te third challenge is how \name then inverts this analog spreading effect of $N$ orthogonal codes to get back per antenna $B$ bandwidth-signals signals?
We show that these efficient $N$ spreading `on-off' codes are in-fact orthogonal in time, and can be inverted by isolating the different time samples occupied by each code.
This is done in the digital domain by simply splicing the digitized samples to ensure the de-spreading of codes.
In a way, this analog spreading + digital de-spreading via configurable RF switches creates `$N$ virtual RF chains' across the $NB$ bandwidth of the physically laid RF chain.
That is, even though there did not exist a physical path to $N$ antennas, it gets created virtually post-digitization.
Note that, similar to freq. multiplexing, we can use design knob of variable sampling bandwidth to vary the number of virtual chains as number of users $N$ varies.
% This is visually illustrated in Fig. \ref{fig:intro_spread}.

% The second challenge here is how can we take this $N$ virtual RF chain concept and apply to $M>N$ antennas, to truly enable spatial multiplexing?

However, we started with $M>N$ antennas, but we have only $N$ virtual RF chains from the spreading-de-spreading in $NB$ bandwidth.
Hence, the final challenge is how can \name use the entire array of $M$ antennas over these $N$ created virtual RF chains?
The two key insights here are that virtual RF chains allow for both, multiple antennas to be connected to a single virtual RF chain, as well as a single antenna connected to multiple RF chain.
This is made possible by the orthogonality of the codes, in the way that we can add to codes together for an antenna so that it shows up in both the spliced samples of virtual RF chain created by both these codes.
Further, giving same spreading code to multiple antennas allows them to be connected together in the same virtual chain.
% The basic principle why this works is that RF chains are created by the analog spreading + digital de-spreading effect which can be abstracted and applied across multiple antennas to enable a many to many connection between antennas and virtual RF chains, making the entire $M$ antenna array available to the $N$ virtual RF chains.
This way, we can have one virtual RF chain using a group of antennas which are co-phased for a user, and grouping them would in a way perform beamforming towards a particular user.
This allows \name to create narrower beams by using more number of $M$ antennas, than $N$ virtual chains, with the many-to-many connection allowing all antennas to be shared across all virtual chains.
Hence, \name achieves mMIMO like performance at user-proportionate power for $N$ virtual RF chains without being antenna-proportionate as mMIMO.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% This is because virtual RF chains are created by analog spreading via $N$ time-orthogonal codes, so to make two antennas appear in same virtual chain we can add the spreading codes for the particular antenna. 
% Hence, it would shows up in time-spliced samples post-digitization across both the virtual chains.
% Having multiple antennas for one virtual RF chain is straightforward, and can be done by supplying the particular spreading code to each antenna
% The key insight here is that since virtual RF chains are created by analog spreading-digital despreading, we can have antennas co-phased for one user to spread with the same code, so that they constructively add up in the virtual RF chain generated by that code.
% This way, we can have one virtual RF chain using a group of antenna beamforming towards it.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% A natural question here would be if $M$ antennas are split up amongst $N$ RF chains?
% We show that infact $2$ virtual RF chains can share the same antenna since the spreading codes are orthogonal, so we can add the spreading codes of the $2$ virtual RF chains for one antenna to make it appear in both the RF chains.
% Hence, this allows a many-to-many connection between the $M$ antennas and $N$ virtual RF chains, and effectively allows all the $N$ virtual chains to use the full array for beamforming.
% This captures the required goal of narrow beams by using $M>N$ antennas, while using $N$ virtual RF chains.
% can we share the $N$ virtual RF chains effectively across higher number of antennas to create the required narrow beams?

% The key insight here is that unlike a physical RF chain, which is created by laying the physical hardware to each antenna, virtual RF chains are an abstraction created by the spreading-despreading effect.
% So, in \name we can group many antennas by spreading them in a similar way, so the de-spreading operation gives a combined signal across all these antennas.
% Further, we show that since the spreading codes are orthogonal, a single antenna can be spread across two virtual RF chains as well.
% So, \name allows a many to many connection between $M$ antennas and $N$ virtual RF chains.
% This allows \name to group antennas strategically such that they perform approximate analog beamforming towards one user per virtual RF chain.
% The residual interference left is then cancelled digitally by inverting the channels and doing zero-forcing post-coding  (shown after de-spreading block, Fig. \ref{fig:intro_spread}).

% By addressing the challenges listed above, \name truly enables `user-proportionate' spatial multiplexing with $M$ antennas connected via the analog spreading network and a single $NB$ bandwidth RF chain.
% % Hence, the net power consumption of \name would be that of OFDMA + total power across the required analog spreading.
% % So, the last challenge in designing \name is how can the
% To design the analog network with ultra-low power consumption,we show that the required analog spreading operation can be achieved via simple RF switches toggling at strategically chosen $N$ distinct on-off codes, which give the required unique spreading for $N$ virtual RF chains.
% RF switches enable this at $<1$mW power draw, which is minimal compared to $100$'s of mW power draw of RF chains.
% This is not surprising, since in the field of backscatter communications, the same RF switches perform the frequency shifting operations at $\mu$W levels.


% Thus, to summarize, \name designs a new MIMO architecture which connects $M$ antennas to single RF chain of OFDMA via $M$ RF switches. \name basically creates $N$ virtual RF chain via analog spreading effect of RF switches, and de-spread digitally in the $NB$ bandwidth OFDMA RF chain. 
% \name also is a `flexible' architecture, it can create $N$ virtual RF chains on demand, so if there are lesser/more users it can adaptively reduce/increase the number of virtual chains.
% By being almost same power level as OFDMA, as well as using multiple antennas to create mMIMO like narrow beams, \name achieves both EE and SE. 
\todo{Improve last para}
We implement \name prototype with $M=8$ antennas to flexibly serve $2,3,4$ users. We test \name over multiple user positions in a conference room setting, as well as traditional MIMO and OFDMA baselines. Our key results include similar performance metrics with MIMO with $3\times$ less power requirements, achieving the same network capacity as compared to OFDMA with $4\times$ lesser spectrum requirements, which experimentally confirm the SE and EE claims.
At the same time, if there is a single MIMO capable user, \name can be used to serve multiple streams, and we show this by increasing throughput of single user by $3$ times.
Finally, we end with a case study on how \name can make various classes of base stations more energy efficient and cut down on power bills.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{new_figs/BM_fig.pdf}
%     \caption{How power consumption varies with number of users for freq. \& spatial multiplexing, with typical values of power consumption tabulated}
%     \label{fig:bm_fig_new}
% \end{figure*}

% and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.



% The main reason for MIMO not achieving EE is the requirement of separate RF chains for each antenna, and this issue 
% Taking a step towards breaking this SE-EE tradeoff, in this paper we present \name, which for the first time, shows an architecture which can maximize both SE and EE. 
% The key insight here is to add low-power analog circuitry to each antenna such that 
% The key insight which enables \name to do so, is that MIMO and OFDMA systems of today can be married together, by using configurable, low-power RF circuits per antenna, to get best of both worlds.
% The idea is to have the multiple MIMO `configurable' antennas combinedly share the single user-proportionate sampling bandwidth RF chain of OFDMA. 
% Each antenna in \name can be set to separate configurations to give unique identity to the antennas signal before they combine together and go through the RF chain.
% By isolating the signals based on the unique identity, \name can isolate the per-antenna signals in the digital domain.
% Hence, this approach basically creates a virtual signal path towards each separate antenna configuration in digital domain, and we dub this process as creation of `Virtual RF chains (VRF)'.
% These VRFs also allow for grouping of multiple antennas by setting them to same configurations, so $N$ virtual RF chains can effectively share $M>N$ antennas among themselves.
% This enables practical MIMO operation for $N$ interfering users, while harnessing advantages offered by $M>N$ antennas, and keeping power consumption to user-proportionate sampling level of single RF chain.
% % Hence, the concrete approach behind \name is that, to serve $N$ users in a user-proportionate power manner via $M>N$ antennas, \name creates $N$ `virtual RF chains' from a single physical RF chain sampled at $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power efficiency of OFDMA.

% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.

% The basic idea is that we can use the increased sampling bandwidth of a single RF chain to carve out virtual signal paths to each antenna in the digital domain, in a process dubbed as creation of `virtual RF chains'.
% This way \name is able to harness MIMO operation by laying a single physical RF chain, and abstracting out multiple virtual RF chains as demand-fit.
% Further, this process is done in an optimal user-proportionate manner where \name can club together multiple antennas in a single virtual RF chain to harness the gains of many more antennas than number of users and show practical MIMO operation in realistic environments.
% This basically allows the single RF chain to get `virtualized' over the many antennas, in the sense that all antennas share the same RF chain but have a separate virtual digital path created , which allows for creation of virtual RF chains in the digital domain.
% Further, by 
% This is made possible by a combined analog-digital antenna combining approach which ensures that the required benefits of many more antennas than number of users get 
% Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

% The first design consideration for \name is how to even realize this concept of a VRF? 
% To motivate this, we first show how that the desired behaviour from the configurable RF circuit is to create a `frequency spreading' effect, so that the $B$ bandwidth user signals get spread into $NB$ total bandwidth.
% However, a challenge here is that this spreading operation needs to be done with minimal power consumption, otherwise the net power requirements would end up being antenna proportionate as we need this circuit for each antenna.
% Hence, \name inspirchallengees from backscatter communication's RF-switches that create frequency shifts with minimal <100uW power requirements \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, when toggled with certain frequency on-off clock.

% This rules out naive solutions like RF mixers which can create the intended frequency spreading effect, but at expense of insertion losses and non-negligible power consumption.
% Instead, \name uses RF switches, which also are capable of creating these frequency shifts when toggled with a certain frequency on-off clock.
% Further, this operation has minimal power requirements, and similar RF switches have been used for channel shifting purposes in backscatter systems with <10uW power requirements that can also be made batteryless \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}.
% The concrete idea here is that, to serve $N$ users in a user-proportionate power manner,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power efficiency of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
% It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
% We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

% Next, we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ different antenna groups so as to enable the creation of $N$ virtual RF chains. 
% Thus, we can use RF switches to configure antennas on-off strategically to create VRFs. However, how exactly should we configure these switches such that we can create $N$ VRFs for $N$ different antenna groups?
% For this, we show how \name can create $N$ orthogonal on-off clocks having $B$ frequency, corresponding to user bandwidth and $1/N$ duty cycle each, but different initial phases.
% The idea is that a particular group of antennas antennas can be configured with one of these $N$ orthogonal on-off clocks, and signals of these antennas would get combined in the analog domain and get downconverted+digitized. 
% Then in digital domain the summed signals from these different antennas can be isolated from since these summed combined signals would have the unique clock marking them different from the other groups using the rest $N-1$ clocks.
% The key insight which allows separating these $N$ clocks from each other is that when
% these $N$ different $B$ frequency codes are sampled at $NB$ they show up at different sample indexes in time, and this allows \name to separate the VRFs set up by each of the $N$ unique on-off clocks.

% Finally, the last piece in the puzzle is how to select these $N$ different antenna groupings from the available $M$ antennas. One key feature of \name's VRFs is that it allows a many to many connection with antennas. That is, it not only allows us to turn on multiple antennas per VRF, we can also have one antenna showing up in multiple VRFs. This is because the clocks are orthogonal in time, and to have one antenna show up in two virtual chains, we can simply add two orthogonal clocks corresponding to the two VRFs. This allows \name to implement a switching matrix $\mathbf{S}$ in analog domain, which maps the user channels across $M$ antennas into $N$ user-proportionate VRFs. We also show a heuristic method, labelled as BABF, which beamforms towards one-user per VRF in order to enable practical user-proportionate MIMO.


% Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
% Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
% That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

% So far we have discussed how \name gets one antenna stream per virtual RF chain.
% But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
% A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
% Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
% Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


% To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
% The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
% In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
% Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
% \name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.




% Hence, massive MIMO ends up being  by having antenna proportionate power, as OFDMA can achieve the same goal by being user-proportionate.
% But, this comes at a cost of multiplicative increase in spectrum with OFDMA, which makes OFDMA power-inefficient.



% 


% Mainly these efficiency metrics can be either the traditionally considered spectral efficiency (bps per hertz) to advocate judicious use of spectrum, or energy efficiency
% both energy efficiency (bps per watt) and spectrum efficiency (bps per hertz). That is, in the coming decade, it is imperative to maximize both, how many bits can you communicate per watt usage, and number of bits packed in unit spectrum (Fig.). 



==> intros/intro_mcom_v4.tex <==
\section{Introduction}

Over the past decade, wireless networks have grown exponentially, and thereof have accrued humongous carbon footprint, with the net carbon emissions rivalling that of aviation sector\cite{footprint1,footprint2}.
% At the same time, the predicted demand of wireless networks is expected to exponentiate even upwards over the next decade .
Extensive case studies have highlighted the need for wireless networks to `\textbf{grow sustainably}' over the next decade\cite{}, and even consumer sentiment also highlight this, with more than 70\% consumers willing to switch to a greener alternative\cite{}. For wireless networks, the above translates to acheiving efficient use of licensed spectrum and energy consumed.
Packing more bits per unit spectrum would support the growing data-rate by achieving spectrally efficient systems.
However, in communicating these more number of bits, the energy consumed should grow in a sub-linear manner, for making the wireless networks energy efficient. 
Ideally, wireless networks should achieve both spectral and energy efficiency (EE) and should be flexible, as number of users ($N$) decrease the energy used should proportional scale down.
% whereas communicating number of bits in a proportionate energy manner
% % should linear or sub-linearly increase the 
% per joule energy spent would make the networks greener. 
% Therefore, the expectation for future networks is to be
%the next generation wireless network that would jointly optimize for both spectrum efficiency (SE) as well as energy efficiency (EE), while adding new users or more throughput, will truly achieve the killer `green' mobile network selling point. 
%Furthermore, if such networks are 
% energy-proportional and flexible, by energy-proportional they can scale up the throughput with linear or sub-linear increase in energy consumption and by flexible they can scale up and down the energy consumption as load varies, besides optimizing for both spectrum efficiency (SE) as well as energy efficiency (EE).

%Therefore one key selling point for next generation mobile networks would be how `green' they can grow while connecting more users and/or support higher throughput, to cater towards both consumer, as well as sustainable incentive pushes. 
% Thus, it is imperative for wireless networks to not just keep increasing net throughput and/or users, but also maintaining or improving the energy efficiency.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{new_figs/intro_arch.pdf}
    \caption{\name solves for energy efficiency by creating a new massive MIMO architecture with flexible user-proportionate power consumption}
    \label{fig:intro_arch}
\end{figure}

% \begin{figure}[t]
%     % \begin{adjustwidth}{-15pt}{} 
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \setlength{\figureheight}{0.6\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     % \input{results/8ant_multipos}    
%     \input{results/compute_pow_spectrum}
%     % \caption{Power \& Spectrum Required}
%     \label{fig:intro_fig_new}
%     \end{subfigure}
%     % \end{adjustwidth}
%     \caption{How today's multi-user techniques stand}
% \end{figure}



Existing solutions for scaling wireless networks largely address spectrum and energy efficiencies in isolation, and are rigid. 
A energy-proportionate approach to scale wireless networks is to add more spectrum bands such that the users communicate at different frequencies in an interference-free manner (referred to as frequency multiplexing). Let's say each user is provided $B$ bandwidth, and therefore $N$ users consume a total of $NB$ spectrum. 
To support this $NB$ spectrum, the energy consumption scales by $N\times$ compared to supporting $B$ bandwidth. The extra energy is spent to support receiving/transmitting the $NB$ bandwidth signal\footnote{The ADC/DAC energy consumption scale up linearly to a threshold point, beyond that they scale exponentially\todo{agrim: may be talk about RF energy as well and citation?}}, resulting in linear scaling of energy proportionate to data bits ($N$).
% requires extra-ordinary spectrum to scale up, 
However, frequency multiplexing requires new spectrum band for each new user, which is an expensive and cumbersome process, 
but it achieves user/throughput proportionate energy scaling.
It also achieves flexibility since if the number of user drops to $K < N$, the transceiver could just sample $KB$ bandwidth and therefore, would scale down the energy consumption as well. 
Hence the net sampling bandwidth of frequency multiplexing offers a simple design knob which can be adjusted in accordance to user load.

% Thus this sampling bandwidth can be abstracted to software layers and frequency multiplexing can be `vi

% In recent times, 
% another popular approach to add more users or throughput
An alternate to frequency multiplexing is massive MIMO (mMIMO), which creates spatial multiplexing.
% by many multiple antennas and used by both WiFi and 5G.
mMIMO creates $N$ distinct spatial streams one for each user by performing linear combination of the massive number of antennas signals $M$, to serve $N$ users over the same spectrum. 
Thus, mMIMO has a spectrum-cost of fixed $B$ bandwidth, but packs in $N$ times more bits, improving spectral efficiency by $N\times$ compared to frequency multiplexing.
As shown in Fig. \ref{fig:intro_arch} (a), this is achieved by digitally interfacing the $M>>N$ number of antennas, which creates the $N$ spatial streams in digital domain (with mMIMO processing). Each antenna has its own RF interfacing hardware (for up/downcomversion, amplification) referred to as a RF chain, followed by the base-band unit which receives/transmits the $B$ bandwidth signals for each of the $M$ antennas, and performs digital computations O($MB$) to achieve mMIMO processing and generate $N$ user streams. 
Hence, mMIMO energy consumption is antenna proportional ($M\times$) to just get user-proportional ($N\times$) data bits across, thus super-linear energy consumption! 
% Thus, traditional mMIMO architecture sacrifices energy efficiency to pack more bits to achieve spectral efficiency. 
% For mMIMO processing, the $M$ antenna signals are combined appropriately to isolate the $N$ user signals from the interfered signals mix at each antenna.
% Therefore, the energy consumption is antenna-proportionate instead of user-proportionate, thus mMIMO sacrifices EE to pack more bits in the same spectrum band and achieve SE. 
Furthermore, mMIMO architectures are not flexible, that is they can not turn down energy consumption proportionately if the number of users drop. 
% It is because the $M$ antennas and their RF chains have been laid physically and typical mMIMO implementations only backhaul the $N$ per-user streams with mMIMO processing implemented on the RF chips\cite{}.
This is because if mMIMO turns off a certain number of RF chains, it has to drop some antennas, which would come at a performance degradation due to dropping to antennas as mMIMO would loose the degree-of-freedom~\cite{}.
Thus, traditional mMIMO architecture does not posses a trivial design knob which can be changed to make it adapt to differing user-loads without dropping performance, hence lacks flexibility.
% , unlike the simple sampling bandwidth knob in frequency multiplexing.
% This is because the architecture mMIMO can not be virtualized, because of the complexity. 


% This is because it is not trivial to turn since the mMIMO backhauls only the per-user $N$ streams.
% the signals (massive-MIMO processing) from these many antennas  
% appropriately to 
% , this way all the users communicate in same frequency bands but the massive-MIMO processing creates interference-free signals per user. 

% Thus even though OFDMA achieves EE, it is far less SE compared to MIMO.
% However, these spectral-efficiency improvements come at cost of exponential energy-usage in massive-MIMO. 
% In massive-MIMO implementations, we require many more antennas, $M$ than number of users, $N$ ($M>>N$) to enable interference free signals per user\cite{}. 



% It is 
% It is because as number of users increase, the sampling bandwidth increases proportionately, and all this sampled bandwidth contains proportionately many bits. 
% So the EE stays optimal as users increase.

% % In comparison, OFDMA implements frequency multiplexing, which puts users in different spectrum bands. 
% % Since the users have different frequency, there is no need to create a spatial beam and OFDMA can use a single antenna and hence a single RF chain. 
% % OFDMA requires sampling the aggregate spectrum, and hence the power consumption is proportional to the net sampling bandwidth, which in turn is user-proportionate.
% Say if number of users are $N$ each having bandwidth $B$, OFDMA transmits/receives the aggregate RF bandwidth $NB$ to communicate the data to/from $N$ users. 
% The hardware implementation of OFDMA is hence straightforward, consists of basically a single TX/RX chain which connects the digital processor to the antenna and communicates the $NB$ signals.
% The power consumption is user proportionate, as users in network increase/decrease OFDMA can increase/decrease the bandwidth and hence not waste power.
% via an antenna
% That is, 
% In OFDMA, the single RF chain samples the aggregate bandwidth occupied by the number of users, and hence the single RF chain's power is user-proportionate.


% but sacrifices SE by putting multiple users in different frequency band\cite{}, so the base station does not need to handle the interference.
% As a consequence, OFDMA just needs a single antenna, hence a single RF chain, which needs to sample the net spectrum occupied by all the users.
% For this, OFDMA would have sampling bandwidth proportionate to number of users, thus the power consumption is user-proportionate, making it achieve EE.
% Multiple existing works have pointed to this SE-EE tradeoff\cite{}, and current research consensus is that the tradeoff can not be broken but needs to be addressed by careful design of networks that they operate on a compromised `green' point of operation.


% As a consequence of MIMO not being EE, it limits usecase 
% MIMO approaches use multiple antennas to address SE by performing spatial multiplexing. 
% Spatial multiplexing allows users to share the spectrum resources, since they are being served by distinct beams created via the multi-antenna array.
% However, this requires specialized circuits , referred to as RF chains, to transmit/receive signals per-antenna.
% Thus, the power consumption grows proportional to number of RF chains, and hence number of antennas, since each antenna needs its own RF chain. 

% Hence, the power consumption is not user-proportionate, and massive MIMO sacrifices EE by setting up many more RF chains to serve a smaller number of users.

% This allows users to share the same spectrum, as they are separated in the spatial domain by the means of beamforming.
% This is achieved by creation of spatial beams towards each user by a concept also referred to as digital beamforming (DBF).
% However, this requires each antenna to have separate RF interfacing hardware\cite{} which interfaces the antenna with the baseband signal processing unit, also referred to as a `RF chain'. 
% which connect the baseband digital processor to the antenna and consists of various circuits like ADC/DAC, down/up conversion mixers, filters, LNA/PA.


In this paper we break the antenna-proportionate energy consumption required to achieve mMIMO multiplexing to user-proportionate energy consumption, while continuing to use all antennas for mMIMO operation, and achieving flexibility (dropping energy consumption as users drop) and spectral efficiency (using only bandwidth B).
To this end, we present the design and implementation of a new massive-MIMO architecture, dubbed as \name.
% which keeps energy consumption to user-proportionate ($N\times$) levels, while interfacing the required $M>>N$ antennas for mMIMO operation.
\name connects each of the $M$ massive-MIMO antennas to an ultra-low power per-antenna configurable analog-network, as shown in Fig \ref{fig:intro_arch} (b). This analog network can intuitively apply a distinct and unique signature to signal received from each antenna, spreading the signal in a distinct manner across a wider bandwidth with very minimal power (\todo{uWatts}). The analog-network output from each antennae is combined and passed through a single down-conversion chain, such an approach allows \name to add any number of antenna while only consuming minimal extra energy. The combined signal is then sampled at user-proportionate sampling rate ($NB$), to allows for the digital computations at user-proportionate rate O($NB$), consuming sampling and compute energy proportional to user-proportionate rate. 

The final goal of \name is to construct the $N$ streams each of bandwidth $B$, from the combined signal sampled at $NB$; the $N$ streams when combined digitally with mMIMO processing should isolate to per-user signal. To ensure that the $M$ antennas diversity gains are captured correctly via the analog-spreading network, \name develops a algorithm to choose proper codes for analog-spreading, such that multiple antennas are grouped accordingly to create $N$ virtual RF chains. That is, \name superimposes codes of multiple antennas strategically such that they beamform via the analog network towards one user per virtual RF chain, such that when, combined with the mMIMO processing it creates interference-free user streams.  
The digital de-spreading and analog-spreading operation can be conducted for transmission as well, to achieve user-proportionate energy consumption for both receive and transmit. 
Furthermore, \name energy consumption can be scaled flexibly via sampling bandwidth design knob, akin to frequency multiplexing.
That is, if the number of users drop to $K$ users, the combined signal across the $M$ antennas is digitized at the $KB$ sampling rate. 



To achieve this, \name designs an algorithm which smartly configures each antennae's analog-network to map to each of the N streams, such that each of the $N$ streams can be used to decode the $N$ users signal. 

With the user-proportionate ($NB$) sampled bandwidth, the digitized signal when passed through a digital de-spreading block can isolate to $N$ signals each of bandwidth $B$. Said differently, we can only have N signature. Each antennae should be assigned a group of these $N$ signature, or super-position of these $N$ signature. Therefore,  


% thus consuming energy proportionate to the number of users supported. 
% This analog spreading + digital de-spreading creates $N$ virtual RF chains, which are fed to MIMO processing to retrieve per-user streams. 

% Thus \name offers the simple sampling bandwidth design knob for flexibility, akin to frequency multiplexing solution.

To achieve \name architecture, the first challenge is to how to create these spreaded bandwidth signatures in analog-network which allows creation of the virtual RF chains. 
Furthermore, we need to achieve this spreading operation in an ultra-low power fashion, which would allow \name to add more antennas easily without requiring exorbitant energy consumption. 
\name's solution to the two problems is to create a simple $M\to 1$ analog network of $M$ antennas each connected to faster-than-bandwidth RF switches with minimal loss ($<1$ dB) insertion losses, with active power draw of about 1mW.  
These switches are modulated with sub-sample level time-period on-off codes, which create the desired analog spreading signature.
This signature can then be used to control how different antenna groups can get combined in the analog network, before these go through the shared downconversion and digitization interface by the single RF chain. 

% Furthermore, the switches are modulated with code which uses `on-off' configurability at each antenna to provide a distinct `on-off' signature (code). 
% We build this analog network via RF switches connected to each antenna, which are energy efficient as they have extremely low insertion losses ($<1$ dB) an
% Recall that the digital sampling is conducted at 
% how do we design analog-pre-processing network such that each antenna signal identity is managed? 
Hence, the second challenge in \name architecture is how to isolate the $N$ 
The first key insight of \name here is that since we have $NB$ bandwidth at disposal, and the user signals are $B$ bandwidth, we can isolate $N$ antenna groups at a time.
To use this $N\times$ higher bandwidth, we can spread the antenna signals via distinct $B$ frequency `on-off' codes which create signal harmonics and spread the $B$ bandwidth signal across $NB$ bandwidth.
We show how $N$ orthogonal $B$ frequency codes can be designed which spread the signals in an efficient manner across the $NB$ bandwidth and prevents signal leakage and distortions.

% However, we
% So, in order to isolate the per-antenna signals, we can use these $N$ degrees of freedom to treat $N$ antennas as $N$ users and 
% Since all the antennas share the same RX/TX chain, the signals would get combined into a single added signal, losing the per-antenna signature.
% analog spreading `on-off' codes for each antenna, so that before getting combined each antenna gets a unique $NB$ bandwidth signature.
% , as shown by different color boxes in Fig. \ref{fig:intro_spread}.

% By giving each antenna a $NB$ bandwidth signature, we preserve the per-antenna signatures even when they share a single downconversion chain.
% It is because we have $N$ different orthogonal methods to spread $B$ bandwidth signals into $NB$ bandwidth, and these orthogonal spreading methods can be then inverted to get back the per-antenna signals.

% allows for isolation of $N$
% This analog spreading effect basically preserves the antenna's signature before they get combined into a single RF chain, get downconverted and digitized.
% After obtaining the $NB$ digitizes samples, we can de-spread the codes to isolate the per-antenna signature, and hence isolate the $B$ bandwidth original signal of that antenna.
% Since we have $N$ degrees of freedom, we can generate $N$ such distinct orthogonal codes to isolate $N$ antennas signals even when they share the same RF chain.
Te third challenge is how \name then inverts this analog spreading effect of $N$ orthogonal codes to get back per antenna $B$ bandwidth-signals signals?
We show that these efficient $N$ spreading `on-off' codes are in-fact orthogonal in time, and can be inverted by isolating the different time samples occupied by each code.
This is done in the digital domain by simply splicing the digitized samples to ensure the de-spreading of codes.
In a way, this analog spreading + digital de-spreading via configurable RF switches creates `$N$ virtual RF chains' across the $NB$ bandwidth of the physically laid RF chain.
That is, even though there did not exist a physical path to $N$ antennas, it gets created virtually post-digitization.
Note that, similar to freq. multiplexing, we can use design knob of variable sampling bandwidth to vary the number of virtual chains as number of users $N$ varies.
% This is visually illustrated in Fig. \ref{fig:intro_spread}.

% The second challenge here is how can we take this $N$ virtual RF chain concept and apply to $M>N$ antennas, to truly enable spatial multiplexing?

However, we started with $M>N$ antennas, but we have only $N$ virtual RF chains from the spreading-de-spreading in $NB$ bandwidth.
Hence, the final challenge is how can \name use the entire array of $M$ antennas over these $N$ created virtual RF chains?
The two key insights here are that virtual RF chains allow for both, multiple antennas to be connected to a single virtual RF chain, as well as a single antenna connected to multiple RF chain.
This is made possible by the orthogonality of the codes, in the way that we can add to codes together for an antenna so that it shows up in both the spliced samples of virtual RF chain created by both these codes.
Further, giving same spreading code to multiple antennas allows them to be connected together in the same virtual chain.
% The basic principle why this works is that RF chains are created by the analog spreading + digital de-spreading effect which can be abstracted and applied across multiple antennas to enable a many to many connection between antennas and virtual RF chains, making the entire $M$ antenna array available to the $N$ virtual RF chains.
This way, we can have one virtual RF chain using a group of antennas which are co-phased for a user, and grouping them would in a way perform beamforming towards a particular user.
This allows \name to create narrower beams by using more number of $M$ antennas, than $N$ virtual chains, with the many-to-many connection allowing all antennas to be shared across all virtual chains.
Hence, \name achieves mMIMO like performance at user-proportionate power for $N$ virtual RF chains without being antenna-proportionate as mMIMO.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% This is because virtual RF chains are created by analog spreading via $N$ time-orthogonal codes, so to make two antennas appear in same virtual chain we can add the spreading codes for the particular antenna. 
% Hence, it would shows up in time-spliced samples post-digitization across both the virtual chains.
% Having multiple antennas for one virtual RF chain is straightforward, and can be done by supplying the particular spreading code to each antenna
% The key insight here is that since virtual RF chains are created by analog spreading-digital despreading, we can have antennas co-phased for one user to spread with the same code, so that they constructively add up in the virtual RF chain generated by that code.
% This way, we can have one virtual RF chain using a group of antenna beamforming towards it.
% Thus, we can beamform to the $N$ users separately via $N$ virtual RF chains, as shown towards right end of Fig. \ref{fig:intro_spread}. 
% A natural question here would be if $M$ antennas are split up amongst $N$ RF chains?
% We show that infact $2$ virtual RF chains can share the same antenna since the spreading codes are orthogonal, so we can add the spreading codes of the $2$ virtual RF chains for one antenna to make it appear in both the RF chains.
% Hence, this allows a many-to-many connection between the $M$ antennas and $N$ virtual RF chains, and effectively allows all the $N$ virtual chains to use the full array for beamforming.
% This captures the required goal of narrow beams by using $M>N$ antennas, while using $N$ virtual RF chains.
% can we share the $N$ virtual RF chains effectively across higher number of antennas to create the required narrow beams?

% The key insight here is that unlike a physical RF chain, which is created by laying the physical hardware to each antenna, virtual RF chains are an abstraction created by the spreading-despreading effect.
% So, in \name we can group many antennas by spreading them in a similar way, so the de-spreading operation gives a combined signal across all these antennas.
% Further, we show that since the spreading codes are orthogonal, a single antenna can be spread across two virtual RF chains as well.
% So, \name allows a many to many connection between $M$ antennas and $N$ virtual RF chains.
% This allows \name to group antennas strategically such that they perform approximate analog beamforming towards one user per virtual RF chain.
% The residual interference left is then cancelled digitally by inverting the channels and doing zero-forcing post-coding  (shown after de-spreading block, Fig. \ref{fig:intro_spread}).

% By addressing the challenges listed above, \name truly enables `user-proportionate' spatial multiplexing with $M$ antennas connected via the analog spreading network and a single $NB$ bandwidth RF chain.
% % Hence, the net power consumption of \name would be that of OFDMA + total power across the required analog spreading.
% % So, the last challenge in designing \name is how can the
% To design the analog network with ultra-low power consumption,we show that the required analog spreading operation can be achieved via simple RF switches toggling at strategically chosen $N$ distinct on-off codes, which give the required unique spreading for $N$ virtual RF chains.
% RF switches enable this at $<1$mW power draw, which is minimal compared to $100$'s of mW power draw of RF chains.
% This is not surprising, since in the field of backscatter communications, the same RF switches perform the frequency shifting operations at $\mu$W levels.


% Thus, to summarize, \name designs a new MIMO architecture which connects $M$ antennas to single RF chain of OFDMA via $M$ RF switches. \name basically creates $N$ virtual RF chain via analog spreading effect of RF switches, and de-spread digitally in the $NB$ bandwidth OFDMA RF chain. 
% \name also is a `flexible' architecture, it can create $N$ virtual RF chains on demand, so if there are lesser/more users it can adaptively reduce/increase the number of virtual chains.
% By being almost same power level as OFDMA, as well as using multiple antennas to create mMIMO like narrow beams, \name achieves both EE and SE. 
\todo{Improve last para}
We implement \name prototype with $M=8$ antennas to flexibly serve $2,3,4$ users. We test \name over multiple user positions in a conference room setting, as well as traditional MIMO and OFDMA baselines. Our key results include similar performance metrics with MIMO with $3\times$ less power requirements, achieving the same network capacity as compared to OFDMA with $4\times$ lesser spectrum requirements, which experimentally confirm the SE and EE claims.
At the same time, if there is a single MIMO capable user, \name can be used to serve multiple streams, and we show this by increasing throughput of single user by $3$ times.
Finally, we end with a case study on how \name can make various classes of base stations more energy efficient and cut down on power bills.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{new_figs/BM_fig.pdf}
%     \caption{How power consumption varies with number of users for freq. \& spatial multiplexing, with typical values of power consumption tabulated}
%     \label{fig:bm_fig_new}
% \end{figure*}

% and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.



% The main reason for MIMO not achieving EE is the requirement of separate RF chains for each antenna, and this issue 
% Taking a step towards breaking this SE-EE tradeoff, in this paper we present \name, which for the first time, shows an architecture which can maximize both SE and EE. 
% The key insight here is to add low-power analog circuitry to each antenna such that 
% The key insight which enables \name to do so, is that MIMO and OFDMA systems of today can be married together, by using configurable, low-power RF circuits per antenna, to get best of both worlds.
% The idea is to have the multiple MIMO `configurable' antennas combinedly share the single user-proportionate sampling bandwidth RF chain of OFDMA. 
% Each antenna in \name can be set to separate configurations to give unique identity to the antennas signal before they combine together and go through the RF chain.
% By isolating the signals based on the unique identity, \name can isolate the per-antenna signals in the digital domain.
% Hence, this approach basically creates a virtual signal path towards each separate antenna configuration in digital domain, and we dub this process as creation of `Virtual RF chains (VRF)'.
% These VRFs also allow for grouping of multiple antennas by setting them to same configurations, so $N$ virtual RF chains can effectively share $M>N$ antennas among themselves.
% This enables practical MIMO operation for $N$ interfering users, while harnessing advantages offered by $M>N$ antennas, and keeping power consumption to user-proportionate sampling level of single RF chain.
% % Hence, the concrete approach behind \name is that, to serve $N$ users in a user-proportionate power manner via $M>N$ antennas, \name creates $N$ `virtual RF chains' from a single physical RF chain sampled at $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power efficiency of OFDMA.

% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.

% The basic idea is that we can use the increased sampling bandwidth of a single RF chain to carve out virtual signal paths to each antenna in the digital domain, in a process dubbed as creation of `virtual RF chains'.
% This way \name is able to harness MIMO operation by laying a single physical RF chain, and abstracting out multiple virtual RF chains as demand-fit.
% Further, this process is done in an optimal user-proportionate manner where \name can club together multiple antennas in a single virtual RF chain to harness the gains of many more antennas than number of users and show practical MIMO operation in realistic environments.
% This basically allows the single RF chain to get `virtualized' over the many antennas, in the sense that all antennas share the same RF chain but have a separate virtual digital path created , which allows for creation of virtual RF chains in the digital domain.
% Further, by 
% This is made possible by a combined analog-digital antenna combining approach which ensures that the required benefits of many more antennas than number of users get 
% Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

% The first design consideration for \name is how to even realize this concept of a VRF? 
% To motivate this, we first show how that the desired behaviour from the configurable RF circuit is to create a `frequency spreading' effect, so that the $B$ bandwidth user signals get spread into $NB$ total bandwidth.
% However, a challenge here is that this spreading operation needs to be done with minimal power consumption, otherwise the net power requirements would end up being antenna proportionate as we need this circuit for each antenna.
% Hence, \name inspirchallengees from backscatter communication's RF-switches that create frequency shifts with minimal <100uW power requirements \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, when toggled with certain frequency on-off clock.

% This rules out naive solutions like RF mixers which can create the intended frequency spreading effect, but at expense of insertion losses and non-negligible power consumption.
% Instead, \name uses RF switches, which also are capable of creating these frequency shifts when toggled with a certain frequency on-off clock.
% Further, this operation has minimal power requirements, and similar RF switches have been used for channel shifting purposes in backscatter systems with <10uW power requirements that can also be made batteryless \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}.
% The concrete idea here is that, to serve $N$ users in a user-proportionate power manner,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power efficiency of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
% Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
% It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
% We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

% Next, we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ different antenna groups so as to enable the creation of $N$ virtual RF chains. 
% Thus, we can use RF switches to configure antennas on-off strategically to create VRFs. However, how exactly should we configure these switches such that we can create $N$ VRFs for $N$ different antenna groups?
% For this, we show how \name can create $N$ orthogonal on-off clocks having $B$ frequency, corresponding to user bandwidth and $1/N$ duty cycle each, but different initial phases.
% The idea is that a particular group of antennas antennas can be configured with one of these $N$ orthogonal on-off clocks, and signals of these antennas would get combined in the analog domain and get downconverted+digitized. 
% Then in digital domain the summed signals from these different antennas can be isolated from since these summed combined signals would have the unique clock marking them different from the other groups using the rest $N-1$ clocks.
% The key insight which allows separating these $N$ clocks from each other is that when
% these $N$ different $B$ frequency codes are sampled at $NB$ they show up at different sample indexes in time, and this allows \name to separate the VRFs set up by each of the $N$ unique on-off clocks.

% Finally, the last piece in the puzzle is how to select these $N$ different antenna groupings from the available $M$ antennas. One key feature of \name's VRFs is that it allows a many to many connection with antennas. That is, it not only allows us to turn on multiple antennas per VRF, we can also have one antenna showing up in multiple VRFs. This is because the clocks are orthogonal in time, and to have one antenna show up in two virtual chains, we can simply add two orthogonal clocks corresponding to the two VRFs. This allows \name to implement a switching matrix $\mathbf{S}$ in analog domain, which maps the user channels across $M$ antennas into $N$ user-proportionate VRFs. We also show a heuristic method, labelled as BABF, which beamforms towards one-user per VRF in order to enable practical user-proportionate MIMO.


% Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
% Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
% That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

% So far we have discussed how \name gets one antenna stream per virtual RF chain.
% But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
% A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
% Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
% Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


% To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
% The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
% In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
% Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
% \name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.




% Hence, massive MIMO ends up being  by having antenna proportionate power, as OFDMA can achieve the same goal by being user-proportionate.
% But, this comes at a cost of multiplicative increase in spectrum with OFDMA, which makes OFDMA power-inefficient.



% 


% Mainly these efficiency metrics can be either the traditionally considered spectral efficiency (bps per hertz) to advocate judicious use of spectrum, or energy efficiency
% both energy efficiency (bps per watt) and spectrum efficiency (bps per hertz). That is, in the coming decade, it is imperative to maximize both, how many bits can you communicate per watt usage, and number of bits packed in unit spectrum (Fig.). 



==> intros/intro_mumimo.tex <==
\section{Introduction}
% Crisp: users are growing, keep getting more spectrum
Over the past decade, wireless networks have become robust, widely deployed and have transformed the daily lives of human beings in immeasurable ways.
This has lead to a boom of consumer devices, smartphone, tablets, smart-watches, all of which utilize wireless connections like Wi-Fi or LTE.
As the adoption of the technology increases further, with internet of things potentially connecting even more devices wirelessly, today's wireless networks face a challenge to scale up with number of users, and manage this ever-increasing demand. 
We already see our Wi-Fi routers performance degrading as number of devices increase, with complaints of poor public Wi-Fi in malls, conference rooms, haunting the network designers  \cite{confwifi,wifimegamimo}. 
Similarly, LTE network struggles to keep up it's robust performance in high density areas, like concerts, airports and stadiums  \cite{ltecrowded}.

% Why the degradation, and the solution
One reason for this performance degradation has been that as number of devices in a network increase, they all compete for the communication resources, like spectrum. 
% In order to communicate in a multi-user network, users share these resources amongst themselves, either by not communicating in the same frequency band as other users, or holding back from transmitting in a time slot when other user is communicating.
A wireless protocol like Wi-Fi, or LTE has to strictly follow the spectrum guidelines from FCC, and they can not increase the spectrum arbitrarily to serve more users.
Thus, multi-user concurrent transmissions typically occupy different frequency bands in the allocated spectrum to prevent any interference between each other (Fig. \ref{fig:introfig1} (a)).
As number of devices in the network increase, with the spectrum kept constant, each communicating device gets lesser spectrum chunk for itself, and hence we see the performance degradation.
The only way to prevent this performance degradation is to somehow handle the interference caused by multiple users transmitting concurrently in the same frequency band.
% The most intuitive solution to this performance degradation is to add more spectrum to the network, which translates to more number of resources per user, and thus improved performance.
% However, adding spectrum is a tedious process, involving new protocol designs and FCC approvals.
% To prevent this network degradation, a way is to design wireless networks such that the network can handle multiple users transmitting concurrently.

% Need to add capacity without adding spectrum
Serving multiple interfering users forms the intended goal of digital beamforming and MU-MIMO approaches. % one to one
% Antennas are easy to put on base station
The basis of these approaches lie in leveraging multiple antennas to allow the creation of multiple independent spatial channels over the same frequency band, so that multiple users can utilize different spatial channels in order to communicate at the same time and frequency band.
Creation of multiple spatial channels in the same time-freqeuncy slot entails that mu-MIMO can bring about a multiplicative increase to the capacity and be a panacea to the multi-user scalability problem plaguing Wi-Fi.
Thus, in the WiFi 802.11ac protocol released back in 2016, mu-MIMO was introduced to commodity devices and was pitched to be a defining change for the future network design. 
However, mu-MIMO failed to deliver on the promise of the multiplicative gain, and infact there are reports that enabling mu-MIMO option in 802.11ac routers even leads to reduced performance as compared to a standard resource sharing model with single users occupying communication resources.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/intro_fig_1.pdf}
    \caption{Comparison of \name with current wireless networks. Due to creation of new fractional time-slots by fast switching, \name can serve multiple users operating over the same time slot and frequency band}
    \label{fig:introfig1}
\end{figure}

% mu MIMO failed collosally and massive mimo is too complex, what are the ways ahead
The key reason for this failure has been that the assumption that mu-MIMO can create independent spatial channels is not always possible. 
The capability to do so heavily depends on where the users are located, and there are user configurations where the channels are correlated and the mu-MIMO created spatial channels face a lot of cross-talk and leads to reduced performance.
At these user configurations, mu-MIMO would perform worse then single user resource sharing communication networks, and this has been reported both experimentally and in research.
People have tried to address this problem by designing intelligent user-grouping algorithms to select only those users in a group where mu-MIMO is able to create these spatial streams successfully without crosstalk \cite{}. However, the deployment of these algorithms in a real-life network with moving users with changing network statistics and the latency in deciding user groups ultimately hinders these efforts.

In contrast, \name addresses this problem by making mu-MIMO give spatial multiplexing gain for any possible user configuration. 
The insight \name has is to focus on the fundamentals of mu-MIMO, which is to utilize multiple antennas to increase the capacity.
The reason mu-MIMO fails to perform at particular user configurations is that the operating point for number of spatial streams is governed by number of antennas, that is with 4 antenna routers mu-MIMO tries to create 4 independent spatial channels.
Say if we have 8 antennas at our disposal, the task of creating 4 independent spatial channels would be more robust and work for arbitrary user configurations.
However, the current beamforming solutions are not scalable with number of antennas, as for each antenna we require a separate downconversion and sampling chain.
\name achieves this by designing a beamforming solution which scales well with number of antennas, by utilizing multiple antennas connected to just a single RF chain.

% Inspired from OFDMA assymetricity, we make a contribution towards increasing a new digital beamformer
% OFDMA inspired mu-MIMO



==> intros/intro_new_arch.tex <==
% !TEX root = paper.tex

\section{Introduction}\label{sec:intro}

% Spectrum is scarce, TDMA is slow
The massive adoption of wireless technologies has led to an ever increasing demand for serving more and more devices with never ending throughput demands.
The only way to do this scalably has been to serve only one device at a time, which reduces throughput or utilize non-overlapping frequency bands, which exacerbates demand for spectrum.
% The amount of devices connected to wireless networks has been blowing up as the networks become more accessible and robust. 
% Today on an average, a single person carries multiple devices connected to the same network, like a phone, tablet and smart watches.
% Thus, any wireless Access Point (AP) will almost always be connected to multiple devices.
% The easiest way for the AP to handle multiple connections is to put the multiple devices in different time slots or non-overlapping frequency bands.
% The first approach reduces throughput, whereas the second approach demands more spectrum.
% However, spectrum is a scarce resource, and thus to scale to the number of devices without trading off throughput, we need concurrent user transmissions without adding new spectrum.
% MIMO has tried to solve this exact issue, fails
Enabling spectrum efficient and concurrent multi user communications has been the core push behind mu-MIMO multiplexing technologies. mu-MIMO approaches do this by creating $K$ independent spatial streams in order to serve $K$ users by utilizing $K$ antennas. Each antenna samples the summed signal from the $K$ interfering users at different positions in space.
Creation of these spatial streams is almost akin to solving $K$ equations with $K$ variables, with these equations being what each $K$-th antenna samples and these variables being the $K$ users' signals.

% Thus, in order to serve $K$ users simultaneously, the radio needs to get the received samples from each antenna.
% The only approach we have today is to take the signal from each antenna and bring the signal to the radio via a RF chain.
% Each RF chain utilizes a downconverting mixer to map these RF signals to baseband, followed by sampling of this baseband signal by a ADC.
% Finally, these digitized baseband signals from these $K$ RF chains form these $K$ equations, which the radio solves to discern the users' signals. 
% This approach of utilizing $K$ antennas and $K$ RF chains is referred to as digital beamforming.

Thus, mu-MIMO has the potential to solve the spectrum crunch today's wireless networks face.
However, the technology has led to minimal adoptation.
The core reason has been that the earlier implementations (mu-MIMO mode in 802.11ac Wi-Fi) failed to delivering multiplicative gains entailed by enabling multi-user transmissions. 
This was because the $K$ equations $K$ variables example is too naive to work with real-life wireless channels. 
Often this system of equations turns out to be non-solvable, or in other words, the wireless channel is said to not have a full rank.
The way to mitigate this problem, and always serve $K$ users robustly, is to 
sample more number of equations with more antennas and have systems where $K_{\text{ant}}>K$ antennas serve $K$ users.

In order to utilize more antennas and alleviate these issues with mu-MIMO there have been two approaches,
Massive MIMO utilizing digital beamforming \cite{} and hybrid beamforming \cite{}.
Digital beamforming solves this problem by digitally sampling each antenna's received signal by means of a separate RF chain per antenna (Fig. \ref{fig:intro_arch} (a)).
A RF chain basically serves two purposes, first it downconverts the received antenna signals to baseband by a mixer, and then samples it digitally by using an ADC.
Thus in order to serve $K$ users, massive MIMO approaches require $K_{text{Ant}}>K$ number of antennas and RF chains.
On the other hand, in hybrid beamforming approaches, $K_{\text{Ant}}$ antennas are connected to only $K$ RF chains by an analog circuit (Fig. \ref{fig:intro_arch} (b)). 
Hybrid beamformers would design this circuit typically with a network of phase shifters, and the aim of this network is to transform the $K_{\text{Ant}}$ signals into $K$ effective signals in such a way that the created $K$ signals are full rank. Thus, hybrid beamformers serve $K$ users with $K_{\text{Ant}}$ antennas but using only $K$ RF Chains.
The main argument against digital beamformers remain the inefficiencies they bring in by serving lesser users than their net sampling capability. Hybrid beamformers optimize this by sampling only with $K$ RF chains, however require challenging analog design, dealing with imperfections and quantization noise as a result of operating in analog domain. This has led to these approaches mostly being studied theoretically, or with system level trace-driven emulations, and thus very few experimental implementations today, with only one known implementation at sub-6 bandwidths \cite{}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_arch.pdf}
    \caption{Comparison of standard multi-user beamforming architectures vs \name}
    \label{fig:intro_arch}
\end{figure}
% Digital beamformers typically 
% This leads multi-user approaches to a state of dichotomy, where we are not sure 

Thus, \name attempts to address this lacuna by designing a new architecture, which connects multiple antennas to a single RF chain via a network of RF switches which can toggle the antennas \emph{on}-\emph{off} (Fig. \ref{fig:intro_arch} (c)).
By toggling the antennas \emph{on}-\emph{off} across time, \name utilizes a very new concept of utilizing time as an alternate axis to space in order to create time-interleaved RF chains from a single physical RF chains. 
This allows \name to combine digitally amongst these virtual RF chains akin to how a digital beamformer does, albeit with just a single downconversion chain.
Further, since these virtual RF chains are emanating out of just a single downconversion chain, we can easily attach more number of antennas than these virtual RF chains, and use the switches as an analog combining network similar to how hybrid beamformers use phase shifters.
At the same time, by combining over these switched values networks over these time interleaved digital chains, allows \name to avoid issues which hybrid beamformers face with specialized analog design and quantization problems with the analog phase shifters.
To this end, \name utilizes RF switches, one of the most readily and low-powered hardware component, to create a  new immensely powerful architecture.

% Core concept of time combining

This leads to the first design principle of \name's new architecture, which is the creation of virtual RF chains interleaved across time.
The inspiration for this idea is simple, in \name architecture, if we switch one antenna \emph{on}, and other antennas \emph{off} for certain time samples, during those time samples we can discern the channel observed at that particular antenna.
At some other time samples, we can turn a second antenna \emph{on}, and observe the channel at the second antenna, and so on.
Thus, by turning individual antennas on-off in an antenna array, we can use the single wire \name to isolate the channels observed across multiple antennas (Fig. \ref{fig:intro_time_interleaved_rfcs}).
This draws a parallel to how digital beamforming observes individual antenna channels. 
What digital beamforming achieves by utilizing samples across the ADCs, sampling the antenna space directly, \name achieves though digital samples, interleaved across time by switching antennas \emph{on} and \emph{off}.
However, this requires the time interleaved signal to be oversampled by a factor of the desired spatial multiplexing gain required, since we need to fit that many signals into one oversampled stream.

Thus the second design principle of \name, is to utilize higher sampling bandwidth to procure the desired multiplexing gain. 
In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. 
\name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virt.pdf}
    \caption{Time interleaved virtual RF chains: An antenna array with RF switches, which turn each antenna on turn by turn and thus the single ADC samples the combined stream having antenna signals interleaved with each other}
    \label{fig:intro_time_interleaved_rfcs}
\end{figure}

Finally, the last design principle of \name's design is to utilize more number of antennas $K_{\text{Ant}}$ than number of virtual RF chains $K$, for robust multiplexing gains.
By hardening of multiplexing gains, we mean that in any $K$ user configuration possible, the multiplexing gain from \name architecture will be close to $K$.
However, the generalization to more number of antennas than RF chains is very difficult to implement with today's digital beamformers.
Unlike, the previous architectures, this $K_{\text{Ant}}>K$ generalization in \name architecture is very natural.
This is because the fundamental unit in digital beamformer was the downconverting mixer, whereas in hybrid beamformer we required a phase shifter in addition to the mixer to create the generalization.
In \name architecture, the humble RF switch behaves like both, it helps to create the digital streams in the first place by toggling in synch with the sampling clock, and now, the same switching network will also act as an analog combining network to toggle multiple antennas on for the same number of virtual RF chains.

Having $K_{\text{Ant}}>K$ antennas to toggle on-off for each these $K$ virtual chains allow us to strategically project the higher dimensional $K\times K_{\text{Ant}}$ channel $\mathbf{H}$ observed via each of the antennas for $K$ users, in order to harden the multiplexing gains from the $K$ virtual RF chains.
This is achieved by strategic choice of $K_{\text{Ant}}\times K$ binary switching matrix $\mathbf{S}$, which can be implemented accurately by \name's RF switch network connecting each of the $K$ virtual RF connected to $K_{\text{Ant}}$ antenna
to create an uncorrelated equivalent $K\times K$ channel $\mathbf{HS}$, which always allows for robust multiplexing gains across any spatial user configuration. This is also backed by our evaluation, where we see a drastic improvement when we utilize $K_{\text{Ant}}=8$ for $K=4$ users.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single wire interface at a higher sample rate to replicate what traditional digital beamformers typically do with multiple wire slower interfaces, at the same time avoiding requirement of multiple downconversion chains. Further, \name shows that such architectures are naturally generalizable to a hybrid architectures with more number of antennas than number of RF chains, which allows us to harden the multiplexing gains and thus enable robust mu-MIMO operation. We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users by utilizing a hybrid architecture.
% \name designs one of the most power-efficient muliplexing architectures possible, since \name utilizes just a single downconverting mixer, still at the same time, generating impressive multiplexing gains.
% This leads us to the the first design principle of \name, which is to overclock a single ADC instead of using multiple slower channel ADCs in order to generate multiplexing gain. 
% In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. 
% If we use just a single RF chain, if we keep the same sampling rate, this would lead to violation of information entropy.
% Thus, \name utilizes a $K$ times sampling bandwidth for the single ADC in its design, as compared to $K$ different ADCs sampling at lower rate as compared to digital beamforming. \name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
% We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.
% This allows \name's hybrid architectures to mimic what digital beamformers do, 

% However, to facilitate the formation of these $K$ independent spatial streams, a core requirement is on utilizing multiple antennas.
% Fundamentally, $K$ antennas allow sampling of spatial signals from $K$ positions, and these supporting $K$ RF chains then carry the information about these spatial streams to the radio.
% The radio finally processes these $K$ antenna streams, and intermixes them to discern the individual signals from $K$ different users in a technique called as digital beamforming. 
% It is almost akin to solving $K$ equations with $K$ variables, with these equations being what each antenna samples and these variables being each of the users' signals.


 

==> intros/intro_new_arch_v1.tex <==
% !TEX root = paper.tex

\section{Introduction}\label{sec:intro}
% to feature 
% Spectrum is scarce, TDMA is slow
The massive adoption of wireless technologies has led to an ever increasing demand for serving more and more devices with never ending throughput demands~\todo{Cite} . To meet these demands for each device, we could utilize non-overlapping frequency bands to serve each device (Frequency Division Multiple Access (FDMA)), which exacerbates the demand for scarce spectrum. Therefore, enabling spectrum efficient and concurrent multi-user communications has been the core push for the last decade. It is why Multiple Input Multiple Output (MIMO) multiplexing technologies were introduced\footnote{in 2011 for WiFi with 11 ac standard referred as mu-MIMO}, which uses the same spectrum to serve $K$ users by utilizing $K_{ant}$ antennas, i.e., create $K$ independent spatial streams, one for each user.  
During the concurrent uplink from $K$ users on the same spectrum, each antenna at the access point samples the summed signal from the $K$ users. With the $K_{ant}$, the access point resolves the signal of each of the $K$ user -- it is almost akin to using $K_{ant}$ equations  to resolve for $K$ variables -- each users signal as shown in Fig. xx, thus requiring $K_{ant}>K$. %With these equations being what each $K$-th antenna samples and these variables being the $K$ users' signals as shown in Fig. xx. 
Thus, $K_\text{ant}$ MIMO has the potential to solve the spectrum crunch today's wireless networks face. 

However, in practice the often deployed system has been the $K_{\text{ant}}=K$ MIMO (also referred as multi-user-MIMO (mu-MIMO)) which fails to consistently deliver multiplicative gains entailed by enabling multi-user transmissions. The core reason has been that often the $K$ antennas measure correlated channels between users, i.e. they do not provide independent measurement as theoretically conceived, thus making the system of K-equations and K-variables degenerate. In other words, often this system of equations turns out to be non-solvable, or the said wireless channel does not have a full rank. The way to mitigate this problem, and always serve $K$ users robustly, is to sample more number of equations with more antennas and have systems where $K_{\text{ant}}\gg K$ antennas to serve $K$ users, referred to as massive MIMO.

In order to realize massive MIMO and alleviate these issues with mu-MIMO, there have been two popular architectures: Massive MIMO utilizing digital beamforming \todo{Cite}  and hybrid beamforming \todo{Cite} . Digital beamforming solves this problem by digitally sampling each antenna's received signal by the means of a separate Radio Frequency (RF) chain per antenna (Fig. \ref{fig:intro_arch} (a)). An RF chain basically consists of two parts, first the received signals is downconverted from the received antenna to baseband using a mixer, and then sampled it digitally using an Analog-to-Digital Converter (ADC) with sampling-rate equivalent to bandwidth. The ADC samples from each of the $K_{\text{ant}}$ are processed via a signal processing network in digital domain to output the samples corresponding to each of the $K$ users. Digital beamformers needs to process large number of samples and down-stream it to only $K$ streams, instead of the sampled $K_{\text{ant}}$ streams. Thus, digital beamformers require first, many more RF chains (down-conversion and Local Oscillator (LO) distribution is extremely power hungry) compared to number of users, second requires sampling with many more ADC compared to number of users, and finally, requiring extensive compute to process these samples to only use at a later stage $K$ ADC equivalent samples, making them power-hungry and computationally expensive. Furthermore, digital beamformers lacks the flexibility, i.e., when channel is good -- one may not need as many antennas -- however majority of power is burnt in setting up the RF chains for the antennas.

On the other hand, the hybrid beamforming approaches minimizes the number of RF chains and signal processing complexity, by implementing the a part of the signal processing required to project $K_{\text{ant}}$ dimensional received signals onto $K$ streams in analog domain. Hence, in these architectures, $K_{\text{ant}}$ antennas are connected to an analog processing network which creates only $K$ outputs, which then requires only $K$ RF chains (Fig. \ref{fig:intro_arch} (b)), thus sampling rates equivalent to the number of users. 
Hybrid beamformers would design this analog circuit network typically with a network of phase shifters, and the aim of this network is to transform the $K_{\text{ant}}$ signals into $K$ output signals in such a way that the created $K$ output signals are full rank, or form a solvable system of equations. Thus, hybrid beamformers serve $K$ users with $K_{\text{ant}}$ antennas but using only $K$ RF Chains, saving on RF chains and signal processing computations compared to digital beamforming. However, hybrid beamformers require challenging analog design, which often only supports narrow-band, and ends up having a lot of insertion losses and imperfect due to limited resolution of phase-shifter which leads to quantization noises. Also, hybrid beamformers still require these $K$ RF chains, as the multiplexing gains are still provided only via the digital combining across these physically laid RF chains. 
% This has led to these approaches mostly being studied theoretically, or with system level trace-driven emulations, and thus few experimental implementations today \todo{Cite} .

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virtualization.pdf}
    \caption{Comparison of standard multi-user beamforming architectures vs \name}
    \label{fig:intro_arch}
\end{figure}
% Digital beamformers typically 
% This leads multi-user approaches to a state of dichotomy, where we are not sure 

% Thus, \name addresses this lacuna by designing a
In stark contrast to these two widely held methods, Time Interleaved Multiple Outputs (\name) designs a new class of architecture which can provide multiplexing gain while just requiring a single physically laid RF chain connected to a multi antenna array.
This is done by virtualizing the concept of having physical RF chains laid in space to be instead created in digital domain by interleaving samples across time.
This design choice of \name makes it a flexible architecture that can achieve digital beamforming without requiring extensive RF chains, and can flexible change the sampling rate to adapt number of virtual RF chains as per demand and thereof computation to save energy. At the same time \name can mimic a hybrid beamformer creating samples equivalent to number of user and utilizing more number of antennas without exacerbating signal processing costs. 

\name achieves this with a simple architecture, wherein it connects multiple antennas to a single RF chain via a network of simple analog RF switches which can toggle the antennas \emph{on}-\emph{off} synchronized with ADC's sampling rate(Fig. \ref{fig:intro_arch} (c)). To this end, \name utilizes RF switches, one of the most readily and low-powered hardware component, to create a new immensely powerful architecture, with a single downconversion chain -- saving on the analog power consumption. 
By synchronized toggling of the antennas \emph{on}-\emph{off} across time with ADC sampling (in MHz), \name develops a simple yet powerful concept of utilizing time axis to capture the space axis -- essentially creating time-interleaved RF chain for all antennae from a single physical RF chains.
This allows \name to combine digitally amongst these virtual RF chains akin to how a digital beamformer does, albeit with just a single downconversion chain -- requiring no LO distribution and multiple mixers operating at GHz frequencies.
Further, since these virtual RF chains are emanating out of just a single downconversion chain, we can easily attach more number of antennas with switches in analog domain, and create these virtual RF chains. 
Finally, by combining over the switched values, choosing multiple antennae to be on or off, we create a analog combining network, over these time interleaved digital chains, allows \name to achieve networks like hybrid beamformers and also avoid issues of hybrid beamformers by flexibly choosing higher sampling rate as necessary for the channel, eliminating fixed K chains requirement. % face with specialized analog design and quantization problems with the analog phase shifters.

% Core concept of time combining

This leads to the first design principle of \name's new architecture, which is the creation of virtual RF chains interleaved across time.
The inspiration for this idea is simple, in \name architecture, if we switch one antenna \emph{on}, and other antennas \emph{off} for certain time samples, during those time samples we can discern the channel observed at that particular antenna.
At some other time samples, we can turn a second antenna \emph{on}, and observe the channel at the second antenna, and so on.
Thus, by turning individual antennas on-off in an antenna array, we can use the single wire \name to isolate the channels observed across multiple antennas (Fig. \ref{fig:intro_time_interleaved_rfcs}).
This draws a parallel to how digital beamforming observes individual antenna channels. 
What digital beamforming achieves by utilizing samples across the ADCs, sampling the antenna space directly, \name achieves though digital samples, interleaved across time by switching antennas \emph{on} and \emph{off}.
However, this requires the time interleaved signal to be oversampled by a factor of the desired spatial multiplexing gain required, since we need to fit that many signals into one oversampled stream.

Thus the second design principle of \name, is to utilize higher sampling bandwidth to procure the desired multiplexing gain. 
In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. 
\name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virt.pdf}
    \caption{Time interleaved virtual RF chains: An antenna array with RF switches, which turn each antenna on turn by turn and thus the single ADC samples the combined stream having antenna signals interleaved with each other}
    \label{fig:intro_time_interleaved_rfcs}
\end{figure}

Finally, the last design principle of \name's design is to utilize more number of antennas $K_{\text{ant}}$ than number of virtual RF chains $K$, for robust multiplexing gains.
By hardening of multiplexing gains, we mean that in any $K$ user configuration possible, the multiplexing gain from \name architecture will be close to $K$.
However, the generalization to more number of antennas than RF chains is very difficult to implement with today's digital beamformers.
Unlike, the previous architectures, this $K_{\text{ant}}>K$ generalization in \name architecture is very natural.
This is because the fundamental unit in digital beamformer was the downconverting mixer, whereas in hybrid beamformer we required a phase shifter in addition to the mixer to create the generalization.
In \name architecture, the humble RF switch behaves like both, it helps to create the digital streams in the first place by toggling in sync with the sampling clock, and now, the same switching network will also act as an analog combining network to toggle multiple antennas on for the same number of virtual RF chains.

Having $K_{\text{ant}}>K$ antennas to toggle on-off for each these $K$ virtual chains allow us to strategically project the higher dimensional $K\times K_{\text{ant}}$ channel $\mathbf{H}$ observed via each of the antennas for $K$ users, in order to harden the multiplexing gains from the $K$ virtual RF chains.
This is achieved by strategic choice of $K_{\text{ant}}\times K$ binary switching matrix $\mathbf{S}$, which can be implemented accurately by \name's RF switch network connecting each of the $K$ virtual RF connected to $K_{\text{ant}}$ antenna
to create an uncorrelated equivalent $K\times K$ channel $\mathbf{HS}$, which always allows for robust multiplexing gains across any spatial user configuration. This is also backed by our evaluation, where we see a drastic improvement when we utilize $K_{\text{ant}}=8$ for $K=4$ users.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single wire interface at a higher sample rate to replicate what traditional digital beamformers typically do with multiple wire slower interfaces, at the same time avoiding requirement of multiple downconversion chains. Further, \name shows that such architectures are naturally generalizable to a hybrid architectures with more number of antennas than number of RF chains, which allows us to harden the multiplexing gains and thus enable robust mu-MIMO operation. We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users by utilizing a hybrid architecture.
% \name designs one of the most power-efficient muliplexing architectures possible, since \name utilizes just a single downconverting mixer, still at the same time, generating impressive multiplexing gains.
% This leads us to the the first design principle of \name, which is to overclock a single ADC instead of using multiple slower channel ADCs in order to generate multiplexing gain. 
% In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. 
% If we use just a single RF chain, if we keep the same sampling rate, this would lead to violation of information entropy.
% Thus, \name utilizes a $K$ times sampling bandwidth for the single ADC in its design, as compared to $K$ different ADCs sampling at lower rate as compared to digital beamforming. \name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
% We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.
% This allows \name's hybrid architectures to mimic what digital beamformers do, 

% However, to facilitate the formation of these $K$ independent spatial streams, a core requirement is on utilizing multiple antennas.
% Fundamentally, $K$ antennas allow sampling of spatial signals from $K$ positions, and these supporting $K$ RF chains then carry the information about these spatial streams to the radio.
% The radio finally processes these $K$ antenna streams, and intermixes them to discern the individual signals from $K$ different users in a technique called as digital beamforming. 
% It is almost akin to solving $K$ equations with $K$ variables, with these equations being what each antenna samples and these variables being each of the users' signals.


 

==> intros/intro_new_arch_v2.tex <==
% !TEX root = paper.tex

\section{Introduction}\label{sec:intro}
% to feature 
% 

% Spectrum is scarce, TDMA is slow
The massive adoption of wireless technologies has led to an ever increasing demand for serving more and more devices with never ending throughput demands~\cite{araujo2016massive, hoydis2013massive}. To meet these demands for each device with scarce spectrum, multi-user MIMO (mu-MIMO) technologies were introduced, which had potential to enable spectrum efficient and concurrent multi-user communications~\cite{liu2012downlink, castaneda2016overview}. The idea was simply to use the same spectrum to serve $K$ users by utilizing $M = K$ antennas, i.e., create $K$ independent spatial streams, one for each user. However, in practice this $M=K$ MIMO system%(also referred as multi-user-MIMO (mu-MIMO)) 
has failed to consistently deliver multiplicative gains entailed by enabling multi-user transmissions. The core reason has been that often the $M$ antennas have correlated channels for users, i.e. they do not provide independent channels as theoretically conceived, thus making the system of $M=K$-equations (antennas) and $K$-variables (user signal) degenerate. In other words, often this system of equations turns out to be non-solvable, or the said wireless channel does not have a full rank. 

The way to mitigate this problem, and always serve $K$ users robustly, is to sample many more number of equations (more antennas) and have systems where $M\gg K$ antennas to serve $K$ users, referred to as massive MIMO. The challenge with enabling massive MIMO is multiple Radio Frequency (RF) chains and supporting much higher sampling rate and computation thereof. A popular architecture for Massive MIMO utilizes digital beamforming \cite{ding2020agora, araujo2016massive}, as shown in Fig. \ref{fig:intro_arch} (a). Digital beamforming uses separate RF chain per antenna, followed by an ADC sampling. RF chains require an Local Oscillator (LO) at GHz frequencies, which is fed to mixer which downconverts the signal. %An RF chain basically consists of two parts, first the received signals is downconverted from the received antenna to baseband using a mixer, and then sampled it digitally using an Analog-to-Digital Converter (ADC) with sampling-rate equivalent to bandwidth. 
% The multiple RF chains required are power-hungry, as they need to distribute LO and then perform downconversion for each antenna \cite{mondal201825}\todo{Cite more}. Furthermore, the ADC samples from each of the $M$ antenna are processed via a signal processing network in digital domain to output the samples corresponding to each of the $K$ users. 
%Digital beamformers needs to process large number of samples and down-stream it to only $K$ streams, instead of the sampled $M$ streams. 
As a consequence of $M\gg K$, digital beamformers require first, many more RF chains (down-conversion and LO distribution is extremely power hungry) compared to number of users, second requires sampling with many more ADC compared to number of users, and finally, requiring extensive compute to process these samples to only use at a later stage $K$ ADC equivalent samples, making them power-hungry and computationally expensive \cite{mondal201825,mondal201725,mondal201921,barati2020energy}. Furthermore, digital beamformers lacks the flexibility, i.e., when channel is good -- one may not need as many antennas -- however majority of power is burnt in setting up the RF chains for the antennas. 
% \todo{Power-hungry is used 4 times in this paragraph, make it concise.}

%% move to related work: 
% On the other hand, the hybrid beamforming approaches minimizes the number of RF chains and signal processing complexity, by implementing the a part of the signal processing required to project $K_{\text{ant}}$ dimensional received signals onto $K$ streams in analog domain. Hence, in these architectures, $M$ antennas are connected to an analog processing network which creates only $K$ outputs, which then requires only $K$ RF chains (Fig. \ref{fig:intro_arch} (b)), thus sampling rates equivalent to the number of users. Hybrid beamformers would design this analog circuit network typically with a network of phase shifters, and the aim of this network is to transform the $K_{\text{ant}}$ signals into $K$ output signals in such a way that the created $K$ output signals are full rank, or form a solvable system of equations. Thus, hybrid beamformers serve $K$ users with $K_{\text{ant}}$ antennas but using only $K$ RF Chains, saving on RF chains and signal processing computations compared to digital beamforming. However, hybrid beamformers require challenging analog design, which often only supports narrow-band, and ends up having a lot of insertion losses and imperfect due to limited resolution of phase-shifter which leads to quantization noises. Also, hybrid beamformers still require these $K$ RF chains, as the multiplexing gains are still provided only via the digital combining across these physically laid RF chains. 
% This has led to these approaches mostly being studied theoretically, or with system level trace-driven emulations, and thus few experimental implementations today \todo{Cite} .

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virtualization.pdf}
    \caption{Standard multi-user beamforming arch. vs \name}
    % \vspace{3pt}
    \label{fig:intro_arch}
\end{figure}
% Digital beamformers typically 
% This leads multi-user approaches to a state of dichotomy, where we are not sure 

% Virtual RF Chain here
In stark contrast to the previous Massive MIMO approches, we present Time Interleaved Multiple Outputs (\name), a new class of architecture for base-station/access points that can provide multiplexing gain while \emph{just requiring a single physically laid RF chain} connected to a multi antenna array, thereby saving on energy (shown in Fig. 1b). 
\name achieves this by virtualizing the concept of having physical RF chains per antenna, and instead creates virtual RF chains in digital domain by interleaving samples across time (Fig. \ref{fig:intro_time_interleaved_rfcs}). 
This virtualization is made possible by toggling the antennas \emph{on}-\emph{off} synchronized with receiver's sampling ADC (Fig.~\ref{fig:intro_arch}(b)), by utilizing RF switches connected to each antenna. 
RF switches are one of the most readily and lowest-powered hardware component, which helps \name create a new immensely powerful architecture, with a single downconversion chain -- saving on the analog power consumption. 
By synchronized toggling of the antennas \emph{on}-\emph{off} across time with ADC sampling (in MHz), \name develops a powerful concept of utilizing time axis to capture the space axis -- essentially creating time-interleaved RF chain for capturing all antennas from a single physical RF chain.
This allows \name to combine digitally amongst these virtual RF chains akin to how a digital beamformer does, albeit with just a single downconversion chain -- requiring no LO distribution and multiple mixers operating at GHz frequencies.

Because of the virtualization of physically laid RF chains, \name becomes a highly flexible architecture that on one end, can achieve a fully digital beamforming without requiring extensive downconversion chains, and on other end, can flexibly change the sampling rate to adapt the number of virtual RF chains as per demand and thereof computation to save energy. 
Finally, \name can also generalize very easily to a large number of $M$ antennas connected to fewer $K$ virtual RF chains, by mimic analog combining of $M>K$ signals from each of the antennas, to form $K$ output signals summed from different antennas combination, before being sampled in digital domain for virtual RF chain creation. 
% This cuts down on number of ADC samples while utilizing increased dimensionality given by large number of antennas, without exacerbating signal processing costs, to generate necessary multiplexing gains to serve all the users. 
This allows \name to achieve networks like hybrid beamformers~\cite{kim201828,kuhne2020bringing,ghasempour2018multi,xie2015hekaton} and also avoid issues of hybrid beamformers by flexibly choosing higher sampling rate as necessary for the channel, eliminating fixed K physical RF chains requirement. % face with specialized analog design and quantization
% virtual RF chain

% Virtual RF chain enables both digital and analog
% BABF now
In order to implement this combining when $M>K$, \name makes a key observation, which is to utilize analog networks where they work the best, viz. increasing of signal power, and digital combiners where they work the best, viz. combining signals with accurate phase and wideband operation to cancel interference. To this end, we present a binarized analog beamforming (BABF) algorithm, which utilizes the constructive combining gains from multiple antennas per virtual RF chain, and thus creates an uncorrelated digital channel which the digital beamformer abstraction then utilizes to kill the interference to almost noise floor (Fig. \ref{fig:raw_ofdm_svg}), enabling very robust spectrally efficient multi-user communications.
%  problems with the analog phase shifters.

% Further, since these virtual RF chains are emanating out of just a single downconversion chain, we can easily attach more antennas with switches in analog domain, to scale well with the number of antennas and allows \name to tap into the increased antennas dimensionality. 
% BABF algorithm ....

% Core concept of time combining
% Thus, in summary, \name designs a powerful new beamforming architecture to generate spatially multiplexed signals.
% This is essentially based on the two design principles in \name architecture. 
% First, \name virtualizes the concept of a physically laid RF chain by utilizing time interleaved samples as it's virtual RF chain.
% This is achieved by synchronised on-off switching of a particular antenna for certain time samples, during those time samples we can discern the channel observed at that particular antenna (Fig. \ref{fig:intro_time_interleaved_rfcs}).
% This draws a parallel to how digital beamforming observes individual antenna channels using physically laid RF chains.
% However, in order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single physical RF chain. 
% However, this requires the time interleaved signal to be oversampled by the desired spatial multiplexing gain required, since we need to fit that many signals into one oversampled stream.

% The second design principle of \name, is to utilize higher sampling bandwidth to procure the desired multiplexing gain, and virtualize different beamforming strategies. 
% \name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
% We show the mathematical analysis of this step of creating virtual RF chains by utilizing a single higher sampling ADC accompanied by synchronously switching antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers, as well as hybrid beamforming architectures which utilize more number of antennas than RF chains. 
% The equivalence is made possible because the circuit element which gives us capability to do digital beamforming, viz. the RF switch can generalize very naturally to a hybrid architecture, made possible by turning multiple of these antennas on-off appropriately.
% This allows \name to utilize constructive combining across the multiple antennas receiving in-phase signals, by turning these set of antennas to be on, in an algorithm we refer to as Binarized Analog Beamforming (BABF).
% Essentially, we employ a binarized variant of the analog beamforming solution which allows us to increase signal power for one user per virtual RF chain.
% This breaks channel correlations between users in the virtual RF chains, as one user is co-phased per slot via BABF, and hence, \name enjoys very robust multiplexing gains courtesy of utilizing more number of antennas than number of users, at the same time keeping the sampling requirements to be same.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{intros/intro_virt_v2.pdf}
    \caption{Equivalence of TIMO's virtual RF chains with traditional MIMO's physical RF chains: TIMO uses a single ADC with 4x sampling rate and a network of RF switches that interleave the signal from each antenna over smaller time units. This creates 4 virtual RF chains which can provide the digital samples of 4 antennas equivalent to mu-MIMO system with four physical low-sampling ADCs. {\footnotesize (Figure better read in color)}
    \vspace{5pt}
    % develops Time interleaved virtual RF chains: An antenna array with RF switches, which turn each antenna on turn by turn and thus the single ADC samples the combined stream having antenna signals interleaved with each other \todo{Clearly distinguish with Traditional approach. Even explain high sampling ADC in this Figure.}
    }
    \label{fig:intro_time_interleaved_rfcs}
\end{figure}

% Finally, the last design principle of \name's design is to utilize more number of antennas $M$ than number of virtual RF chains $K$, for robust multiplexing gains.
% By hardening of multiplexing gains, we mean that in any $K$ user configuration possible, the multiplexing gain from \name architecture will be close to $K$.
% However, the generalization to more number of antennas than RF chains is very difficult to implement with today's digital beamformers.
% Unlike, the previous architectures, this $M>K$ generalization in \name architecture is very natural.
% This is because the fundamental unit in digital beamformer was the downconverting mixer, whereas in hybrid beamformer we required a phase shifter in addition to the mixer to create the generalization.
% In \name architecture, the humble RF switch behaves like both, it helps to create the digital streams in the first place by toggling in sync with the sampling clock, and now, the same switching network will also act as an analog combining network to toggle multiple antennas on for the same number of virtual RF chains.

% Having $M>K$ antennas to toggle on-off for each these $K$ virtual chains allow us to strategically project the higher dimensional $K\times M$ channel $\mathbf{H}$ observed via each of the antennas for $K$ users, in order to harden the multiplexing gains from the $K$ virtual RF chains.
% This is achieved by strategic choice of $M\times K$ binary switching matrix $\mathbf{S}$, which can be implemented accurately by \name's RF switch network connecting each of the $K$ virtual RF connected to $M$ antenna
% to create an uncorrelated equivalent $K\times K$ channel $\mathbf{HS}$, which always allows for robust multiplexing gains across any spatial user configuration. This is also backed by our evaluation, where we see a drastic improvement when we utilize $M=8$ for $K=4$ users.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single wire interface at a higher sample rate to replicate what traditional digital beamformers typically do with multiple wire slower interfaces, at the same time avoiding requirement of multiple downconversion chains. Further, \name shows that such architectures are naturally generalizable to a hybrid architectures with more number of antennas than number of RF chains, which allows us to harden the multiplexing gains and thus enable robust mu-MIMO operation. We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with \todo{$4$ times} less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users by utilizing a hybrid architecture.
% \name designs one of the most power-efficient muliplexing architectures possible, since \name utilizes just a single downconverting mixer, still at the same time, generating impressive multiplexing gains.
% This leads us to the the first design principle of \name, which is to overclock a single ADC instead of using multiple slower channel ADCs in order to generate multiplexing gain. 
% In order to get a spatial multiplexing gain of $K$, we would need to create $K$ virtual RF chains, thus requiring us to accommodate $K$ times sampling of a single RF chain. 
% If we use just a single RF chain, if we keep the same sampling rate, this would lead to violation of information entropy.
% Thus, \name utilizes a $K$ times sampling bandwidth for the single ADC in its design, as compared to $K$ different ADCs sampling at lower rate as compared to digital beamforming. \name creates virtual RF chains over time using just a single physical RF chain, similar to how digital beamforming approaches utilize multiple physical RF chains by having multiple slower clocked ADCs.
% We analyze this step of creating virtual RF chains by utilizing a single higher sampling ADCs accompanied by switchable antennas, and show that by controlling RF switches appropriately, we can have an equivalence between \name and slower clocked digital beamformers. This is also backed up by our hardware evaluation results, that is, ceteris paribus, we get similar performances from both these approaches, even though \name is far less hardware intensive as the standard approach, requiring just a single physical RF chain.
% This allows \name's hybrid architectures to mimic what digital beamformers do, 

% However, to facilitate the formation of these $K$ independent spatial streams, a core requirement is on utilizing multiple antennas.
% Fundamentally, $K$ antennas allow sampling of spatial signals from $K$ positions, and these supporting $K$ RF chains then carry the information about these spatial streams to the radio.
% The radio finally processes these $K$ antenna streams, and intermixes them to discern the individual signals from $K$ different users in a technique called as digital beamforming. 
% It is almost akin to solving $K$ equations with $K$ variables, with these equations being what each antenna samples and these variables being each of the users' signals.


 

==> intros/intro_roshan.tex <==
% !TEX root = paper.tex

\section{Introduction}
\label{sec:intro}

% power efficiency while saving spectrum
Current wireless systems contribute as high as 1.4\% of global carbon footprint. 
In comparison, aviation industry has a footprint of 2\%. 
So, the wireless systems industry is aiming to reduce this footprint by 45\% by 2030, by optimizing for power consumption ~\cite{ish,link}.
This is going to be a gargantuan task, with billions of more devices getting connected ~\cite{billions,devices} and increasing data rate trends ~\cite{data,trends}.
% As seen recently, 
Thus the wireless systems are going to face a challenging time to reduce power consumption to target while keeping up the with data rates while to add new users/devices.
% Hence, there is a requirement to develop a communication system that can keep up with the data rates while adding new users, in a gr 
The easiest way to address this challenge is to add new spectrum to the mix.
But spectrum is scarce, expensive and needs to be utilized in an efficient way~\cite{recent,fcc,aviation,fight}.
Hence, the need of the hour is to figure out a way to add users and maintaining data rates, while optimizing both spectrum-efficiency and power consumption.


% Energy + Spectrum
% But how do we go by optimizing for power consumption? 
In the current systems, like WiFi6's OFDMA~\cite{xx} the increasing users are served by slicing the fixed aggregate spectrum into multiple slices that serve each user. 
While, this makes the system need constant power to process the fixed amount of spectrum making it power efficient it would lead to low-data rates per user leading to spectrum inefficiency.
On the other hand, there is an increasing research towards Massive MIMO systems for serving large number of users (let's say $N$) by deploying larger antenna arrays ($N_{\text{ant}} > N$) on the base station to utilize the spectrum efficiently~\cite{massive,mimo,papers}. 
These multi-antenna ($N_{\textit{ant}}$) Massive MIMO arrays would in turn require $N_{\textit{ant}}$ individual RF front end processing chains (RF-chains), which would increase the overall power consumption by $N_{\textit{ant}}\times$~\cite{massive,mimo,power,consumption,papers}.
Additionally, while the OFDMA system needs to backhaul $N$ data-streams for serving $N$ users, the $N_{\textit{ant}}$ Massive MIMO system would need to backhaul $N_{\textit{ant}}$ data streams for serving $N$ users. This additional $N_{ant}$ backhualing ends up using compute power inefficiently.
Thus, a \textit{Green} communication system to reduce the carbon footprint needs to be (1) Spectrum efficient, (2) Compute power efficient, and (3) Power Efficient at the front-end design. 
\todo{should we consider scalability or flexibility?}

While, there has been research towards hybrid-beamforming~\cite{beamforming,works} that tries to solve for power-spectrum trade-off, they only meet the first two requirements of the three. 
These hybrid architectures basically, connect $N_{\textit{ant}}$ to $N$ RF-chains via analog circuits and feedback only $N$ streams to efficiently use compute. 
The analog circuits are typically network of phase shifters, and the phases are set such that the combined $N$ streams getting backhauled permit the creation of $N$ spatial streams.
However, these hybrid beamformers optimize only for the compute power consumption by reducing the number of backhaul streams but do not optimize for the front end RF-chain power consumption as they would still require $N$ physical RF-chains.
Hence, even with the most ideal hybrid beamformer, for let's say $8$ user system, we would require 1x spectrum, 8x RF front end power and 8x sampling+compute power. 
In this paper, we ask a question if the golden goose system can push this to the lowest of limits, i.e. serving $8$ users with 1x spectrum, 1x RF front end power and 8x sampling+compute power.

This golden goose communication system would be most power efficient, where all the power consumption is just happening to get the data bits across.
In order to serve $8$ users, $8$x sampling+compute power can not be reduced further to avoid info-theoretic implications; we cant get more data rate without getting more digital bits sampled and processed.
However the golden goose system eliminates any other inefficient power consumption; by optimizing for compute as well as front end power consumption.
Taking a step towards realization of this golden goose system, in this paper we present \name, which meets these stringent requirements by developing a system which utilizes just a single RF chain (to justify 1x RF front end power), at the same time handling $N$ users communicating simultaneously on the same spectrum.

They key-insight which allows \name to come up with such single RF chain design is to marry the concepts of OFDMA with that of massive MIMO.
The essential idea is that \name creates $N$ virtual RF chains from a single physical RF chain's sampled bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power benefits of OFDMA's single physical RF-chain design.
Fundamentally, as shown in Figure~\ref{fig:comingup} if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
We enable this $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.
% This draws a parallel to OFDMA, in that it samples $NB$ spectrum and gives interference-free $B$ bandwidth slices to $N$ individual users. 
% Similarly \name uses a single RF chain which abstracts out slices of the sampled $NB$ bandwidth to $N$ antennas serving $N$ users, thus consuming only 1x RF front end power.

% This design principle of creating these $N$ virtual RF-chains by providing $N$ distinct frequency shifts to each antenna's $B$ bandwidth RF-signal such that they occupy different parts of the sampled $NB$ bandwidth, leads to the following key technical challenges 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virtualization.pdf}
    \caption{\name architecture with a single RF chain \todo{Draft from previous submission}}
    % \vspace{3pt}
    \label{fig:intro_arch}
\end{figure}

The important question that now arises is how one can provide these $N$ distinct frequency shifts across $N$ antennas without consuming $N\times$ the power to justify our $1\times$ RF front end power claim. 
To answer this, \name takes an inspiration from backscatter communication, where RF-switches have been popularly used to perform similar frequency shifts to signals, with minimal to no additional power requirements.
The insight here is that with $NB$ sampled bandwidth, we can create $N$ different phase frequency shifts of $B$ bandwidth, such that each antenna's signal has a discernable frequency shift.
This enables \name to recover the $N$ antenna signals from the $NB$ sampled single RF chain, allowing capability to handle $N$ users with just 1x RF front end power.

Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
That is, if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

So far we have discussed how \name gets one antenna stream per virtual RF chain.
But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
Although this satisfies 1x spectrum requirements, nearly 1x front end consumption, it will have ($N_{\text{ant}}$)x compute+sampling.
Here, \name borrows design elements from hybrid beamforming literature and generalize our virtual RF chains to utilize more than one antenna per virtual chain, to make the compute power requirements Nx as well by creating only $N$ virtual RF chains to serve $N$ users.
% With $N_{\text{ant}}>N$ generalization, we observe another advantage of the virtual RF chain design. 
% \name capitalizes on the fact that unlike physically laid RF chains which are connected to one antenna at a time, our virtual RF chains are connected to all the antennas simultaneously.
% % Thus, unlike a physical RF chain, which is one antenna per chain, \name's architecture allows connecting multiple antennas per virtual RF chain seamlessly.
% That is, we can have a $N_{\text{ant}}$ \name architecture, with $N$ virtual RF chain, and each virtual RF chain is connected to all the $N_{\text{ant}}$ antennas.

To do so, \name designs a algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
In BABF, we figure out the maximal group of antennas which are \emph{in-phase} for a particular user, and turn this group `on' via the switches implementing frequency shifts for that particular virtual RF chain, in effect beamforming towards that user.
\emph{By beamforming one user per RF chain, instead of one antenna per RF chain}, we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
\name architecture to do so demands only 1x spectrum, 1x RF front end power and $N$x compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.

\todo{From the old intro right now, will update after evals are done} Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be both green, and adapt to averse channel conditions upon demand by scaling up resources.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.

% The current systems either optimize for only power (OFDMA) or only the spectrum (massive MIMO).
% For example consider how base stations would serve 8 users today.
% In OFDMA, the total spectrum requirements would be 8x, and the base station would sample these spectrum slices.
% On the other hand, in massive MIMO, spectrum requirements would be 1x, however, the base station would need to sample 8x spatial streams, instead of 8x spectrum slices.
% Sampling $8$ spatial streams requires multi-antenna architectures, with more than $8$ antennas, whereas sampling interference free spectrum slices requires just $1$ antenna.
% Say as an example, massive MIMO does this with 16 antennas.
% Thus, the power requirements for massive MIMO, would be 16x power of sampling streams as compared to OFDMA, which samples from a single antenna.
% Worse, massive MIMO also needs digital demodulation and processing blocks for these 16 streams from 16 antennas to serve 8 users, in comparison to processing just the 8x spectrum streams as with OFDMA, being 2x worse even on data processing power requirements.

% In summary, we can see that today there's a huge power cost associated with being spectrum efficient: both in terms of additional hardware requirement, and signal processing stemming from multi-antenna architectures.

% In OFDMA, total spectrum required would be 200 MHz, with each user occupying a narrow 20 MHz slice of the spectrum.


% Besides being most energy efficient, the base-stations are required to support multiple users. An interesting is observation is that most energy efficient base stations, however, end up being spectrally inefficient or low data-rate when supporting multi-users.
% That is, the best scenario for the base station is to have the users in non-overlapping frequency bands, called Frequency Division Multiple Access (FDMA) more popularly OFDMA in cellular context. The base station can just sample the parts of bandwidths where user's are transmitting. Often this approach provide reliable non-interfering channels but leads to either spectrum inefficiency or low-data rate.

==> intros/intro_roshan_v1.tex <==
% !TEX root = paper.tex

\section{Introduction}
\label{sec:intro}

% power efficiency while saving spectrum
Current wireless systems contribute as high as 1.4\% of global carbon footprint, close to aviation industry that has a footprint of 2\%. Therefore, the wireless industry is aiming to reduce this footprint by 45\% by 2030, by optimizing for energy consumption ~\cite{ish,link}. 
This is going to be a gargantuan task even with advancements in efficient radio designs, with billions of more devices getting connected ~\cite{billions,devices} and increasing data rate trends ~\cite{data,trends}.
% As seen recently, 
Thus the wireless systems, more specifically, the next generation base-stations are going to face a challenging time to reduce energy footprint to meet the target, while keeping up the with data rates to add new users/devices. 
% Hence, there is a requirement to develop a communication system that can keep up with the data rates while adding new users, in a gr 
Hence, the need of the hour is to develops base-stations that are ideal or green i.e., 1) figure out a way to add users and maintaining data rates for each user, while optimizing both spectrum-efficiency and power consumption 2) flexible and Scale-able, the energy consumption is proportional to the amount of data communicated.  


% Energy + Spectrum
% But how do we go by optimizing for power consumption? 
To achieve a green communication system, a straight forward way for base-stations to keep up is by adding new spectrum to support more users and maintaining data-rate and leverage radio design enhancements in sub-6 GHz to reduce energy consumption\footnote{mmwave and THz spectrum tend to be not reliable i.e. easily blocked by blockage and mobility}. However spectrum is scarce in sub-6 GHz, and expensive and needs to be utilized in an efficient way~\cite{recent,fcc,aviation,fight}. 
For example, in WiFi6's OFDMA~\cite{xx} the increasing users are served by slicing the fixed aggregate spectrum into multiple slices that serve each user, providing a narrow slice of non-interfering channel. While, this makes the AP need constant energy to process the fixed number of users of spectrum making it energy efficient, but it would lead to low-data rates per user, which can be referred to leading to spectrum inefficiency. 

To overcome the limited spectrum per user, there is an increasing trend towards Massive MIMO systems for serving large number of users (let's say $N$) concurrently over entire spectrum by deploying larger antenna arrays ($N_{\text{ant}} > N$) on the base station and create spatially non-interfering channels to serve each user, thus providing  spectrum efficiency~\cite{massive,mimo,papers}. However, these multi-antenna ($N_{\textit{ant}}$) Massive MIMO arrays results in extreme energy in-efficiency and lacks flexibility. First, massive MIMO would in turn require $N_{\textit{ant}}$ individual (radio) RF front end processing chains (RF-chains), which would increase the overall power consumption by $N_{\textit{ant}}\times$~\cite{massive,mimo,power,consumption,papers}. An ideal green system should only need to perform computation and typically backhaul only $N$ data-streams for serving $N$ users, but the Massive MIMO system would need to backhaul and compute on $N_{\textit{ant}} >> N $ data streams for serving $N$ users. Furthermore, the backhaul and compute of the data, doesn't reduce even if the number of users are reduced in the system (reduced antenna leads to loosing the degree of freedom). Thus, the additional $N_{ant}$ backhualing ends up using compute power inefficiently.

% \todo{should we consider scalability or flexibility?}

% While, there has been research towards hybrid-beamforming~\cite{beamforming,works} that tries to solve for power-spectrum trade-off, they only meet the first two requirements of the three. 
% These hybrid architectures basically, connect $N_{\textit{ant}}$ to $N$ RF-chains via analog circuits and feedback only $N$ streams to efficiently use compute. 
% The analog circuits are typically network of phase shifters, and the phases are set such that the combined $N$ streams getting backhauled permit the creation of $N$ spatial streams.
% However, these hybrid beamformers optimize only for the compute power consumption by reducing the number of backhaul streams but do not optimize for the front end RF-chain power consumption as they would still require $N$ physical RF-chains.
% Hence, even with the most ideal hybrid beamformer, for let's say $8$ user system, we would require 1x spectrum, 8x RF front end power and 8x sampling+compute power. 
% In this paper, we ask a question if the golden goose system can push this to the lowest of limits, i.e. serving $8$ users with 1x spectrum, 1x RF front end power and 8x sampling+compute power.

The green communication system would be most power efficient, where all the power consumption is proportional to amount of data moved across the system. %happening to get the data bits across.
Next, the green communication system should minimize the power consumption of the RF-chains to a minimal and constant, instead of $N\times$ consumption, a fixed value, which would be amortized by increasing $N$. 
% However the golden goose system eliminates any other inefficient power consumption; by optimizing for compute as well as front end power consumption.
Taking a step towards realization of the green communication system, in this paper we present \name, which meets all these stringent requirements by developing a system which utilizes just a single RF front-end chain (constant 1x RF front end power consumption), at the same time supporting data-rate of $N$ users communicating simultaneously on the entire spectrum concurrently. By supporting N users, we mean it can enable $N$ non-interfering channels over the entire spectrum. Furthermore, \name achieves green communication system, where it can serve $N$ users on entire spectrum, with just $N\times$ sampling+compute power, which can not be reduced further to avoid info-theoretic implications; we cannot get more data rate without getting more digital samples processed. Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus increasing energy/power consumption with increasing users. 

The first key challenge for \name is to achieve (constant $1\times$ RF front end power consumption) while supporting the massive MIMO architecture. 
They key-insight which allows \name to come up with such single RF chain design is to marry the concepts of OFDMA with that of massive MIMO. Intuitively, it maps different spatial directions/users on the spectrum to non-overlapping frequencies very much like OFDMA. More accurately,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO while enjoying power benefits of OFDMA's single physical RF-chain design.
Fundamentally, as shown in Figure~\ref{fig:comingup} if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
We enable this $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.
% This draws a parallel to OFDMA, in that it samples $NB$ spectrum and gives interference-free $B$ bandwidth slices to $N$ individual users. 
% Similarly \name uses a single RF chain which abstracts out slices of the sampled $NB$ bandwidth to $N$ antennas serving $N$ users, thus consuming only 1x RF front end power.

% This design principle of creating these $N$ virtual RF-chains by providing $N$ distinct frequency shifts to each antenna's $B$ bandwidth RF-signal such that they occupy different parts of the sampled $NB$ bandwidth, leads to the following key technical challenges 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/greenmo_intro_fig.pdf}
    \caption{\name architecture puts forward a best of both worlds communication architecture: As power efficient as OFDMA and as spectrum efficient as Massive MIMO}
    % \vspace{3pt}
    \label{fig:intro_arch}
\end{figure}

The important question that now arises is how one can provide these $N$ distinct frequency shifts across $N$ antennas without consuming $N\times$ the power to justify our $1\times$ RF front end power claim. 
To answer this, \name takes an inspiration from backscatter communication, where RF-switches have been popularly used to perform similar frequency shifts to signals, with minimal to no additional power requirements.
The insight here is that with $NB$ sampled bandwidth, we can create $N$ different phase frequency shifts of $B$ bandwidth, such that each antenna's signal has a discernable frequency shift.
This enables \name to recover the $N$ antenna signals from the $NB$ sampled single RF chain, allowing capability to handle $N$ users with just $1\times$ RF front end power.

Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
That is, if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

So far we have discussed how \name gets one antenna stream per virtual RF chain.
But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
Although this satisfies 1x spectrum requirements, nearly 1x front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
Here, instead \name  generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennae. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}>> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}>> N$) and the compute power requirements of $N\times$.
% With $N_{\text{ant}}>N$ generalization, we observe another advantage of the virtual RF chain design. 
% \name capitalizes on the fact that unlike physically laid RF chains which are connected to one antenna at a time, our virtual RF chains are connected to all the antennas simultaneously.
% % Thus, unlike a physical RF chain, which is one antenna per chain, \name's architecture allows connecting multiple antennas per virtual RF chain seamlessly.
% That is, we can have a $N_{\text{ant}}$ \name architecture, with $N$ virtual RF chain, and each virtual RF chain is connected to all the $N_{\text{ant}}$ antennas.

To perform the mapping of antenna or antennae to virtual RF chains, \name designs a algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
In BABF, we figure out the maximal group of antennas which are \emph{in-phase} for a particular user, and turn this group `on' via the switches implementing frequency shifts for that particular virtual RF chain, in effect beamforming towards that user.
\emph{By beamforming one user per RF chain, instead of one antenna per RF chain}, we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
\name architecture to do so demands only 1x spectrum, 1x RF front end power and $N\times$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.

\todo{From the old intro right now, will update after evals are done} Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be both green, and adapt to averse channel conditions upon demand by scaling up resources.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4\times$ less hardware requirements, achieving the same network capacity as compared to FDMA with $4\times$ lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.

% The current systems either optimize for only power (OFDMA) or only the spectrum (massive MIMO).
% For example consider how base stations would serve 8 users today.
% In OFDMA, the total spectrum requirements would be 8x, and the base station would sample these spectrum slices.
% On the other hand, in massive MIMO, spectrum requirements would be 1x, however, the base station would need to sample 8x spatial streams, instead of 8x spectrum slices.
% Sampling $8$ spatial streams requires multi-antenna architectures, with more than $8$ antennas, whereas sampling interference free spectrum slices requires just $1$ antenna.
% Say as an example, massive MIMO does this with 16 antennas.
% Thus, the power requirements for massive MIMO, would be 16x power of sampling streams as compared to OFDMA, which samples from a single antenna.
% Worse, massive MIMO also needs digital demodulation and processing blocks for these 16 streams from 16 antennas to serve 8 users, in comparison to processing just the 8x spectrum streams as with OFDMA, being 2x worse even on data processing power requirements.

% In summary, we can see that today there's a huge power cost associated with being spectrum efficient: both in terms of additional hardware requirement, and signal processing stemming from multi-antenna architectures.

% In OFDMA, total spectrum required would be 200 MHz, with each user occupying a narrow 20 MHz slice of the spectrum.


% Besides being most energy efficient, the base-stations are required to support multiple users. An interesting is observation is that most energy efficient base stations, however, end up being spectrally inefficient or low data-rate when supporting multi-users.
% That is, the best scenario for the base station is to have the users in non-overlapping frequency bands, called Frequency Division Multiple Access (FDMA) more popularly OFDMA in cellular context. The base station can just sample the parts of bandwidths where user's are transmitting. Often this approach provide reliable non-interfering channels but leads to either spectrum inefficiency or low-data rate.

==> intros/intro_sigcom_v1.tex <==
% !TEX root = ../paper.tex

\section{Introduction}\label{sec:intro}

Current wireless systems have a very high carbon footprint of 1.4\% , close to aviation industry that has a footprint of 2\%. So, the wireless industry is aiming to reduce this footprint by 45\% by 2030, by optimizing for energy consumption ~\cite{footprint1,footprint2}. 
This is going to be a gargantuan task even with advancements in efficient radio designs, with billions of more devices getting connected ~\cite{sinha2021state} and increasing data rate trends ~\cite{sharma2021review}.
Thus the wireless systems, more specifically, the next generation base-stations will face a challenging time reducing energy footprint to meet the target, while keeping up with data rates to add new users/devices. 
Hence, the need of the hour is to develop base-stations that are ideal or green i.e., figure out a way to add users and maintaining data rates for each user, (1) while optimizing for both spectrum and power (2) being flexible and Scale-able, so the energy consumption is proportional to the amount of data communicated.  


To achieve a green communication system, a straight forward way for base-stations to keep up is by adding new spectrum to support more users and maintaining data-rate and leverage radio design enhancements in sub-6 GHz to reduce energy consumption\footnote{mmwave and THz spectrum tend to be not reliable i.e. easily blocked by blockage and mobility}. However spectrum is scarce in sub-6 GHz, and expensive and needs to be utilized in an efficient way~\cite{fcc1,fcc2}. 
For example, in WiFi6's OFDMA~\cite{wifi6} the increasing users are served by slicing the fixed aggregate spectrum into multiple slices that serve each user, providing each user a narrow slice of non-interfering channel. 
While, this makes the AP need constant energy to process the fixed number of users, it would lead to low-data rates per user, which defeats the purpose of spectrum efficiency. 

To overcome the limited spectrum per user, there is an increasing trend towards Massive MIMO systems for serving large number of users (let's say $N$) concurrently over entire spectrum by deploying larger antenna arrays ($N_{\text{ant}} > N$) on the base station and create spatially non-interfering channels to serve each user, thus providing  spectrum efficiency~\cite{ding2020agora,yan2019performance,araujo2016massive, hoydis2013massive,liu2012downlink, castaneda2016overview}. However, these multi-antenna ($N_{\textit{ant}}$) Massive MIMO arrays results in extreme energy in-efficiency and lacks flexibility. 
First, massive MIMO would in turn require $N_{\textit{ant}}$ individual (radio) RF front end processing chains (RF-chains), which would increase the overall power consumption by $N_{\textit{ant}}\times$~\cite{mondal201825,mondal201725,mondal201921,barati2020energy}. 
Additionally, an ideal green system should only need to perform computation and typically backhaul only $N$ data-streams for serving $N$ users. 
However, the Massive MIMO system would need to backhaul and compute on $N_{\textit{ant}} >> N $ data streams for serving $N$ users. 
Finally, the backhaul and compute of the data, doesn't reduce even if the number of users are reduced in the system (as reduced antennas lead to loosing the degree of freedom). Thus, the additional $N_{ant}$ backhualing ends up using compute power inefficiently.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{intros/Presentation2.pdf}
    \vspace{-15pt}
    \caption{\name puts forward best of both worlds: (a) As power efficient as OFDMA and (b) as spectrum efficient as Massive MIMO}
    \vspace{5pt}
    \label{fig:intro_arch}    
\end{figure*}

An ideal green communication system should be most power efficient, where all the power consumption is proportional to amount of data moved across the system. 
Next, the green communication system should minimize the power consumption of the RF-chains to be minimal and constant (or $O(1)$), instead of on the orders of the number of users (or $O(N)$ for $N$ users).
% consumption, a fixed value, which would be amortized by increasing $N$. 
Taking a step towards realization of the green communication system, in this paper we present \name, which meets all these stringent requirements by developing a system which utilizes just a single RF front-end chain (constant $O(1)$ RF front end power consumption), at the same time supporting data-rate of $N$ users communicating simultaneously on the entire spectrum concurrently. By supporting $N$ users, we mean it can enable $N$ non-interfering channels over the entire spectrum. Furthermore, \name achieves green communication system, where it can serve $N$ users on entire spectrum, with just $N\times$ sampling+compute power, which can not be reduced further to avoid info-theoretic implications. That is we cannot get more data rate without getting more digital samples processed. Furthermore, \name is flexible, i.e. with decreasing users the compute and sampling is reduced proportionally as well, thus maintaining constant power consumption with decreasing users. 

The first key challenge for \name is to achieve (constant $O(1)$ RF front end power consumption) while supporting the massive MIMO architecture. 
The key-insight which allows \name to come up with a single RF chain design is the amalgamation of the concepts of OFDMA with that of massive MIMO. Intuitively, it maps different spatial directions/users on the spectrum to non-overlapping frequencies very much like OFDMA. More accurately,  \name creates $N$ virtual RF chains from a single physical RF chain's sampled at appropriate $N\times$ bandwidth to deliver the spectral efficiency of massive MIMO (Fig. ~\ref{fig:intro_arch}(b)) while enjoying power benefits of OFDMA's single physical RF-chain design (Fig. ~\ref{fig:intro_arch}(a)).
Fundamentally, as shown in Fig. ~\ref{fig:intro_arch}(c) if antennas are receiving a signal of $B$ bandwidth spectrum, \name's intuition is to fit $N$ antenna signals of $B$ bandwidth each across the $NB$ sampled single RF chain.
It is important to note here that the over the air spectrum received by the antenna is of bandwidth $B$ and the net sampled bandwidth is $NB$. 
We thus enable $N$ virtual RF-chain creation by providing $N$ distinct frequency shifts to each antenna's RF-signal such that they occupy different parts of the sampled $NB$ bandwidth.

No we need to figure out how one can provide these $N$ distinct frequency shifts across $N$ antennas without consuming $O(N)$ the power to justify our $O(1)$ RF front end power claim. 
To do this, \name inspires from backscatter communication's RF-switches that create frequency shifts to signals \cite{zhang2016hitchhike,zhang2017freerider,dunna2021syncscatter,liu2020vmscatter,kellogg2014wi}, with minimal to no additional power requirements.
Thus with $NB$ sampled bandwidth, we can create $N$ different phase frequency shifts of $B$ bandwidth each, such that each antenna's signal has a discernable frequency shift.
This enables \name to recover the $N$ antenna signals from the $NB$ sampled single RF chain, allowing capability to handle $N$ users with just $O(1)$ RF front end power.

Additionally, this intuitive design choice of employing RF switches combined with configurable sampling rate to virtualize the concept of an RF chain, makes \name a highly flexible architecture.
Thus, by varying the sampling and switching frequencies of the architecture, \name can increase/decrease the number of RF chains on the fly, allowing \name to flexibly adjust to the user conditions.
That is, unlike existing Fig. ~\ref{fig:intro_arch}(c) solutions if the user load decreases, \name can automatically reduce the number of RF chains to flexibly meet the new demands.
% In comparison, the solutions which used multiple physical RF chains (massive MIMO) would end up burning power in the laid down RF chains as they can not flexibly increase/decrease the number of physical RF chains.

So far we have discussed how \name gets one antenna stream per virtual RF chain.
But, with $N$ antennas and $N$ virtual RF chains we can not serve $N$ users in a robust manner.
A naive solution here would be to do $N_{\text{ant}}>N$ antennas and create $N_{\text{ant}}$ virtual RF chains, so that we can borrow from massive MIMO solutions employing this many physical RF chains, to robustly serve $N$ users.
Although this satisfies $O(1)$ spectrum requirements and nearly $O(1)$ front end consumption, it will have ($N_{\text{ant}}\times$) compute+sampling.
Here, instead \name generalizes our virtual RF chains, where a virtual RF chain can utilize or connect or combine to one or more antennas. Thus, \name uses the generalized concept to create only $N$ virtual RF chains to serve $N$ users, but still continuing to leverage ($N_{\text{ant}}> N$) antennas. Thus achieving both spatial diversity of ($N_{\text{ant}}> N$) and the compute power requirements of $O(N)$.


To perform the mapping of antennas to virtual RF chains, \name designs an algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this virtual hybrid beamforming with simple $0-1$ RF switches.
The key idea is that, \name uses $N_{\text{ant}}$ antennas per virtual RF chains, to beamform towards one user per virtual RF chain, instead of isolating per-antenna signals via the virtual RF chain.
In BABF, we strategically switch the antennas to \emph{beamform to one user per RF chain, instead of one antenna per RF chain}. 
Thus we show that we can serve $N$ same frequency band users with $N_{\text{ant}}$ antennas and $N$ virtual RF chains.
\name architecture to do so demands only $O(1)$ spectrum, $O(1)$ RF front end power and $O(N)$ compute+sampling power, being the first green architecture which can keep up with the power and spectrum efficiency requirements of the new decade.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be green and drastically cut down both on RF front end power as well as sampling+compute power.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $3\times$ less power requirements, achieving the same network capacity as compared to FDMA with $4\times$ lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.


==> intros/intro_software.tex <==
\section{Introduction}

% Energy as a required parameter
As wireless systems move to the new decade, there are new approaches to expand the coverage and make the systems more flexible.
For example, there is a lot of push towards portable base stations on drones/trucks, using LEO satellites as wireless backhaul in the sky, smaller de-centralized base stations on homes' rooftops; instead of conventional specialized base stations located sparsely across the major population bottlenecks.
Since these new portable base-stations need to be powered either via batteries, in case of drones, or hybrid solar+battery powered in case of satellites and rooftops, the energy consumption metrics of base stations becomes a critical parameter.
Further, with the turn of new decade, even the conventionally located base station are required to be green and not guzzle up a lot of power.

% Energy + Spectrum
The most energy efficient base stations, however, end up being spectrally inefficient when supporting multi-users.
That is, the best scenario for the base station is to have the users in non-overlapping frequency bands, called Frequency Division Multiple Access (FDMA), and then, the base station can just sample the parts of bandwidths where user's are transmitting.
However, with increasing density of deployment and scarce spectrum, this is not a practical scenario.
% transition better 
Often the base stations need to handle multiple users communicating simultaneously on the same spectrum.
This has been typically addressed via massive MIMO approaches, which utilize signal processing techniques to use multiple antennas for handling multiple users with same spectrum.

Although massive MIMO is most spectrally efficient, it fails to meet power efficiency.
% Massive MIMO's core concept is to utilize spatial degrees of freedom furnished by a multi-antenna architecture.
Effectively, each antenna in a massive MIMO architecture brings about a new spatial degree of freedom, which provides capability to handle multiple users transmitting on same spectrum.
In order to capture each degree of freedom from an antenna, it ends up setting up dedicated hardware, referred to as `RF Chains', to downconvert the RF signal received at the antenna and then sample it digitally to make the antennas' degrees of freedom available for signal processing tasks.
This requirement of multiple RF chains to capture enough degrees of freedom needed to handle multiple users makes massive MIMO power inefficient.
In comparison, FDMA has frequency separated users, so it doesn't need to capture the required degrees of freedom to perform the additional signal processing, and hence can just use a single RF chain being highly power-efficient.

In addition to being power-inefficient, massive MIMO schemes ends up being highly inflexible as compared to FDMA.
When number of users decrease in the network, FDMA can choose to flexibly reduce the sampling to parts of spectrum still occupied, and this can be controlled easily via software. 
In comparison, massive MIMO systems would end up burning power to capture the required degrees of freedom via the network of RF chains, and the number of these RF chains can not be controlled via software as these are physically laid hardware, and not an abstraction unlike the parts of spectrum being sampled in case of FDMA.
Thus, FDMA is highly power-efficient and flexible communications architecture; but at a cost of required spectrum resources, which are scarce.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virtualization.pdf}
    \caption{\name architecture with a single RF chain \todo{Draft from previous submission}}
    % \vspace{3pt}
    \label{fig:intro_arch}
\end{figure}

% and then perform signal processing to isolate each user's signal from the received interfered signals.
% Key reasons: Flexibility+channel conditions
% power
% The key reason why massive MIMO fails to meet energy efficiency metrics 

% The key reasons why massive MIMO fails to meet the power efficiency metrics is that the process of serving multiple users requires cancelling of the interfering signals, and the efficacy of this largely depends on the underlying channel conditions.
% Theoretically, the optimum point of operation would be to have $N$ antennas in a MIMO system to serve $N$ users, but because of averse channel consitions, massive MIMO ends up requiring $N_{\text{ant}}>N$ to serve $N$ users.
% In order to capture signals from $N_{\text{ant}}$ antennas, massive MIMO has to lay dedicated hardware to each antenna, referred to as `RF chains'.
% Thus, to serve $N$ users, massive MIMO has to first, deal with power consumption from $N_{\text{ant}}$ RF chains, and second, the digital signal processing required of these $N_{\text{ant}}$ data streams.

% flexibility
% If the number of users decrease from $N$, or if the channel conditions become favorable to not actually need $N_{\text{ant}}$ RF chains, the massive MIMO solution becomes over-designed and inflexible, with the power getting burnt in the physically laid RF chains.
% In comparison, FDMA has $N$ frequency separated users, and now the base station would require just a single RF chain and signal processing would sample the $N$ data streams, and the system can also reduce the sampling if number of users decrease without wasting power.

% our solution
Looking ahead to green communications and new avenues of flexible wireless coverage requiring portable base stations, it is the need of the hour to devise a communication system which is as, power efficient and flexible as FDMA, and as spectrum efficient as massive MIMO.
In this paper, we present \name, which is the first multi-antenna architecture to address these challenges. 
The key insight which makes \name come up with such an architecture is to not capture the antennas' degrees of freedom via physical RF chain, 
and instead, virtualize the creation of RF chains over frequency domain. 
In other words, \name basically aims to creates many virtual RF chains over the sampled spectrum, from a singly laid physical RF chain.
This allows \name to effectively behave like FDMA; requiring just a single physically laid RF chains, and controlling the sampled spectrum on the fly. 
By choosing to alter the sampling rate \name can flexibly increase/decrease the number of virtual RF chains created in response to channel conditions and number of users.
At the same time \name does not demand users to be separated in frequency domain, and it handles the interfering users by performing signal processing over the virtualized RF chains.
Thus, \name 
% is both, a spectrally efficient, as well as a power efficient multi-user architecture, which 
will pave the way ahead of how base-stations can optimize the power consumption and open doors to new portable deployments.

% how our solution works
A natural question is, how \name actually virtualizes the concept of a physically laid RF chain? 
A physically laid RF chain connected to an antenna essentially amplifies the weak signal at antenna, downconverts it and finally digitizes it for signal processing ahead.
\name utilizes an architecture where all antennas are connected via a singly laid RF chain, allowing for hardware reuse, and simultaneous downconversion and digitization of all the antenna signals in one go.

But, in this process the individual antenna signals get combined with each other, and this won't allow capturing of per-antenna degrees of freedom required for interference suppression, so how does \name get back the degrees of freedom from the combined antenna signals?
To do so, \name utilizes RF switches connected to each antenna, in order to create different \emph{on-off} signatures for each antenna, which gives the signals from each antenna a discernable identity allowing them to be separated from each other via simple digital signal processing in software.
% RF switches are extremely low-powered circuit elements, and have been used 

% application: green
Thus, \name utilizes a switched-antenna array design connected to a single physically laid RF chain, with capability to create multiple virtual RF chains at a software level, making it an extremely flexible architecture.
In contrast, Massive MIMO today is niether flexible; nor as power-efficient as \name.
Another problem with massive MIMO today is the huge amount of data which is backhauled to software, or prcoessed on ASICs/FPGA for isolating the per-user's signals.
Beyond saving a lot of power consumption as compared to traditional multi-user techniques, by hardware reuse of the single RF chain across antennas, \name also optimizes on the amount of data backhauled for MIMO signal processing.
By optimizing both the energy consumption, as well as required data backhauling, \name creates a truly green architecture.

% \name also brings forth the only architecture which can simultaneously enable two applications: first, using only $N$ digital streams to serve $N$ users, and second, in very averse channel conditions, flexibly increase the sampling rate to keep on serving $N$ users in a robust manner.

% coarse 0-1 beamforming at RF
% fine beamfo
Massive MIMO requires having number of antennas $N_{\text{ant}}>N$ users, so that the captured degrees of freedom far exceed number of users to allow robust interference suppression. 
Hence, in order to get the $N$ per-user streams, baseband samples of $N_{\text{ant}}>N$ have to be backhauled and processed.
Alternately, an ASIC has to process these $N_{\text{ant}}$ streams in hardware, to backhaul only the $N$ processed per-user streams.
Either way, there is a tradeoff of massive data transfer, or massive processing requirement on the base-station.

Unlike Massive MIMO, in order to tap into the increased spatial degrees of freedom from an antenna, \name architecture does not require a dedicated RF chain.
\name capitalizes on the fact that unlike physically laid RF chains which are connected to one antenna at a time, our virtual RF chains are connected to all the antennas simultaneously.
Thus, unlike a physical RF chain, which is one antenna per chain, \name's architecture allows connecting multiple antennas per virtual RF chain seamlessly.
That is, we can have a $N_{\text{ant}}$ \name architecture, with $N$ virtual RF chain, and each virtual RF chain is connected to all the $N_{\text{ant}}$ antennas.
Thus, we can essentially backhaul only the baseband samples corresponding to $N$ virtual RF chains, while using $N_{\text{ant}}$ antennas to serve $N$ users; to optimize the amount of data utilized for signal processing

The key insight \name has here, to utilize multiple antennas per virtual RF chain, is to use these $N_{\text{ant}}$ antennas to beamform towards one user per virtual RF chains, instead of isolating per-antenna signals via the virtual RF chain.
That is, instead of keeping one antenna on per virtual RF chain, we can turn on all the antennas which are \emph{in-phase} for one user in that particular virtual RF chain.
Since we sample $N$ streams for $N$ users, we have $N$ virtual RF chains and thus we can use this method to beamform towards one user per virtual RF chain.
\name designs a simple algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this beamforming with simple $0-1$ RF switches.
\emph{By prioritizing one user per RF chain, instead of one antenna per RF chain}, we show that serving $N$ same frequency band users with just $N$ digital streams, is indeed possible.

Similar to \name, hybrid beamformers also aim to use $N_{\text{ant}}>N$ antennas connected to $N$ physically laid RF chains via analog circuits, analog beamforming + digital combining in order to address green communications.
However, first, these are fixed deployments, which are not flexible unlike \name.
Second, multi-user interference cancellation is a very channel dependent process, and there will be some channels where it won't be possible for hybrid architectures to perform as well as full digital architectures which sample.
Thus there will be some off-cases where it won't be possible to serve users with just $N$ sampled digital streams.
Unlike hybrid beamformers, by varying the sampling rate, \name can go from a hybrid architecture, to a fully digital architecture; 
Thus we keep on supporting the $N$ users reliably without overdesigning for worst case, or coming up with a fixed design to work well on average but fail to guarantee the quality of service.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be both green, and adapt to averse channel conditions upon demand by scaling up resources.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.

==> intros/intro_software_v1.tex <==
\section{Introduction}

% Energy as a required parameter
As wireless systems move to the new decade, there are new approaches to expand the coverage and make the systems more flexible. For example, there is a lot of push towards portable base stations on drones/trucks, smaller de-centralized base stations on homes' rooftops; instead of conventional specialized base stations located sparsely across the major population bottlenecks, and even using LEO satellites as wireless backhaul in the sky.
Since these new portable base-stations need to be powered either via batteries, in case of drones, or hybrid solar+battery powered in case of satellites and rooftops, the energy consumption metrics of base stations becomes a critical parameter.
Further, with the turn of new decade, even the conventionally located base station are required to be green and not guzzle up a lot of power.

% Energy + Spectrum
Besides being most energy efficient, the base-stations are required to support multiple users. An interesting is observation is that most energy efficient base stations, however, end up being spectrally inefficient or low data-rate when supporting multi-users.
That is, the best scenario for the base station is to have the users in non-overlapping frequency bands, called Frequency Division Multiple Access (FDMA) more popularly OFDMA in cellular context. The base station can just sample the parts of bandwidths where user's are transmitting. Often this approach provide reliable non-interfering channels but leads to either spectrum inefficiency or low-data rate. 

However, with increasing density of deployment and scarce spectrum, this is not a practical scenario.
% transition better 
Often the base stations need to handle multiple users communicating simultaneously on the same spectrum.
This has been typically addressed via massive MIMO approaches, which utilize signal processing techniques to use multiple antennas for handling multiple users with same spectrum.

Although massive MIMO is most spectrally efficient, it fails to meet power efficiency.
% Massive MIMO's core concept is to utilize spatial degrees of freedom furnished by a multi-antenna architecture.
Effectively, each antenna in a massive MIMO architecture brings about a new spatial degree of freedom, which provides capability to handle multiple users transmitting on same spectrum.
In order to capture each degree of freedom from an antenna, it ends up setting up dedicated hardware, referred to as `RF Chains', to downconvert the RF signal received at the antenna and then sample it digitally to make the antennas' degrees of freedom available for signal processing tasks.
This requirement of multiple RF chains to capture enough degrees of freedom needed to handle multiple users makes massive MIMO power inefficient.
In comparison, FDMA has frequency separated users, so it doesn't need to capture the required degrees of freedom to perform the additional signal processing, and hence can just use a single RF chain being highly power-efficient.

In addition to being power-inefficient, massive MIMO schemes ends up being highly inflexible as compared to FDMA.
When number of users decrease in the network, FDMA can choose to flexibly reduce the sampling to parts of spectrum still occupied, and this can be controlled easily via software. 
In comparison, massive MIMO systems would end up burning power to capture the required degrees of freedom via the network of RF chains, and the number of these RF chains can not be controlled via software as these are physically laid hardware, and not an abstraction unlike the parts of spectrum being sampled in case of FDMA.
Thus FDMA is highly power-efficient and flexible communications architecture; but at a cost of required spectrum resources, which are scarce.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{intros/intro_virtualization.pdf}
    \caption{\name architecture with a single RF chain \todo{Draft from previous submission}}
    % \vspace{3pt}
    \label{fig:intro_arch}
\end{figure}

% and then perform signal processing to isolate each user's signal from the received interfered signals.
% Key reasons: Flexibility+channel conditions
% power
% The key reason why massive MIMO fails to meet energy efficiency metrics 

% The key reasons why massive MIMO fails to meet the power efficiency metrics is that the process of serving multiple users requires cancelling of the interfering signals, and the efficacy of this largely depends on the underlying channel conditions.
% Theoretically, the optimum point of operation would be to have $N$ antennas in a MIMO system to serve $N$ users, but because of averse channel consitions, massive MIMO ends up requiring $N_{\text{ant}}>N$ to serve $N$ users.
% In order to capture signals from $N_{\text{ant}}$ antennas, massive MIMO has to lay dedicated hardware to each antenna, referred to as `RF chains'.
% Thus, to serve $N$ users, massive MIMO has to first, deal with power consumption from $N_{\text{ant}}$ RF chains, and second, the digital signal processing required of these $N_{\text{ant}}$ data streams.

% flexibility
% If the number of users decrease from $N$, or if the channel conditions become favorable to not actually need $N_{\text{ant}}$ RF chains, the massive MIMO solution becomes over-designed and inflexible, with the power getting burnt in the physically laid RF chains.
% In comparison, FDMA has $N$ frequency separated users, and now the base station would require just a single RF chain and signal processing would sample the $N$ data streams, and the system can also reduce the sampling if number of users decrease without wasting power.

% our solution
Looking ahead to green communications and new avenues of flexible wireless coverage requiring portable base stations, it is the need of the hour to devise a communication system which is as, power efficient and flexible as FDMA, and as spectrum efficient as massive MIMO.
In this paper, we present \name, which is the first multi-antenna architecture to address these challenges. 
The key insight which makes \name come up with such an architecture is to not capture the antennas' degrees of freedom via physical RF chain, 
and instead, virtualize the creation of RF chains over frequency domain. 
In other words, \name basically aims to creates many virtual RF chains over the sampled spectrum, from a singly laid physical RF chain.
This allows \name to effectively behave like FDMA; requiring just a single physically laid RF chains, and controlling the sampled spectrum on the fly. 
By choosing to alter the sampling rate \name can flexibly increase/decrease the number of virtual RF chains created in response to channel conditions and number of users.
At the same time \name does not demand users to be separated in frequency domain, and it handles the interfering users by performing signal processing over the virtualized RF chains.
Thus, \name 
% is both, a spectrally efficient, as well as a power efficient multi-user architecture, which 
will pave the way ahead of how base-stations can optimize the power consumption and open doors to new portable deployments.

% how our solution works
A natural question is, how \name actually virtualizes the concept of a physically laid RF chain? 
A physically laid RF chain connected to an antenna essentially amplifies the weak signal at antenna, downconverts it and finally digitizes it for signal processing ahead.
\name utilizes an architecture where all antennas are connected via a singly laid RF chain, allowing for hardware reuse, and simultaneous downconversion and digitization of all the antenna signals in one go.

But, in this process the individual antenna signals get combined with each other, and this won't allow capturing of per-antenna degrees of freedom required for interference suppression, so how does \name get back the degrees of freedom from the combined antenna signals?
To do so, \name utilizes RF switches connected to each antenna, in order to create different \emph{on-off} signatures for each antenna, which gives the signals from each antenna a discernable identity allowing them to be separated from each other via simple digital signal processing in software.
% RF switches are extremely low-powered circuit elements, and have been used 

% application: green
Thus, \name utilizes a switched-antenna array design connected to a single physically laid RF chain, with capability to create multiple virtual RF chains at a software level, making it an extremely flexible architecture.
In contrast, Massive MIMO today is niether flexible; nor as power-efficient as \name.
Another problem with massive MIMO today is the huge amount of data which is backhauled to software, or prcoessed on ASICs/FPGA for isolating the per-user's signals.
Beyond saving a lot of power consumption as compared to traditional multi-user techniques, by hardware reuse of the single RF chain across antennas, \name also optimizes on the amount of data backhauled for MIMO signal processing.
By optimizing both the energy consumption, as well as required data backhauling, \name creates a truly green architecture.

% \name also brings forth the only architecture which can simultaneously enable two applications: first, using only $N$ digital streams to serve $N$ users, and second, in very averse channel conditions, flexibly increase the sampling rate to keep on serving $N$ users in a robust manner.

% coarse 0-1 beamforming at RF
% fine beamfo
Massive MIMO requires having number of antennas $N_{\text{ant}}>N$ users, so that the captured degrees of freedom far exceed number of users to allow robust interference suppression. 
Hence, in order to get the $N$ per-user streams, baseband samples of $N_{\text{ant}}>N$ have to be backhauled and processed.
Alternately, an ASIC has to process these $N_{\text{ant}}$ streams in hardware, to backhaul only the $N$ processed per-user streams.
Either way, there is a tradeoff of massive data transfer, or massive processing requirement on the base-station.

Unlike Massive MIMO, in order to tap into the increased spatial degrees of freedom from an antenna, \name architecture does not require a dedicated RF chain.
\name capitalizes on the fact that unlike physically laid RF chains which are connected to one antenna at a time, our virtual RF chains are connected to all the antennas simultaneously.
Thus, unlike a physical RF chain, which is one antenna per chain, \name's architecture allows connecting multiple antennas per virtual RF chain seamlessly.
That is, we can have a $N_{\text{ant}}$ \name architecture, with $N$ virtual RF chain, and each virtual RF chain is connected to all the $N_{\text{ant}}$ antennas.
Thus, we can essentially backhaul only the baseband samples corresponding to $N$ virtual RF chains, while using $N_{\text{ant}}$ antennas to serve $N$ users; to optimize the amount of data utilized for signal processing

The key insight \name has here, to utilize multiple antennas per virtual RF chain, is to use these $N_{\text{ant}}$ antennas to beamform towards one user per virtual RF chains, instead of isolating per-antenna signals via the virtual RF chain.
That is, instead of keeping one antenna on per virtual RF chain, we can turn on all the antennas which are \emph{in-phase} for one user in that particular virtual RF chain.
Since we sample $N$ streams for $N$ users, we have $N$ virtual RF chains and thus we can use this method to beamform towards one user per virtual RF chain.
\name designs a simple algorithm which we refer to as `Binarized Analog Beamforming (BABF)' to enable this beamforming with simple $0-1$ RF switches.
\emph{By prioritizing one user per RF chain, instead of one antenna per RF chain}, we show that serving $N$ same frequency band users with just $N$ digital streams, is indeed possible.

Similar to \name, hybrid beamformers also aim to use $N_{\text{ant}}>N$ antennas connected to $N$ physically laid RF chains via analog circuits, analog beamforming + digital combining in order to address green communications.
However, first, these are fixed deployments, which are not flexible unlike \name.
Second, multi-user interference cancellation is a very channel dependent process, and there will be some channels where it won't be possible for hybrid architectures to perform as well as full digital architectures which sample.
Thus there will be some off-cases where it won't be possible to serve users with just $N$ sampled digital streams.
Unlike hybrid beamformers, by varying the sampling rate, \name can go from a hybrid architecture, to a fully digital architecture; 
Thus we keep on supporting the $N$ users reliably without overdesigning for worst case, or coming up with a fixed design to work well on average but fail to guarantee the quality of service.

Thus, to summarize, \name designs a new beamforming architecture which utilizes a single RF chain to create many virtual RF chains, and show that this flexible architecture can be both green, and adapt to averse channel conditions upon demand by scaling up resources.  We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users over traditional architectures.

==> intros/intro_spectrum.tex <==
% Spectrum+ADC sampling most important commodities of networks
\section{Introduction}

% Generally assumed to be symmetric, you always sample whatever exists out there
% As we race ahead in technology, can we resuse these gains without changing hardware?
% dual band argument
% Further, 

% Spctrum needs to be shared typically
Spectrum is the most essential resource for wireless networks. Access to free, unused spectrum allows for wide bandwidth high data rate wireless communications. However, we do not have unlimited spectrum at our hands, and being a limited resource, spectrum needs to be shared between all the devices connected to a network, and even the neighbourhood networks. That is, no two devices transmitting concurrently typically share the same spectrum (Fig. \ref{fig:introfig1} (a)). 

% What is sampling BW and it's relation with spectrum
In order to receive the given spectrum, it is required to have downconverters which bring the signals to base-band, and then a ADC which needs to sample the aggregate over-the-air bandwidth occupied by users. Typically this sampling bandwidth is the same as the net bandwidth of all transmissions dictated by the spectrum occupancy of the frequency bands of interest. 

% What happens when number of users increase, and the current trend of things
As the number of users in a network increase without an additional increase in total spectrum, the frequency band occupied by single user shrink, leading to reduced data rate to each user. To keep the same data rate for each user, this method of sharing spectrum by having users in different frequency band requires more spectrum to be added into the network, which is not always possible since spectrum is a shared resource and can not be increased arbitrarily. However, the receiver sampling rate is a local parameter, and with improved technology, can be increased to sample higher spectrum. 
Thus, there is a trend to go to higher center frequencies \cite{}, where spectrum is readily available, in order to keep up with the evolving communication technology which is able to design faster and more efficient receivers.

% We are doing something different, using faster rate receiver without requiring extra spectrum, but this introduces interference
In this paper, \name asks if this can be avoided, and if we can keep on using more adept receiver technologies without asking for more over-the-air spectrum. The relevance of problem \name targets can even be seen in current wireless protocols. WiFi-6 has modems which are capable to sample an aggregate bandwidth of 160 MHz, but at the same time there are modes in which they would sample only 20/40/80 MHz bandwidth \cite{} in scenarios like airports/malls where there are neighbouring modems which are sharing the net 160 MHz spectrum. 
That is, say if AP can only use 40 MHz spectrum over-the-air, it would be able to serve only $4$ 10 MHz users even though it has full technical capabilities to serve $16$ of them due to the higher sampling bandwidth available.
The only way to avoid utilizing higher aggregate spectrum across users is to have them occupy the same frequency band (Fig. \ref{fig:introfig1} (b)), such that the occupied spectrum is limited to the users' bandwidth, and does not sum up with additional users. However, this introduces multi-user interference in the chosen band of interest. 


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/intro_fig_1.pdf}
    \caption{Comparison of \name with current wireless networks. Due to creation of new fractional time-slots by fast switching, \name can serve multiple users operating over the same time slot and frequency band}
    \label{fig:introfig1}
\end{figure}

% Previous methods to kind-of do this actually dont do this at all
Serving multiple interfering users also forms the intended goal of digital beamforming MU-MIMO approaches. 
The basis of these approaches lie in leveraging multiple antennas to allow the creation of multiple independent spatial channels over the same frequency band, so that multiple users can utilize different spatial channels in order to communicate at the same time and frequency band.
However, these technologies require sampling spectrum at each antenna, which needs a downconversion chain and an ADC for each antenna. 
Also, these technologies do not utilize the available higher sampling bandwidth effectively.
\name asks a more fundamental question, can we handle multiple interfering users with just a single RF chain, requiring just a higher sampling ADC? 
The benefits of this would then be two fold, first, systems having just a single RF chain can also enjoy an efficient utilization of the available sampling bandwidth, and second, if any system has more RF chains available, \name can work in tandem with digital beamforming to tap into even more multiplicative gain possible. Said simply, if \name with 1 RF chain can serve 4 users, \name with 2 RF chains can serve 8 users in accordance with the 2x multiplexing offered by an additional RF chain.

Hence, \name designs a single RF chain receiver capable of utilizing the full sampling bandwidth available without actually requiring users to be in different frequency bands. To achieve this elusive goal, \name designs a novel multi-antenna single-wire interface, which is adept in handling the multi-user interference caused as many users occupy the same frequency band. As a consequence of utilizing a single wire interface, \name's antenna array is also scalable to add more antennas without overburdening the system complexities, which also help harden the multiplexing gains and guarantee robust performance. 

The first design principle of \name is to use RF switches in order to discern individual antenna streams from the combined single interface samples. The idea is that an increased sampling rate would allow forming of redundant fractional time samples, and by selecting one specific antenna to be \emph{on} for these fractional time samples, we can hone into the channel for that specific antenna by interpolating across these fractional time samples. The interpolation will be exact as per Shannon-Nyquist theorem, since the signal of interest from transmitter has lower bandwidth than the sampling bandwidth. 

Moving ahead, \name generalizes this step of discerning the per-antenna channel into a concrete analysis.
Selecting the fractional time slots and interpolating across gives us a lower bandwidth signal which is as good as a separate lower bandwidth signal sampled by a slower ADC.
Thus, by utilizing these time separated fractional time slots, \name creates virtual RF chains over time similar to how digital beamforming approaches utilize physical RF chains by having multiple slower clocked ADCs.
The analysis reveals that by switching appropriately, we can have an equivalence between \name and slower clocked digital beamformers, which is then also backed up by our results, that is, ceteris paribus, we get similar performances from both these approaches.

Going one step further, we notice that a generalization of \name's switching based approach to more number of antennas than number of fractional time slots is very natural. 
Basically, we can switch multiple antennas on for the fractional time slot in order to utilize constructive combining gains from these antennas to our advantage.
This draws a parallel to hybrid beamformers, which have more antennas than number of RF chains.
In case of \name, we utilize more antennas than number of virtual RF chains. Interestingly, this form of doing hybrid beamforming automatically creates a fully connected hybrid beamformer, the gold standard amongst the currently existing hybrid beamformers. This is because all antennas are connected to the created virtual RF chains by default. In comparison to hybrid beamforming for physically located RF chains, one needs to pay the hardware cost of connecting all antennas to all RF chains, by having that many more phase shifters required to connect than as compared to selecting some antennas for one RF chain and some for others. In case of \name's generalization, since the RF chains are a virtual abstract of the single wire sampled signal, all the antennas are connected automatically to each virtual RF chains without requiring more amount of switches to the effect.

Utilizing more number of antennas than number of virtual RF chains allows \name to harden the multiplexing gains entailed by the number of virtual RF chains available. This is a very concrete problem with mu-MIMO approaches of today, that we can not actually have $K$ users reliably multiplexed with $K$ antenna digital beamformer \cite{}. Due to this, there has been research on creating mu-MIMO schedulers \cite{}, which would select the group of users which can be multiplexed successfully, in order to fully utilize the available RF chains. Unlike these approaches, \name solves the problem head-on, by utilizing more number of antennas and strategic switching sequences to create an uncorrelated equivalent channel, which always allows for robust multiplexing gains across any spatial user configuration. This is also backed by our evaluation, where we see a drastic improvement with hybrid architecture when number of users are same as number of virtual RF chains.

Thus, to summarize, \name designs a novel antenna array which utilizes a single wire interface at a higher sample rate to replicate what traditional digital beamformers typically do with multiple wire slower interfaces, at the same time avoiding requirement of multiple downconversion chains. Further, \name shows that such architectures are naturally generalizable to a fully connected hybrid architecture with more number of antennas than number of RF chains, which allows us to harden the multiplexing gains and allow for robust mu-MIMO operation. We implement and test our antenna array prototype with WARPv3 SDR and 802.11 OFDM waveforms with $4$ users, over multiple user positions in a conference room setting, as well as digital beamforming and FDMA baselines. Our key results include similar performance metrics with digital beamforming with $4$ times less hardware requirements, achieving the same network capacity as compared to FDMA with $4$ times lesser spectrum requirements, and $>10$ dB improvement in $90$ percentile performance for average SINR across the 4 users by utilizing a hybrid architecture.




==> intros/intro_v1.tex <==
% !TEX root = paper.tex

\section{Introduction}

% Current status
Over the past decade, wireless networks have become robust, widely deployed and have transformed the daily lives of human beings in immeasurable ways.
However, as the number of users in a network scales up, as well as number of devices per user explodes with wearables and IoT, these networks face a drastic challenge in how to manage this ever increasing demand. 
It is well known that most of the Wi-Fi routers performance degrades as number of devices increase, with complaints of poor public Wi-Fi in malls, conference rooms, still haunting the network designers. 
Similarly, LTE network struggles to keep up it's robust performance in high density areas, like concerts, airports and stadiums.

% Why this happens
A key reason for this performance degradation has been that as number of devices in a network increase, they all compete for the communication resources, like spectrum, or time slots. 
In order to communicate in a multi-user network, users share these resources amongst themselves, either by not communicating in the same frequency band as other users, or holding back from transmitting in a time slot when other user is communicating.
A key requirement to this resource sharing is that no two users occupy the same frequency band simultaneously (Fig. \ref{fig:introfig1} (a)).
Thus, as number of devices in the network increase, with the spectrum kept constant, each communicating device gets lesser resources, and thus the performance degradation.

The most intuitive solution to this performance degradation is simple, add more spectrum to the network, which translates to more number of resources per user, and thus improved performance.
However, adding spectrum is a tedious process, involving new protocol designs and FCC approvals.
Thus, to prevent the network degradation from resource sharing without adding new spectrum, a way is to design wireless networks such that the network can handle multiple users communicating over the same spectrum simultaneously.
Since multiple users can now occupy same spectrum simultaneously, this leads to a multiplicative increase in the network capacity.
Serving multiple interfering users forms the intended goal of digital beamforming and MU-MIMO approaches, which utilize multiple antennas to cancel the interference caused as a result of users operating over the same spectrum simultaneously.
Although this solution allows to increase the network capacity, these solutions typically get limited by the number of spatial RF chains they can support, since it is not trivial and scalable to keep on increasing the number of RF chains to support more and more users in the network.
% However, a challenge here is to handle the interference caused as a result of users operating over the same spectrum and same time slot resources.

% To handle this multi-user interference, base stations are equipped with multiple antennas. 
% With multiple antennas, the base station's degrees of freedom increases, and it can use this increased dimensionality to cancel out the interference.
% Intuitively, this can be thought as the base station using one antenna for one user, and cancelling out the cross-talk by signal processing methods. 
% This is the main goal of digital beamforming, and MU-MIMO, and the standard solutions to achieve this require multiple spatial RF chains for each antenna to meet the multi-user requirement.
% Although this solution allows to increase the network capacity, these solutions typically get limited by the number of spatial RF chains they can support, since it is not trivial to keep on increasing the number of RF chains to support more users in the network.

Thus, the wireless network engineer is caught up in a loop, where increasing number of users means increasing number of spatial RF chains, which is not feasible after a certain point, and we can not simply keep on adding new spectrum to the mix.
So how do we address this scalable multi-user network design problem, without adding RF chains, or utilizing more spectrum?
\name makes a key observation here, that even though spectrum typically can not be increased, there is the other resource which we have not counted for, the time slots in the network.
So, the question \name asks is, can we create new time slots, by introducing multiple fractional time slots within one time slot (Fig. \ref{fig:introfig1} (b)), and get the desired multiplicative gain in the network capacity without adding RF chains or spectrum?
% So the question \name asks is, can we introduce some sub-sample time slots, and more importantly can these act as new resources in the network?

% Start with sub-sample, go to B, kB and end with oversampling at the BTS side
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/intro_fig_1.pdf}
    \caption{Comparison of \name with current wireless networks. Due to creation of new fractional time-slots by fast switching, \name can serve multiple users operating over the same time slot and frequency band}
    \label{fig:introfig1}
\end{figure}
First and foremost, what does it mean when we introduce these fractional time slots? Say, the base station needs to serve $K$ interfering users, and in hope of doing so, it creates $K$ new fractional time slots within one time slot.
Now, if the users also started operating in these $K$ fractional time slots, 
this solution would become same as increasing the bandwidth $K$ times, since bandwidth is inversely related to sampling time, and thus requiring more spectrum. 
Here, lies the first key insight of \name, where we introduce these fractional time slots \textit{only} at the base station, with the users still transmitting at the original intended time slots. 
Thus, what happens is that we increase the operating bandwidth locally at the base-station by $K$ times, whereas the bandwidth actually transmitted by the users remains the same, thus not needing any extra spectrum over the air.
% More importantly, it makes sense that the base station does 
% we only need increased bandwidth at the base station, since only the base station has to serve $K$ users in the network, and the users can keep on operating at the original bandwidth.
The hope here is that since only the base station needs to serve $K$ users in the network, with the users just caring about their own transmissions, and the base station is the only entity which actually needs this $K$ times processing bandwidth.
From a hardware requirement, this operating bandwidth asymmetricity makes sense, since the base station will have a more capable hardware to introduce these fractional time slots, and can do it easily, as compared to the mobile users.



% Next para tell the antenn array part
However, is using just the increased $K$ times bandwidth enough to handle $K$ users at the base station, without adding RF chains?
Since the users still transmit in the original time slot, and at the same frequency band, their signals interfere with each other.
Thus, we get $K$ users interfered signals across these newly created $K$ fractional time slots.
Definitely, to handle this $K$ user interference, we need to have at least $K$ antennas in the system, but how do we introduce this required dimensionality, without increasing RF chains, as the posed requirement for our solution?

To do so, \name creates a novel single-wire antenna array, which consists of `switched-antennas'. By a `switched-antenna' we basically mean an antenna accompanied with a RF switch, which can toggle the antenna on-off. To serve $K$ users, we create a $K$ switched-antenna array, and the signals from all these antennas are combined to a single wire interface requiring just one RF chain to operate. 
Since we combined all the $K$ switched antenna signals into one RF chain, how do we actually utilize the $K$ different antenna signals, in order to address the $K$ user interference?

This is where \name's approach to increase bandwidth at the base-station marries the approach to use a single-wire switched antenna array.
Basically, over the $K$ newly created fractional time-slots, we can create $K$ orthogonal 0-1 codes, which can then be implemented in analog domain using the $K$ RF switches accompanying each switched-antenna. 
This allows us to isolate the channels associated with each of the $K$ antennas, even if all their signals are added up, since we can isolate them using these on-off codes created by the toggling the RF switches. 

Intuitively, \name's novel switched antenna array, coupled with the $K$ orthogonal codes and the increased $K$ times bandwidth allows creation of $K$ virtual RF chains over these newly created $K$ fractional time slots.
Now, similar to how traditional digital beamforming combines signal over multiple spatial RF chains, \name combines signals over these $K$ virtual RF chains over time, to cancel out the interference.
Hence, without increasing the number of RF chains, \name's design serves $K$ users, by efficiently utilizing a single wire $K$ antenna array, accompanied with increased $K$ times bandwidth.

Thus our approach increases the effective capacity of a single RF chain by $K$ times, where $K$ is the factor by which we increase our sampling bandwidth at the base station. However, if the base station already had $S$ RF chains, at each RF chain, we create $K$ more virtual RF chains, which leads to $SK$ number of RF chain. 
This increases the number of users which can be served by a $S$ RF chain base station to $SK$, leading to a multiplicative increase in the perceived network capacity of a $S$ RF chain base station.

In order to combine across the $SK$ spatio-temporal RF chains to serve $SK$ users, we make a key observation, that irrespective of the physical location and multipath scattering, we can always cancel out all the $SK-1$ interfering users to handle the $SK$ users transmitting simultaneously, by combining across the $SK$ RF chains. 
This is enabled by efficiently using the null space of the channel matrix formed by collecting channels of each user to the multiple switched antennas.
This null space combining is also supplemented with a novel antenna selection algorithm by selecting the appropriately co-phased antennas to utilize the constructive combining gains. 

We build and test \name's switched array prototype with a SDR receiver, programmed to operate with $K$ times the bandwidth in accordance with our strategy to increase the operating bandwidth of the base station. We show that we are able to decode the $SK$ users, with just $S$ RF chains, and achieve the same performance as one would get by using a digital beamformer with $SK$ spatial RF chains, or using $K$ times more bandwidth across the users, to prove that we get this increased multiplicative capacity without actually increasing either the spatial RF chains, or requesting users to transmit at higher bandwidths.
At the same time, we significantly outperform our fair baselines, like a digital beamformer having $S$ RF chains and $SK$ antenna analog beamforming solution, by achieving $XX\%$ increased throughput and $XX\%$ higher SINR. 
We show our system working with a wideband OFDM waveform, and perform evaluations in both, an office indoor environment, as well as an outdoor environment.
% Although one may think that introducing sub-sample time slots is equivalent to actually increasing the spectrum itself, since bandwidth and time are related inversely to each other. 
% However, here, our key insight is that we will only perform sub-sampling at the receiver base station, and not at the indiviudal users.
% That is, what we actaully do by our sub-sampling, is 

==> requirements/requirements.tex <==
% !TEX root = paper.tex

\section{Requirements}\label{sec:reqs}


==> results/results.tex <==
% !TEX root =../paper.tex





\section{Evaluations}

Having described the design, implementation and showed an example captured trace of \name, we will now go over various experiments performed to verify the design choices and showcase the power + spectrum efficiency of \name. First, we will go over the experimental setting, then show microbenchmarks and ablation studies, \name and end by showing the end-to-end evaluations and brief case studies on power savings entailed via \name architecture.

\subsection{Evaluation setting}

\begin{figure}[t]
\begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp-setup-photo-only.pdf}
    \subcaption{Experimental Setting}
        \label{fig:multi_user_conf_actual}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp-setup-floor-map.pdf}
        \subcaption{Setting Floorplan}
        \label{fig:multi_user_conf_floor}
    \end{subfigure}
% \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp-setup-with-num.pdf}
%         \caption{Experimental Setting: Actual image and floorplan}
%         \label{fig:multi_user_conf_floor}
%     \end{subfigure}
% \begin{subfigure}[t]{0.3\textwidth}
%     \centering
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/bar_chart}    
%     % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
%     \caption{Power consumption for 4 users (mW)}
%     % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
%     \label{fig:pow_calc}
%     \end{subfigure}
%     \vspace{7pt}
\caption{We test \name in a conference room setting (a), and the numbers $0,1,\ldots 9$ in (b) represent the $4$ user positions for the 10 configurations where we test \name and baselines, (c) shows the power consumption metrics of our setup}
\end{figure}



To evaluate \name, we consider a office environment (conference room setting, rough dimensions of 12m*5m, Fig. \ref{fig:multi_user_conf_actual}) with TV screens/desks/whiteboards which would act as reflectors and make it a multipath setting.
We fix the location of \name PCB, which acts as an AP, roughly in middle of the room, and vary the positions of the $2,3,4$ users across 10 configurations scattered around the room, and with various degrees of closeness to capture the overall performance trends in the experimental setting considered.
For the experiments we set the transmit power such that we have SNR of about 17-20 dB, and utilize QAM-16 constellation with 0.5 rate convolutional channel code.
This choice of SNRs is consistent with the recent works on MIMO systems \cite{ding2020agora}.

% We evaluate the power consumption, SINR, system capacity, Goodput and Energy per joule performance for 2,3,4 users at various positions in a conference room setting (Fig. \ref{fig:multi_user_conf_actual}), to capture the overall performance trends in the experimental setting considered. The room which we choose has rough dimensions of 12m*5m, and is populated with objects like tables, chairs, whiteboard and TV screens, which make the setting rich with scattering effects. 
% For the experiments we set the transmit power such that we have SNR of about 17-20 dB, and utilize QAM-16 constellation with 0.5 rate convolutional channel code.
% This choice of SNRs is consistent with the recent works on MIMO systems \cite{ding2020agora}.
% This constellation was tested to work reliably for these SNRs, given the phase noise of our implementation with users on an USRP and AP being WARPv3.
% We implement 5 different test configurations anutilized baselines: 4 antenna \name, 4 antenna DBF, 8 antenna \name, 8 antenna DBF (Trace level) and Interference free OFDMA oracle.
\subsection{End to end evaluations}




% \subsection{Evaluations}
\begin{figure*}
    
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/8ant_multipos_sajjad}    
    \caption{8 Ant \name improves SINR for 4 users}
    \label{fig:8ant_res}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/tput_sajjad}
    % \input{results/8ant_multipos}   
    \input{results/trace_sim}
    \caption{Trace level comparisons with 8 antenna DBF}
    \label{fig:trace_lvl}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/capacity}   
    \caption{Increasing number of antennas allow reaching FDMA capacity}
    \label{fig:fdma_cap}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/tput_sajjad}   
    \caption{Throughput results}
    \label{fig:tput}
    \end{subfigure}
        \vspace{7pt}
    \caption{Experiment CDFs for SINR plotted across multiple packets collected for multiple user locations in the conference room setting, and Average Goodput with errorbars representing std. deviation across multiple packets. We can see that with $8\times4$ \name, we always meet the target SINR which allows robust goodput performance for all users, and also meets FDMA oracle capacity}
    \vspace{5pt}
\end{figure*}

\begin{figure}[t]
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \centering
    \setlength{\figureheight}{0.55\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegrapandhics[width=\linewidth]{results/init_figs/Selection_820.png}
     
    \input{results/bp_joule}
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \caption{Energy efficiency results}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \caption{}
    \label{fig:bp_joule}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
    % \includegrapandhics[width=\linewidth]{results/init_figs/Selection_820.png}
    % \input{results/pow_rf.pdf}
    \includegraphics[width=\linewidth]{results/pow_rf.pdf}
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \caption{Power consumption with \# of RF Chains}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \caption{}
    \label{fig:energy_rfc}
    \end{subfigure}
        \vspace{-5pt}
    \caption{(a) Energy Efficiency, (b) Power consumption with \# of RFC}
    \vspace{3pt}
    % \label{fig:fdma_comp}
\end{figure}





% \noindent \textbf{5.1 Evaluation Setting}:\\


% \begin{enumerate}[itemsep=0pt,leftmargin=5pt]
    % \item \textbf{4 antenna \name}: Here we utilize 4 switched antennas combined to a single output, used to create 4 virtual RF chains  (Fig. \ref{fig:mmse_comp})
    % \item \textbf{4 antenna DBF}: Since we use WARPv3 as our evaluation platform, we have availability of 4 physical RF chains via the MIMO expansion daughtercard, to implement 4 antenna digital beamforming (Fig. \ref{fig:mmse_comp})
    % \item \textbf{8 antenna \name}: Here we use PCB which has 8 switched antennas combined to a single output (Fig. \ref{fig:pcb_pic})
    % \item \textbf{Interference free-oracle}: To test how well \name suppresses interference, we also test with an oracle which has users in different frequency bands 
    % \item \textbf{8 antenna DBF (trace level)}: We utilize our 8 antenna switched PCB to $4$ channel traces at a time via the WARP's 4 physical RF chains, and then time-align these traces to evaluate at a trace level how a 8 antenna DBF would perform in comparison to \name
% \end{enumerate}

% \item \textbf{4 antenna \name}: Here we utilize 4 switched antennas combined to a single output, used to create 4 virtual RF chains  (Fig. \ref{fig:mmse_comp})
%     \item \textbf{4 antenna DBF}: Since we use WARPv3 as our evaluation platform, we have availability of 4 physical RF chains via the MIMO expansion daughtercard, to implement 4 antenna digital beamforming (Fig. \ref{fig:mmse_comp})
%     \item \textbf{8 antenna \name}: Here we use PCB which has 8 switched antennas combined to a single output (Fig. \ref{fig:pcb_pic})
%     \item \textbf{Interference free-oracle}: To test how well \name suppresses interference, we also test with an oracle which has users in different frequency bands 
%     \item \textbf{8 antenna DBF (trace level)}: We utilize our 8 antenna switched PCB to $4$ channel traces at a time via the WARP's 4 physical RF chains, and then time-align these traces to evaluate at a trace level how a 8 antenna DBF would perform in comparison to \name

% Virtual RF chains offer various advantages over their physical counterparts. 
% First, because of hardware re-use of downconversion chains across the antennas, creation of $N$ virtual RF chains costs is much less power consuming than $N$ physical RF chains.
% Second, virtual RF chains can scale easily to number of antennas; addition of new antennas doesn't need a new RF chain, which allows \name to use more number of antennas than number of virtual RF chains to allow MIMO signal processing commensurate to users' bandwidth; paving the way ahead for green communications.
% In addition, \name allows creation of RF chains via software, instead of laying them physically, thus making \name a flexible architecture.
% Since \name uses just a single RF chain, similar to FDMA, \name actually enables a multi-antenna architecture which is as spectrally efficient as massive MIMO and as power efficient as FDMA.
% In this section, we evaluate each of these claims, and provide microbenchmarks for our design.
% Hence, the while evaluating \name we first confirm that the virtual RF chains give same performance as compared to their physical counterparts.
% Then, we show evaluations which support \name's claim towards design of a green communication architecture, wherein we serve $N$ user by just utilizing $N$ times oversampled ADC and a single RF chain, at the same time using a higher number of antennas $N_{\text{ant}}$.
% We also compare the energy metrics of our design and prove the optimallity of our design by comparing to a oracle interference-free FDMA baseline.
% Finally, we also illustrate our approach of increasing the sampling rate when channel conditions are bad, by considering a very bad multi-user scenario where the users' channels are extremely correlated.
% Towards the end we also evaluate microbenchmarks for various components of \name design to quantify the performance metrics.


% We have evaluated \name architecture to deliver uplink mu-MIMO multiplexing gains with just a single RF chain connected to multiple switched antennas. The core principle behind \name is the usage of strategic toggling sequences for the RF switches, which enable the creation of time interleaved virtual RF chains. \name would then combines across these virtual RF chains in digital domain to cancel interference and thus serve multiple users with a single RF chain. Thus \name can be very helpful in situations where the networks need to serve multiple users simultaneously, for example during conferences when the occupancy shoots up drastically.

\noindent \textbf{5.2 RFE and Sampling power consumption}: 
WARPv3's RF transceiver MAX2829 \cite{MAX2829}, performs the downconversion and filtering. From the datasheet, we can see that 4 antenna DBF would require RFE power of 1632 mW (4$\times$408 mW) power when operating in synchronous MIMO mode, while only 354 mW for \name operating by itself, as is the case with \name and interference-free oracle which employs FDMA.
Finally, \name uses a network of switches for creating per-antenna spectrum variations leading to virtual RF chain creation; This has near negligible power consumption, similar to how these switches being used for backscatter communications which exploit this near negligible power for battery-less operation. The HMC197BE switches used in \name design require just 0.001 mW of static power, and even including the active power they draw from the MHz clock sources, it is fairly less than 1 mW. Hence total RFE power consumption for 8 antenna \name is approximately 354+8 = 362 mW (assuming 1mW per switch), for FDMA it is 354 mW and for DBF it is 1632 mW.
% As users drop down from $4$ to say $3$ or $2$, the RFE power for \name and FDMA will not change as this is the fixed power consumption by the single front end chain. But for digital beamfroming, as users drop down, 

ADC power varies linearly with the sampling frequency \cite{barati2020energy}, which is true for the AD9963 ADC used for WARP, as evident from the datasheet \cite{AD9963}. 
Thus, the power consumption of 4 ADCs is same to that of one ADC with 4x higher sampling. From the datasheets of AD9963, we have power consumption as 400 mW for 40 MHz sampling operation used for \name and FDMA, whereas 4 physical RF chains with 10 MHz would use 4*100 = 400 mW as well. Thus for all the three confiurations, the sampling power would be 400mW.

Therefore, total power consumption of \name is ~762 mW (354+400+8 mW) which is 3x lower than MIMO (1632+400 = 2032 MW), and almost the same as single antenna FDMA oracle, which would be 754 mW (354+400mW).

Fig. \ref{fig:pow_calc} shows the power consumption metrics for each of the strategy. As seen clearly, it is not the sampling power which dominates the power consumption, but the power consumed in the front end by these multiple RF chains. 
% One might argue that these calculations are for WARPv3, which is a slightly older SDR, but even the state of art mmWave receiver also show this trend of power consumption being dominated by the downconversion hardware and not ADCs/DACs \cite{yan2019performance}.

\noindent\textbf{5.3 SINR performance comparison of 4 antenna \name with DBF}:
\name is the first work to use virtual RF chains.
Hence, it is important to show the performance comparison with physical RF chains.
We do so by creating a faithful test setup to compare virtual RF chains with physical RF chains (Fig. \ref{fig:mmse_comp}). 
% The test-setup allows us to use the same antennas for capturing the received samples from WARP with both $4$ virtual RF chains created by \name's approach, and $4$ physical RF chains digital beamforming.
Basically we use external switches to have the same antennas connected to either 4 physical RF chains directly, or 4 virtual RF chains via RF switched array.
Thus, we can compare the 2 approaches faithfully, as both of them capture the samples from the same antennas.

The SINR performance of both the methods indeed turn out to be very similar (Fig. \ref{fig:4ant_sinr}). 
For these CDFs, we collect 30 packets at each of the 10 locations of $4$ users in the conference room, which gives 300 sample SINRs these plots. We can clearly see the performance for both the methods to be very similar (within $\pm$ 0.5 dB for median error).
Thus $4$ virtual RF chains, with total power consumption as 762 mW provides same SINR metrics as $4$ physical RF chains, with total power consumption 2032 mW, which is 3x more than \name.
However, as the number of users increase from $2$ to $4$, the performance of both the two approaches deteriorate, and with $4$ users, for almost $40\%$ of the packets, the SINR is lesser than $10$ dB (Fig. \ref{fig:4ant_sinr}). \\
% This result is consistent with many of the research papers \cite{pasandi2021muvis,sur2016practical}, agreeing on the fact that serving $N$ users with just $N$ antennas is not a robust operation point.
% In this setup, we use RF switches external to the switches we use for our switched antennas, and the purpose of these SPDT RF switches is to toggle between two states. The first state of the setup is ``RFC-RF1", which connects the $4$ antenna array to the PCB which implements \name architecture, and takes the output emanating from the PCB and feeds it to a single RF chain on WARP. The other state, 
% ``RFC-RF2" connects the same antenna array to each of the physical RF chains on WARP to implement traditional digital beamforming. 
% Evaluation in such conference room, or auditorium settings has been a constant feature of research works on multi-user communications \cite{flores2016scalable,kuhne2020bringing}. 
% The SINR here is computed from the EVM metric of the receieved constellation after digital combining is done, as the noise would be coming from the residual interference and noise.
% Goodput is measured by mapping the received constellation back to bits, passing through vitterbi decoder corresponding to the 0.5 rate convolutional code, and then measuring the number of bit errors.
% Unlike traditional digital beamformers, which have to now spend even more power to add new RF chains, \name can guarantee performance for $N$ users with $N$ streams by extending to more number of antennas easily.

\noindent\textbf{5.4 Optimizing sampling+compute power by serving 4 users reliably with $4$ virtual RF chains}:
In order to improve the performance as number of users $N$ approach number of virtual RF chains $N$, we increase the antennas and use our BABF algorithm to prioritize 1 user per RF chain.
% We utilize the $8$ antenna version of our \name architecture, as shown in Fig. \ref{fig:pcb_pic} to 
% implement BABF algorithm in order to support $4$ users reliably. Note that we do not increase our oversampling factor, and just attach more switched antennas for this experiment. 

For this experiment, we use the \name PCB which has the capability to utilize $8$ switched antennas, and create $4$ virtual RF chains from the combined $8$ antenna output.
We can electronically turn off antennas in our PCB to simultaneously collect data from $4$, as well as $6$ antenna configurations to understand the effect of increasing number of antennas on the system metrics. 
The SINR and goodput results are shown in Fig. \ref{fig:8ant_res}.
As we increase the antennas to $8$, the SINR shows an immense jump and always exceeds 10 dB, close to what is expected from a robust multi-user transmission scheme.
We observe more than $10$ dB increase in the $90$-th percentile SINR, as compared to $4$ antenna digital beamformer implemented using WARP's physical RF chains.

% It is indeed impressive to see how \name was able to harden the multiplexing gains for $4$ users without actually increasing the number of virtual RF chains just by utilizing more switched antennas, which bear a very minimal extra power and implementation cost.




% \begin{figure*}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/random_seq_sajjad}    
%     % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
%     % \vspace{-3pt}
%     \caption{Choice of $\mathbf{S}$}
%     % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
%     \label{fig:random_seq}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/unsynch_sajjad}   
%     % \vspace{-3pt}
%     \caption{Synch. vs Unsynch. users}
%     \label{fig:unsynch}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     \input{results/lts_fig}
%     % \input{results/8ant_multipos}    
%     % \vspace{-3pt}
%     \caption{Varying channel estimation accuracy}
%     \label{fig:chan_est}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     \input{results/sim_res}
%     % \input{results/8ant_multipos}    
%     % \vspace{-3pt}
%     \caption{Large scale simulations}
%     \label{fig:sim_fig}
%     \end{subfigure}
%         \vspace{7pt}
%     \caption{Ablation studies to adjudge \name's performance (a)-(c), and a large scale simulation result (d)}
%     \vspace{5pt}
% \end{figure*}

% \noindent\textbf{Trace level comparisons with Digital Beamformers having more than $4$ RF chains:
% Unlike \name, which can support $4$ users robustly without increasing sampling power consumption, by just adding more antennas+RF switches, Digital beamforming adds new RF chains to do so. 
% Thus, a nai
Unlike \name, digital beamforming approaches utilize a naive way of improving performance for $4$ users, which is to add more RF chains to sample from more antennas.
Since WARPv3 has support only for $4$ physical RF chains, we do a trace level comparison to $6,8$ RF chain DBF by collecting $4$ antennas channels at a time and then synchronizing them in post-processing.
We observe that \name even outperforms a $6$ antenna digital beamformer (Fig. \ref{fig:trace_lvl}), and comes $\sim3$ dB close to $8$ antenna digital beamformer at median performachainsnce, all the while having at least $4$x lower power consumption.


\noindent\textbf{5.5 Comparison with interference-free oracle}:
% Since \name utilizes $4$ times higher \emph{sampling bandwidth} as the user's transmitting bandwidth, it is only natural to compare the same with an equivalent frequency based multiplexing (FDMA) system. 
% However, only the sampling bandwidth for FDMA and \name are the same, \name utilizes $4$ times lesser spectrum resources while sampling at a higher rate. 
For the FDMA oracle, the users occupy $4$ different $10$ MHz bands, and the WARP would sample this aggregate $40$ MHz bandwidth in order to serve these $4$ non-interfering users.
In contrast, for \name, the $4$ users occupy the same $10$ MHz band, and the WARP receiver samples a higher sampling bandwidth $40$ MHz, in order to create the $4$ virtual RF chains required to multiplex the 4 users signals.
Thus in order to be spectrum-efficient, \name has to cancel the in-band interference in the occupied 10 MHz bandwidth
Even with added task of interference cancellation, we see that with more number of antennas ($8$) than number of users ($4$), we get system capacity on on par with FDMA oracle (Fig. \ref{fig:fdma_cap}). 

\noindent \textbf{5.6 Energy efficiency metrics (bits per joules)}: Finally, we revisit the power calculations briefly in the context of our goodput results.
As seen in Fig. \ref{fig:tput}, we can get goodput close to interference-free oracle levels using \name architecture with 8 antennas. 
This result can also be viewed in the lens of bits per joules (Fig. \ref{fig:bp_joule}) by seeing how much power got expended in the process.
As the number of RF chains increase from $2$ to $4$, we see constant $O(1)$ 354 mW RF front end (RFE) power demand for \name, as explained in Section 5.2.
The ADC power requirements are $100mW$ per 10 MHz data sampled and that increases as $O(N)$ with users.
On the other end, for digital beamforming, RFE power scales linearly with $N$, given by $408*N$, since the WARPv3 MAX2829 IC uses $408$ mW per RF chain in MIMO mode.
Hence, we get energy consumption trends as shown in Fig. \ref{fig:energy_rfc}.
This explains the energy per joule Fig. \ref{fig:bp_joule}, more particularly, the dip for DBF at $4$ user operation.
This is because, the DBF goodput shows a downward trend for $4$ users, whereas power has kept on increasing linearly, which further exacerbates the energy efficiency between DBF and \name.

% \noindent\textbf{Spectrum saving and Power saving with TIMO}: So far, we have seen that TIMO serves four users utilizing 4x lower spectrum than equivalent FDMA system and 4x lower RF-chains than equivalent MIMO system while performing similar to FDMA and MIMO systems. Here we explain the implication of saving these spectrum and hardware resources on modern communication systems as shown in Figure \ref{fig:pow}. First, TIMO is spectrally efficient as it utilizes only 10 MHz bandwidth to serve 4 users while an equivalent FDMA system requires a large 40 MHz spectrum. Thus, TIMO achieves 4x higher spectral efficiency than FDMA. 
% The second implication is that TIMO is power efficient as it saves the number of RF chains by a factor of four compared to a MIMO system.  \textit{In summary, TIMO makes the best of both worlds by being as power-efficient as FDMA systems and as spectrum efficient as MIMO systems. This leads to a scalable mu-MIMO design that can multiplex an order of magnitude higher users simultaneously.}\
% While MIMO hardware consists of 4 ADCs along with 4 down conversion chains, the TIMO hardware consists of only one high-sampling ADC and a single downconversion chain, 
% * ADC power is linear in  terms of sampling frequency \todo{cite}. Utilizing 4x faster ADC has same power 4x power slower ADC. For 
% * Howvere, we save on, we don;t need 4 downconversion chains. And in our implementation with warp v3, the ADC consume 400 mW for both case. \todo{cite datasheet}. Downconversion chip MAX2829 utilizes 354 mW for SISOimplementation and 4x 408 mW = 1632 mW when used in a MIMO mode. 754 mW for us and 2032 mW for DF.
% * Switches need 0.001 mW static power and even including the active power they draw from the MHz clock sources, it is less than 1 mW . 
% * We are close to fDMS because switches are minimal power. 
% By getting the same capacity result as FDMA, at the same time using $4$ times lower aggregate bandwidth than FDMA, \name builds a single RF chain receiver which is spectrally very efficient.
% At the same time, \name utilizes similar power metrics to the single antenna FDMA approach, since the switches, including the DC power as well as power drawn from the MHz clocking inputs, have very minimal power ($<$ 1 dBm), and the antennas are entirely passive.
% Thus, as compared to other multiplexing approaches to be spectrally efficient, like digital beamforming, which are power inefficient, \name offers both, a spectrally, as well as power efficiently solution to obtain multiplexing gains.
% For this result, we use the switches to increase the signal power of one user at each time slot, so that we get uncorrelated channels enabling higher spatial multiplexing gains. To evaluate the effectiveness of our algorithm, we choose 100 random trials to choose the switching matrix $\mathbf{S}$, and 100 trials with our algorithm, and plot the CDF in Fig. \ref{fig:random_seq}. Our approach of choosing inphase antennas for one user at a time always outprforms a randomly chosen matrix $\mathbf{S}$.

% \noindent\textbf{5.7 Ablation studies}:
% % Finally, to conclude our evaluations, we show ablation studies for
% % \begin{enumerate}[itemsep=0pt]
% %     \item Effectiveness of BABF algorithm
% %     \item Synchronized vs Unsynchronized users
% %     \item Channel estimation accuracy 
% % \end{enumerate}
% % , having users unsynchronized and channel estimation accuracy play a factor into \name's approach. For all these results we fix a $4$ user configuration in the conference room setting and collect multiple packets by varying these parameters to carefully understand the effects.

% First, to evaluate the effectiveness of BABF, we choose 100 random choices of $\mathbf{B}$, and collect $10$ packets with each choice, and repeat the same with $100$ packets collected by choosing $\mathbf{B}$ via BABF algorithm which chooses in-phase switches for one user per virtual RF chain. We plot the CDF in Fig. \ref{fig:random_seq}, and observe that BABF $\mathbf{B}$ matrix always outperforms a randomly chosen $\mathbf{B}$.

% Second, to show robustness against unsynchronized users, we first synchronize the users to each other by utilizing same reference clock and start time, and thus all the transmitters have same CFO and tightly synchronized sampling times.
% Then, we repeat the experiment by having unsynchronized usees, suchthat each user has a different clock, leading to different CFOs for each user.
% As clearly seen from Fig. \ref{fig:unsynch}, we get almost the same performance when the transmitters are synchronised with each other as compared to when they are unsynchronized.
% % Infact, we get minimally higher SINR with unsynchronized since due to sampling offsets, the unsynchronized transmissions often end up having some samples to be interference free, whereas for the synchronized transmissions, all the user's signals interfere all the times, hence being a more stringent evaluation.

% Third, the interference cancellation performance also depends on the accuracy of channel estimates procured. We can always average the channel across multiple LTS's to get a higher channel estimation accuracy. Thus, we repeat the experiment with more number of LTS's than the prescribed $2$ LTS's as per 802.11 protocol, and observe that we get only about $1.5$ dB difference in median performance as the number of LTS's increase to $10$, which shows that \name's algorithms can work without imposing a high cost of channel estimation latency.
\begin{figure}[t]
    % \begin{adjustwidth}{-15pt}{} 
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mmse_comp_network.pdf}
        \caption{Physical vs Virtual RFC}
        \label{fig:mmse_comp}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.9\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/mmse_comparison_sajjad}
    \caption{SINR CDF for 2, 3, 4 users}
    % \caption{Throughput comparison with SISO and Digital beamforming. Our method closely matches the digital beamforming baseline, however, both these methods fail to provide the 4x possible increase in rate}
    \label{fig:4ant_sinr}
    \end{subfigure}
    % \end{adjustwidth}
    % \begin{subfigure}[t]{0.22\textwidth}
    % \centering
    % \setlength{\figureheight}{0.5\linewidth}
    % \setlength{\figurewidth}{0.8\linewidth}
    % % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % % \input{results/8ant_multipos}    
    % \input{results/pow_spectrum}
    % \caption{Power \& Spectrum Required}
    % \label{fig:pow_spectrum}
    % \end{subfigure}
        % \vspace{7pt}
    \vspace{2pt}
    \caption{Microbenchmarks (1): Do the created virtual RF chains have similar performance to physical RF chains?}
    \label{fig:fdma_comp}
\end{figure}

\begin{figure}
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \centering
    \setlength{\figureheight}{0.5\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/random_seq_sajjad}    
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \vspace{-3pt}
    \caption{Choice of $\mathbf{S}$}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \label{fig:random_seq}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
    \setlength{\figureheight}{0.5\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/unsynch_sajjad}   
    % \vspace{-3pt}
    \caption{Synch. vs Unsynch. users}
    \label{fig:unsynch}
    \end{subfigure}
    \caption{Microbenchmarks (2): What is the performance gain of BABF switching, and do the transmitters need synchronization?}
\end{figure}


\subsection{Microbenchmarks}
The main design concepts of \name are creation of virtual RF chains from the spreaded bandwidth and BABF switching to beamform towards one user per virtual chain.
Further, since the creation of virtual RF chains require slicing across samples, like collecting every $\{4n\},\{4n+1\},\{4n+2\},\{4n+3\}$ samples, it may appear that the transmitters also need to be synchronized for the whole \name approach to work.

\textbf{Physical vs Virtual RF chains}: Hence, we first create a faithful test setup to ascertain the fidelity of \name's virtual RF chains versus traditional MIMO's physical RF chains (Fig. \ref{fig:mmse_comp}).
Since we want a fair one to one comparison, we do not turn on multiple antennas per virtual RF chain and restrict to one antenna per virtual chain.
The test setup ensures that the wireless channels captured by $4$ physical RF chains is same as the $4$ virtual RF chains channel via \name PCB.
We collect the $2,3,4$ users interfering traces from this setup, and evaluate the average SINR across the users to evaluate the interference cancellation capacity of virtual vs physical RF chains.
Because the insertion losses from the switches are minimal ($\sim 0.5$ dB) and the PCB is designed with optimal Wilkinson networks at $2.4$ GHz, we see that the SINR metrics remain same for both physical and virtual RF chains. 
This validates the \name PCB design and implementation.

\textbf{Why BABF?}: Next, we start utilizing one big advantage of virtual RF chains, that we can toggle multiple antennas on-off in a virtual chain to get advantage of analog combining gains. Using the BABF approach, this allows us to get a well-conditioned equivalent channel matrix $\mathbf{H}\mathbf{S}$ which is diagonal heavy.
Hence, as a consequence, the digital beamforming block which inverts the wireless channel works more efficiently and the final SINRs so obtained are much better.
These results are quantified as shown in Fig. \ref{fig:random_seq}, where for one user configuration we evaluate the final SINRs by choosing $\mathbf{S}$ randomly, and via BABF, and we repeat this 100 times to plot the CDF.
BABF always works better than any random choice of $\mathbf{S}$, and on an average (median line) it works $10$ dB better.
This justifies the design choice of adopting BABF approach of computing $\mathbf{S}$.
% Note that BABF is computed deterministically, whereas to get to median random matrix performance we would need to try 50 random combinations and then choose the best one.

\textbf{Synchronized vs Unsynchronized Users}: \textcolor{red}{!!!Write it better!!!} \name basically does a spatial operation; so it does not matter if the transmitters are synchronized or not.
So, to show this result, we conduct experiments where we synchronize the $4$ users to share the same clock, and repeat it without synchronization.
We observe similar performance as expected, shown in Fig. \ref{fig:unsynch}.
However, since \name needs to obtain per-user channels, it is required that the users are at least loosely synchronized such that their LTS's do not collide, and this level of loose synchronization is guaranteed by modern cellular protocols, however the users do not need to share the whole clocks.



% \subsubsection{Virtual vs Physical RF chains}
% \subsubsection{SAM+BABF implementation}

\noindent \textbf{Scaling to higher number of antennas and users}: 
Our hardware experiments are limited to handling $4$ users and $8$ antennas, however, the techniques introduced in this paper are fairly general and can be implemented for higher number of antennas and more number of users with specialized RF switches and better evaluation platform.
% since the commercially available HMC197BE RF switch we use has $\sim 10ns$ on time. 
% Thus, we can not handle faster bandwidth switching than 50 MHz, and further
% our evaluation platform WARPv3 which supports only 40 MHz sampling.
% However, the techniques introduced in this paper are fairly general and can be implemented for higher number of antennas and more number of users with specialized RF switches and better evaluation platform.

To motivate this, we perform simulations by placing users in similar environments to our evaluation setting, and modelling the multipath wireless channel via ray-tracing.
In simulations, the users transmit OFDM signals and the channels are applied to the OFDM signals by calculating the distances from the environment reflectors in simulation setting and applying appropriate time delays+amplitude weights in the received OFDM signal. 
All the receive processing uses the identical codes used for hardware evaluations. Hence, this simulation framework gives results which by and large follow the trends expected from experimental evaluations.

Fig. \ref{fig:sim_fig} shows simulation results and comparison for 64 antennas usecase to serve 8 users. This is considered a standard baseline with multi-user Dense deployments, which on an average require serving $8$ streams concurrently \cite{yan2019performance}.
\name uses 64 antennas and creates 8 virtual RF chains to serve the 8 users, and almost always obtains >10dB SINR.
We can see even in simulations serving $8$ users with $8$ RF chain digital beamforming is infeasible.
We also show comparisons with ideal partially and fully connected hybrid beamformers with $8$ physical RF chains. Our simulations assume perfect phase quantization, and still \name outperforms partially connected beamformers. The reason is that unlike partially connected beamformers \name does not split the antenna array between the physical RF chains, since all the antennas are by default connected to the virtual RF chains.

\name's performance comes about $5dB$ close on an average, to the full 64 chain DBF and fully connected HBF, even though using at least 64x lower power and 64x lower circuit elements.  

% Now, there are some ways to get around these limitations. One method is to to expect some sort-of coordination from users, such that either they align their transmissions to minimize interference, or the users introduce random cyclic delays to allow for de-correlation of the channels. However, both these methods require channel feedback to the users, which is very difficult to achieve in practise, with multiple challenges like accuracy of quantized feedback, staleness of channel estimates which hinder these deployments in practical scenarios. A potentially better method is to increase the number of antennas at the base-station, since that increases the aperture and allows for finer beams to be formed which can de-correlate the users. However, increasing number of antennas is not a scalable operation with digital beamforming, since we require extra RF chains for the same to support the increased antennas. On the flipside, \name uses just a single RF chain, and thus can increase the number of antennas in a more scalable manner, and this allows \name to deal with spatially close users (Fig. \ref{fig:8ant_exampleloc}). 

% To evaluate this claim, we choose the following user configuration, where the users are quite co-located, which is practise could be a single user with their phones and tablets acting as two close located device. We keep on increasing the number of antennas in our implementation till we start seeing acceptable SINR performance (>10 dB for all the users), which we empirically observe happens at number of antennas to be 8 (Fig. \ref{fig:8ant_exampleloc}. In comparison, we have the performance by a 4 antenna digital beamformer which doesn't have the capability of handling such scenarios and the SINR is only around 4 dB or even lower for some users.








% \begin{figure}[H]
%     \begin{subfigure}{0.23\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{results/init_figs/Screenshot_20210323-102643_Samsung Notes.jpg}
%         \caption{Indoor Setting}
    
%     \end{subfigure}
%     \begin{subfigure}{0.23\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{results/init_figs/Screenshot_20210323-102643_Samsung Notes.jpg}
%         \caption{Outdoor Setting}
    
%     \end{subfigure}
%     \label{fig:my_label}
% \end{figure}


% We evaluate the effectiveness of \name in handling multiple users in two settings, first one an indoor office setting, and second one an outdoor setting. For each setting we evaluate BER/Throughput/EVM at multiple user locations and plot the CDF to obtain the performance statistics of \name. \name uses 4 antennas, followed by 4 switches, which are then combined and read via a single RF Chain. 
% Hence, \name lies somewhere between a conventional MIMO design with multiple antennas supported by multiple RF chains, and a single antenna with a single RF chain solutions.
% Thus, we compare \name results with a SISO link, as well as an equivalent 4 antenna MMSE baseline.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{results/init_figs/Screenshot_20210323-105406_Samsung Notes.jpg}
%     \caption{Eval Results}
%     \label{fig:my_label}
% \end{figure}

% \subsection{BER Results}


==> results_1.tex <==
% !TEX root =../paper.tex



\section{Evaluations}

Having described the design, implementation and showed an example captured trace of \name, we will now go over various experiments performed to verify the design choices and showcase the power + spectrum efficiency of \name. First, we will go over the experimental setting, then show microbenchmarks and ablation studies, \name and end by showing the end-to-end evaluations and brief case studies on power savings entailed via \name architecture.

\subsection{Evaluation setting}

\begin{figure}[t]
\begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp-setup-photo-only.pdf}
    \subcaption{Experimental Setting}
        \label{fig:multi_user_conf_actual}
\end{subfigure}
\begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp-setup-floor-map.pdf}
        \subcaption{Setting Floorplan}
        \label{fig:multi_user_conf_floor}
    \end{subfigure}
% \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp-setup-with-num.pdf}
%         \caption{Experimental Setting: Actual image and floorplan}
%         \label{fig:multi_user_conf_floor}
%     \end{subfigure}
% \begin{subfigure}[t]{0.3\textwidth}
%     \centering
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.8\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/bar_chart}    
%     % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
%     \caption{Power consumption for 4 users (mW)}
%     % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
%     \label{fig:pow_calc}
%     \end{subfigure}
%     \vspace{7pt}
\caption{We test \name in a conference room setting (a), and the numbers $0,1,\ldots 9$ in (b) represent the $4$ user positions for the 10 configurations where we test \name and baselines, (c) shows the power consumption metrics of our setup}
\end{figure}



To evaluate \name, we consider a office environment (conference room setting, rough dimensions of 12m*5m, Fig. \ref{fig:multi_user_conf_actual}) with TV screens/desks/whiteboards which would act as reflectors and make it a multipath setting.
We fix the location of \name PCB, which acts as an AP, roughly in middle of the room, and vary the positions of the $2,3,4$ users across 10 configurations scattered around the room, and with various degrees of closeness to capture the overall performance trends in the experimental setting considered.
For the experiments we set the transmit power such that we have SNR of about 17-20 dB, and utilize QAM-16 constellation with 0.5 rate convolutional channel code.
This choice of SNRs is consistent with the recent works on MIMO systems \cite{ding2020agora}.

% We evaluate the power consumption, SINR, system capacity, Goodput and Energy per joule performance for 2,3,4 users at various positions in a conference room setting (Fig. \ref{fig:multi_user_conf_actual}), to capture the overall performance trends in the experimental setting considered. The room which we choose has rough dimensions of 12m*5m, and is populated with objects like tables, chairs, whiteboard and TV screens, which make the setting rich with scattering effects. 
% For the experiments we set the transmit power such that we have SNR of about 17-20 dB, and utilize QAM-16 constellation with 0.5 rate convolutional channel code.
% This choice of SNRs is consistent with the recent works on MIMO systems \cite{ding2020agora}.
% This constellation was tested to work reliably for these SNRs, given the phase noise of our implementation with users on an USRP and AP being WARPv3.
% We implement 5 different test configurations anutilized baselines: 4 antenna \name, 4 antenna DBF, 8 antenna \name, 8 antenna DBF (Trace level) and Interference free OFDMA oracle.
\subsection{End to end evaluations}




% \subsection{Evaluations}
\begin{figure*}
    
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/8ant_multipos_sajjad}    
    \caption{8 Ant \name improves SINR for 4 users}
    \label{fig:8ant_res}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/tput_sajjad}
    % \input{results/8ant_multipos}   
    \input{results/trace_sim}
    \caption{Trace level comparisons with 8 antenna DBF}
    \label{fig:trace_lvl}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/capacity}   
    \caption{Increasing number of antennas allow reaching FDMA capacity}
    \label{fig:fdma_cap}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % \input{results/8ant_multipos}    
    \input{results/tput_sajjad}   
    \caption{Throughput results}
    \label{fig:tput}
    \end{subfigure}
        \vspace{7pt}
    \caption{Experiment CDFs for SINR plotted across multiple packets collected for multiple user locations in the conference room setting, and Average Goodput with errorbars representing std. deviation across multiple packets. We can see that with $8\times4$ \name, we always meet the target SINR which allows robust goodput performance for all users, and also meets FDMA oracle capacity}
    \vspace{5pt}
\end{figure*}

\begin{figure}[t]
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \centering
    \setlength{\figureheight}{0.55\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegrapandhics[width=\linewidth]{results/init_figs/Selection_820.png}
     
    \input{results/bp_joule}
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \caption{Energy efficiency results}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \caption{}
    \label{fig:bp_joule}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
    % \includegrapandhics[width=\linewidth]{results/init_figs/Selection_820.png}
    % \input{results/pow_rf.pdf}
    \includegraphics[width=\linewidth]{results/pow_rf.pdf}
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \caption{Power consumption with \# of RF Chains}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \caption{}
    \label{fig:energy_rfc}
    \end{subfigure}
        \vspace{-5pt}
    \caption{(a) Energy Efficiency, (b) Power consumption with \# of RFC}
    \vspace{3pt}
    % \label{fig:fdma_comp}
\end{figure}





% \noindent \textbf{5.1 Evaluation Setting}:\\


% \begin{enumerate}[itemsep=0pt,leftmargin=5pt]
    % \item \textbf{4 antenna \name}: Here we utilize 4 switched antennas combined to a single output, used to create 4 virtual RF chains  (Fig. \ref{fig:mmse_comp})
    % \item \textbf{4 antenna DBF}: Since we use WARPv3 as our evaluation platform, we have availability of 4 physical RF chains via the MIMO expansion daughtercard, to implement 4 antenna digital beamforming (Fig. \ref{fig:mmse_comp})
    % \item \textbf{8 antenna \name}: Here we use PCB which has 8 switched antennas combined to a single output (Fig. \ref{fig:pcb_pic})
    % \item \textbf{Interference free-oracle}: To test how well \name suppresses interference, we also test with an oracle which has users in different frequency bands 
    % \item \textbf{8 antenna DBF (trace level)}: We utilize our 8 antenna switched PCB to $4$ channel traces at a time via the WARP's 4 physical RF chains, and then time-align these traces to evaluate at a trace level how a 8 antenna DBF would perform in comparison to \name
% \end{enumerate}

% \item \textbf{4 antenna \name}: Here we utilize 4 switched antennas combined to a single output, used to create 4 virtual RF chains  (Fig. \ref{fig:mmse_comp})
%     \item \textbf{4 antenna DBF}: Since we use WARPv3 as our evaluation platform, we have availability of 4 physical RF chains via the MIMO expansion daughtercard, to implement 4 antenna digital beamforming (Fig. \ref{fig:mmse_comp})
%     \item \textbf{8 antenna \name}: Here we use PCB which has 8 switched antennas combined to a single output (Fig. \ref{fig:pcb_pic})
%     \item \textbf{Interference free-oracle}: To test how well \name suppresses interference, we also test with an oracle which has users in different frequency bands 
%     \item \textbf{8 antenna DBF (trace level)}: We utilize our 8 antenna switched PCB to $4$ channel traces at a time via the WARP's 4 physical RF chains, and then time-align these traces to evaluate at a trace level how a 8 antenna DBF would perform in comparison to \name

% Virtual RF chains offer various advantages over their physical counterparts. 
% First, because of hardware re-use of downconversion chains across the antennas, creation of $N$ virtual RF chains costs is much less power consuming than $N$ physical RF chains.
% Second, virtual RF chains can scale easily to number of antennas; addition of new antennas doesn't need a new RF chain, which allows \name to use more number of antennas than number of virtual RF chains to allow MIMO signal processing commensurate to users' bandwidth; paving the way ahead for green communications.
% In addition, \name allows creation of RF chains via software, instead of laying them physically, thus making \name a flexible architecture.
% Since \name uses just a single RF chain, similar to FDMA, \name actually enables a multi-antenna architecture which is as spectrally efficient as massive MIMO and as power efficient as FDMA.
% In this section, we evaluate each of these claims, and provide microbenchmarks for our design.
% Hence, the while evaluating \name we first confirm that the virtual RF chains give same performance as compared to their physical counterparts.
% Then, we show evaluations which support \name's claim towards design of a green communication architecture, wherein we serve $N$ user by just utilizing $N$ times oversampled ADC and a single RF chain, at the same time using a higher number of antennas $N_{\text{ant}}$.
% We also compare the energy metrics of our design and prove the optimallity of our design by comparing to a oracle interference-free FDMA baseline.
% Finally, we also illustrate our approach of increasing the sampling rate when channel conditions are bad, by considering a very bad multi-user scenario where the users' channels are extremely correlated.
% Towards the end we also evaluate microbenchmarks for various components of \name design to quantify the performance metrics.


% We have evaluated \name architecture to deliver uplink mu-MIMO multiplexing gains with just a single RF chain connected to multiple switched antennas. The core principle behind \name is the usage of strategic toggling sequences for the RF switches, which enable the creation of time interleaved virtual RF chains. \name would then combines across these virtual RF chains in digital domain to cancel interference and thus serve multiple users with a single RF chain. Thus \name can be very helpful in situations where the networks need to serve multiple users simultaneously, for example during conferences when the occupancy shoots up drastically.

\noindent \textbf{5.2 RFE and Sampling power consumption}: 
WARPv3's RF transceiver MAX2829 \cite{MAX2829}, performs the downconversion and filtering. From the datasheet, we can see that 4 antenna DBF would require RFE power of 1632 mW (4$\times$408 mW) power when operating in synchronous MIMO mode, while only 354 mW for \name operating by itself, as is the case with \name and interference-free oracle which employs FDMA.
Finally, \name uses a network of switches for creating per-antenna spectrum variations leading to virtual RF chain creation; This has near negligible power consumption, similar to how these switches being used for backscatter communications which exploit this near negligible power for battery-less operation. The HMC197BE switches used in \name design require just 0.001 mW of static power, and even including the active power they draw from the MHz clock sources, it is fairly less than 1 mW. Hence total RFE power consumption for 8 antenna \name is approximately 354+8 = 362 mW (assuming 1mW per switch), for FDMA it is 354 mW and for DBF it is 1632 mW.
% As users drop down from $4$ to say $3$ or $2$, the RFE power for \name and FDMA will not change as this is the fixed power consumption by the single front end chain. But for digital beamfroming, as users drop down, 

ADC power varies linearly with the sampling frequency \cite{barati2020energy}, which is true for the AD9963 ADC used for WARP, as evident from the datasheet \cite{AD9963}. 
Thus, the power consumption of 4 ADCs is same to that of one ADC with 4x higher sampling. From the datasheets of AD9963, we have power consumption as 400 mW for 40 MHz sampling operation used for \name and FDMA, whereas 4 physical RF chains with 10 MHz would use 4*100 = 400 mW as well. Thus for all the three confiurations, the sampling power would be 400mW.

Therefore, total power consumption of \name is ~762 mW (354+400+8 mW) which is 3x lower than MIMO (1632+400 = 2032 MW), and almost the same as single antenna FDMA oracle, which would be 754 mW (354+400mW).

Fig. \ref{fig:pow_calc} shows the power consumption metrics for each of the strategy. As seen clearly, it is not the sampling power which dominates the power consumption, but the power consumed in the front end by these multiple RF chains. 
% One might argue that these calculations are for WARPv3, which is a slightly older SDR, but even the state of art mmWave receiver also show this trend of power consumption being dominated by the downconversion hardware and not ADCs/DACs \cite{yan2019performance}.

\noindent\textbf{5.3 SINR performance comparison of 4 antenna \name with DBF}:
\name is the first work to use virtual RF chains.
Hence, it is important to show the performance comparison with physical RF chains.
We do so by creating a faithful test setup to compare virtual RF chains with physical RF chains (Fig. \ref{fig:mmse_comp}). 
% The test-setup allows us to use the same antennas for capturing the received samples from WARP with both $4$ virtual RF chains created by \name's approach, and $4$ physical RF chains digital beamforming.
Basically we use external switches to have the same antennas connected to either 4 physical RF chains directly, or 4 virtual RF chains via RF switched array.
Thus, we can compare the 2 approaches faithfully, as both of them capture the samples from the same antennas.

The SINR performance of both the methods indeed turn out to be very similar (Fig. \ref{fig:4ant_sinr}). 
For these CDFs, we collect 30 packets at each of the 10 locations of $4$ users in the conference room, which gives 300 sample SINRs these plots. We can clearly see the performance for both the methods to be very similar (within $\pm$ 0.5 dB for median error).
Thus $4$ virtual RF chains, with total power consumption as 762 mW provides same SINR metrics as $4$ physical RF chains, with total power consumption 2032 mW, which is 3x more than \name.
However, as the number of users increase from $2$ to $4$, the performance of both the two approaches deteriorate, and with $4$ users, for almost $40\%$ of the packets, the SINR is lesser than $10$ dB (Fig. \ref{fig:4ant_sinr}). \\
% This result is consistent with many of the research papers \cite{pasandi2021muvis,sur2016practical}, agreeing on the fact that serving $N$ users with just $N$ antennas is not a robust operation point.
% In this setup, we use RF switches external to the switches we use for our switched antennas, and the purpose of these SPDT RF switches is to toggle between two states. The first state of the setup is ``RFC-RF1", which connects the $4$ antenna array to the PCB which implements \name architecture, and takes the output emanating from the PCB and feeds it to a single RF chain on WARP. The other state, 
% ``RFC-RF2" connects the same antenna array to each of the physical RF chains on WARP to implement traditional digital beamforming. 
% Evaluation in such conference room, or auditorium settings has been a constant feature of research works on multi-user communications \cite{flores2016scalable,kuhne2020bringing}. 
% The SINR here is computed from the EVM metric of the receieved constellation after digital combining is done, as the noise would be coming from the residual interference and noise.
% Goodput is measured by mapping the received constellation back to bits, passing through vitterbi decoder corresponding to the 0.5 rate convolutional code, and then measuring the number of bit errors.
% Unlike traditional digital beamformers, which have to now spend even more power to add new RF chains, \name can guarantee performance for $N$ users with $N$ streams by extending to more number of antennas easily.

\noindent\textbf{5.4 Optimizing sampling+compute power by serving 4 users reliably with $4$ virtual RF chains}:
In order to improve the performance as number of users $N$ approach number of virtual RF chains $N$, we increase the antennas and use our BABF algorithm to prioritize 1 user per RF chain.
% We utilize the $8$ antenna version of our \name architecture, as shown in Fig. \ref{fig:pcb_pic} to 
% implement BABF algorithm in order to support $4$ users reliably. Note that we do not increase our oversampling factor, and just attach more switched antennas for this experiment. 

For this experiment, we use the \name PCB which has the capability to utilize $8$ switched antennas, and create $4$ virtual RF chains from the combined $8$ antenna output.
We can electronically turn off antennas in our PCB to simultaneously collect data from $4$, as well as $6$ antenna configurations to understand the effect of increasing number of antennas on the system metrics. 
The SINR and goodput results are shown in Fig. \ref{fig:8ant_res}.
As we increase the antennas to $8$, the SINR shows an immense jump and always exceeds 10 dB, close to what is expected from a robust multi-user transmission scheme.
We observe more than $10$ dB increase in the $90$-th percentile SINR, as compared to $4$ antenna digital beamformer implemented using WARP's physical RF chains.

% It is indeed impressive to see how \name was able to harden the multiplexing gains for $4$ users without actually increasing the number of virtual RF chains just by utilizing more switched antennas, which bear a very minimal extra power and implementation cost.




% \begin{figure*}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/random_seq_sajjad}    
%     % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
%     % \vspace{-3pt}
%     \caption{Choice of $\mathbf{S}$}
%     % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
%     \label{fig:random_seq}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
%     \input{results/unsynch_sajjad}   
%     % \vspace{-3pt}
%     \caption{Synch. vs Unsynch. users}
%     \label{fig:unsynch}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     \input{results/lts_fig}
%     % \input{results/8ant_multipos}    
%     % \vspace{-3pt}
%     \caption{Varying channel estimation accuracy}
%     \label{fig:chan_est}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%     \setlength{\figureheight}{0.5\linewidth}
%     \setlength{\figurewidth}{0.85\linewidth}
%     % \includegraphics[draft,width=0.7\linewidth]{draft.png}
%     \input{results/sim_res}
%     % \input{results/8ant_multipos}    
%     % \vspace{-3pt}
%     \caption{Large scale simulations}
%     \label{fig:sim_fig}
%     \end{subfigure}
%         \vspace{7pt}
%     \caption{Ablation studies to adjudge \name's performance (a)-(c), and a large scale simulation result (d)}
%     \vspace{5pt}
% \end{figure*}

% \noindent\textbf{Trace level comparisons with Digital Beamformers having more than $4$ RF chains:
% Unlike \name, which can support $4$ users robustly without increasing sampling power consumption, by just adding more antennas+RF switches, Digital beamforming adds new RF chains to do so. 
% Thus, a nai
Unlike \name, digital beamforming approaches utilize a naive way of improving performance for $4$ users, which is to add more RF chains to sample from more antennas.
Since WARPv3 has support only for $4$ physical RF chains, we do a trace level comparison to $6,8$ RF chain DBF by collecting $4$ antennas channels at a time and then synchronizing them in post-processing.
We observe that \name even outperforms a $6$ antenna digital beamformer (Fig. \ref{fig:trace_lvl}), and comes $\sim3$ dB close to $8$ antenna digital beamformer at median performachainsnce, all the while having at least $4$x lower power consumption.


\noindent\textbf{5.5 Comparison with interference-free oracle}:
% Since \name utilizes $4$ times higher \emph{sampling bandwidth} as the user's transmitting bandwidth, it is only natural to compare the same with an equivalent frequency based multiplexing (FDMA) system. 
% However, only the sampling bandwidth for FDMA and \name are the same, \name utilizes $4$ times lesser spectrum resources while sampling at a higher rate. 
For the FDMA oracle, the users occupy $4$ different $10$ MHz bands, and the WARP would sample this aggregate $40$ MHz bandwidth in order to serve these $4$ non-interfering users.
In contrast, for \name, the $4$ users occupy the same $10$ MHz band, and the WARP receiver samples a higher sampling bandwidth $40$ MHz, in order to create the $4$ virtual RF chains required to multiplex the 4 users signals.
Thus in order to be spectrum-efficient, \name has to cancel the in-band interference in the occupied 10 MHz bandwidth
Even with added task of interference cancellation, we see that with more number of antennas ($8$) than number of users ($4$), we get system capacity on on par with FDMA oracle (Fig. \ref{fig:fdma_cap}). 

\noindent \textbf{5.6 Energy efficiency metrics (bits per joules)}: Finally, we revisit the power calculations briefly in the context of our goodput results.
As seen in Fig. \ref{fig:tput}, we can get goodput close to interference-free oracle levels using \name architecture with 8 antennas. 
This result can also be viewed in the lens of bits per joules (Fig. \ref{fig:bp_joule}) by seeing how much power got expended in the process.
As the number of RF chains increase from $2$ to $4$, we see constant $O(1)$ 354 mW RF front end (RFE) power demand for \name, as explained in Section 5.2.
The ADC power requirements are $100mW$ per 10 MHz data sampled and that increases as $O(N)$ with users.
On the other end, for digital beamforming, RFE power scales linearly with $N$, given by $408*N$, since the WARPv3 MAX2829 IC uses $408$ mW per RF chain in MIMO mode.
Hence, we get energy consumption trends as shown in Fig. \ref{fig:energy_rfc}.
This explains the energy per joule Fig. \ref{fig:bp_joule}, more particularly, the dip for DBF at $4$ user operation.
This is because, the DBF goodput shows a downward trend for $4$ users, whereas power has kept on increasing linearly, which further exacerbates the energy efficiency between DBF and \name.

% \noindent\textbf{Spectrum saving and Power saving with TIMO}: So far, we have seen that TIMO serves four users utilizing 4x lower spectrum than equivalent FDMA system and 4x lower RF-chains than equivalent MIMO system while performing similar to FDMA and MIMO systems. Here we explain the implication of saving these spectrum and hardware resources on modern communication systems as shown in Figure \ref{fig:pow}. First, TIMO is spectrally efficient as it utilizes only 10 MHz bandwidth to serve 4 users while an equivalent FDMA system requires a large 40 MHz spectrum. Thus, TIMO achieves 4x higher spectral efficiency than FDMA. 
% The second implication is that TIMO is power efficient as it saves the number of RF chains by a factor of four compared to a MIMO system.  \textit{In summary, TIMO makes the best of both worlds by being as power-efficient as FDMA systems and as spectrum efficient as MIMO systems. This leads to a scalable mu-MIMO design that can multiplex an order of magnitude higher users simultaneously.}\
% While MIMO hardware consists of 4 ADCs along with 4 down conversion chains, the TIMO hardware consists of only one high-sampling ADC and a single downconversion chain, 
% * ADC power is linear in  terms of sampling frequency \todo{cite}. Utilizing 4x faster ADC has same power 4x power slower ADC. For 
% * Howvere, we save on, we don;t need 4 downconversion chains. And in our implementation with warp v3, the ADC consume 400 mW for both case. \todo{cite datasheet}. Downconversion chip MAX2829 utilizes 354 mW for SISOimplementation and 4x 408 mW = 1632 mW when used in a MIMO mode. 754 mW for us and 2032 mW for DF.
% * Switches need 0.001 mW static power and even including the active power they draw from the MHz clock sources, it is less than 1 mW . 
% * We are close to fDMS because switches are minimal power. 
% By getting the same capacity result as FDMA, at the same time using $4$ times lower aggregate bandwidth than FDMA, \name builds a single RF chain receiver which is spectrally very efficient.
% At the same time, \name utilizes similar power metrics to the single antenna FDMA approach, since the switches, including the DC power as well as power drawn from the MHz clocking inputs, have very minimal power ($<$ 1 dBm), and the antennas are entirely passive.
% Thus, as compared to other multiplexing approaches to be spectrally efficient, like digital beamforming, which are power inefficient, \name offers both, a spectrally, as well as power efficiently solution to obtain multiplexing gains.
% For this result, we use the switches to increase the signal power of one user at each time slot, so that we get uncorrelated channels enabling higher spatial multiplexing gains. To evaluate the effectiveness of our algorithm, we choose 100 random trials to choose the switching matrix $\mathbf{S}$, and 100 trials with our algorithm, and plot the CDF in Fig. \ref{fig:random_seq}. Our approach of choosing inphase antennas for one user at a time always outprforms a randomly chosen matrix $\mathbf{S}$.

% \noindent\textbf{5.7 Ablation studies}:
% % Finally, to conclude our evaluations, we show ablation studies for
% % \begin{enumerate}[itemsep=0pt]
% %     \item Effectiveness of BABF algorithm
% %     \item Synchronized vs Unsynchronized users
% %     \item Channel estimation accuracy 
% % \end{enumerate}
% % , having users unsynchronized and channel estimation accuracy play a factor into \name's approach. For all these results we fix a $4$ user configuration in the conference room setting and collect multiple packets by varying these parameters to carefully understand the effects.

% First, to evaluate the effectiveness of BABF, we choose 100 random choices of $\mathbf{B}$, and collect $10$ packets with each choice, and repeat the same with $100$ packets collected by choosing $\mathbf{B}$ via BABF algorithm which chooses in-phase switches for one user per virtual RF chain. We plot the CDF in Fig. \ref{fig:random_seq}, and observe that BABF $\mathbf{B}$ matrix always outperforms a randomly chosen $\mathbf{B}$.

% Second, to show robustness against unsynchronized users, we first synchronize the users to each other by utilizing same reference clock and start time, and thus all the transmitters have same CFO and tightly synchronized sampling times.
% Then, we repeat the experiment by having unsynchronized usees, suchthat each user has a different clock, leading to different CFOs for each user.
% As clearly seen from Fig. \ref{fig:unsynch}, we get almost the same performance when the transmitters are synchronised with each other as compared to when they are unsynchronized.
% % Infact, we get minimally higher SINR with unsynchronized since due to sampling offsets, the unsynchronized transmissions often end up having some samples to be interference free, whereas for the synchronized transmissions, all the user's signals interfere all the times, hence being a more stringent evaluation.

% Third, the interference cancellation performance also depends on the accuracy of channel estimates procured. We can always average the channel across multiple LTS's to get a higher channel estimation accuracy. Thus, we repeat the experiment with more number of LTS's than the prescribed $2$ LTS's as per 802.11 protocol, and observe that we get only about $1.5$ dB difference in median performance as the number of LTS's increase to $10$, which shows that \name's algorithms can work without imposing a high cost of channel estimation latency.
\begin{figure}[t]
    % \begin{adjustwidth}{-15pt}{} 
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mmse_comp_network.pdf}
        \caption{Physical vs Virtual RFC}
        \label{fig:mmse_comp}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \setlength{\figureheight}{0.6\linewidth}
    \setlength{\figurewidth}{0.9\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/mmse_comparison_sajjad}
    \caption{SINR CDF for 2, 3, 4 users}
    % \caption{Throughput comparison with SISO and Digital beamforming. Our method closely matches the digital beamforming baseline, however, both these methods fail to provide the 4x possible increase in rate}
    \label{fig:4ant_sinr}
    \end{subfigure}
    % \end{adjustwidth}
    % \begin{subfigure}[t]{0.22\textwidth}
    % \centering
    % \setlength{\figureheight}{0.5\linewidth}
    % \setlength{\figurewidth}{0.8\linewidth}
    % % \includegraphics[draft,width=0.7\linewidth]{draft.png}
    % % \input{results/8ant_multipos}    
    % \input{results/pow_spectrum}
    % \caption{Power \& Spectrum Required}
    % \label{fig:pow_spectrum}
    % \end{subfigure}
        % \vspace{7pt}
    \vspace{2pt}
    \caption{Microbenchmarks (1): Do the created virtual RF chains have similar performance to physical RF chains?}
    \label{fig:fdma_comp}
\end{figure}

\begin{figure}
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \centering
    \setlength{\figureheight}{0.5\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/random_seq_sajjad}    
    % \includegraphics[width=0.4\textwidth]{results/init_figs/Selection_821.png}
    % \vspace{-3pt}
    \caption{Choice of $\mathbf{S}$}
    % \caption{Throughput with number of users, 2 RF chains and 8 antenna \name, which allows linear scaling of throughput with 8 users}
    \label{fig:random_seq}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
    \setlength{\figureheight}{0.5\linewidth}
    \setlength{\figurewidth}{0.85\linewidth}
    % \includegraphics[width=\linewidth]{results/init_figs/Selection_820.png}
    \input{results/unsynch_sajjad}   
    % \vspace{-3pt}
    \caption{Synch. vs Unsynch. users}
    \label{fig:unsynch}
    \end{subfigure}
    \caption{Microbenchmarks (2): What is the performance gain of BABF switching, and do the transmitters need synchronization?}
\end{figure}


\subsection{Microbenchmarks}
The main design concepts of \name are creation of virtual RF chains from the spreaded bandwidth and BABF switching to beamform towards one user per virtual chain.
Further, since the creation of virtual RF chains require slicing across samples, like collecting every $\{4n\},\{4n+1\},\{4n+2\},\{4n+3\}$ samples, it may appear that the transmitters also need to be synchronized for the whole \name approach to work.

\textbf{Physical vs Virtual RF chains}: Hence, we first create a faithful test setup to ascertain the fidelity of \name's virtual RF chains versus traditional MIMO's physical RF chains (Fig. \ref{fig:mmse_comp}).
Since we want a fair one to one comparison, we do not turn on multiple antennas per virtual RF chain and restrict to one antenna per virtual chain.
The test setup ensures that the wireless channels captured by $4$ physical RF chains is same as the $4$ virtual RF chains channel via \name PCB.
We collect the $2,3,4$ users interfering traces from this setup, and evaluate the average SINR across the users to evaluate the interference cancellation capacity of virtual vs physical RF chains.
Because the insertion losses from the switches are minimal ($\sim 0.5$ dB) and the PCB is designed with optimal Wilkinson networks at $2.4$ GHz, we see that the SINR metrics remain same for both physical and virtual RF chains. 
This validates the \name PCB design and implementation.

\textbf{Why BABF?}: Next, we start utilizing one big advantage of virtual RF chains, that we can toggle multiple antennas on-off in a virtual chain to get advantage of analog combining gains. Using the BABF approach, this allows us to get a well-conditioned equivalent channel matrix $\mathbf{H}\mathbf{S}$ which is diagonal heavy.
Hence, as a consequence, the digital beamforming block which inverts the wireless channel works more efficiently and the final SINRs so obtained are much better.
These results are quantified as shown in Fig. \ref{fig:random_seq}, where for one user configuration we evaluate the final SINRs by choosing $\mathbf{S}$ randomly, and via BABF, and we repeat this 100 times to plot the CDF.
BABF always works better than any random choice of $\mathbf{S}$, and on an average (median line) it works $10$ dB better.
This justifies the design choice of adopting BABF approach of computing $\mathbf{S}$.
% Note that BABF is computed deterministically, whereas to get to median random matrix performance we would need to try 50 random combinations and then choose the best one.

\textbf{Synchronized vs Unsynchronized Users}: \textcolor{red}{!!!Write it better!!!} \name basically does a spatial operation; so it does not matter if the transmitters are synchronized or not.
So, to show this result, we conduct experiments where we synchronize the $4$ users to share the same clock, and repeat it without synchronization.
We observe similar performance as expected, shown in Fig. \ref{fig:unsynch}.
However, since \name needs to obtain per-user channels, it is required that the users are at least loosely synchronized such that their LTS's do not collide, and this level of loose synchronization is guaranteed by modern cellular protocols, however the users do not need to share the whole clocks.



% \subsubsection{Virtual vs Physical RF chains}
% \subsubsection{SAM+BABF implementation}

\noindent \textbf{Scaling to higher number of antennas and users}: 
Our hardware experiments are limited to handling $4$ users and $8$ antennas, however, the techniques introduced in this paper are fairly general and can be implemented for higher number of antennas and more number of users with specialized RF switches and better evaluation platform.
% since the commercially available HMC197BE RF switch we use has $\sim 10ns$ on time. 
% Thus, we can not handle faster bandwidth switching than 50 MHz, and further
% our evaluation platform WARPv3 which supports only 40 MHz sampling.
% However, the techniques introduced in this paper are fairly general and can be implemented for higher number of antennas and more number of users with specialized RF switches and better evaluation platform.

To motivate this, we perform simulations by placing users in similar environments to our evaluation setting, and modelling the multipath wireless channel via ray-tracing.
In simulations, the users transmit OFDM signals and the channels are applied to the OFDM signals by calculating the distances from the environment reflectors in simulation setting and applying appropriate time delays+amplitude weights in the received OFDM signal. 
All the receive processing uses the identical codes used for hardware evaluations. Hence, this simulation framework gives results which by and large follow the trends expected from experimental evaluations.

Fig. \ref{fig:sim_fig} shows simulation results and comparison for 64 antennas usecase to serve 8 users. This is considered a standard baseline with multi-user Dense deployments, which on an average require serving $8$ streams concurrently \cite{yan2019performance}.
\name uses 64 antennas and creates 8 virtual RF chains to serve the 8 users, and almost always obtains >10dB SINR.
We can see even in simulations serving $8$ users with $8$ RF chain digital beamforming is infeasible.
We also show comparisons with ideal partially and fully connected hybrid beamformers with $8$ physical RF chains. Our simulations assume perfect phase quantization, and still \name outperforms partially connected beamformers. The reason is that unlike partially connected beamformers \name does not split the antenna array between the physical RF chains, since all the antennas are by default connected to the virtual RF chains.

\name's performance comes about $5dB$ close on an average, to the full 64 chain DBF and fully connected HBF, even though using at least 64x lower power and 64x lower circuit elements.  

% Now, there are some ways to get around these limitations. One method is to to expect some sort-of coordination from users, such that either they align their transmissions to minimize interference, or the users introduce random cyclic delays to allow for de-correlation of the channels. However, both these methods require channel feedback to the users, which is very difficult to achieve in practise, with multiple challenges like accuracy of quantized feedback, staleness of channel estimates which hinder these deployments in practical scenarios. A potentially better method is to increase the number of antennas at the base-station, since that increases the aperture and allows for finer beams to be formed which can de-correlate the users. However, increasing number of antennas is not a scalable operation with digital beamforming, since we require extra RF chains for the same to support the increased antennas. On the flipside, \name uses just a single RF chain, and thus can increase the number of antennas in a more scalable manner, and this allows \name to deal with spatially close users (Fig. \ref{fig:8ant_exampleloc}). 

% To evaluate this claim, we choose the following user configuration, where the users are quite co-located, which is practise could be a single user with their phones and tablets acting as two close located device. We keep on increasing the number of antennas in our implementation till we start seeing acceptable SINR performance (>10 dB for all the users), which we empirically observe happens at number of antennas to be 8 (Fig. \ref{fig:8ant_exampleloc}. In comparison, we have the performance by a 4 antenna digital beamformer which doesn't have the capability of handling such scenarios and the SINR is only around 4 dB or even lower for some users.








% \begin{figure}[H]
%     \begin{subfigure}{0.23\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{results/init_figs/Screenshot_20210323-102643_Samsung Notes.jpg}
%         \caption{Indoor Setting}
    
%     \end{subfigure}
%     \begin{subfigure}{0.23\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{results/init_figs/Screenshot_20210323-102643_Samsung Notes.jpg}
%         \caption{Outdoor Setting}
    
%     \end{subfigure}
%     \label{fig:my_label}
% \end{figure}


% We evaluate the effectiveness of \name in handling multiple users in two settings, first one an indoor office setting, and second one an outdoor setting. For each setting we evaluate BER/Throughput/EVM at multiple user locations and plot the CDF to obtain the performance statistics of \name. \name uses 4 antennas, followed by 4 switches, which are then combined and read via a single RF Chain. 
% Hence, \name lies somewhere between a conventional MIMO design with multiple antennas supported by multiple RF chains, and a single antenna with a single RF chain solutions.
% Thus, we compare \name results with a SISO link, as well as an equivalent 4 antenna MMSE baseline.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{results/init_figs/Screenshot_20210323-105406_Samsung Notes.jpg}
%     \caption{Eval Results}
%     \label{fig:my_label}
% \end{figure}

% \subsection{BER Results}

